Massless Phases for the Villain model in $d\geq 3$

We consider the classical Villain rotator model in $\mathbb{Z}^d, d\geq 3$ at sufficiently low temperature, and prove that the truncated two-point function decays asymptotically as $|x|^{2-d}$, with an algebraic rate of convergence. We also obtain the same asymptotic decay separately for the transversal two-point functions. This quantifies the spontaneous magnetization result for the Villain model at low temperature, and rigorously establishes the Gaussian spin-wave conjecture in dimension $d\ge 3$. We believe that our method extends to finite range interactions and to other abelian spin systems and abelian gauge theory in $d\geq 3$.

==> codesbis.tex <==
First we note that, by definition of the operator $\mathcal{L}_\beta$,
\begin{equation*}
    \left\| \nabla \left( w - \eta G_{\delta}  \right) \right\|_{L^2\left( B_{R^{1 + \delta}}, \, \mu_\beta \right)}^2 \leq
     \sum_{x \in B_{R^{1 + \delta}}} \left\langle \L_\beta \left(w - \eta G_{\delta} \right), \left( w - \eta G_{\delta} \right) \right\rangle_{\mu_\beta} \leq \frac{C}{R^{(1 + \delta)(d-2)}}.
\end{equation*}
We first prove the estimate REF; we note that since the functions $w$ and $\eta G$ are equal to $0$ outside the ball $B_{R^{1+\delta}}$, we can apply the Poincar\'e inequality and obtain
\begin{equation*}
     \left\| w - \eta G_\delta   \right\|_{L^2\left( B_{R^{1 + \delta}}, \, \mu_\beta \right)}^2 \leq \frac{C}{R^{(1 + \delta_0)(d-4)}}.
\end{equation*}
We can then restrict the integral on the left side to the annulus $A_R$, use that the volume of $A_R$ is of order $R^d$, and that the cutoff function $\eta$ is equal to $1$ in $A_R$. We obtain
\begin{equation*}
    \left\| w - G_\delta   \right\|_{\underline{L}^2\left( A_R, \, \mu_\beta \right)} \leq \frac{CR^{1+\delta}}{R^{d - 1 -\alpha}}.
\end{equation*}
If the exponent $\delta$ is chosen small enough, in particular smaller than $\frac \alpha 2$, we obtain
\begin{equation*}
    \left\| w - G_\delta  \right\|_{\underline{L}^2\left( A_R, \, \mu_\beta \right)} \leq \frac{CR^{1+\delta}}{R^{d - 1 -\frac{\alpha}{2}}},
\end{equation*}
which gives, by reducing the value of the exponent $\alpha$,
\begin{equation*}
    \left\| w - G_\delta   \right\|_{\underline{L}^2\left( A_R, \, \mu_\beta \right)} \leq \frac{C}{R^{d - 2 -\alpha}}.
\end{equation*}
To complete the proof of the estimate REF, we prove the following inequality
\begin{equation*}
     \left\| w - \bar G_\delta   \right\|_{\underline{L}^2\left( A_R, \, \mu_\beta \right)} \leq \frac{C}{R^{d - 2 -\alpha}}.
\end{equation*}
Using the explicit formula for the two-scale expansion, we see that, for any pair $(x , \phi)\in A_R \times \Omega$
\begin{equation*}
w(x, \phi) - \bar G_\delta (x , \phi) = \sum_{i=1}^d \nabla_i \bar G_\delta (x , \phi) \chi_{m,i}(x , \phi).
\end{equation*}
By the regularity estimate REF on the gradient of the Green's function $\bar G_\delta$ and the quantitative sublinearity of the corrector stated in REF, we have
\begin{align*}
    \left\|\sum_{i=1}^d \nabla_i \bar G_\delta \chi_{m,i}  \right\|_{\underline{L}^2\left( A_R, \, \mu_\beta \right)} & \leq C \left\| \nabla_i \bar G_\delta \right\|_{\underline{L}^2\left( A_R, \, \mu_\beta \right)} \sum_{i=1}^d \left\|  \chi_{m,i}  \right\|_{\underline{L}^2\left( A_R, \, \mu_\beta \right)} \\
    & \leq \frac{C}{R^{d - 1}} R^{d \delta} \left\|  \chi_{m,i}  \right\|_{\underline{L}^2\left( B_{R^{1 + \delta}}, \, \mu_\beta \right)} \\
    & \leq  \frac{C}{R^{d - 1}} R^{d \delta} R^{(1+ \delta) \alpha}.
\end{align*}
By choosing the value of the parameter $\delta$ small enough, and reducing the value of the expoenent $\alpha$, we obtain the estimate REF. Combining the estimates REF and REF completes the proof of the inequality REF.





We now prove the estimate REF pertaining to the gradient of the Green's function. We start from the estimate REF restrict the domain of integration to the annulus $A_R$ and note that the cutoff function $\eta$ is equal to $1$ on $A_R$. This gives
\begin{equation*}
    \left\| \nabla \left( w - G  \right) \right\|_{\underline{L}^2\left( A_R, \, \mu_\beta \right)} \leq \frac{1}{ R^{d}} \sum_{x \in B_{R^{1 + \delta}}} \left\langle \L_\beta \left(w -  G \right), \left( w -  G \right) \right\rangle_{\mu_\beta} \leq \frac{C}{R^{d-1 - \alpha}}.
\end{equation*}
Using the explicit formula REF to compute the gradient of $w$ and obtain
\begin{equation*}
    \nabla w = \nabla \bar G_\delta +
    \sum_{i = 1}^d  \nabla_i \bar G_\delta \nabla \chi_{m,i} + \sum_{i = 1}^d \nabla \nabla_i \bar G_\delta \chi_{m,i}.
\end{equation*}
The third term on the right side can be estimated thanks to the regularity estimates REF and the sublinearity of the corrector REF with an argument similar to the one of the inequality REF and we obtain
\begin{equation*}
    \left\|  \sum_{i = 1}^d \nabla \nabla_i \bar G_\delta \chi_{m,i} \right\|_{\underline{L}^2\left( A_R, \, \mu_\beta \right) } \leq \frac{C}{R^{d-1-\alpha}}.
\end{equation*}
Combining the estimate REF with REF, we deduce
\begin{equation*}
    \left\| \nabla  w -  \nabla \bar G_\delta -
    \sum_{i = 1}^d  \nabla_i \bar G_\delta \nabla \chi_{m,i} \right\|_{\underline{L}^2\left( A_R, \, \mu_\beta \right)} \leq \frac{C}{R^{d-1 - \alpha}}.
\end{equation*}
Their remains to replace the gradient of the finite volume corrector by the full-volume gradient $\nabla \chi_p$ and we use Proposition REF with the regularity estimate REF to obtain
\begin{equation*}
    \left\| \nabla  w -  \nabla \bar G_\delta -
    \sum_{i = 1}^d  \nabla_i \bar G_\delta \nabla \chi_i \right\|_{\underline{L}^2\left( A_R, \, \mu_\beta \right)} \leq \frac{C}{R^{d-1 - \alpha}}.
\end{equation*}
Combining the inequality REF with the estimate REF completes the proof of REF.


Recall if the THM of homogenization of mixed derivative of Green's function.

 The result is recalled below. Before stating the result, we need to introduce three objects: \pdcomment{petit pb de consistence ici, a bien verifier}
\begin{itemize}
    \item For each integer $i \in \{ 1 , \ldots, d \}$, we let $l_{e_i}$ be the linear function defined by the formula
    \begin{equation*}
    l_{e_i} := \left\{\begin{aligned}
    \R^{d} &\to \R^{\binom d2}, \\
    x &\to \left( x \cdot e_i , \ldots, x \cdot e_i \right);
    \end{aligned} \right.
\end{equation*}
\item We let $\ahom$ be the homogenized coefficient associated to the Helffer-Sj{\"o}strand operator$\L$, it is defined in Section~\ref{section5} as the limit of the energy associated to the Dirichlet problem with affine boundary condition (see Definition~\ref{def.defnunustar} and Corollary~\ref{cor:coro5.13}); it is deterministic and depends only on the dimension $d$ and the inverse temperature $\beta$;
\item For each integer $i \in \{ 1 , \ldots , d \}$, we let $\nabla \chi_i$ be the gradient of the infinite-volume corrector. It is defined in Proposition~\ref{prop5.26}. Once equipped with the gradient of the corrector, we can define the exterior derivative $\di^* \chi_i$ by using that the codifferential $\di^*$ is a linear functional of the gradient (see REF).
\end{itemize}

We now state Theorem~\ref{thm:homogmixedder}.

\begin{reptheorem}{thm:homogmixedder}[Homogenization of the mixed derivative of the Green's matrix]
We let $G_{q_2}$ be the Green's matrix defined by the formula
\begin{equation} \label{def:Gq2}
    G_{q_2} = \ahom^{-1} \sum_{i=1}^d \left\langle \cos \left( \phi , q_2\right) \left( n_{q_2} , \di^* l_{e_i} + \di^* \chi_i(0 , \phi) \right)   \right\rangle_{\mu_\beta} \nabla_i G.
\end{equation}
There exist an exponent $\gamma := \gamma(d) >0$ and a constant $C_{q_1}$ which satisfies the estimates
$\left| C_{q_1} \right| \leq  C \left\| q_1 \right\|_1^{k}$, for some $C := C(d , \beta) < \infty$ and $k := k(d) < \infty$, such that for each radius $R \geq 1$, one has the estimate 
\begin{equation} \label{eq:TV192532}
    \left\| \nabla \mathcal{U}_{q_1} - \sum_{i=1}^d \left( e_i + \nabla \chi_{i}\right) \nabla_i  G_{q_2}\right\|_{\underline{L}^2 \left( B_{2R} \setminus B_R , \mu_\beta \right)} \leq \frac{C_{q_1}}{R^{d + \gamma}}.
\end{equation}
\end{reptheorem}

\begin{remark} \label{rem:remark3.578}
From the definition of the function $G_{q_2}$, we have the following inequality, for each $\kappa \in \Zd$,
\begin{equation*}
    \left| G_{q_2}(\kappa) \right| \leq \frac{C_{q_2}}{|\kappa|^{d-1}} \hspace{5mm} \mbox{and} \hspace{5mm} \left|  \nabla G_{q_2}(\kappa) \right|\leq \frac{C_{q_2}}{|\kappa|^{d}}.
\end{equation*}
\end{remark}

==> copyandpaste.tex <==
\section{Treating the error term $\mathcal{E}_{q_1,q_2}$} \label{sec:chap8.5}

This section is devoted to the treatment the error term $\mathcal{E}_{q_1,q_2}$. It is used in the proof of Theorem~\ref{t.main} in Section~\ref{sectionsection4.2789} of Chapter 4.

\begin{proposition} \label{prop:propB1}
Fix two exponents $\gamma, \ep \in ( 0, 1]$ such that $\ep \leq \frac{\gamma}{4(d-2)}$ and two charges $q_1,q_2 \in \mathcal{Q}$. Let $\mathcal{E}_{q_1, q_2} : \Zd \to \R$ be a function which satisfies the pointwise and $L^1$-estimates, for each $\kappa \in \Zd$ and each radius $R \geq 1$,
\begin{equation} \label{app.assumptE}
    \left| \mathcal{E}_{q_1,q_2}(\kappa) \right| \leq \frac{C}{|\kappa|^{d- \ep}} ~\mbox{and}~ \sum_{\kappa \in B_{2R} \setminus B_R} \left| \mathcal{E}_{q_1 , q_2} \left( \kappa \right) \right| \leq C R^{-\gamma}.
\end{equation}
Then the constant $K_{q_1,q_2} := 4\pi^2\sum_{\kappa \in \Zd} \mathcal{E}_{q_1 , q_2} \left( \kappa \right) $ is well-defined in the sense that the sum converges absolutely and one has the expansion
\begin{multline} \label{eq:TV02504}
    4\pi^2\sum_{z_2 , \kappa  \in \Zd}  \nabla G(z_2) \cdot (n_{q_2}) \nabla G_x(z_2 + \kappa) \cdot (n_{q_1})  \mathcal{E}_{q_1,q_2}(\kappa) \\ = K_{q_1 , q_2} \sum_{z_1  \in \Zd}  \nabla G(z_2) \cdot (n_{q_2}) \nabla G(z_2-x) \cdot (n_{q_1})  + O \left(\frac{C_{q_1 , q_2}}{|x|^{d -2 + \frac{\gamma}{4(d-2)}}} \right).
\end{multline}
\end{proposition}

\begin{proof}
We first write
\begin{equation*}
    \nabla G(z_2) \cdot (n_{q_2}) = \sum_{i=1}^d \nabla_i G(z_2) (n_{q_2})_i \hspace{3mm}\mbox{and}\hspace{3mm} \nabla G(z_2 + \kappa - x) \cdot (n_{q_1}) = \sum_{j=1}^d \nabla_j G(z_2 + \kappa - x) (n_{q_1})_j
\end{equation*}
and note that to prove the expansion~\eqref{eq:TV02504} it is sufficient to prove that, for each pair of integers $i , j \in \{ 1 , \ldots , d \}$,
\begin{equation} \label{eq:TV02554}
    4\pi^2\sum_{z_2 , \kappa  \in \Zd}  \nabla_i G(z_2) \nabla_j G_x(z_2 + \kappa) \mathcal{E}_{q_1,q_2}(\kappa) = K_{q_1 , q_2} \sum_{z_2  \in \Zd}  \nabla_i G(z_2)  \nabla_j G(z_2-x)  + O \left(\frac{C_{q_1 , q_2}}{|x|^{d-2 + \frac{\gamma}{4(d-2)}}} \right).
\end{equation}
We fix a pair of integers $i , j \in \{ 1 , \ldots , d \}$ and focus on the proof of~\eqref{eq:TV02554}.
Using the assumption on the function $\mathcal{E}_{q_1,q_2}$ stated in~\eqref{app.assumptE}, one has the estimate
\begin{equation*}
    \sum_{\kappa \in \Zd} \left| \mathcal{E}_{q_1 , q_2} \left( \kappa \right) \right| = \sum_{n = 0}^\infty  \sum_{\kappa \in B_{2^{n+1}} \setminus B_{2^n}}\left| \mathcal{E}_{q_1 , q_2} \left( \kappa \right) \right| \leq C \sum_{n = 0}^\infty 2^{-\gamma n} < \infty.
\end{equation*}
This proves that the sum $\sum_{\kappa \in \Zd}  \mathcal{E}_{q_1 , q_2} \left( \kappa \right)$ is absolutely convergent and that the constant $K_{q_1, q_2}$ is well-defined.
To ease the notation, we let $g$ be the function defined by the formula, for each $\kappa \in \Zd$,
\begin{equation*}
    g(\kappa) := \sum_{z_2  \in \Zd}  \nabla_i G(z_2) \nabla_j G(z_2 + \kappa),
\end{equation*}
so that the expansion~\eqref{eq:TV02554} can be rewritten in this notation
\begin{equation} \label{eq:TV03114}
4\pi^2\sum_{\kappa  \in \Zd}  g(\kappa + x) \mathcal{E}_{q_1,q_2}(\kappa) = K_{q_1 , q_2} g(x)  + O \left(\frac{C_{q_1 , q_2}}{|x|^{d -2+ \frac{\gamma}{4(d-2)}}} \right).
\end{equation}
Before proving the expansion~\eqref{eq:TV03114}, we record a property of the function $g$: by using standard estimates on the Green's function $G$, it can be estimated by the formula
\begin{equation} \label{eq:TV04094}
    \left| g(\kappa) \right| \leq \sum_{z_2  \in \Zd} \left| \nabla_i G(z_2)  \nabla_j G(z_2 + \kappa) \right|  \leq C \sum_{z_2  \in \Zd} \frac{1}{|z_2|^{d-1}} \frac{1}{|z_2 + \kappa|^{d-1}}  \leq  \frac{C}{|\kappa|^{d-2}}.
\end{equation}
The gradient of $g$ can be bounded from above according to the following estimate
\begin{equation} \label{eq:TV03324}
    \left| \nabla g(\kappa) \right| \leq \sum_{z_2  \in \Zd} \left| \nabla_i G(z_2) \nabla \nabla_j G(z_2 + \kappa) \right|  \leq C \sum_{z_2  \in \Zd} \frac{1}{|z_2|^{d-1}} \frac{1}{|z_2 + \kappa|^{d}}  \leq  \frac{C}{|\kappa|^{d-1}}.
\end{equation}
To prove the expansion~\eqref{eq:TV03114}, it is sufficient to prove the estimate
\begin{equation} \label{eq:TV03284}
    \left| \sum_{\kappa \in \Zd} \left( g \left( x + \kappa \right) - g(x) \right)\mathcal{E}_{q_1 , q_2}(\kappa) \right| \leq \frac{C_{q_1,q_2}}{|x|^{d-2+\frac{\gamma}{4(d-2)}}}.
\end{equation}
We split the space into three regions:
\begin{itemize}
    \item The ball of center $0$ and radius $|x|/2$. We use that for each point $\kappa \in B(0 , |x|/2)$, one has the estimate $|\kappa + x| \geq |x|/2$, which implies, by~\eqref{eq:TV03324}, the inequality $\left| \nabla g(\kappa) \right| \leq C |x|^{d-1}$. From this estimate, we deduce that, for each $\kappa \in B(0 , |x|/2)$,
    \begin{equation*}
        \left|g \left( x+ \kappa \right) - g(x) \right| \leq |\kappa| \sup_{z \in B(0 , |x|/2)} \left| \nabla g(z) \right| \leq  \frac{C \left| \kappa \right|}{|x|^{d-1}} .
    \end{equation*}
    We then use this estimate to compute the sum
    \begin{align*}
        \left| \sum_{\kappa \in B \left( 0, \frac{|x|}{2}\right)} \left( g \left( x + \kappa \right) - g(x) \right)\mathcal{E}_{q_1 , q_2}(\kappa) \right| & \leq C \sum_{\kappa \in B \left( 0, \frac{|x|}{2}\right)} \frac{|\kappa|}{|x|^{d-1}} \left| \mathcal{E}_{q_1 , q_2}(\kappa) \right|.
    \end{align*}
We partition the ball $B \left( 0, \frac{|x|}{2}\right)$ into dyadic annuli according to the inclusion $B \left( 0, \frac{|x|}{2}\right) \subseteq \cup_{n=0}^{\lfloor \ln_2\left( |x|/2\right) \rfloor} B_{2^{n+1}} \setminus B_{2^{n}}$, where we use the notation $\lfloor \ln_2\left( |x|/2\right) \rfloor$ to denote the floor of the real number $\ln_2\left( |x|/2\right)$. We additionally note that for each integer $n \in \N$ and each point $\kappa \in B_{2^{n+1}} \setminus B_{2^{n}}$, one has the estimate $|\kappa | \leq C 2^{n}$. Together with the estimate~\eqref{app.assumptE} on the error term $\mathcal{E}_{q_1 , q_2}$, we obtain
    \begin{align} \label{eq:TV04454}
        \left| \sum_{\kappa \in B \left( 0, \frac{|x|}{2}\right)} \left( G \left( x - \kappa \right) - G(x) \right)\mathcal{E}_{q_1 , q_2}(\kappa) \right| & \leq C \sum_{\kappa \in B \left( 0, \frac{|x|}{2}\right)} \frac{|\kappa|}{|x|^{d-1}} \left| \mathcal{E}_{q_1 , q_2}(\kappa) \right| \\ 
        & \leq \frac{C}{|x|^{d-1}} \sum_{n = 0}^{\lfloor \ln_2\left( |x|/2\right) \rfloor} \left| \kappa \right| \sum_{\kappa \in B_{2^{n+1}} \setminus B_{2^n} }  \left| \mathcal{E}_{q_1 , q_2}(\kappa) \right| \notag\\
        & \leq \frac{C}{|x|^{d-1}} \sum_{n = 0}^{\lfloor \ln_2\left( |x|/2\right) \rfloor} 2^n 2^{-\gamma n}\notag \\
        & \leq \frac{C}{|x|^{d-1}} 2^{(1-\gamma) \ln_2\left( |x|/2\right) } \notag\\
        & \leq \frac{C}{|x|^{d-2+\gamma}}. \notag
    \end{align}
    \item The ball of center $-x$ and of radius $|x|^{1-\frac{\gamma}{4(d-2)}}$. In this region, we use the estimate~\eqref{eq:TV04094} on the function $g$ and the pointwise bound on the error term $\mathcal{E}_{q_1,q_2}$ stated in~\eqref{app.assumptE} to obtain
    \begin{align} \label{eq:TV04444}
         \left| \sum_{\kappa \in B \left(-x , |x|^{1-\frac{\gamma}{2(d-2)}} \right)} g \left( x + \kappa \right) \mathcal{E}_{q_1,q_2} \left( \kappa \right) \right| & \leq C \sum_{\kappa \in B \left(x , |x|^{1-\frac{\gamma}{2(d-2)}} \right)} \frac{1}{| \kappa - x|^{d-2}} \frac{1}{|\kappa|^{d- \ep}} \\ & \leq \frac{1}{|x|^{d- \ep}} \sum_{\kappa \in B \left(x , |x|^{1-\frac{\gamma}{2(d-2)}} \right)} \frac{1}{| \kappa - x|^{d-2}} \notag \\ & \leq \frac{C}{|x|^{d - 2 +\frac{\gamma}{2(d-2)} - \ep}} \notag\\
         & \leq \frac{C}{|x|^{d - 2 +\frac{\gamma}{4(d-2)}}}, \notag
    \end{align}
    where we used in the second inequality the lower bound $|\kappa| \geq c |x|$, valid for any point $\kappa \in B\left( x , |x|^{1-\frac{\gamma}{2}} \right)$, and the assumption $\ep \leq \frac{\gamma}{4(d-2)}$ in the fourth inequality.
    \item The complementary of the two previous regions, i.e., the set $C := \Zd \setminus \left( B\left(0, \frac{|x|}{2}\right)  \cup B \left(-x , |x|^{1-\frac{\gamma}{2(d-2)}} \right)\right)$.
    By the inequality~\eqref{eq:TV04094}, we have the estimate, for each $\kappa \in C$,
    \begin{equation*}
        \left| g \left( x - \kappa \right) \right| \leq \frac{C}{|x|^{(1-\frac{\gamma}{2(d-2)})(d-2)}}.
    \end{equation*}
    Using the previous estimate and the inclusion $C \subseteq \cup_{n = \lceil \ln_2 |x|/2 \rceil}^\infty \left( B_{2^{n+1}} \setminus B_{2^n} \right)$, one obtains the inequality
        \begin{align} \label{eq:TV04324}
        \left| \sum_{\kappa \in C} \left( g \left( x + \kappa \right) - g(x) \right)\mathcal{E}_{q_1 , q_2}(\kappa) \right| & \leq C \sum_{\kappa \in C } \frac{1}{|x|^{(1-\frac{\gamma}{2(d-2)} )(d-2)}} \left| \mathcal{E}_{q_1 , q_2}(\kappa) \right| \\
        & \leq \frac{C}{|x|^{(1-\frac{\gamma}{2(d-2)} )(d-2)}} \sum_{n = \lceil \ln_2 |x|/2 \rceil}^\infty \sum_{\kappa \in  B_{2^{n+1}} \setminus B_{2^n}} \left| \mathcal{E}_{q_1 , q_2}(\kappa) \right| \notag \\
        & \leq \frac{C}{|x|^{(1-\frac{\gamma}{2(d-2)} )(d-1)}} \sum_{n = \lceil \ln_2 |x|/2 \rceil}^\infty 2^{-n\gamma} \notag \\
        & \leq \frac{C}{|x|^{(1-\frac{\gamma}{2(d-2)} )(d-2)+ \gamma}}. \notag
    \end{align}
    Computing the exponent in the last line of the inequality~\eqref{eq:TV04324} proves the estimate
    \begin{equation} \label{eq:TV04434}
        \left| \sum_{\kappa \in C} \left( G \left( x - \kappa \right) - G(x) \right)\mathcal{E}_{q_1 , q_2}(\kappa) \right| \leq \frac{C}{|x|^{(d-2)+ \frac{\gamma}{2}}}.
    \end{equation}
\end{itemize}
Combining the estimates~\eqref{eq:TV04454},~\eqref{eq:TV04444} and~\eqref{eq:TV04434} completes the proof of Lemma~\ref{prop:propB1}.


\end{proof}


==> copyandpastebis.tex <==
\chapter{Quantitative homogenization of the Green's matrix} \label{sec:section6}

\section{Statement of the main result}
In this section, we prove the homogenization of the mixed gradient of the Green's matrix; the result we prove is stated below. We first introduce the Green's matrix associated to the homogenized operator $\ahom \Delta$: we denote by $\bar G : \Zd \to \R^{\binom d2 \times \binom d2}$ the fundamental solution of the elliptic system
\begin{equation} \label{def.barGTV145288}
    -\frac{\ahom}{\beta} \Delta \bar G = \delta_0 ~\mbox{in}~\Zd.
\end{equation}

\begin{theorem}[Homogenization of the mixed derivative of the Green's matrix] \label{thm:homogmixedder}
We fix a charge $q_1 \in \mathcal{Q}$ such that $0$ belongs to the support of $n_{q_1}$, let $\mathcal{U}_{q_1}$ be the solution of the Helffer-Sj{\"o}strand equation
\begin{equation} \label{eq:defmathcalU}
\L \mathcal{U}_{q_1} = \cos \left( \phi , q_1\right) q_1 ~\mbox{in}~\Zd \times \Omega,
\end{equation}
and let $\bar G_{q_1} : \Zd \to \R^{\binom d2}$ be the Green's matrix defined by the formula, for each integer $k \in \left\{ 1 , \ldots , \binom d2 \right\}$,
\begin{equation*}
    \bar G_{q_1, k} = \sum_{1 \leq i \leq d} \sum_{1 \leq j\leq \binom d2} \left\langle \cos \left( \phi , q_1\right) \left( n_{q_1} , \di^* l_{e_{ij}} + \di^* \chi_{ij} \right)   \right\rangle_{\mu_\beta} \nabla_i \bar G_{kj}.
\end{equation*}
There exist an inverse temperature $\beta_0 := \beta_0(d) <\infty$, an exponent $\gamma := \gamma(d) >0$ and a constant $C_{q_1}$ which satisfies the estimate
$\left| C_{q_1} \right| \leq  C \left\| q_1 \right\|_{L^1}^{k}$ for some $C := C(d) <\infty$ and $k := k(d) < \infty$, such that for each $\beta \geq \beta_0$ and each radius $R \geq 1$, one has the inequality
\begin{equation} \label{eq:TV19253}
    \left\| \nabla \mathcal{U}_{q_1} - \sum_{1 \leq i \leq d} \sum_{1 \leq j\leq \binom d2} \left( e_{ij} + \nabla \chi_{ij}\right) \nabla_i \bar G_{q_1, j}\right\|_{\underline{L}^2 \left( A_R , \mu_\beta \right)} \leq \frac{C_{q_1} \beta}{R^{d + \gamma}}.
\end{equation}
\end{theorem}

\begin{remark}
Since the codifferential $\di^*$ is a linear functional of the gradient, the map $\di^* \chi_{ij}$ is well-defined even if we have only defined the gradient of the infinite-volume corrector: we have the formula $\di^* \chi_{ij} :=  L_{2, \di^*} \left( \nabla \chi_{ij} \right)$.
\end{remark}

\begin{remark}
We recall the definition of the annulus $A_R := B_{2R} \setminus B_R$. The volume of the annulus $A_R$ is of order $R^d$.
\end{remark}

\begin{remark} \pdcomment{rephrase and improve + solve the question of the dependence in the inverse temperature}
 The maps $(x , \phi) \to \left( e_{ij} + \nabla \chi_{ij} \right)$ and $x \to \nabla_i \bar G_{q_1}$ are valued in $\R^{d \times \binom d2}$ and $\R^{\binom d2 \times \binom d2}$ respectively; the product $\left( e_{ij} + \nabla \chi_{ij} \right) \nabla_i \bar G_{q_1}$ is valued in $\R^{d \times \binom d2}$. There is an underlying scalar product between the two terms to make the notation meaningful. We do not introduce a specific notation for the scalar product to simplify the equations. 
\end{remark}

\iffalse \begin{remark}
We allow the constant $C_{q_1}$ to depend on the constant $q_1$. The point of the argument is to use this result in the proof of Theorem~\ref{t.main} by multiplying the left side of the inequality~\eqref{eq:TV19253} by the term $z \left( \beta , q\right)$ to sum over all the charges $q_1 \in \mathcal{Q}$ (under the condition that $0$ belongs to the support of the charge). Since, by the estimate, the coefficient $z \left( \beta , q\right)$ decays exponentially fast in the $L^1$-norm of the charge $q_1$, we can allow the constant $C_{q_1}$ to grow algebraically fast in the $L^1$-norm of the charge $q_1$ and this growth will be absorbed by the exponential decay of the coefficient $z \left( \beta , q\right)$.
\end{remark} \fi

\begin{remark}
Since the the form $q_1$ can be written $\di n_{q_1}$, we expect the two gradients $\nabla \mathcal{U}_{q_1}$ and $\nabla \bar G_{q_1}$ to behave like mixed derivatives of the Green's matrix, i.e., they should be of order $R^{-d}$ in the annulus $A_R$. The proposition asserts that the difference between the two terms $\nabla_i \mathcal{G}$ and $\sum_{i,j} \left( e_{ij} + \nabla \chi_{ij} \right) \nabla_i \bar G$ is quantitatively smaller than the typical size of the two terms considered separately.
\end{remark}

\section{Outline of the argument}

The strategy of the proof of Theorem~\ref{thm:homogmixedder} relies on a classical strategy in homogenization: the two-scale-expansion. The proofs presented in the chapter make essentially use of two ingredients established in Chapters 5 and 6:
\begin{itemize}
    \item The quantitative sublinearity of the finite-volume corrector and the estimate on the $H^{-1}$-norm of the flux stated in Proposition~\ref{prop:prop5.25} of Chapter 6;
    \item The $C^{0 , 1-\ep}$-regularity theory established in Chapter~\ref{section:section4}.
\end{itemize}
We now give an outline of the proof of Theorem~\ref{thm:homogmixedder}. The argument is split into two subsections:
\begin{itemize}
    \item In Section~\ref{sec:section6.1}, we perform the two-scale expansion and obtain a result of homogenization for the gradient of the Green's matrix as stated in Proposition~\ref{prop:prop6.1};
    \item In Section~\ref{sec:section6.2}, we use the result of Proposition~\ref{prop:prop6.1} and perform the two-scale expansion a second time to obtain the quantitative homogenization of the mixed derivative of the Green's matrix stated in Theorem~\ref{thm:homogmixedder}.
\end{itemize}

\subsection{Homogenization of the gradient of the Green's matrix}
In Section~\ref{sec:section6.1}, we prove the homogenization of the gradient of the Green's matrix stated in Proposition~\ref{prop:prop6.1} below.

\begin{proposition}[Homogenization of the Green's matrix] \label{prop:prop6.1}
Let $\mathcal{G}$ be the Green's matrix associated to the Helffer-Sj{\"o}strand equation
\begin{equation} \label{def:GreenGf19}
    \mathcal{L}  \mathcal{G} =  \delta_0 \hspace{3mm} \mbox{in} \hspace{3mm} \Zd \times \Omega.
\end{equation}
There exist  an inverse temperature $\beta_0(d) < \infty$, an exponent $\gamma := \gamma(d) > 0$ and a constant $C:=C(d) < \infty$ such that for any $\beta > \beta_0$, any radius $R \geq 1$, any integer $i \in \{ 1 , \ldots , d \}$, one has the estimate
\begin{equation} \label{eq:TVmainprop6.2}
\left\| \nabla_i \mathcal{G} - \sum_{i,j} \left( e_i + \nabla \chi_{ij} \right) \nabla_i \bar G \right\|_{\underline{L}^2 \left(A_R,  \mu_\beta\right)} \leq C R^{ 1 - d - \gamma}.
\end{equation}
\end{proposition}

\iffalse \begin{remark}
We expect the gradient of the function $\mathcal{G}$ to behave like the gradient of the standard Green's matrix; in particular, it should be of order $R^{1-d}$ in the annulus $A_R$. The proposition asserts that the difference between the two terms $\nabla_i \mathcal{G}$ and $\sum_{i,j} \left( e_i + \nabla \chi_{ij} \right) \nabla_i \bar G $ is quantitatively smaller than the typical size of the two terms taken separately.
\end{remark} \fi

The argument relies on a two-scale expansion. To set up the argument, we first select an inverse temperature $\beta$ large enough, depending only on the dimension $d$, such that the quantitative sublinearity of the finite-volume corrector and of its flux stated in Proposition~\ref{prop:prop5.25} hold with exponent $\alpha > 0$. Following the argument explained at the beginning of Section~\ref{sec:section5.4}, we can choose the parameter $\beta$ large enough so that all the results presented in Chapter~\ref{section:section4} pertaining to the $C^{0,1-\ep}$-regularity theory for the Helffer-Sj{\"o}strand operator $\mathcal{L}$ are valid with a regularity exponent $\ep$ which is small compared to the exponent $\alpha$ (we assume for instance that the ratio between $\ep$ and $\alpha$ is smaller than $100d^2$). We also fix an exponent $\delta$ which is both larger than $\ep$ and smaller than $\alpha$ and corresponds to the size of a mesoscopic boundary layer which needs to be removed in the argument (we assume for instance that the ratios between the exponents $\alpha$ and $\delta$ and between the exponents $\ep$ and $\delta$ are both smaller than $10d$). To summarize, we have three exponents in the argument, which can be ordered by the following relations
\begin{equation} \label{eq:TVexpord}
    0 < \underbrace{\ep}_{\mathrm{regularity}} \ll \underbrace{\delta}_{\mathrm{boundary}\, \mathrm{layers}}  \ll  \underbrace{\alpha}_{\mathrm{homogenization}}.
\end{equation}
We additionally assume that the exponents $\ep$, $\delta$ and $\alpha$ are chosen in a way that they depend only on the dimension $d$. The exponent $\gamma$ in the statement of Proposition~\ref{prop:prop6.2} depends only $\ep$, $\delta$ and $\alpha$ (and thus only on the dimension $d$).

We now give an outline of the proof of the inequality~\eqref{eq:TVmainprop6.2}; the details can be found in Step 1 of the proof of Proposition~\ref{prop:prop6.2}. The first step of the argument is to approximate the Green's matrices $\mathcal{G}$ and $\bar G$; the main issue is that the spatial Dirac function $\delta_0$ in the definitions of the Green's matrices $\mathcal{G}$ in~\eqref{def:GreenGf19} and $\bar G$ in~\eqref{def.barGTV145288} is too singular and causes some problems in the analysis. To remedy this issue, we replace the Dirac function $\delta_0$ by a smoother function and make use of the boundary layer exponent $\delta$: we let $\rho_\delta$ be a discrete function from $\Zd$ to $\R^{\binom d2 \times \binom d2}$, we denote its components by $\left( \rho_{\delta, ij} \right)_{1 \leq i , j \leq \binom d2}$ and assume that they satisfy the four properties
\begin{equation} \label{prop.rhodelta}
\supp \rho_\delta \subseteq B_{R^{1 - \delta}}, ~ 0 \leq \rho_{\delta, ij}  \leq C R^{-(1-\delta) d } , ~\sum_{x \in \Zd} \rho_{\delta, ij}(x) = \indc_{\{i=j\}}, ~\mbox{and} ~\forall k \in \N, ~\left| \nabla^k \rho_{\delta, ij} \right| \leq \frac{C}{R^{(d + k)(1 - \delta)}},
\end{equation}
and define the functions $ \mathcal{G}^\delta : \Zd \times \Omega \to \R^{\binom d2 \times \binom d2}$ and $\bar G_\delta:  \Zd  \to \R^{\binom d2 \times \binom d2}$ to be the solution of the systems
\begin{equation} \label{def:GdeltaGhomdelta}
    \L \mathcal{G}_\delta = \rho_\delta ~\mbox{in} ~\Omega \times \Zd, \hspace{5mm} - \frac{\ahom}{\beta} \Delta \bar G_\delta =  \rho_\delta ~\mbox{in} ~\Zd.
\end{equation}
We then prove, by using the $C^{0,1-\ep}$-regularity theory established in Section~\ref{section3.4} of Chapter 5, that the functions $\mathcal{G}_\delta$, $\bar G_\delta$ are good approximations of the functions
$\mathcal{G}_\delta$, $\bar G_\delta$ respectively. This is the subject of Lemma~\ref{prop:prop6.2} where we prove the estimates
\begin{equation} \label{eq:TV0421}
    \left\| \nabla \mathcal{G}_\delta - \nabla \mathcal{G} \right\|_{L^\infty \left( A_R , \mu_\beta \right)} \leq CR^{1 - d - \gamma} \hspace{5mm} \mbox{and} \hspace{5mm} \left\| \nabla \bar G_\delta - \nabla \bar G \right\|_{L^\infty \left( A_R , \mu_\beta \right)} \leq CR^{1 - d - \gamma}.
\end{equation}
By the estimates~\eqref{eq:TV0421}, we see that to prove Proposition~\ref{prop:prop6.2} it is sufficient to prove the inequality, for each integer $i \in \{1 , \ldots , d \}$,
\begin{equation} \label{eq:TV1013}
    \left\| \nabla_i \mathcal{G}_\delta - ( e_i + \nabla \chi_{ij}) \nabla_i \bar G_\delta \right\|_{\underline{L}^2 \left( A_R , \mu_\beta \right)} \leq C R^{1 - d - \gamma}.
\end{equation}
We now sketch the proof of the inequality~\eqref{eq:TV1013}. We let $m$ be the integer uniquely defined by the inequalities $3^m \leq R^{1 + \delta} < 3^{m+1}$, consider the collection finite-volume correctors $\left( \chi_{m , i} \right)_{i = 1 , \ldots, d}$. We then define the two-scale expansion $\mathcal{H}$ according to the formula
\begin{equation} \label{def.Ho2sc}
    \mathcal{H}_\delta := \bar G_\delta + \sum_{i= 1}^d \left(\nabla_i \bar G_\delta\right) \chi_{m , i}.
\end{equation}
The strategy is then to compute the value of $\mathcal{L} \mathcal{H}$ by using the explicit formula on $\mathcal{H}$ stated in~\eqref{def.Ho2sc} and to prove that it is quantitatively close to the map $\rho_\delta$ in the correct functional space; precisely, we prove the $H^{-1}$-estimate
\begin{equation} \label{eq:insertineq}
    \left\| \mathcal{L} \mathcal{H}_\delta - \rho_\delta \right\|_{\underline{H}^{-1} \left( B_{R^{1+\delta} , \mu_\beta} \right)} \leq C R^{1-d  - \gamma}.
\end{equation}
Obtaining this result relies on the quantitative behavior of the corrector and of the flux established in Proposition~\ref{prop:prop5.25}. Once one has a good control over the $H^{-1}$-norm of $\mathcal{L} \mathcal{H} - \rho_\delta$, the inequality~\eqref{eq:TV1013} can be deduced from the following two arguments:
\begin{itemize}
    \item We use that the function $\mathcal{G}_\delta$ satisfies the equation $\mathcal{L} \mathcal{G}_\delta = \rho_\delta$ to obtain that the $H^{-1}$-norm of the term $\mathcal{L} \left( \mathcal{H} - \mathcal{G}_\delta \right)$ is small. We then introduce a cutoff function $\eta : \Zd \to \R$ which satisfies:
    \begin{equation*}
    \supp \eta \subseteq A_R, ~ 0 \leq \rho \leq 1 , ~\eta = 1 ~\mbox{on}~ \left\{ x \in \Zd \, : \, 1.1 R \leq |x| \leq 1.9 |x| \right\}, ~\mbox{and} ~\forall k \in \N, ~\left| \nabla^k \eta \right| \leq \frac{C}{R^k},
\end{equation*}
    and use the function $\eta \left( \mathcal{H} - \mathcal{G}_\delta \right)$ as a test function in the definition of the $H^{-1}$-norm of the inequality~\eqref{eq:insertineq}. We obtain that the $L^2$-norm of the difference $\left( \nabla \mathcal{H} - \nabla \mathcal{G}_\delta \right)$ is small (the cutoff function is used to ensure that the function $\eta \left( \mathcal{H} - \mathcal{G}_\delta \right)$ is equal to $0$ on the boundary of the ball $B_{R^{1+\delta}}$ and can thus be used as a test function). The precise estimate we obtain is written below
    \begin{equation} \label{eq:TV15488de}
        \left\| \nabla \mathcal{H}_\delta - \nabla \G_\delta \right\|_{L^2 \left( \Zd , \mu_\beta \right)} \leq CR^{\frac d2 + 1 - d - \gamma};
    \end{equation}
    \item By using the formula~\eqref{def.Ho2sc}, we can compute an explicit formula for the gradient of the two-scale expansion $\mathcal{H}$. We then use the quantitative sublinearity of the corrector stated in Proposition~\ref{prop:prop5.25} and the property of the gradient of the infinite volume corrector stated in Proposition~\ref{prop5.26} to deduce that the $L^2$-norm of the difference $\nabla \mathcal{H}_\delta - \sum_{i,j} ( e_i + \nabla \chi_{ij}) \nabla_i \bar G$ is small; the precise result we obtain is the following
    \begin{equation} \label{eq:TV09109}
        \left\| \nabla \mathcal{H}_\delta - \sum_{i,j} ( e_i + \nabla \chi_{ij}) \nabla_i \bar G \right\|_{L^2 \left( \Zd  \mu_\beta \right)} \leq C R^{\frac d2 + 1 - d - \gamma}.
    \end{equation}
\end{itemize}
The inequality~\eqref{eq:TV1013} is then a consequence of the inequalities~\eqref{eq:TV15488de} and~\eqref{eq:TV09109}.

\subsection{Homogenization of the mixed derivative of the Green's matrix} \label{sec3.2chap60851}
In Section~\ref{sec:section6.2}, we use Proposition~\ref{prop:prop6.1} to prove Theorem~\ref{thm:homogmixedder}. The argument is decomposed into three steps:
\begin{itemize}
    \item In Step 1, we use Proposition~\ref{prop:prop6.1} and the symmetry of the Helffer-Sj{\"o}strand operator $\mathcal{L}$ to prove the inequality in expectation
    \begin{equation} \label{eq:TV15057}
    \left( R^{-d} \sum_{z\in A_R} \left| \left\langle \mathcal{U}_{q_1}(z, \cdot ) \right\rangle_{\mu_\beta} - \bar G_{q_1}(z) \right|^2 \right)^\frac 12 \leq \frac{C}{R^{d - 1+\gamma}}.
    \end{equation}
     \iffalse
    The inequality~\eqref{eq:TV15057} states that the function $z \mapsto \left\langle \mathcal{U}_{q_1}(z) \right\rangle_{\mu_\beta}$ is close to the function $\bar G_{q_1}$ in the $\underline{L}^2(A_R)$-norm.
   
     The functions $\mathcal{U}_{q_1}$ and $\bar G_{q_1}$ have a large-scale behavior similar to the one of a gradient of the Green's function (and decay like $R^{1-d}$).
     \fi
    \item In Step 2, we prove the variance estimate, for each point $z \in \Zd$,
    \begin{equation} \label{eq:TV15087}
         \var \left[ \mathcal{U}_{q_1}(z, \cdot) \right] \leq \frac{C_{q_1}}{|z|^{2d-2\ep}}.
    \end{equation}
    Since we expect the function $z \mapsto \mathcal{U}_{q_1}(z)$ to decay like $|z|^{1-d}$; its variance should be of order $|z|^{2-2d}$. The estimate~\eqref{eq:TV15087} states that the variance of the random variable $\phi \to \mathcal{U}_{q_1}(z, \phi)$ is (quantitatively) smaller than its size; this means that the random variable $\mathcal{U}_{q_1}(z)$ contracts on its expectation. We then use the result established in Step 1 to obtain refine the result: since by~\eqref{eq:TV15057}, one knows that the expectation of $\mathcal{U}_{q_1}(z)$ is close to the function $\bar G_{q_1}$, one deduces that the function $\mathcal{U}_{q_1}$ is close to the function $\bar G_{q_1}$ in the $\underline{L}^2(A_R, \mu_\beta)$-norm. The precise estimate we obtain is the following
    \begin{equation} \label{eq:TV08289}
    \left\| \mathcal{U}_{q_1} - \bar G_{q_1} \right\|_{\underline{L}^2 \left( A_R , \mu_\beta \right)} \leq \frac{C_{q_1}}{R^{d-1-\gamma}}.
    \end{equation}
    The proof of the inequality~\eqref{eq:TV15087} does not rely on tools from stochastic homogenization; we appeal to the Brascamp-Lieb inequality and used the differentiated Helffer-Sj{\"o}strand introduced in Section~\ref{sec.section4.5} of Chapter REF.
    \item In Step 3, we prove the estimate~\eqref{eq:TV19253}, the proof is similar to the argument presented in the proof of Proposition~\ref{prop:prop6.1} and relies on a two-scale expansion. The argument is split into three substeps. We first define the two-scale expansion $\mathcal{H}_{q_1}$ by the formula
    \begin{equation} \label{eq:defHq12sc5}
    \mathcal{H}_{q_1} := \bar G_{q_1} + \sum_{i,j} \nabla_i \bar G_{q_1} \chi_{m,i}.
    \end{equation}
    We can then use that the function $\bar G_{q_1}$ is solution to the homogenized equation $\ahom \Delta \bar G_{q_1} = 0$ in the annulus $A_R$ to prove that the $\underline{H}^{-1}\left(A_R , \mu_\beta \right)$-norm of the term $ \L \mathcal{H}_{q_1}$ over the annulus $A_R$ is small; this is the subject of Substep 3.1 where we prove
    \begin{equation} \label{eq:TV10438}
        \left\| \L \mathcal{H}_{q_1} \right\|_{\underline{H}^{-1}\left(A_R , \mu_\beta \right)} \leq \frac{C_{q_1}}{R^{d + \gamma}}.
    \end{equation}
    The proof is essentially a notational modification of the proof of the estimate~\eqref{eq:insertineq} (and is even simpler since we do not have to take into account the exponent $\delta$ and the function $\rho_\delta$). Once we have proved that the inequality~\eqref{eq:TV10438}, we use that the function $\mathcal{U}_{q_1}$ satisfies the identity $\L \mathcal{U}_{q_1} = 0$ in the set $A_R \times \Omega$ to deduce that the $\underline{H}^{-1}\left(A_R , \mu_\beta \right)$-norm of the term $\L \left( \mathcal{H}_{q_1} - \mathcal{U}_{q_1}\right) = \L  \mathcal{H}_{q_1}$ is small. We then introduce the annulus $A_R^1 := \left\{ x \in \Zd \, : \, 1.1 R \leq |x| \leq 1.9 R \right\}$ and a cutoff function $\eta$ satisfying the properties:
\begin{equation*}
    \supp \eta \subseteq A_R, ~ 0 \leq \rho \leq 1 , ~\eta = 1 ~\mbox{on}~ A_R^1, ~\mbox{and} ~\forall k \in \N, ~\left| \nabla^k \eta \right| \leq \frac{C}{R^k}.
\end{equation*}
We note that the choice of the values $1.1$ and $1.9$ in the definition of the annulus $A_R^1$ is arbitrary; any pair of real numbers belonging to the interval $(1,2)$ would be sufficient for our purposes. We then use the function $\eta \left( \mathcal{H}_{q_1} - \mathcal{U}_{q_1} \right)$ as a test function in the definition of the $\underline{H}^{-1}\left(A_R , \mu_\beta \right)$-norm of the term $\L \left( \mathcal{H}_{q_1} - \mathcal{U}_{q_1}\right)$ and use the $\underline{L}^2 \left( A_R , \mu_\beta \right)$-estimate~\eqref{eq:TV08289} to obtain that the $\underline{L}^2 \left( A_R^1 , \mu_\beta \right)$-norm of the difference $\nabla \mathcal{H}_{q_1} - \nabla \mathcal{U}_{q_1}$ is small. This is the subject of Substep 3.2 where we prove
\begin{equation} \label{eq:TV09249}
    \left\| \nabla \mathcal{U}_{q_1} - \nabla \mathcal{H}_{q_1} \right\|_{\underline{L}^2 \left( A_R^1 , \mu_\beta \right)} \leq \frac{C_{q_1}}{R^{d+\gamma}}.
\end{equation}
\item Step 4 is the conclusion of the argument, we use the explicit formula for the two-scale expansion $\mathcal{H}_{q_1}$ given in~\eqref{eq:defHq12sc5}, the quantitative sublinearity of the corrector stated in Proposition~\ref{prop:prop5.25} and the quantitative estimate for the difference of the finite and infinite-volume gradient of the corrector stated in Proposition~\ref{prop5.26} to prove the estimate
\begin{equation} \label{eq:TV12347}
    \left\| \nabla \mathcal{H}_{q_1} - \sum_{i,j} \left( e_i + \nabla \chi_{ij} \right) \nabla_i \bar G_{q_1} \right\|_{\underline{L}^2 \left( A_R , \mu_\beta \right)} \leq \frac{C_{q_1}}{R^{d+ \gamma}}.
\end{equation}
The argument is a notational modification of the one used to prove~\eqref{eq:defHq12sc5}. We finally combine the estimates~\eqref{eq:TV09249} and~\eqref{eq:TV12347} to obtain the estimate~\eqref{eq:TV19253} and complete the proof of Theorem~\ref{thm:homogmixedder}.
\end{itemize}



\medskip


\section{Two-scale expansion and homogenization of the gradient of the Green's matrix} \label{sec:section6.1}

This section is devoted to the proof of Proposition~\ref{prop:prop6.1}. We first collect some preliminary results in Section~\ref{premest3.1chap6} and then prove the result in Sections~\ref{sec3.2chap60851},~\ref{sec3.3chap60851} and~\ref{sec3.4chap60851} following the outline given in Section~\ref{sec3.2chap60851}.

\pd{Discussion about the exponent $\gamma$}  To ease the notation, we allow the value of the exponent $\gamma$ to vary from line to line and do not keep track of its value; the only important property is that it should always remain strictly larger than $0$.

\subsection{Preliminary estimates} \label{premest3.1chap6} In this section, we collect and prove some preliminary estimates which are used in the proof of Proposition~\ref{prop:prop6.1}.

\begin{proposition} \label{prop:prop6.2}
The following properties hold:
\begin{itemize}
\item There exists an exponent $\gamma_\delta > 0$ such that one has the estimates
\begin{equation} \label{eq:TV20383}
\left\|\nabla \G (x, \cdot) - \nabla \G_\delta(x , \cdot ) \right\|_{L^\infty \left(A_R,  \mu_\beta \right)} \leq \frac{C}{R^{d-1 + \gamma_\delta}} \hspace{5mm} \mbox{and} \hspace{5mm}  \left\|\nabla \bar G - \nabla \bar G_\delta \right\|_{L^\infty (A_R)} \leq \frac{C}{R^{d-1 + \gamma_\delta}};
\end{equation}
\item The Green's matrix $\G_\delta$ satisfies the following $L^\infty$-estimates
\begin{equation} \label{eq:TV090191}
    \left\| \G_\delta  \right\|_{L^\infty \left( \Zd , \mu_\beta  \right)} \leq  \frac{C}{R^{(1-\delta) (d-2) }} ~\mbox{and}~ \left\| \nabla \G_\delta  \right\|_{L^\infty \left( \Zd , \mu_\beta  \right)} \leq \frac{C}{R^{(1-\delta) (d-1 - \ep) }},
\end{equation}
as well as the estimates
\begin{equation} \label{eq:TVdes13370}
    \left\| \G_\delta \right\|_{L^\infty \left( A_{R^{1+\delta}}, \mu_\beta  \right)} \leq \frac{C}{R^{(1+\delta)(d-2)}}  ~\mbox{and}~  \left\| \nabla \G_\delta \right\|_{L^\infty \left( A_{R^{1+\delta}}, \mu_\beta  \right)} \leq \frac{C}{R^{(1+\delta)(d-1- \ep)}};
\end{equation}
\item The homogenized Green's matrix $\bar G_\delta$ satisfies the regularity estimate, for each integer $k \in \N$,
    \begin{equation} \label{eq:spatregbarGgeq3}
         \left\| \nabla^k \bar G_\delta \right\|_{L^\infty \left( \Zd , \mu_\beta \right)} \leq \frac{C}{R^{(1-\delta)(d-2+k)}},
    \end{equation}
as well as the estimate
        \begin{equation} \label{eq:spatregbarGgeq34}
         \left\| \nabla^k \bar G_\delta \right\|_{L^\infty \left( A_{R^{1+\delta}} , \mu_\beta \right)} \leq \frac{C}{R^{(1+\delta)(d-2+k)}}.
    \end{equation}
\end{itemize}
\end{proposition}


\begin{proof}[Proof of Proposition~\ref{prop:prop6.2}]
The proof relies on the regularity estimates established in Chapter~\ref{section:section4}. We first note that, by definitions of the functions $\G$ and $\G_\delta$, we have the identities 
\begin{equation} \label{eq:TV13219}
    \G \left( x , \phi \right) = \G_1 \left( x , \phi ;0 \right) \hspace{5mm} \mbox{and} \hspace{5mm} \G_\delta \left( x , \phi \right) = \sum_{y \in B_{R^{1-\delta}}} \rho_\delta(y) \G_1\left( x , \phi ; y \right).
\end{equation}
Using that the map $\rho_\delta$ has total mass $1$ and the regularity estimate on the Green's matrix stated in Proposition~\ref{cor:corollary4.14}, we obtain, for each point $x$ in the annulus $A_R$,
\begin{align*}
    \left\| \nabla_x \G (x , \phi ; 0) - \nabla_x \G_\delta (x , \phi ; y) \right\|_{L^\infty \left( \mu_\beta \right)}  & \leq  \sum_{y \in B_{R^{1-\delta}}} \rho_\delta (y) \left\|  \nabla_x \G_1 (x ,  \phi ; 0 ) -  \nabla_x  \G_1 (x , \phi ; y)  \right\|_{L^\infty \left( \mu_\beta \right)} \\
    & \leq R^{1 - \delta} \sup_{y \in B_{R^{1- \delta}}} \left\| \nabla_x \nabla_y \G (x , \phi ; y ) \right\|_{L^\infty \left( \mu_\beta \right)} \\
    & \leq R^{1 - \delta} \sup_{y \in B_{R^{1-\delta}}}|x - y|^{- d - \ep}\\
    & \leq R^{1 - \delta} R^{- d - \ep}.
\end{align*}
 This completes the proof of the estimate~\eqref{eq:TV20383} with the exponent $\gamma_\delta = \delta - \ep$ which is strictly positive by the assumption~\eqref{eq:TVexpord}.
 
The estimate on the homogenized Green's matrix is similar and even simpler since we only have to work with the Green's matrix associated to the discrete Laplacian on $\Zd$ (and not the Helffer-Sj{\"o}strand operator $\L$); we omit the details.

The proof of the inequality~\eqref{eq:TV090191} relies on the estimates on the Green's matrix and its gradient established in Corollary~\ref{cor:cor5.23} of Chapter 5. We use the identity~\eqref{eq:TV13219} and write, for each point $x \in \Zd$,
\begin{align*}
    \left\| \G_\delta \left( x , \cdot \right) \right\|_{L^\infty \left( \mu_\beta \right)}  = \sum_{y \in B_{R^{1-\delta}}} \rho_\delta(y) \left\| \G_1 \left( x , \phi ; y \right)  \right\|_{L^\infty \left( \mu_\beta \right)} \leq \frac{1}{R^{(1-\delta) d }} \sum_{y \in B_{R^{1-\delta}}} \frac{C}{|x- y|^{d-2}} 
    & \leq  \frac{1}{R^{(1-\delta) d }} \sum_{y \in B_{R^{1-\delta}}} \frac{C}{| y|^{d-2}} \\
    & \leq \frac{1}{R^{(1-\delta) (d-2) }}.
\end{align*}
A similar computation shows the bound for the gradient of the Green's matrix and the bounds~\eqref{eq:TVdes13370} in the annulus $A_{R^{1+\delta}}$.

To prove the regularity estimate~\eqref{eq:spatregbarGgeq3}, we use the definition of the map $\bar G_\delta$ given in~\eqref{def:GdeltaGhomdelta} and note that
\begin{equation*}
    -\frac{\ahom}{\beta} \Delta \left(\nabla^k \bar G_\delta \right) = \nabla^k \rho_\delta ~\mbox{in}~\Zd.
\end{equation*}
We then use the the properties of the function $\rho_\delta$ stated in~\eqref{prop.rhodelta} and the standard estimates on the homogenized Green's matrix $\bar G$. We obtain, for each point $x \in \Zd$,
\begin{equation*} 
    \left| \nabla^k \bar G_\delta(x ) \right| \leq \sum_{y \in B_{R^{1-\delta}}} \left|\nabla^k  \rho_\delta(y) \right| \left| \bar G \left( x - y \right) \right|
     \leq \frac{C}{R^{(d+k)(1-\delta)}} \sum_{y \in B_{R^{1-\delta}}} \frac{1}{|x - y|^{d-2}}
     \leq \frac{C}{R^{(1-\delta)(d-2 + k)}}. \notag
\end{equation*}
There only remains to prove the estimate~\eqref{eq:spatregbarGgeq34}. We select a point $x \in A_{R^{1+\delta}}$ and write
\begin{align*} 
    \left| \nabla^k \bar G_\delta(x ) \right| = \left| \sum_{y \in B_{R^{1-\delta}}}   \rho_\delta(y) \nabla^k \bar G \left( x - y \right) \right|
     \leq \sum_{y \in B_{R^{1-\delta}}} \frac{\left|\rho_\delta (y)\right|}{|x - y|^{d-2+k}}
     &\leq \frac{C}{R^{(d+k)(1+\delta)}} \sum_{y \in B_{R^{1-\delta}}} \left|\rho_\delta (y)\right| \notag \\
    & \leq \frac{C}{R^{(1+\delta)(d-2 + k)}}. \notag
\end{align*}
\end{proof}

We have now collected all the necessary preliminary ingredients for the proof of Proposition~\ref{prop:prop6.1} and devote the rest of Section~\ref{sec:section6.1} to its demonstration. 


%We decompose the proof into three steps, following the sketch presented at the beginning of Section~\ref{sec:section6}. We recall that through the proof, the exponent $\gamma$ is a small, strictly positive exponent which may vary from line to line and can be computed explicitly in terms of the values of $\ep$, $\delta$ and $\alpha$; in particular, it depends only on the dimension $d$. We also recall the ordering between the three exponents $\ep$, $\delta$ and $\alpha$ presented in~\eqref{eq:TVexpord}.

\smallskip

\subsection{Estimating the weak norm of $\L \mathcal{H}_{\delta} - \rho_\delta$} \label{sec3.2chap60851}
In this section, we let $\mathcal{H}_\delta$ be the two-scale expansion introduced in~\eqref{def.Ho2sc} and prove that there exists an exponent $\gamma_{\alpha} > 0$ such that
\begin{equation} \label{eq:TV19578}
    \left\| \L \mathcal{H}_{\delta} - \rho_\delta \right\|_{\underline{H}^{-1}\left(B_{R^{1+\delta}} , \mu_\beta \right)} \leq \frac{C}{R^{d-1+\gamma_{\alpha}}}.
\end{equation}

The strategy is to use the explicit formula for the map $\mathcal{H}_{\delta}$ to compute the value of the term $\mathcal{L} \mathcal{H}$. We then prove that its $\underline{H}^{-1}\left(B_{R^{1+\delta}} , \mu_\beta \right)$-norm is small by using the quantitative properties of the corrector stated in Proposition~\ref{prop:prop5.25} of Chapter 6. 
We first write
\begin{equation} \label{eq:TV0957897}
    \L \mathcal{H}_\delta = \underbrace{\Delta_\phi \mathcal{H}_\delta}_{\textnormal{Substep 1.1}} + \underbrace{\frac1{2\beta} \sum_{n \geq 1} \frac{1}{\beta^{\frac n2}} \Delta^{n+1} \mathcal{H}_\delta}_{\textnormal{Substep 1.2}} - \underbrace{\frac1{2\beta} \Delta \mathcal{H}_\delta + \sum_{q \in \mathcal{Q}} \nabla_q^* \cdot \a_q \nabla_q \mathcal{H}_\delta}_{\textnormal{Substep 1.3}}.
\end{equation}
We treat the three terms in the right side in three distinct substeps.

\medskip

\textit{Substep 1.1} 
In this substep, we treat the term $\Delta_\phi \mathcal{H}_{\delta}$. Since the homogenized Green's matrix $\bar G_\delta$ does not depend on the field $\phi$, we have the formula
\begin{equation} \label{eq:mainsub1.1hom}
    \Delta_\phi \mathcal{H}_\delta = \Delta_\phi \bar G_\delta  + \sum_{i,j} \nabla_i \bar G_\delta \left( \Delta_{\phi} \chi_{m,i}\right).
\end{equation}

\medskip


\textit{Sustep 1.2.} In this substep, we study the iteration of the Laplacian of the two-scale expansion. We prove the identity
\begin{equation} \label{eq:TV14557}
 	 \sum_{n \geq 1} \frac{1}{\beta^{\frac n2}} \Delta^{n+1} \mathcal{H}_{\delta} =  \sum_{i,j} \sum_{n \geq 1}  \frac{1}{\beta^{\frac n2}} \nabla_i \bar G_\delta \Delta^{n+1} \chi_{m,i} + R_{\Delta^n},
\end{equation}
where $R_{\Delta^n}$ is an error term which satisfies the $\underline{H}^{-1}\left( B_{R^{1+\delta}} , \mu_\beta \right)$-estimate
\begin{equation}  \label{eq:TV145677}
\left\| R_{\Delta^n} \right\|_{\underline{H}^{-1}\left( B_{R^{1+\delta}}, \mu_\beta \right)} \leq \frac{C}{R^{d-1+\gamma_{\alpha}}}.
\end{equation}
We use the following identity for the iteration of the Laplacian on a product of functions: given two smooth functions $f , g \in \C^\infty \left( \Rd \right)$, we have the identity
\begin{equation} \label{eq:expandLap}
    \Delta^n \left( f g \right) = \sum_{k=0}^{n} \sum_{l = 0}^k \binom{n- k}{l} \left( \nabla^{k} \Delta^l  f  \right) \times \left( \nabla^{k} \Delta^{n- k - l} g \right).
\end{equation}
We note that this formula is valid for continuous functions (with the continuous Laplacian), it can be adapted to the discrete setting by taking into considerations translations of the functions $f$ and $g$. Since this adaptation does not affect the overall strategy of the proof, we ignore this technical difficulty in the rest of the argument and apply the formula~\eqref{eq:expandLap} to the two-scale expansion $\mathcal{H}_{\delta}$ as such. We obtain
\begin{equation} \label{eq:TV11087}
\Delta^n \mathcal{H}_{\delta} = \Delta^n \bar G_\delta + \sum_{i,j} \sum_{k=0}^{n} \sum_{l = 0}^k \binom{n- k}{l} \left( \nabla^{k} \Delta^l  \nabla_i  \bar G_\delta  \right) \times \left( \nabla^{k} \Delta^{n- k - l} \chi_{m,i} \right) .
\end{equation}
We first focus on the term $\Delta^n \bar G_\delta$ in the identity~\eqref{eq:TV11087} and prove that it is small in the $\underline{H}^{-1} \left( B_{R^{1+\delta}} , \mu_\beta \right)$-norm. Using the regularity estimate~\eqref{eq:spatregbarGgeq3}, we have, for each integer $n \geq 2$,
\begin{align} \label{eq:TV14407}
    \left\| \Delta^n \bar G_\delta  \right\|_{\underline{H}^{-1} \left( B_{R^{1+\delta}} , \mu_\beta \right)}  \leq C R^{1+\delta}\left\| \Delta^n \bar G_\delta  \right\|_{\underline{L}^{2} \left( B_{R^{1+\delta}} , \mu_\beta \right)} 
    & \leq  C R^{1+\delta}\left\| \Delta^n \bar G_\delta  \right\|_{L^{\infty} \left( B_{R^{1+\delta}} \right)} \\
    & \leq  \frac{C^{2n} R^{1+\delta}}{R^{(1-\delta)(d - 2 + 2n)}} \notag \\
    & \leq \frac{C^{2n} R^{1+\delta}}{R^{(1-\delta)(d - 2 + 4)}} \notag \\
    & \leq \frac{C^{2n} }{R^{d-1 + \gamma_1}}, \notag
\end{align}
where we have set $\gamma_1 := 2 + \delta (d+1) > 0$.

Using the regularity estimate~\eqref{eq:spatregbarGgeq3} a second time, we can estimate the terms of the right side of the identity~\eqref{eq:TV11087} with more than 3 derivatives on the homogenized Green's matrix $\bar G_\delta$. We obtain the following inequality: for each integer $i \in \{ 1 , \ldots, d\}$, and each pair of integers $k, l \in \{ 1 , \ldots, d \}$ such that $l \leq n-k$ and $k + 2 l \geq 2$,
\begin{align} \label{eq:TV11047}
\lefteqn{ \left\| \left( \nabla^{k} \Delta^l  \nabla_i \bar G_\delta  \right) \times \left( \nabla^{k} \Delta^{n- k - l} \chi_{m,i} \right) \right\|_{\underline{H}^{-1}(B_{R^{1+\delta}}, \mu_\beta)} } \qquad & \\  & \leq C R^{1+\delta} \left\| \left( \nabla^{k} \Delta^l  \nabla_i \bar G_\delta \right) \times \left( \nabla^{k} \Delta^{n- k - l} \chi_{m,i} \right) \right\|_{\underline{L}^2(B_{R^{1+\delta}}, \mu_\beta)}\notag \\
 & \leq  C R^{1+\delta} \left\|  \nabla^{k} \Delta^l  \nabla_i \bar G_\delta \right\|_{L^\infty \left( B_{R^{1+\delta}}  \right)} \times \left\|  \nabla^{k} \Delta^{n- k - l} \chi_{m,i}  \right\|_{\underline{L}^2(B_{R^{1+\delta}}, \mu_\beta)} \notag \\
 & \leq \frac{C^{k + 2l} R^{1+\delta}}{R^{(1-\delta)(d-1+2l + k)}} \left\|  \nabla^{k} \Delta^{n- k - l} \chi_{m,i}  \right\|_{\underline{L}^2(B_{R^{1+\delta}}, \mu_\beta)}. \notag
 \end{align}
 We use that the discrete operator $ \nabla^{k} \Delta^{n- k - l}$ is bounded in the space $L^2 \left( B_{R^{1+\delta}} \right)$ and Proposition~\ref{prop:prop5.25} of Chapter 6 to estimate the $L^2$-norm of the corrector. We obtain
 \begin{equation} \label{eq:TV11037}
      \left\|  \nabla^{k} \Delta^{n- k - l} \chi_{m,i}  \right\|_{\underline{L}^2(B_{R^{1+\delta}}, \mu_\beta)} \leq C^{2n - 2l} \left\|   \chi_{m,i}  \right\|_{\underline{L}^2(B_{R^{1+\delta}}, \mu_\beta)} \leq  C^{2n - 2l} R^{(1+\delta)(1-\alpha)}.
 \end{equation}
 Putting the estimate~\eqref{eq:TV11047} and~\eqref{eq:TV11037} together and using the inequality $3 \leq 2l+k \leq 2n$, we deduce that
 \begin{equation} \label{eq:TV14387}
       \left\| \left( \nabla^{k} \Delta^l  \nabla_i \bar G_\delta  \right) \times \left( \nabla^{k} \Delta^{n- k - l} \chi_{m,i} \right) \right\|_{\underline{H}^{-1}(B_{R^{1+\delta}}, \mu_\beta)} \leq  \frac{C^{2n} R^{1+\delta}}{R^{(1-\delta)(d+2)}} R^{(1+\delta)(1-\alpha)} \leq \frac{C^{2n}}{R^{d-1 + \gamma_{1}}},
 \end{equation}
where we have set $\gamma_{1} := 1 + \alpha - \alpha \delta + \delta \left( d-1 \right) + \delta >0$.

We then estimate the $H^{-1}$-norm of the terms corresponding to the parameters $k=1$ and $l=0$ in the sum in the right side of the identity~\eqref{eq:TV11087}. To estimate it, we select a function $h \in H^1_0 \left(B_{R^{1+\delta}}, \mu_\beta \right)$ such that $\left\| h \right\|_{\underline{H}^1 \left( B_{R^{1+\delta}}, \mu_\beta \right)}\leq 1$. We use the function $h$ as a test function, perform an integration by parts in the first line, use the Cauchy-Schwarz inequality in the second line and the continuity of the Laplacian in the third line. We obtain 
\begin{align} \label{eq:TV14097}
\lefteqn{\frac{1}{R^{(1+\delta)d}}\sum_{x \in B_{R^{1+\delta}}} \left\langle \left( \nabla \nabla_i \bar G_\delta \left( x , \cdot \right)  \right) \times \left( \nabla \Delta^{n- 1} \chi_{m,i} (x , \cdot ) \right)  h(x , \cdot)  \right\rangle_{\mu_\beta} } \qquad & \\ 
			& = \frac{1}{R^{(1+\delta)d}} \sum_{x \in B_{R^{1+\delta}}} \left\langle \chi_{m,i} (x , \cdot )   \nabla \Delta^{n- 1} \left( \left( \nabla \nabla_i \bar G_\delta \left( x , \cdot \right)  \right) h  (x , \cdot )\right) \right\rangle_{\mu_\beta} \notag \\
			& \leq  \left\| \chi_{m,i} \right\|_{L^2 \left( B_{R^{1+\delta}}, \mu_\beta \right) }   \left\| \nabla \Delta^{n- k}\left( \nabla \nabla_i \bar G_\delta  h \right) \right\|_{\underline{L}^2 \left( B_{R^{1+\delta}} , \mu_\beta \right)} \notag \\
			& \leq C^{n} \left\| \chi_{m,i} \right\|_{L^2 \left( B_{R^{1+\delta}}, \mu_\beta \right) }   \left\| \nabla \left( \nabla \nabla_i \bar G_\delta  h \right) \right\|_{\underline{L}^2 \left( B_{R^{1+\delta}} , \mu_\beta \right)} .\notag
\end{align}
Using the regularity estimate for the homogenized Green's matrix stated in~\eqref{eq:spatregbarGgeq3} and the inequality $\left\| h \right\|_{\underline{L}^2 \left(B_{R^{1+\delta}} , \mu_\beta \right)} \leq C R^{1+\delta}$ (which is a consequence of the assumption $\left\| h \right\|_{\underline{H}^1 \left(B_{R^{1+\delta}} , \mu_\beta \right)} \leq 1$ and the Poincar\'e inequality), we obtain
\begin{align} \label{eq:TV14047}
    \left\| \nabla \left(\left( \nabla \nabla_i \bar G_\delta \right) h \right) \right\|_{\underline{L}^2 \left( B_{R^{1+\delta}} , \mu_\beta \right)} & \leq \left\| \nabla^3 \bar G_\delta h \right\|_{\underline{L}^2 \left( B_{R^{1+\delta}} , \mu_\beta \right)} + \left\| \nabla^2 \bar G_\delta  \nabla h \right\|_{\underline{L}^2 \left( B_{R^{1+\delta}} , \mu_\beta \right)} \\
    & \leq  \frac{CR^{1+\delta}}{R^{\left( 1-\delta \right)\left(d + 1 \right)}}  +  \frac{C}{R^{\left( 1-\delta \right)d}} \notag \\ &
    \leq \frac{C}{R^{d - \delta (d+2)}}. \notag
\end{align}
We then combine the estimate~\eqref{eq:TV14097} with the inequality~\eqref{eq:TV14047} and the quantitative sublinearity of the corrector stated in Proposition~\ref{prop:prop5.25} of Chapter 6. We obtain
\begin{equation} \label{eq:TV14397}
    \frac{1}{R^{(1+\delta)d}}\sum_{x \in B_{R^{1+\delta}}} \left\langle \left( \nabla \nabla_i \bar G_\delta \left( x , \cdot \right)  \right) \times \left( \nabla \Delta^{n- 1} \chi_{m,i} (x , \cdot ) \right)  h(x , \cdot)  \right\rangle_{\mu_\beta} \leq \frac{C^n R^{\left(1+\delta\right)(1 - \alpha) }}{R^{d - \delta (d+2)}} \leq  \frac{C^n}{R^{d - 1 + \gamma_{\alpha} }},
\end{equation}
where we have set $\gamma_{\alpha} :=\alpha (1+\delta) - \delta (d+3) > 0$.

\smallskip

By combining the identity~\eqref{eq:TV11087} with the estimates~\eqref{eq:TV14407},~\eqref{eq:TV14387},~\eqref{eq:TV14397} and choosing the inverse temperature $\beta$ large enough so that the series $\left( \frac{C^n}{\beta^{\frac n2}}\right)_{n \in \N}$ is summable, we obtain the main result~\eqref{eq:TV14557} and~\eqref{eq:TV145677} of this substep.

\medskip

\textit{Substep 1.3.}  In this substep, we study the term pertaining to the charges in the identity~\eqref{eq:TV0957897}. We prove the expansion
\begin{equation} \label{eq:mainsub1.3hom}
 \frac{1}{2\beta} \Delta \mathcal{H}_{\delta} + \sum_{q\in \mathcal{Q}} \nabla_q^* \cdot \a_q \nabla_q \mathcal{H}_{\delta}  = \frac{\ahom}{\beta}  \Delta \bar G_\delta + \sum_{i,j} \frac{1}{2\beta} \nabla_i  \bar G_\delta \Delta \chi_{m,i} +   \sum_{i,j}  \sum_{q\in \mathcal{Q}} \nabla_i  \bar G_\delta \nabla_q^* \cdot \a_q \nabla_q \chi_{m,i}+ R_{Q}.
\end{equation}
where $R_{Q}$ is an error term which satisfies the $\underline{H}^{-1}\left( B_{R^{1+\delta}} , \mu_\beta \right)$-norm estimate
\begin{equation}  \label{eq:TV14567}
\left\| R_{Q} \right\|_{\underline{H}^{-1}\left( B_{R^{1+\delta}} \mu_\beta \right)} \leq \frac{C}{R^{d-1+\gamma_{\alpha}}}.
\end{equation}
We first compute the gradient and the Laplacian of the two-scale expansion $\mathcal{H}$ and obtain the formulas
\begin{equation} \label{eq:formnablaH2sc}
\nabla \mathcal{H}_{\delta} = \nabla  \bar G_\delta  + \sum_{i,j} \left[ \nabla \nabla_i  \bar G_\delta  \chi_{m,i} + \nabla_i  \bar G_\delta   \nabla \chi_{m,i} \right],
\end{equation}
and
\begin{equation} \label{eq:formnablaH2scLap}
    \Delta \mathcal{H}_{\delta}  = \Delta \bar G_\delta + \sum_{i,j} \left( \Delta \nabla_i  \bar G_\delta  \right) \chi_{m,i} + 2 \left( \nabla \nabla_i  \bar G_\delta  \right) \cdot \left( \nabla \chi_{m,i} \right)  + \left(  \nabla_i  \bar G_\delta  \right) \Delta \chi_{m,i}. \\
\end{equation}
We first treat the term $\Delta \mathcal{H}$ and use the two following ingredients:
\begin{enumerate}
    \item[(i)] First we introduce the notation $R_{Q,1} := \sum_{i,j} \left( \Delta \nabla_i  \bar G_\delta  \right) \chi_{m,i} $. By using the regularity estimate~\eqref{eq:spatregbarGgeq3} on the homogenized Green's matrix and the quantitative sublinearity of the corrector stated in 
    Proposition~\ref{prop:prop5.25} of Chapter 6, we prove that this term is an error term and estimate its $\underline{H}^{-1} \left( B_{R^{1+\delta}} , \mu_\beta \right)$-norm according to the following computation
    \begin{align*}
        \left\| R_{Q,1} \right\|_{\underline{H}^{-1} \left( B_{R^{1+\delta}} , \mu_\beta \right)} & \leq C R^{1+\delta} \left\|  R_{Q,1} \right\|_{\underline{L}^{2} \left( B_{R^{1+\delta}} , \mu_\beta \right)} \\
        & \leq \sum_{i,j} C R^{1+\delta} \left\|  \left( \Delta \nabla_i  \bar G_\delta  \right) \right\|_{L^{\infty} \left( B_{R^{1+\delta}} , \mu_\beta \right)} \left\|  \chi_{m,i} \right\|_{\underline{L}^{2} \left( B_{R^{1+\delta}} , \mu_\beta \right)}\\
        & \leq \frac{C R^{1+\delta} R^{\left( 1 + \delta \right)\left(1-\alpha\right)}}{R^{(1-\delta) (d+1)}} \\
        & \leq \frac{C}{R^{d-1 + \gamma_\alpha}},
    \end{align*}
    where we have set $\gamma_\alpha :=\alpha (1+\delta) - \delta (d+3) > 0$.
    \smallskip
    \item[(ii)] Second, we use the identity $\Delta \bar G_{\delta} = \sum_{i,j} \nabla \cdot \left( \nabla_i \bar G_\delta  e_i \right)$.
\end{enumerate}
We obtain
\begin{equation} \label{eq:TV21228}
     \Delta \mathcal{H}_{\delta}  = \sum_{i,j}  \left( \nabla \nabla_i  \bar G_\delta  \right) \cdot \left( e_i + \nabla \chi_{m,i} \right) + \sum_{i,j} \left(  \nabla_i  \bar G_\delta  \right) \Delta \chi_{m,i} + R_{Q,1}.
\end{equation}
We then treat the term pertaining to the charges; the objective is to prove the identity 
\begin{equation} \label{eq:TV19558}
\sum_{q\in \mathcal{Q}} \nabla_q^* \cdot \a_q \nabla_q \mathcal{H}_{\delta} = \sum_{i = 1}^d \sum_{q \in \mathcal{Q}}  \left( \di^* \nabla_i \bar G_\delta \right) \a_q \nabla_q \left( l_{e_{ij}} + \chi_{m,i} \right) n_q + \sum_{q \in \mathcal{Q}} \nabla_i  \bar G_\delta \nabla_q^* \cdot \a_q \nabla_q \left( l_{e_{ij}} + \chi_{m,i} \right) + R_{Q,2},
\end{equation}
where $R_{Q,2}$ is an error term which satisfies the estimate
\begin{equation} \label{eq:TV19568}
    \left\| R_{Q,2} \right\|_{\underline{H}^{-1}\left(B_{R^{1+\delta}} , \mu_\beta \right)} \leq \frac{C}{R^{d-1-\gamma_{\alpha}}}.
\end{equation}
To prove this result, we select a test function $h$ which belongs to the space $H^1_0 \left(B_{R^{1+\delta}} , \mu_\beta \right)$ and satisfies the estimate $\left\| h \right\|_{\underline{H}^1 \left(B_{R^{1+\delta}} , \mu_\beta \right)} \leq 1$. For each charge $q \in \mathcal{Q}$, we select a point $x_q$ which belongs to the support of the charge $q$ arbitrarily. We then write
\begin{equation} \label{eq:TV21447}
    \sum_{q\in \mathcal{Q}} \a_q \nabla_q \mathcal{H}_{\delta} \nabla_q h :=  \sum_{q\in \mathcal{Q}}  \a_q \left( n_q , \di^* \mathcal{H}_{\delta} \right) \left( n_q , \di^* h \right).
\end{equation}
We use the exact formula for $\mathcal{H}_{\delta}$, and note that we have the identity $\di^* \bar G_\delta = \sum_{i,j} \nabla_i \bar G_\delta \di^* l_{e_{ij}}$. We obtain \pdcomment{recall this identity at the beginning + add a comment about 3.27 somewhere}
\begin{equation} \label{eq:TV21357}
    \di^* \mathcal{H}_{\delta}  = \di^* \bar G_\delta + \sum_{i = 1}^d \nabla_i \bar G_\delta \di^* \chi_{m,i} +  \sum_{i = 1}^d \di^* \nabla_i \bar G_\delta \chi_{m,i}
             = \sum_{i = 1}^d \nabla_i \bar G_\delta \left( \di^* l_{e_{ij}} + \di^* \chi_{m,i} \right) + \sum_{i,j} \di^* \nabla_i \bar G_\delta \chi_{m,i}.
\end{equation}
Putting the identity~\eqref{eq:TV21357} back into~\eqref{eq:TV21447}, we obtain
\begin{equation} \label{eq:TV22007}
     \sum_{q \in \Qa} \a_q \nabla_q \mathcal{H}_{\delta} \nabla_q h = \underbrace{\sum_{i = 1}^d \sum_{q \in \Qa}  \a_q \left( n_q , \nabla_i \bar G_\delta \left( \di^* l_{e_{ij}} + \di^* \chi_{m,i} \right) \right) \left( n_q , \di^* h \right)}_{\eqref{eq:TV22007}-(i)}  +  \underbrace{\sum_{q \in \Qa}  \a_q \left( n_q , \di^* \nabla_i \bar G_\delta \chi_{m,i} \right) \left( n_q , \di^* h \right)}_{\eqref{eq:TV22007}-(ii)} .
\end{equation}
The second term~\eqref{eq:TV22007}-(ii) is an error term which is small can be estimated thanks to the regularity estimate~\eqref{eq:spatregbarGgeq3} and Young's inequality. We obtain
\begin{align*}
     \lefteqn{ \left| \left\langle \sum_{q \in \Qa}  \a_q \left( n_q , \di^* \nabla_i \bar G_\delta \chi_{m,i} \right) \left( n_q , \di^* h \right) \right\rangle_{\mu_\beta} \right|} \qquad & \\ &  \leq \sum_{q \in \Qa} e^{-c \sqrt{\beta} \left\| q \right\|_{L^1}} \left\| n_q \right\|_2^2 \left\| \nabla^2 \bar G_\delta\right\|_{L^\infty \left( \Zd , \mu_\beta \right)} \left\| \chi_{m,i} \right\|_{L^2 \left( \supp n_q , \mu_\beta \right)} \left\| \nabla h \right\|_{L^2 \left( \supp n_q , \mu_\beta \right)} \\
     & \leq \frac{C}{R^{(1-\delta)(d+1)}}  \sum_{q \in \Qa} e^{-c \sqrt{\beta} \left\| q \right\|_{L^1}} \left\| n_q \right\|_2^2 \left\| \chi_{m,i} \right\|_{L^2 \left( \supp n_q , \mu_\beta \right)} \left\| \nabla h \right\|_{L^2 \left( \supp n_q , \mu_\beta \right)} \\
     & \leq \frac{C}{R^{(1-\delta)(d+1)}}  \sum_{q \in \Qa} e^{-c \sqrt{\beta} \left\| q \right\|_{L^1}} \left\| n_q \right\|_2^2 \left( R^{1 + \alpha} \left\| \chi_{m,i} \right\|_{L^2 \left( \supp n_q , \mu_\beta \right)}^2 + R^{- 1 - \alpha} \left\| \nabla h \right\|_{L^2 \left( \supp n_q , \mu_\beta \right)}^2 \right).
\end{align*}
We then use the inequality, for each point $x \in \Zd$,
\begin{equation} \label{eq:TV09127}
    \sum_{q \in \Qa} e^{-c \sqrt{\beta} \left\| q \right\|_{L^1}} \left\| n_q \right\|_2^2 \indc_{\{ x \in \supp n_q\}} \leq C.
\end{equation}
We deduce that
\begin{equation*}
    \left| \left\langle \sum_{q \in \Qa}  \a_q \left( n_q , \di^* \nabla_i \bar G_\delta \chi_{m,i} \right) \left( n_q , \di^* h \right) \right\rangle_{\mu_\beta} \right| \leq \frac{CR^{-1 + \alpha}}{R^{(1-\delta)(d+1)}}  \left\| \chi_{m,i} \right\|_{L^2 \left(B_{R^{1+\delta}, \mu_\beta } \right)}^2 + \frac{CR^{1-\alpha}}{R^{(1-\delta)(d+1)}} \left\| \nabla h \right\|_{L^2 \left(B_{R^{1+\delta}, \mu_\beta } \right)}^2.
\end{equation*}
We then use Proposition~\ref{prop:prop5.25} and the assumption $\left\| \nabla h \right\|_{\underline{L}^2 \left(B_{R^{1+\delta}, \mu_\beta } \right)} \leq 1$. We obtain
\begin{equation} \label{eq:TV1854812}
    \left| \frac{1}{R^{(1+\delta)d}} \left\langle \sum_{q \in \Qa}  \a_q \left( n_q , \di^* \nabla_i \bar G_\delta \chi_{m,i} \right) \left( n_q , \di^* h \right) \right\rangle_{\mu_\beta} \right| \leq \frac{C R^{1-\alpha}}{R^{(1-\delta)(d+1)}} \leq \frac{C}{R^{d-1 + \gamma_{\alpha}}},
\end{equation}
where we have set $\gamma_{\alpha} = \alpha - \delta \left( d+1 \right)$.

To treat the term~\eqref{eq:TV22007}-(i), we make use of the point $x_q$ and write
\begin{align*}
     \sum_{q\in \mathcal{Q}}  \a_q \left( n_q , \nabla_i \bar G_\delta \left( \di^* l_{e_{ij}} + \di^* \chi_{m,i} \right) \right) \left( n_q , \di^* h \right) & = \sum_{q\in \mathcal{Q}}   \a_q \left( n_q ,  \left( \di^* l_{e_{ij}} + \di^* \chi_{m,i} \right) \right) \left( n_q , \nabla_i \bar G_\delta \di^* h \right) \\
     & + \sum_{q\in \mathcal{Q}} \a_q \left( n_q ,\left( \nabla_i \bar G_\delta - \nabla_i \bar G_\delta(x_q) \right)  \left( \di^* l_{e_{ij}} + \di^* \chi_{m,i} \right) \right) \left( n_q , \di^* h \right) \\
     & +  \sum_{q\in \mathcal{Q}} \a_q \left( n_q   \left( \di^* l_{e_{ij}} + \di^* \chi_{m,i} \right) \right) \left( n_q , \left( \nabla_i \bar G_\delta - \nabla_i \bar G_\delta(x_q) \right) \di^* h \right).
\end{align*}
The terms on the second and third lines are error terms which are small, they can be estimated by the regularity estimate~\eqref{eq:spatregbarGgeq3} on the gradient of the homogenized Green's matrix and Young's inequality. We obtain
\begin{align*}
    \lefteqn{\left| \left\langle \sum_{q\in \mathcal{Q}} \a_q \left( n_q ,\left( \nabla_i \bar G_\delta - \nabla_i \bar G_\delta(x_q) \right)  \left( \di^* l_{e_{ij}} + \di^* \chi_{m,i} \right) \right) \left( n_q , \di^* h \right) \right\rangle_{\mu_\beta} \right|  } \qquad & \\ & \leq \sum_{q\in \mathcal{Q}} e^{-c \sqrt{\beta} \left\| q \right\|_{L^1}} \left\| n_q \right\|_2 \left\| \nabla \bar G_\delta - \nabla \bar G_\delta (x_q)\right\|_{L^\infty \left( \supp n_q , \mu_\beta \right)} \left\|  \nabla \chi_{m,i} \right\|_{L^2 \left( \supp n_q , \mu_\beta \right)} \left\| \nabla h \right\|_{L^2 \left( \supp n_q , \mu_\beta \right)} \\
    & \leq \frac{C}{R^{(1-\delta)d}} \sum_{q\in \mathcal{Q}} e^{-c \sqrt{\beta} \left\| q \right\|_{L^1}} \left\| n_q \right\|_2  \left( \left\|  \nabla \chi_{m,i} \right\|_{L^2 \left( \supp n_q , \mu_\beta \right)}^2 +  \left\| \nabla h \right\|_{L^2 \left( \supp n_q , \mu_\beta \right)}^2 \right). 
\end{align*}
We then the estimate~\eqref{eq:TV09127}, the bound $\left\| \nabla \chi_{m,i} \right\|_{\underline{L}^2 \left( B_{R^{1+\delta}} , \mu_\beta \right)} \leq C$ on the gradient of the corrector and the assumption $\left\| \nabla h \right\|_{\underline{L}^2 \left( B_{R^{1+\delta}} , \mu_\beta \right)} \leq 1$ to conclude that
\begin{equation} \label{eq:TV18538}
    \left| \frac{1}{R^{(1+\delta)d}} \left\langle \sum_{q\in \mathcal{Q}} \a_q \left( n_q ,\left( \nabla_i \bar G_\delta - \nabla_i \bar G_\delta(x_q) \right)  \left( \di^* l_{e_{ij}} + \di^* \chi_{m,i} \right) \right) \left( n_q , \di^* h \right) \right\rangle_{\mu_\beta} \right|  \leq \frac{C}{R^{(1-\delta)d}} \leq \frac{C}{R^{(d-1) + \gamma_1}},
\end{equation}
where we have set $\gamma_1 = 1 - \delta >0$.
The same argument proves the inequality
\begin{equation} \label{eq:TV18528}
     \left|  \frac{1}{R^{(1+\delta)d}} \left\langle \sum_{q\in \mathcal{Q}} \a_q \left( n_q   \left( \di^* l_{e_{ij}} + \di^* \chi_{m,i} \right) \right) \left( n_q , \left( \nabla_i \bar G_\delta - \nabla_i \bar G_\delta(x_q) \right) \di^* h \right) \right\rangle_{\mu_\beta} \right| \leq \frac{C}{R^{(d-1) + \gamma}},
\end{equation}
with the same exponent $\gamma_1 >0$. Combining the identity~\eqref{eq:TV22007} with the estimates~\eqref{eq:TV1854812},~\eqref{eq:TV18538},~\eqref{eq:TV18528}, we have obtained the following result: for each function $h \in H^1_0 \left( B_{R^{1+\delta}} , \mu_\beta \right)$ such that $\left\| h \right\|_{\underline{H}^1 \left(B_{R^{1+\delta}} , \mu_\beta \right)} \leq 1$, one has the estimate
\begin{equation*}
     \frac{1}{R^{(1+\delta)d}} \sum_{q \in \Qa} \a_q \nabla_q \mathcal{H} \nabla_q h =   \frac{1}{R^{(1+\delta)d}} \sum_{q\in \mathcal{Q}}   \a_q \left( n_q ,  \left( \di^* l_{e_{ij}} + \di^* \chi_{m,i} \right) \right) \left( n_q , \nabla_i \bar G_\delta \di^* h \right) + O \left( \frac{C}{R^{d - 1 + \gamma_\alpha}} \right).
\end{equation*}
We then use the identity $\nabla_i \bar G_\delta \di^* h = \di^*  \left(\nabla_i \bar G_\delta h \right) -  \di^* \nabla_i \bar G_\delta h$ and deduce that
\begin{multline} \label{eq:TV19548}
    \sum_{q \in \Qa} \a_q \nabla_q \mathcal{H} \nabla_q h =  \sum_{q\in \mathcal{Q}}   \a_q \left( n_q ,  \left( \di^* l_{e_{ij}} + \di^* \chi_{m,i} \right) \right) \left( n_q , \di^* \left( \nabla_i \bar G_\delta  h\right) \right) \\ + \sum_{q\in \mathcal{Q}}   \a_q \left( n_q ,  \left( \di^* l_{e_{ij}} + \di^* \chi_{m,i} \right) \right) \left( n_q , \di^* \nabla_i \bar G_\delta  h \right) + O \left( \frac{C}{R^{d - 1 + \gamma_\alpha}} \right).
\end{multline}
The inequality~\eqref{eq:TV19548} is equivalent to the identity~\eqref{eq:TV19558} and the estimate~\eqref{eq:TV19568}.

We now complete the proof of~\eqref{eq:mainsub1.3hom}. To prove this identity, it is sufficient, in view of~\eqref{eq:TV21228} and~\eqref{eq:TV19558}, to prove the estimate
\begin{equation} \label{eq:07499}
    \frac1{2\beta}\sum_{i,j}  \left( \nabla \nabla_i  \bar G_\delta  \right) \cdot \left( e_i + \nabla \chi_{m,i} \right) + \sum_{i = 1}^d \sum_{q \in \Qa}  \left( \di^* \nabla_i \bar G_\delta \right) \a_q \nabla_q \left( l_{e_{ij}} + \chi_{m,i} \right) n_q = \frac{\ahom}{\beta} \Delta \bar G_\delta + R_{Q,3},
\end{equation}
where the term $R_{Q,3}$ satisfies the estimate
\begin{equation} \label{eq:07509}
    \left\| R_{Q,3} \right\|_{\underline{H}^{-1}\left( B_{R^{1+\delta}} , \mu_\beta\right)} \leq \frac{C}{R^{1-d+ \gamma_\alpha}}.
\end{equation}
The proof relies on the quantitative estimate for the $\underline{H}^{-1}\left( B_{R^{1+\delta}} , \mu_\beta\right)$-norm of the flux corrector stated in Proposition~\ref{prop:prop5.25} of Chapter 6 and the regularity estimate~\eqref{eq:spatregbarGgeq3} on the homogenized function $\bar G_\delta$. We select a function $h \in H^1_0 \left( B_{R^{1+\delta}} , \mu_\beta \right)$ such that $\left\| h \right\|_{\underline{H}^1 \left( B_{R^{1+\delta}} , \mu_\beta \right)} \leq 1$ and use it as a test function. We write
\begin{align} \label{eq:TV07399}
    \lefteqn{\frac{1}{R^{(1+\delta)d}} \left| \left\langle  \sum_{x \in B_{R^{1+\delta}}}\sum_{i,j} \frac 1{2\beta} \left( \nabla \nabla_i  \bar G_\delta(x , \cdot )  \right) \cdot \left( e_i + \nabla \chi_{m,i}(x , \cdot) \right) h(x , \cdot)  \right. \right.} \qquad & \\ & \left. \left. + \sum_{i = 1}^d \sum_{q \in \mathcal{Q}}   \a_q \nabla_q \left( l_{e_{ij}} + \chi_{m,i} \right) \left( n_q, \di^* \nabla_i \bar G_\delta h \right) - \sum_{x \in B_{R^{1+\delta}}} \sum_{i = 1}^d \frac{\ahom}{\beta} \Delta  \bar G_\delta(x , \cdot ) h(x , \cdot) \right\rangle_{\mu_\beta}\right| \notag \\ & \leq C \sum_{i,j}  \left\| \frac 1{2 \beta} \left(e_i +  \nabla \chi_{m,i}\right) + \sum_{q \in \mathcal{Q}} \a_q \nabla_q \left( l_{e_{ij}} + \chi_{m,i} \right) n_q - \frac{\ahom}{\beta} e_i \right\|_{\underline{H}^{-1}\left( B_{R^{1+\delta}} , \mu_\beta \right)} \left\| \nabla^2 \bar G_\delta  h \right\|_{\underline{H}^1 \left(B_{R^{1+\delta}} , \mu_\beta \right)}. \notag
\end{align}
We then use Proposition~\ref{prop:prop5.25} of Chapter 6 to write \pdcomment{here something to do}
\begin{equation} \label{eq:TV07379}
    \sum_{i,j}  \left\| \frac 1{2 \beta} \left( e_i +  \nabla \chi_{m,i}\right) + \sum_{q \in \mathcal{Q}} \a_q \nabla_q \left( l_{e_{ij}} + \chi_{n,i} \right) n_q - \frac{\ahom}{\beta} e_i \right\|_{\underline{H}^{-1}\left( B_{R^{1+\delta}} , \mu_\beta \right)} \leq CR^{(1+\delta)(1-\alpha)}
\end{equation}
and the regularity estimate~\eqref{eq:spatregbarGgeq3} to write 
\begin{align} \label{eq:TV07299}
    \left\| \nabla^2 \bar G_\delta  h \right\|_{\underline{H}^1 \left(B_{R^{1+\delta}} , \mu_\beta \right)} & \leq  \frac{1}{R^{1+\delta}}\left\|  \nabla^2 \bar G_\delta  \right\|_{L^\infty \left( B_{R^{1+\delta}} , \mu_\beta \right)}\left\|   h \right\|_{\underline{L}^2 \left( B_{R^{1+\delta}} , \mu_\beta \right)} + \left\|  \nabla^3 \bar G_\delta  \right\|_{L^\infty \left( B_{R^{1+\delta}} , \mu_\beta \right)}\left\|  h \right\|_{\underline{L}^2 \left( B_{R^{1+\delta}} , \mu_\beta \right)}  \\ & \qquad + \left\|  \nabla^2 \bar G_\delta  \right\|_{L^\infty \left( B_{R^{1+\delta}} , \mu_\beta \right)}\left\| \nabla h \right\|_{\underline{L}^2 \left( B_{R^{1+\delta}} , \mu_\beta \right)} \notag \\
    & \leq C \left(\frac{1}{R^{d(1-\delta)}} + \frac{1}{R^{(d-1)(1-\delta)}} + \frac{R^{1+\delta}}{R^{(d+1)(1-\delta)}} \right) \notag\\
    & \leq \frac{1}{R^{d - \delta\left( d+2 \right)}} \notag
\end{align}
Combining the estimates~\eqref{eq:TV07399},~\eqref{eq:TV07379} and~\eqref{eq:TV07299}, we have obtained that, for each function $h \in H^1_0 \left( B_{R^{1+\delta}} , \mu_\beta \right)$ such that $\left\| h \right\|_{\underline{H}^1 \left( B_{R^{1+\delta}} , \mu_\beta \right)} \leq 1$,
\begin{align} \label{eq:07489}
    \lefteqn{\frac{1}{R^{(1+\delta)d}} \left| \left\langle  \sum_{x \in B_{R^{1+\delta}}}\sum_{i,j}  \left( \nabla \nabla_i  \bar G_\delta(x , \cdot )  \right) \cdot \left( e_i + \nabla \chi_{m,i}(x , \cdot) \right)  \right. \right.} \qquad & \\ & \left. \left. \qquad + \sum_{i = 1}^d \sum_{\di q = 0}   \a_q \nabla_q \left( l_{e_{ij}} + \chi_{m,i} \right) \left( n_q, \di^* \nabla_i \bar G_\delta h \right) - \sum_{x \in B_{R^{1+\delta}}} \sum_{i = 1}^d \ahom \Delta  \bar G_\delta(x , \cdot ) h(x , \cdot) \right\rangle_{\mu_\beta}\right| \notag \\ & \leq \frac{CR^{(1+\delta)(1-\alpha)}}{R^{d - \delta\left( d+2 \right)}} \notag \\
    & \leq \frac{C}{R^{d-1 + \gamma_{\alpha}}}, \notag
\end{align}
where we have set $\gamma := \alpha (1 + \delta) - \delta (d+3)$. Since the inequality~\eqref{eq:07489} is valid for any function $h \in H^1_0 \left( B_{R^{1+\delta}} , \mu_\beta \right)$ such that $\left\| h \right\|_{\underline{H}^1 \left( B_{R^{1+\delta}} , \mu_\beta \right)} \leq 1$, the estimate~\eqref{eq:07489} is equivalent to the identity~\eqref{eq:07499} and the $H^{-1}\left( B_{R^{1+\delta}} , \mu_\beta \right)$-norm estimate~\eqref{eq:07509}. The proof of~\eqref{eq:07499}, and thus of~\eqref{eq:mainsub1.3hom}, is complete. 

\medskip

\textit{Substep 1.4} In this substep, we conclude Step 1 and prove the estimate~\eqref{eq:TV19578}. We use the identity~\eqref{eq:TV0957897} and the identities~\eqref{eq:mainsub1.1hom} proved in Substep 1,~\eqref{eq:TV14557} proved in Substep 2 and~\eqref{eq:mainsub1.3hom} proved in Substep 3. We obtain
\begin{align} \label{eq:TV08399}
    \L \mathcal{H}_\delta & = \frac{\ahom}{\beta}  \Delta \bar G_\delta \\ & \quad + \sum_{i,j}  \nabla_i  \bar G_\delta \left(  \Delta_{\phi} \chi_{m,i}  + \frac{1}{2\beta} \Delta \chi_{m,i} + \sum_{q\in \mathcal{Q}}  \nabla_q^* \cdot \a_q \nabla_q \left( l_{e_{ij}} + \chi_{m,i} \right)  + \frac 1{2\beta} \sum_{n \geq 1}  \frac{1}{\beta^{\frac n2}} \Delta^{n+1} \chi_{m,i} \right) \notag \\ & \quad + R_{Q}  + R_{\Delta^n}. \notag
\end{align}
We then treat the three lines of the previous display separately. For the first line we use the identity
\begin{equation} \label{eq:TV09239}
     - \frac{\ahom}{\beta}  \Delta \bar G_\delta =\rho_\delta ~\mbox{in}~\Zd.
\end{equation}
For the second line, we use that, by the definition of the finite-volume corrector given in Definition~\ref{def.finivolcorr}, this map is a solution of the Helffer-Sj{\"o}strand equation $\L \left( l_{e_{ij}} + \chi_{m,i} \right) = 0$ in the set $B_{R^{1+\delta}} \times \Omega$. We obtain
\begin{align} \label{eq:TV09249}
    \sum_{i,j}  \nabla_i  \bar G_\delta \left(  \Delta_{\phi} \chi_{m,i}  + \frac{1}{2\beta} \Delta \chi_{m,i} + \sum_{q\in \mathcal{Q}}  \nabla_q^* \cdot \a_q \nabla_q \left( l_{e_{ij}} + \chi_{m,i} \right)+   \frac1{2\beta} \sum_{n \geq 1}  \frac{1}{\beta^{\frac n2}} \Delta^{n+1} \chi_{m,i} \right) & =  \sum_{i,j}  \nabla_i  \bar G_\delta \L \left( l_{e_{ij}} + \chi_{m,i} \right) \\& = 0. \notag
    \end{align}
For the third line, we use the estimates~\eqref{eq:TV145677} and~\eqref{eq:TV14567} on the error terms $R_{Q}$ and $R_{\Delta^n}$ respectively. We obtain
\begin{equation} \label{eq:TV09259}
    \left\| R_{Q}+R_{\Delta^n} \right\|_{\underline{H}^{-1}\left(B_{R^{1+\delta}} , \mu_\beta \right)} \leq \frac{C}{R^{d-1+\gamma_\alpha}}.
\end{equation}
A combination of the identities~\eqref{eq:TV08399},~\eqref{eq:TV09239},~\eqref{eq:TV09249} and~\eqref{eq:TV09259} proves the inequality
\begin{equation*}
    \left\| \mathcal{L} \mathcal{H}_\delta - \rho_\delta \right\|_{\underline{H}^{-1}\left(B_{R^{1+\delta}} , \mu_\beta \right)} \leq \frac{C}{R^{d-1+\gamma_\alpha}}.
\end{equation*}
The proof of the estimate~\eqref{eq:TV19578} is complete.


\medskip

\subsection{Estimating the $L^2$-norm of the term $\nabla \G_\delta - \nabla \mathcal{H}_{\delta}$} \label{sec3.3chap60851}
The objective of this section is to prove that the gradient of the Green's matrix $\nabla \G_\delta$ and the gradient of the two-scale expansion $\nabla \mathcal{H}_\delta$ are close in the $\underline{L}^2 \left( A_R , \mu_\beta \right)$-norm. More specifically, we prove that there exists an exponent $\gamma_\delta > 0$ such that one has the estimate 
\begin{equation} \label{eq:TV1004020}
    \left\| \nabla \G_\delta - \nabla \mathcal{H}_\delta  \right\|_{\underline{L}^2 \left( A_R , \mu_\beta \right)} \leq \frac{C}{R^{(d-1) + \gamma_\delta}}.
\end{equation}
To prove this inequality, we work on the larger set $B_{R^{1+\delta}/2}$ and prove the estimate
\begin{align} \label{eq:TV10039}
    \left\| \nabla \G_\delta - \nabla \mathcal{H}_\delta  \right\|_{\underline{L}^2 \left( B_{R^{1+\delta}/2} , \mu_\beta \right)} \leq  \frac{C}{R^{(1+\delta)(d-1 - \ep/2)}}.
\end{align}
The inequality~\eqref{eq:TV1004020} implies~\eqref{eq:TV10039}; indeed by using that the annulus $A_R$ is included in the ball $B_{R^{1+\delta}}$ we can compute
\begin{align*}
    \left\| \nabla \G_\delta - \nabla \mathcal{H}_{\delta}  \right\|_{\underline{L}^2 \left( A_R , \mu_\beta \right)} & \leq \left(\frac{\left| B_{R^{1+\delta}/2}\right|}{\left| A_R \right|} \right)^\frac 12 \left\| \nabla \G_\delta - \nabla \mathcal{H}_{\delta}  \right\|_{\underline{L}^2 \left( B_{R^{1+\delta}/2} , \mu_\beta \right)} \\ 
    & \leq C \left( \frac{R^{d(1+\delta)}}{R^d}\right)^\frac12 \frac{C}{R^{(1+\delta)(d-1 - \ep/2)}} \\
    & \leq \frac{C}{R^{d-1 + \gamma_\delta}},
\end{align*}
where we have set $\gamma_\delta := \delta (\frac d2-1 - \ep/2)$.
We now focus on the proof of the estimate~\eqref{eq:TV10039}. The strategy is to first use the identity $\mathcal{L} \G_\delta =  \rho_{\delta}$ to rewrite the estimate~\eqref{eq:TV19578} in the following form
\begin{equation} \label{eq:TV10569}
    \left\| \L \left( \mathcal{H}_\delta -  \G_\delta \right)  \right\|_{\underline{H}^{-1} \left( B_{R^{1+\delta}} , \mu_\beta \right)} \leq \frac{C}{R^{d-1+\gamma_\alpha}}.
\end{equation}
We then use the function $\G_\delta - \mathcal{H}$ as a test function in the definition of the $H^{-1}$-norm in the inequality~\eqref{eq:TV10569} to obtain the $H^1$-estimate stated in~\eqref{eq:TV10039}, as described in the outline of the proof at the beginning of Chapter~\ref{sec:section6}. The overall strategy is relatively straightforward; however, one has to deal with the following technical difficulty. By definition of the $H^{-1}$-norm, one needs to use a function in $H^1_0 \left( B_{R^{1+\delta}} , \mu_\beta \right)$ as a test function; in particular the function must be equal to $0$ outside the ball $B_{R^{1+\delta}}$, this condition is not verified by the function $\G_\delta - \mathcal{H}$ which is thus not a suitable test function. To overcome this issue, we introduce a cutoff function $\eta: \Zd \to \R$ supported in the ball $B_{R^{1+ \delta}}$ which satisfies the properties
\begin{equation} \label{eq:propeta}
    0 \leq \eta \leq \indc_{B_{R^{ 1 + \delta }}}, ~ \eta = 1 ~\mbox{in}~ B_{\frac{R^{ 1 + \delta }}{2}} , ~\mbox{and}~ \forall k \in \N, \, \left| \nabla^k \eta \right|\leq \frac{C}{R^{ (1 + \delta ) k }},
\end{equation}
and use the functions $\eta \left( \G_\delta - \mathcal{H} \right)$ as a test function. The main difficulty is thus to treat the cutoff function. Nevertheless, this difficulty is similar to the one treated in the proof of the Caccioppoli inequality stated in Proposition~\ref{Caccio.ineq}. We thus omit some of the details of the argument and refer the reader to the proof of Proposition~\ref{Caccio.ineq} of Chapter 5 for the missing elements of the argument.

We use the function $\eta \left( \G_\delta - \mathcal{H}_{\delta} \right)$ as a test function in the inequality~\eqref{eq:TV10569}. We obtain
\begin{align} \label{eq:TV11239}
    \frac{1}{R^{(1+\delta)d}}\sum_{x \in B_{R^{1+\delta}}} \left\langle \eta \left( \G_\delta - \mathcal{H}_{\delta}\right) \L \left( \G_\delta - \mathcal{H}_{\delta} \right)  \right\rangle_{\mu_\beta} & \leq \left\| \L \left( \G_\delta - \mathcal{H}_{\delta} \right) \right\|_{\underline{H}^{-1} \left( B_{R^{1+\delta}} , \mu_\beta \right)} \left\|  \eta \left( \G_\delta - \mathcal{H}_{\delta} \right)  \right\|_{\underline{H}^1 \left( B_{R^{1+\delta}} , \mu_\beta \right)} \\
    & \leq \frac{C}{R^{d-1 + \gamma_{\alpha}}} \left\| \eta \left( \G_\delta - \mathcal{H}_{\delta} \right) \right\|_{\underline{H}^1 \left( B_{R^{1+\delta}} , \mu_\beta \right)}. \notag
\end{align}
We then treat the terms in the left and right sides of the inequality~\eqref{eq:TV11239} separately. Regarding the left side, we prove the estimate
\begin{equation} \label{eq:TV15049}
    \left\| \eta \left( \G_\delta - \mathcal{H}_{\delta} \right) \right\|_{\underline{H}^1 \left( B_{R^{1+\delta}} , \mu_\beta \right)} \leq \frac{C}{R^{d-1 - \delta d}}.
\end{equation}
The proof relies on the properties of the cutoff function $\eta$ stated in~\eqref{eq:propeta}, the regularity estimate on the Green's matrix stated in Proposition~\ref{prop:prop6.2} of Chapter 5, the $L^\infty$-bound on the homogenized Green's matrix $\G_{\mathrm{hom}}^\delta$ stated in~\eqref{eq:spatregbarGgeq3} and the bounds on the corrector and its gradient recalled below
\begin{equation*}
    \left\| \chi_{m,i} \right\|_{\underline{L}^2 \left( B_{R^{1+\delta}} , \mu_\beta  \right)} \leq C R^{(1+\delta)(1-\alpha)},~ \left\| \nabla \chi_{m,i} \right\|_{\underline{L}^2 \left( B_{R^{1+\delta}} , \mu_\beta  \right)} \leq C  ~\mbox{and}~ \beta \sum_{x \in \Zd} \left\| \nabla \chi_{m,i} \right\|_{\underline{L}^2 \left( B_{R^{1+\delta}} , \mu_\beta  \right)} \leq C  .
\end{equation*}
We first write
\begin{multline} \label{eq:TV11579}
    \left\| \eta \left( \G_\delta - \mathcal{H}_{\delta} \right) \right\|_{\underline{H}^1 \left( B_{R^{1+\delta}} , \mu_\beta \right)} \leq \underbrace{\frac{1}{R^{1+\delta}} \left\| \eta \left( \G_\delta - \mathcal{H}_{\delta} \right) \right\|_{\underline{L}^2 \left( B_{R^{1+\delta}} , \mu_\beta \right)}}_{\eqref{eq:TV11579}-(i)} + \underbrace{ \left\| \nabla \eta \left( \G_\delta - \mathcal{H}_{\delta} \right) \right\|_{\underline{L}^2 \left( B_{R^{1+\delta}} , \mu_\beta \right)} }_{\eqref{eq:TV11579}-(ii)} \\ + \underbrace{ \left\| \eta \left( \nabla \G_\delta - \nabla \mathcal{H}_{\delta} \right) \right\|_{\underline{L}^2 \left( B_{R^{1+\delta}} , \mu_\beta \right)}}_{\eqref{eq:TV11579}-(iii)}+ \underbrace{\beta \sum_{x \in \Zd}  \left\| \eta \left( \partial_x \G_\delta - \partial_x \mathcal{H}_{\delta} \right) \right\|_{\underline{L}^2 \left( B_{R^{1+\delta}} , \mu_\beta \right)}}_{\eqref{eq:TV11579}-(iv)},
\end{multline}
and treats the four terms in the right side separately. For the term~\eqref{eq:TV11579}-(i), we use that the function $\eta$ is non-negative and smaller than $1$ to write
\begin{equation*}
    \frac{1}{R^{1+\delta}} \left\| \eta \left( \G_\delta - \mathcal{H}_{\delta} \right) \right\|_{\underline{L}^2 \left( B_{R^{1+\delta}} , \mu_\beta \right)} \leq \frac{1}{R^{1+\delta}} \left( \left\| \G_\delta  \right\|_{\underline{L}^2 \left( B_{R^{1+\delta}} , \mu_\beta \right)} + \left\| \mathcal{H}_{\delta}  \right\|_{\underline{L}^2 \left( B_{R^{1+\delta}} , \mu_\beta \right)} \right).
\end{equation*}
We then estimate the $L^2$-norm of the Green's matrix $ \G_\delta$ thanks to the estimate
\begin{equation*}
    \left\| \G_\delta  \right\|_{\underline{L}^2 \left( B_{R^{1+\delta}} , \mu_\beta \right)} \leq \left\| \G_\delta \right\|_{L^\infty \left( \Zd , \mu_\beta \right)} \leq \frac{C}{R^{(1-\delta)(d-2)}}.
\end{equation*}
The $L^2$-norm of the two-scale expansion $\mathcal{H}$ can be estimated according to the following computation
\begin{align*}
     \left\| \mathcal{H}_{\delta}  \right\|_{\underline{L}^2 \left( B_{R^{1+\delta}} , \mu_\beta \right)} & \leq  \left\| \bar G  \right\|_{\underline{L}^2 \left( B_{R^{1+\delta}} , \mu_\beta \right)} + \sum_{i,j} \left\| \nabla_i \bar G  \right\|_{L^\infty \left( B_{R^{1+\delta}} , \mu_\beta \right)} \left\| \chi_{m,i} \right\|_{\underline{L}^2 \left( B_{R^{1+\delta}} , \mu_\beta \right)} \\
     & \leq \frac{C}{R^{(1-\delta)(d-2)}} + \frac{C R^{(1 + \delta)(1-\alpha)}}{R^{(1-\delta)(d-1)}} \\
     & \leq \frac{C}{R^{(1-\delta)(d-2)}},
\end{align*}
where we have used the inequality $\alpha \gg \delta$ in the third inequality.
A combination of the three previous displays shows the estimate
\begin{equation} \label{eq:TV15019}
    \frac{1}{R^{1+\delta}} \left\| \eta \left( \G_\delta - \mathcal{H} \right) \right\|_{\underline{L}^2 \left( B_{R^{1+\delta}} , \mu_\beta \right)} \leq \frac{C}{R^{1+\delta} \times R^{(1-\delta)(d-2)}} \leq \frac{C}{ R^{d-1 - \delta (d-3)}}.
\end{equation}
The proof of the term~\eqref{eq:TV11579}-(ii) is identical, we use the estimate $\left| \nabla \eta \right| \leq \frac{C}{R^{1+\delta}}$ and apply the estimate obtained for the term~\eqref{eq:TV11579}-(ii). We obtain
\begin{equation} \label{eq:TV15029}
     \left\| \nabla \eta \left( \G_\delta - \mathcal{H}_{\delta} \right) \right\|_{\underline{L}^2 \left( B_{R^{1+\delta}} , \mu_\beta \right)} \leq \frac{C}{ R^{d-1 - \delta (d-3)}}.
\end{equation}
For the term~\eqref{eq:TV11579}-(iii), we first write
\begin{equation*}
     \left\| \eta \left( \nabla \G_\delta - \nabla \mathcal{H}_{\delta} \right) \right\|_{\underline{L}^2 \left( B_{R^{1+\delta}} , \mu_\beta \right)} \leq \left\| \nabla \G_\delta  \right\|_{L^\infty \left(\Zd , \mu_\beta \right)} + \left\| \nabla \mathcal{H}  \right\|_{\underline{L}^2 \left( B_{R^{1+\delta}} , \mu_\beta \right)}.
\end{equation*}
The $L^\infty$-norm of the Green's matrix $\nabla \G_\delta $ is estimated by Proposition~\ref{prop:prop6.2}. We have
\begin{equation*}
    \left\| \nabla \G_\delta  \right\|_{L^\infty \left(\Zd , \mu_\beta \right)} \leq \frac{C}{R^{(1-\delta)(d-1-\ep)}}.
\end{equation*}
For the $L^2$-norm of the two-scale expansion $\mathcal{H}$, we use the formula~\eqref{eq:formnablaH2sc} and write
\begin{align*}
    \left\| \nabla \mathcal{H}_{\delta}  \right\|_{\underline{L}^2 \left( B_{R^{1+\delta}} , \mu_\beta \right)} & \leq  \left\| \nabla  \bar G_\delta \right\|_{L^\infty \left( \Zd  \right)}  + \sum_{i,j} \left\| \nabla \nabla_i  \bar G_\delta \right\|_{L^\infty \left( \Zd  \right)} \left\| \chi_{m,i} \right\|_{\underline{L}^2 \left( B_{R^{1+\delta}} , \mu_\beta  \right)} \\ & \quad + \sum_{i,j} \left\| \nabla_i  \bar G_\delta \right\|_{L^\infty \left( \Zd  \right)}  \left\| \nabla \chi_{m,i} \right\|_{\underline{L}^2 \left( B_{R^{1+\delta}} , \mu_\beta  \right)} \\
    & \leq \frac{C}{R^{(1-\delta)(d-1-\ep)}} + \frac{CR^{(1+\delta)(1-\alpha)}}{R^{(1-\delta)(d-\ep)}} + \frac{C}{R^{(1-\delta)(d-1-\ep)}} \\
    & \leq \frac{C}{R^{d-1 - \ep - \delta (d-1-\ep)}}.
\end{align*}
A combination of the three previous displays together with the inequality $\delta \gg \ep$ yields the estimate
\begin{equation} \label{eq:TV15039}
    \left\| \eta \left( \nabla \G_\delta - \nabla \mathcal{H} \right) \right\|_{\underline{L}^2 \left( B_{R^{1+\delta}} , \mu_\beta \right)}  \leq \frac{C}{R^{d-1- \delta d}}.
\end{equation}
There remains to estimate the term~\eqref{eq:TV11579}-(iv). We first write
\begin{equation} \label{eq:TVde10120}
    \beta \sum_{x \in \Zd}  \left\| \eta \left( \partial_x \G_\delta - \partial_x \mathcal{H} \right) \right\|_{\underline{L}^2 \left( B_{R^{1+\delta}} , \mu_\beta \right)} \leq \underbrace{\beta \sum_{x \in \Zd}  \left\| \eta \partial_x \G_\delta  \right\|_{\underline{L}^2 \left( B_{R^{1+\delta}} , \mu_\beta \right)}}_{\eqref{eq:TVde10120}-(i)} +  \underbrace{\beta \sum_{x \in \Zd} \left\| \eta \partial_x \mathcal{H}_{\delta}  \right\|_{\underline{L}^2 \left( B_{R^{1+\delta}} , \mu_\beta \right)}}_{\eqref{eq:TVde10120}-(ii)}
\end{equation}
and estimate the two terms in the right side separately. For the term~\eqref{eq:TVde10120}-(i), we use that the map $\G_\delta$ solves the equation $\mathcal{L} \G_\delta = \rho_\delta$ and use the map $\eta^2 \G_\delta$ as a test function. We obtain
\begin{multline*}
\beta \sum_{x \in \Zd}  \left\| \eta \partial_x \G_\delta  \right\|_{L^2 \left( B_{R^{1+\delta}} , \mu_\beta \right)} = - \frac 1{2}\sum_{x \in \Zd}  \left\langle \nabla \G_\delta (x, \cdot) \cdot \nabla \left( \eta^2 \G_\delta \right)(x, \cdot) \right\rangle_{\mu_\beta} -   \beta \sum_{q \in \mathcal{Q}}  \left\langle \nabla_q \G_\delta \cdot \a_q \nabla_q \left( \eta^2 \G_\delta \right) \right\rangle_{\mu_\beta} \\ -  \frac 1{2} \sum_{n \geq 1} \sum_{x \in \Zd}  \frac{1}{\beta^{ \frac n2}} \left\langle  \nabla^{n+1} \G_\delta(x, \cdot) \cdot \nabla^{n+1} \left( \eta^2 \G_\delta \right)(x,\cdot) \right\rangle_{\mu_\beta} + \beta \sum_{x \in \Zd} \rho_\delta(x) \left\langle \G_\delta(x , \cdot) \right\rangle_{\mu_\beta}.
\end{multline*}
We then estimate the four terms in the right sides using the pointwise estimates on the function $\G_\delta$ and its gradient stated in Proposition~\ref{prop:prop6.2}, the properties on the functions $\rho_\delta$ and $\eta$ stated in~\eqref{prop.rhodelta} and~\eqref{eq:propeta} respectively. We omit the technical details and obtain the estimate
\begin{equation} \label{eq:TVde10220}
    \beta \sum_{x \in \Zd}  \left\| \eta \partial_x \G_\delta  \right\|_{\underline{L}^2 \left( B_{R^{1+\delta}} , \mu_\beta \right)} \leq \frac{C}{R^{(1-\delta)(d-1-\ep)}}.
\end{equation}


The term~\eqref{eq:TVde10120}-(ii) involving the two-scale expansion is the easiest one to estimate; using the explicit formula for the map $\mathcal{H}_\delta$ and the fact that the function $\bar G_\delta$ does not depend on the field $\phi$, we have the identity
\begin{equation*}
    \partial_x \mathcal{H}_{\delta} := \sum_{i,j} \nabla_i \bar G_\delta \partial_x \chi_{m,i}.
\end{equation*}
We deduce that
\begin{align} \label{eq:TVdec10340}
    \beta \sum_{x \in \Zd} \left\| \eta \partial_x \mathcal{H}_{\delta}  \right\|_{\underline{L}^2 \left( B_{R^{1+\delta}} , \mu_\beta \right)} & \leq \beta \sum_{x \in \Zd} \left\|  \partial_x \mathcal{H}_{\delta}  \right\|_{\underline{L}^2 \left( B_{R^{1+\delta}} , \mu_\beta \right)} \\
    & \leq C  \sum_{i,j} \left\| \nabla \bar G_\delta \right\|_{L^{\infty \left( \Zd \right)}}  \beta \sum_{x \in \Zd} \left\| \partial_x \chi_{m,i} \right\|_{\underline{L}^2 \left( B_{R^{1+\delta}} , \mu_\beta \right)} \notag \\
    & \leq \frac{C}{R^{(1-\delta)(d - 1 - \ep)}}. \notag
\end{align}
Combining the inequalities~\eqref{eq:TVde10120},~\eqref{eq:TVde10220} and~\eqref{eq:TVdec10340} yields
\begin{equation} \label{eq:TVdec1034045}
    \beta \sum_{x \in \Zd}  \left\| \eta \left( \partial_x \G_\delta - \partial_x \mathcal{H}_{\delta} \right) \right\|_{\underline{L}^2 \left( B_{R^{1+\delta}} , \mu_\beta \right)} \leq \frac{C}{R^{d-1 - \ep - \delta \left( d - 1 - \ep \right)}} \leq \frac{C}{R^{d-1 -  \delta  d }}.
\end{equation}

The inequality~\eqref{eq:TV15049} is then obtained by combining the estimates~\eqref{eq:TV15019}, \eqref{eq:TV15029},~\eqref{eq:TV15039} and~\eqref{eq:TVdec1034045}. We then put the inequality back into the inequality~\eqref{eq:TV11239} and deduce that
\begin{equation} \label{eq:TV06520}
     \frac{1}{R^{(1+\delta)d}}\sum_{x \in B_{R^{1+\delta}}} \left\langle \eta \left( \G_\delta - \mathcal{H}_{\delta}\right) \L \left( \G_\delta - \mathcal{H}_{\delta} \right)  \right\rangle_{\mu_\beta} \leq \frac{C}{R^{d-1 + \gamma_\alpha} \times R^{d-1 - \delta d}} \leq  \frac{C}{R^{2d-2 + \gamma_\alpha}},
\end{equation}
where we have used in the second inequality that the exponent $\gamma_\alpha$ is of order $\alpha$; it is thus much larger than the value $\delta d$ and we may write $\gamma_\alpha - \delta d = \gamma_\alpha$ following the notation convention explained at the beginning of Section~\ref{sec:section6.1}.

In the rest of this step, we treat the left side of~\eqref{eq:TV06520} and prove the inequality
\begin{equation} \label{eq:TV11321}
     \left\| \nabla \G_\delta - \nabla \mathcal{H}_{\delta} \right\|_{\underline{L}^2 \left( B_{\frac{R^{1+\delta}}{2}} , \mu_\beta \right)} \leq \frac{1}{R^{(1+\delta)d}}\sum_{x \in B_{R^{1+\delta}}} \left\langle \eta \left( \G_\delta - \mathcal{H}_{\delta}\right) \L \left( \G_\delta - \mathcal{H}_{\delta} \right)  \right\rangle_{\mu_\beta} + \frac{C}{R^{(1+\delta)(2d-2 - \ep) }} .
\end{equation}
First, by definition of the Helffer-Sj{\"o}strand operator $\mathcal{L}$, we have the identity
\begin{align} \label{eq:TV08101}
\sum_{x \in \Zd} \left\langle \eta \left( \G_\delta - \mathcal{H}_{\delta}\right) \L \left( \G_\delta - \mathcal{H}_{\delta} \right)  \right\rangle_{\mu_\beta} & = \sum_{x , y \in \Zd} \eta(x) \left\langle \left( \partial_y \G_\delta (x , \cdot)  - \partial_y \mathcal{H}_{\delta} (x , \cdot) \right)^2 \right\rangle_{\mu_\beta} \\ & + \frac 1{2\beta}\sum_{x \in \Zd}  \left\langle  \left( \nabla \G_\delta  - \nabla \mathcal{H}_{\delta}\right)(x , \cdot) \cdot \nabla \left( \eta \left( \G_\delta-  \mathcal{H}_{\delta} \right)\right)(x , \cdot)  \right\rangle_{\mu_\beta} \notag \\ & +  \sum_{q \in \mathcal{Q}}  \left\langle \nabla_q \left(  \G_\delta -  \mathcal{H}_{\delta}\right) \cdot \a_q \nabla_q \left( \eta \left(  \G_\delta  - \mathcal{H}_{\delta} \right) \right) \right\rangle_{\mu_\beta} \notag \\ & +  \frac 1{2\beta} \sum_{n \geq 1} \sum_{x \in \Zd}  \frac{1}{\beta^{ \frac n2}} \left\langle  \nabla^{n+1} \left(  \G_\delta  -  \mathcal{H}_{\delta} \right)(x , \cdot) \cdot \nabla^{n+1} \left( \eta \left(  \G_\delta  -  \mathcal{H}_{\delta} \right) \right)(x,\cdot) \right\rangle_{\mu_\beta}. \notag
\end{align}
We then estimate the four terms on the right side separately. For the first one, we use that it is non-negative
\begin{equation*}
    \sum_{x , y \in \Zd} \eta(x)^2 \left\langle \left( \partial_y \G_\delta (x , \cdot)  - \partial_y \mathcal{H}_{\delta} (x , \cdot) \right)^2 \right\rangle_{\mu_\beta}  \geq 0.
\end{equation*}
For the second one, we expand the gradient of the product $\eta \left( \G_\delta  - \mathcal{H} \right)$ and write
\begin{align} \label{eq:TV09490}
    \lefteqn{\sum_{x \in \Zd}  \left\langle  \left( \nabla \G_\delta  - \nabla \mathcal{H}_{\delta}\right)(x , \cdot) \cdot \nabla \left( \eta \left( \G_\delta-  \mathcal{H}_{\delta} \right)\right)(x , \cdot)  \right\rangle_{\mu_\beta}} \qquad & \\ &
    = \sum_{x \in \Zd}  \eta(x)  \left\langle  \left( \nabla \G_\delta  - \nabla \mathcal{H}_{\delta}\right)(x , \cdot) \cdot   \nabla \left( \G_\delta-  \mathcal{H}_{\delta} \right)(x , \cdot)  \right\rangle_{\mu_\beta} \notag \\
    & \quad + \sum_{x \in \Zd}  \left\langle  \left( \nabla \G_\delta  - \nabla \mathcal{H}_{\delta}\right)(x , \cdot) \cdot  \nabla \eta(x)\left( \G_\delta-  \mathcal{H}_{\delta} \right)(x , \cdot)  \right\rangle_{\mu_\beta}. \notag
\end{align}
we divide the identity~\eqref{eq:TV09490} by the volume factor $R^{(1+\delta)d}$ and use the properties of the function $\eta$ stated in~\eqref{eq:propeta}. In particular, we use that the gradient of $\eta$ is supported in the annulus $A_{R^{1+\delta}} := B_{R^{1+\delta}} \setminus B_{\frac{R^{1+\delta}}{2}}$ and obtain
\begin{multline} \label{eq:TV07591}
    \frac{1}{R^{(1+\delta)d}} \sum_{x \in \Zd}  \left\langle  \left( \nabla \G_\delta  - \nabla \mathcal{H}_\delta\right)(x , \cdot) \cdot \nabla \left( \eta \left( \G_\delta-  \mathcal{H}_\delta \right)\right)(x , \cdot)  \right\rangle_{\mu_\beta} \geq c \left\| \eta \left( \nabla \G_\delta  - \nabla \mathcal{H}_\delta \right) \right\|_{\underline{L}^2 \left( B_{R^{1+\delta}} , \mu_\beta \right)}^2 \\ -  \frac{C}{R^{1+\delta}} \left\| \nabla \G_\delta  \ - \nabla \mathcal{H}_\delta \right\|_{\underline{L}^2 \left( A_{R^{1+\delta}} , \mu_\beta \right)} \left\|  \G_\delta  - \mathcal{H}_\delta \right\|_{\underline{L}^2 \left( A_{R^{1+\delta}} , \mu_\beta \right)}.
\end{multline}
By a computation similar to the one performed for the term ~\eqref{eq:TV11579}-(iii), but using the estimates~\eqref{eq:TV20383} for the Green's matrices in the distant annulus $A_{R^{1+\delta}}$, instead of the $L^\infty$-estimates~\eqref{eq:TV090191} and~\eqref{eq:spatregbarGgeq3}. We obtain
\begin{equation} \label{eq:TV07601}
    \left\| \nabla \G_\delta  \ - \nabla \mathcal{H}_\delta \right\|_{\underline{L}^2 \left( A_{R^{1+\delta}} , \mu_\beta \right)} \leq \frac{C}{R^{(1+\delta)(d -1 - \ep)}}~\mbox{and}~\left\|  \G_\delta  - \mathcal{H}_\delta \right\|_{\underline{L}^2 \left( A_{R^{1+\delta}}, \mu_\beta \right)} \leq \frac{C}{R^{(1+\delta)(d-2)}}.
\end{equation}
A combination of the inequalities~\eqref{eq:TV07591} and~\eqref{eq:TV07601} proves the estimate
\begin{equation} \label{eq:TV11111}
    \frac{1}{R^{(1+\delta)d}} \sum_{x \in \Zd}  \left\langle  \left( \nabla \G_\delta  - \nabla \mathcal{H}_\delta\right)(x , \cdot) \cdot \nabla \left( \eta \left( \G_\delta-  \mathcal{H}_\delta \right)\right)(x , \cdot)  \right\rangle_{\mu_\beta} + \frac{C}{R^{(1+\delta)(2d-2 - \ep)}} \geq c  \left\| \eta \left( \nabla \G_\delta  - \nabla \mathcal{H} \right) \right\|_{\underline{L}^2 \left( B_{R^{1+\delta}} , \mu_\beta \right)}^2.
\end{equation}
The other terms in the right side of the identity~\eqref{eq:TV08101} involving the sum over the iteration of the Laplacian and over the charges $q \in \mathcal{Q}$ are treated similarly. Instead of expanding the gradient as it was done in~\eqref{eq:TV09490}, we use the commutation estimates (see~\eqref{eq:Caccio1925} and~\eqref{eq:TV1549C} in the proof of Proposition~\ref{Caccio.ineq} in Chapter 5), for each integer $n \in \N$, and each pair $(x , \phi) \in \Zd \times \Omega$,
\begin{equation}
\left| \nabla^n \left( \eta \left ( \G_\delta  - \mathcal{H}_\delta \right) \right) (x , \phi)  -  \eta(x) \nabla^n\left ( \G_\delta  - \mathcal{H}_\delta \right)(x , \phi)  \right| \leq \frac{C^n}{R^{1+\delta}} \sum_{z \in B(x,n)} | \G_\delta ( z, \phi)  - \mathcal{H}_\delta( z, \phi)|.
\end{equation}
and for each charge $q \in \mathcal{Q}$, each point $x$ in the support of the charge $q$ and each field $\phi \in \Omega$,
\begin{equation*}
\left| \nabla_q \left( \eta \left ( \G_\delta  - \mathcal{H}_\delta \right) \right) - \eta(x) \nabla_q  \left( \G_\delta  - \mathcal{H}_\delta \right) \right| \leq \frac{C}{R^{1+\delta}} \left(\diam q \right) \left\|q \right\|_{1} \sum_{z \in \supp q} | \G_\delta  - \mathcal{H}|.
\end{equation*}
The details of the argument are similar to the one presented in the proof of the Caccioppoli inequality (Proposition~\ref{Caccio.ineq} of Chapter 5) and are omitted. The result we obtain is stated below
\begin{equation} \label{eq:TV11121}
    \frac{1}{R^{(1+\delta)d}}  \sum_{q \in \mathcal{Q}}  \left\langle \nabla_q \left(  \G_\delta -  \mathcal{H}_\delta\right) \cdot \a_q \nabla_q \left( \eta \left(  \G_\delta  - \mathcal{H}_\delta \right) \right) \right\rangle_{\mu_\beta}  + \frac{C}{R^{(1+\delta)(2d-2 - \ep) }} \geq -C e^{-c \sqrt{\beta}} \left\| \eta \left( \nabla \G_\delta  - \nabla \mathcal{H}_\delta \right) \right\|_{L^2 \left( \Zd , \mu_\beta \right)}^2
\end{equation}
and
\begin{align} \label{eq:TV11131}
    \lefteqn{ \frac{1}{R^{(1+\delta)d}}  \sum_{n \geq 1} \sum_{x \in \Zd}  \frac{1}{\beta^{ \frac n2}} \left\langle  \nabla^{n+1} \left(  \G_\delta  -  \mathcal{H}_\delta \right)(x , \cdot) \cdot \nabla^{n+1} \left( \eta \left(  \G_\delta  -  \mathcal{H}_\delta \right) \right)(x,\cdot) \right\rangle_{\mu_\beta} + \frac{C}{R^{(1+\delta)(2d-2 - \ep) }} }  \qquad \qquad\qquad\qquad \qquad\qquad\qquad & \\ & \geq   \sum_{n \geq 1} \sum_{x \in \Zd}  \frac{1}{\beta^{ \frac n2}} \left\langle \eta(x) \left| \nabla^{n+1} \left(  \G_\delta  -  \mathcal{H}_\delta \right)(x , \cdot) \right|^2 \right\rangle_{\mu_{\beta}} \notag \\
    & \geq 0. \notag
\end{align}
We then combine the identity~\eqref{eq:TV08101} with the estimates~\eqref{eq:TV11111},~\eqref{eq:TV11121} and~\eqref{eq:TV11131} and assume that the inverse temperature $\beta$ is large enough. We obtain
\begin{align*}
     \frac{1}{R^{(1+\delta)d}} \sum_{x \in \Zd} \left\langle \eta \left( \G_\delta - \mathcal{H}\right) \L \left( \G_\delta - \mathcal{H}_\delta \right)  \right\rangle_{\mu_\beta} +  \frac{C}{R^{(1+\delta)(2d-2 - \ep) }} & \geq c \left\| \eta \left( \nabla \G_\delta  - \nabla \mathcal{H}_\delta \right) \right\|_{\underline{L}^2 \left( \Zd , \mu_\beta \right)}^2 \\ & \geq c \left\|  \nabla \G_\delta  - \nabla \mathcal{H}_\delta  \right\|_{\underline{L}^2 \left( B_{R^{1+\delta}/2}, \mu_\beta \right)}^2. \notag
\end{align*}
The proof of the inequality~\eqref{eq:TV11321} is then complete. To complete the proof of Step 2, we combine the estimates~\eqref{eq:TV06520} and~\eqref{eq:TV11321}. We obtain
\begin{equation*}
     \left\| \nabla \G_\delta - \nabla \mathcal{H}_\delta \right\|_{L^2 \left( B_{\frac{R^{1+\delta}}{2}} , \mu_\beta \right)}^2 \leq \frac{C}{R^{2d-2 + \gamma_\alpha}} + \frac{C}{R^{(1+\delta)(2d-2 - \ep) }} \leq \frac{C}{R^{(1+\delta)(2d-2 - \ep)}},
\end{equation*}
where the last inequality is a consequence of the fact that $\gamma_\alpha$ is of order $\alpha$ and of the ordering $\alpha \gg \delta \gg \ep$. The proof of the estimate~\eqref{eq:TV10039} is complete.

\medskip

\subsection{Homogenization of the gradient of the Green's matrix} \label{sec3.4chap60851}
In this section, we post-process the conclusion~\eqref{eq:TV10039} of Section~\ref{sec3.3chap60851} and prove that the gradient of the Green's matrix $\nabla \mathcal{G}$ is close to the map $\sum_{i,j} \left( e_i + \nabla \chi_{ij} \right) \nabla_i \bar G$. The objective is to prove that there exists an exponent $\gamma_\delta > 0$ such that
\begin{equation} \label{eq:TV14282}
    \left\| \nabla \G - \sum_{i,j} \left( e_i + \nabla \chi_{ij} \right) \nabla_i \bar G \right\|_{\underline{L}^2 \left( A_R , \mu_\beta \right)}  \leq \frac{C}{R^{d-1 + \gamma_{\delta}}}.
\end{equation}
We first use the regularity estimates stated in Proposition~\ref{prop:prop6.2} and the $L^2$-bound on the gradient of the infinite-volume corrector, for each $x \in \Zd$, each integers $i \in \{ 1 , \ldots , d \}$ and $j\in \{1 , \ldots, \binom d2 \}$, $\left\| \nabla \chi_{ij}(x , \cdot) \right\|_{L^2 \left( \mu_\beta \right)} \leq C$. We write
\begin{align} \label{eq:TV14272}
    \lefteqn{\left\| \nabla \left( \G - \G_\delta \right) - \sum_{i,j} \left( e_i + \nabla \chi_{ij} \right) \nabla_i \left( \bar G_\delta - \bar G \right) \right\|_{\underline{L}^2 \left( A_R , \mu_\beta \right)}} \qquad & \\ & \leq \left\| \nabla \left( \G - \G_\delta \right) \right\|_{\underline{L}^2 \left( A_R , \mu_\beta \right)} + \sum_{i,j} \left\| \left( e_i + \nabla \chi_{ij} \right) \right\|_{\underline{L}^2 \left( A_R , \mu_\beta \right)} \left\| \nabla_i \left( \bar G_\delta - \bar G \right) \right\|_{L^\infty \left( A_R , \mu_\beta \right)}  \notag \\
    & \leq \frac{C}{R^{d-1+\gamma_\delta}}. \notag
\end{align}
Using the inequality~\eqref{eq:TV14272}, we see that to prove~\eqref{eq:TV14282} it is sufficient to prove the estimate 
\begin{equation} \label{eq:TV15172}
 \left\| \nabla \G_\delta - \sum_{i,j} \left( e_i + \nabla \chi_{ij} \right) \nabla_i \bar G_\delta \right\|_{\underline{L}^2 \left( A_R , \mu_\beta \right)}  \leq \frac{C}{R^{d-1 + \gamma_\delta}}.
 \end{equation}
We then use the main estimate~\eqref{eq:TV10039} and deduce that, to prove the inequality~\eqref{eq:TV15172}, it is sufficient to prove
\begin{equation} \label{eq:TV15182}
    \left\| \nabla \mathcal{H}_\delta - \sum_{i,j} \left( e_i + \nabla \chi_{ij} \right) \nabla_i \bar G_\delta \right\|_{\underline{L}^2 \left( A_R , \mu_\beta \right)} \leq \frac{C}{R^{d-1 + \gamma_\delta}}.
\end{equation}
The rest of the argument of this step is devoted to the proof of~\eqref{eq:TV15182}. We first use the explicit formula for the gradient of the two-scale expansion $\nabla \mathcal{H}_\delta$ stated in~\eqref{eq:formnablaH2sc} and write 
\begin{align*}
\left\| \nabla \mathcal{H}_\delta - \sum_{i,j} \left( e_i + \nabla \chi_{m,i} \right) \nabla_i \G_\delta \right\|_{\underline{L}^2 \left( A_R , \mu_\beta \right)} \leq \sum_{i,j} \left\|  \nabla \nabla_i  \bar G_\delta  \chi_{m,i} \right\|_{\underline{L}^2 \left( A_R , \mu_\beta \right)}+ \left\| \left(\nabla_i  \bar G_\delta \right) \left( \nabla \chi_{m,i} - \nabla \chi_{ij} \right) \right\|_{\underline{L}^2 \left(A_R , \mu_\beta \right)}.
\end{align*}
We then use the regularity estimate~\eqref{eq:spatregbarGgeq3}, the quantitative sublinearity of the corrector stated in Proposition~\ref{prop:prop5.25} and Proposition~\ref{prop5.26} to quantify the $L^2$-norm of the difference between the gradient of finite-volume corrector and the gradient of the infinite-volume corrector. We obtain
\begin{align} \label{eq:TV13422}
    \left\| \nabla \mathcal{H} - \sum_{i,j} \left( e_i + \nabla \chi_{m,i} \right) \nabla_i \bar G_\delta \right\|_{\underline{L}^2 \left( A_R , \mu_\beta \right)} & \leq \left( \frac{\left| A_R \right|}{\left| B_{R^{1+\delta}} \right|} \right)^\frac 12 \frac{C R^{1-\alpha}}{R^{d - \ep}} + \left( \frac{\left| A_R \right|}{\left| B_{R^{1+\delta}} \right|} \right)^\frac 12 \frac{C R^{-\alpha}}{R^{d - 1 - \ep}} \\
    & \leq \frac{C}{R^{d-1 + \gamma_\alpha}}, \notag
\end{align}
where we have set $\gamma_\alpha := \alpha - \ep - \frac{d \delta}{2}$. Using that the exponent $\gamma_\alpha$ is larger than the exponent $\gamma_\delta$ completes the proof of the estimate~\eqref{eq:TV14282}.




\section{Homogenization of the mixed derivative of the Green's matrix} \label{sec:section6.2}

In this section, we use Proposition~\ref{prop:prop6.1} to prove Theorem~\ref{thm:homogmixedder}. We fix a charge $q_1 \in \mathcal{Q}$ and recall the definitions of the maps $\mathcal{U}_{q_1}$ and $\bar G_{q_1}$ given in the statement of Theorem~\ref{prop:prop6.1}. The proof is decomposed into four sections and follows the outline of the proof given in Section~\ref{sec3.2chap60851}.

and first record some preliminary estimates about the function $\mathcal{U}_{q_1}$ and $\bar G_{q_1}$.

\subsection{Preliminary estimates}

In this section, we record some properties pertaining to the functions $\mathcal{U}_{q_1}$ and $\bar G_{q_1}$ which are used in the argument.

\begin{proposition} \label{prop:prop6.5}
There exists an inverse temperature $\beta_0 := \beta_0(d) < 0$ and a constant $C_{q_1}$ which satisfies the estimate $C_{q_1} \leq C \left\| q_1 \right\|_{L^1}^k$, for some $C(d) < \infty$ and $k(d) < \infty$, such that the following statement holds. For each pair of points $y \in \Zd$ and each integer $k \in \N$, one has the estimates
\begin{equation*}
\left\| \nabla \mathcal{U}_{q_1} \left( y, \cdot \right)\right\|_{L^\infty \left(\mu_\beta \right)} \leq \frac{C_{q_1}}{|y|^{d-\ep}}, \hspace{3mm} \left\| \mathcal{U}_{q_1} \left( y , \cdot \right)\right\|_{L^\infty \left(\mu_\beta \right)} \leq \frac{C_{q_1}}{|y|^{d-1-\ep}} \hspace{3mm} \mbox{and} \hspace{3mm} \left| \nabla^k \bar G_{q_1} (y) \right| \leq \frac{C_{q_1}}{|y |^{d-1 + k}}.
\end{equation*}
\end{proposition}

\begin{proof}
The proof is a consequence of the regularity estimates given in Proposition~\ref{prop.prop4.11} and the identity $q = \di n_q$.
\end{proof}

%We now prove Theorem~\ref{thm:homogmixedder} following the outline described at the beginning of Section~\ref{sec:section6}.

\subsection{Exploiting the symmetry of the Helffer-Sj{\"o}strand operator} \label{sec4.2explsymmHS} The objective of this section is to use Proposition~\ref{prop:prop6.2} and the symmetry of the Helffer-Sj{\"o}strand operator $\mathcal{L}$ to prove the following estimate of the expectations
\begin{equation} \label{eq:TV07495}
    \left( R^{-d} \sum_{z\in A_R} \left| \left\langle \mathcal{U}_{q_1}(z, \cdot) \right\rangle_{\mu_\beta} - \bar G_{q_1}(z) \right|^2 \right)^\frac 12 \leq \frac{C}{R^{d+\gamma_\delta}}.
\end{equation}
We start from the formula
\begin{equation} \label{eq:TV22283}
\left\| \di^* \mathcal{G} - \sum_{i,j} \left( \di^* l_{e_{ij}} + \di^* \chi_{ij} \right) \nabla_i \bar G \right\|_{\underline{L}^2 \left(A_R,  \mu_\beta\right)} \leq \frac{C}{R^{ d-1 + \gamma_\delta}},
\end{equation}
which is a direct consequence of Proposition~\ref{prop:prop6.1} since the codifferential is a linear functional of the gradient.
Using the estimate~\eqref{eq:TV22283}, we deduce that
\begin{multline*}
    R^{-d} \sum_{x \in A_R} \left| \left\langle \cos \left( \phi , q_1(x + \cdot) \right)  \left( n_{q_1}\left( x + \cdot \right), \di^* \mathcal{G} \right) \right\rangle_{\mu_\beta}- \sum_{i,j} \left\langle \cos \left( \phi , q_1(x + \cdot) \right) \left( n_{q_1}\left( x + \cdot \right) \left(\di^* l_{e_{ij}} + \di^* \chi_{ij}\right) \right)  \right\rangle_{\mu_\beta }\nabla_i \bar G(x) \right| \\ \leq \frac{C_{q_1}}{R^{d - 1+\gamma}}.
\end{multline*}
By the translation invariance of the measure $\mu_\beta$ and the stationarity of the gradient of the infinite-volume corrector, we deduce that
\begin{align*}
    \sum_{i,j} \left\langle \cos \left( \phi , q_1(x + \cdot) \right) \left( n_{q_1}\left( x + \cdot \right) \left(\di^* l_{e_{ij}} + \di^* \chi_{ij}\right) \right)  \right\rangle_{\mu_\beta }\nabla_i \bar G(x) & = \sum_{i,j} \left\langle \cos \left( \phi , q_1 \right) \left( n_{q_1} \left( \di^* l_{e_{ij}} + \di^* \chi_{ij} \right) \right)  \right\rangle_{\mu_\beta }\nabla_i \bar G(x) \\
    & = \bar G_{q_1} \left( x \right).
\end{align*}
We now claim that we have the identity, for each point $x \in A_R$,
\begin{equation*}
    \left\langle \cos \left( \phi , q_1(x + \cdot) \right)  \left( n_{q_1}\left( x + \cdot \right), \di^* \mathcal{G} \right) \right\rangle_{\mu_\beta} = \left\langle \mathcal{U}_{q_1(x + \cdot)} (0 , \cdot) \right\rangle_{\mu_\beta}.
\end{equation*}
The proof of this result is a consequence of the symmetry of the Helffer-Sj{\"o}strand operator $\L$. To argue this, we use the computation
\begin{align*}
     \left\langle \cos \left( \phi , q_1(x + \cdot) \right)  \left( n_{q_1}\left( x + \cdot \right), \di^* \mathcal{G} \right) \right\rangle_{\mu_\beta} & =  \left\langle   \left( \cos \left( \phi , q_1(x + \cdot) \right) q_1\left( x + \cdot \right),  \mathcal{G} \right) \right\rangle_{\mu_\beta} \\
     & = \left\langle   \left( \cos \left( \phi , q_1(x + \cdot) \right) q_1\left( x + \cdot \right),  \L^{-1}\delta_0 \right) \right\rangle_{\mu_\beta} \\
     & = \left\langle   \left( \L^{-1} \cos \left( \phi , q_1(x + \cdot) \right) q_1\left( x + \cdot \right), \delta_0 \right) \right\rangle_{\mu_\beta} \\
     & = \left\langle \mathcal{U}_{q_1(x + \cdot)} (0, \cdot) \right\rangle_{\mu_\beta}.
\end{align*}
A combination of the four previous displays implies
\begin{equation} \label{eq:TV8194}
    R^{-d}\sum_{x\in A_R} \left| \left\langle \mathcal{U}_{q_1 \left( x + \cdot \right)}(0, \cdot) \right\rangle_{\mu_\beta} - \bar G_{q_1}( x) \right| \leq \frac{C}{R^{d+\gamma_\delta}}.
\end{equation}
We then use the translation invariance of the measure $\mu_\beta$ and the definition of the map $\mathcal{U}_{q_1}$ as the solution of the Helffer-Sj{\"o}strand equation~\eqref{eq:defmathcalU} to write
\begin{equation} \label{eq:TV21154}
    \left\langle \mathcal{U}_{q_1 \left( x + \cdot \right)}(0, \cdot) \right\rangle_{\mu_\beta} = \left\langle \mathcal{U}_{q_1}(x, \cdot) \right\rangle_{\mu_\beta}.
\end{equation}
Combining the inequality~\eqref{eq:TV8194} with the identity~\eqref{eq:TV21154}, we obtain
\begin{equation*}
    R^{-d}\sum_{x\in A_R} \left| \left\langle \mathcal{U}_{q_1}(x, \cdot) \right\rangle_{\mu_\beta} - \bar G_{q_1}( x) \right| \leq \frac{C}{R^{d+\gamma_\delta}}.
\end{equation*}
We finally upgrade the $L^1$-inequality stated in~\eqref{eq:TV8194} into an $L^2$-inequality: by using Proposition~\ref{prop:prop6.5}, we write
\begin{align*}
    \lefteqn{R^{-d}\sum_{x\in A_R} \left| \left\langle \mathcal{U}_{q_1}(x, \cdot) \right\rangle_{\mu_\beta} - \bar G_{q_1}(x) \right|^2} \qquad & \\ & \leq \left(R^{-d}\sum_{x\in A_R} \left| \left\langle \mathcal{U}_{q_1}(x, \cdot) \right\rangle_{\mu_\beta} - \bar G_{q_1}(x) \right|\right) \left(  \left\| \mathcal{U}_{q_1}(x, \cdot) \right\|_{L^\infty \left(A_R, \mu_\beta\right)}  + \left\| \bar G_{q_1} \right\|_{L^\infty \left(A_R \right)}\right) \\
    & \leq \frac{C_{q_1} }{R^{d-1+\gamma_\delta} \times R^{d-1-\ep}} \\
    & \leq \frac{C_{q_1} }{R^{2d-2+\gamma_\delta}},
\end{align*}
where we have used the convention notation described at the beginning of Section~\ref{sec:section6.1} to absorb the exponent $\ep$ into the exponent $\gamma_\delta$ in the third inequality.

\medskip

\subsection{Contraction of the variance of $\mathcal{U}_{q_1}$} \label{SEctiocontracvar4.3chap7} In this section, we prove that the random variable $\mathcal{U}_{q_1}$ contracts around its expectation. To this end, we prove the variance estimate, for each point $z \in \Zd$,
\begin{equation} \label{eq:TV08015}
    \var \left[ \mathcal{U}_{q_1}(z, \cdot) \right] \leq \frac{C_{q_1}}{|z|^{2d-2\ep}}.
\end{equation}
Let us make a comment about the result: since the size of the random variable $\mathcal{U}_{q_1}(z, \cdot)$ is of order $|z|^{1-d}$ (since is behaves like the gradient of a Green's function), we would expect its variance to be of order $|z|^{2-2d}$. The inequality~\eqref{eq:TV08015} asserts that it is in fact of order $|z|^{2d - 2\ep}$ which is smaller than the typical size of the random variable $\mathcal{U}_{q_1}(z, \cdot)$ by an algebraic factor.

Once this estimate is established, we can combine it with the main result~\eqref{eq:TV07495} of Section~\ref{sec4.2explsymmHS} to prove that the map $\mathcal{U}_{q_1}$ is close to the (deterministic) Green's function $\bar G_{q_1}$ in the $\underline{L}^2 \left( A_R , \mu_\beta \right)$-norm: we obtain the inequality
\begin{equation} \label{eq:TV16256}
    \left\| \mathcal{U}_{q_1} - \bar G_{q_1} \right\|_{\underline{L}^2 \left( A_R , \mu_\beta \right)} \leq \frac{C}{R^{d-1-\gamma_\delta}}.
\end{equation}
We now prove of the variance estimate~\eqref{eq:TV08015}. We first apply the Brascamp-Lieb inequality and write
\begin{equation} \label{eq:TV08435}
     \var \left[ \mathcal{U}_{q_1}(z, \cdot) \right] \leq C \sum_{y,y_1 \in \Zd} \left\| \partial_y \mathcal{U}_{q_1}(z, \cdot)  \right\|_{L^2 \left( \mu_\beta \right)} \frac{C}{|z - z_1|^{d-2}} \left\| \partial_{z_1} \mathcal{U}_{q_1}(z, \cdot)  \right\|_{L^2 \left( \mu_\beta \right)}.
\end{equation}
A consequence of the inequality~\eqref{eq:TV08435} is that to estimate the variance of the random variable $\mathcal{U}_{q_1}(z,\cdot)$, it is sufficient to understand the behavior of the mapping $y \mapsto \partial_y \mathcal{U}_{q_1}(z, \cdot)$. To this end, we appeal to the differentiated Helffer-Sj{\"o}strand equation: following the arguments developed in Section~\ref{sec.section4.5} of Chapter REF, the map $u : (y , z , \phi) \mapsto \partial_y \mathcal{U}_{q_1}(z , \phi)$ is solution of the equation
\begin{equation*}
    \L_{\mathrm{der}} u (x , y , \phi) = -  \sum_{q \in \mathcal{Q}}  z \left( \beta , q\right) \cos \left( \phi , q \right) \left( \mathcal{U}_{q_1}, q \right) q(x) \otimes q(y) + \sin \left( \phi , q_1 \right) q_1 (x) \otimes q_1(y) \hspace{3mm} \mbox{in} \hspace{3mm} \Zd \times \Zd \times \Omega.
\end{equation*}
The function $u$ can be expressed in terms of the derived Green's function $\mathcal{G}_{\mathrm{der}}$ and we write, for each triplet $(x , y , \phi) \in \Zd \ \times \Zd \times \Omega$,
\begin{align*}
     u (x , y , \phi) & = \sum_{q \in \mathcal{Q}} z \left( \beta , q \right) \sum_{x_1 , y_1 \in \Zd} \di^*_{x_1} \di^*_{y_1} \G_{\mathrm{der}, \cos \left( \phi , q \right) \left( \mathcal{U}_{q_1}, q \right)} \left( x , y , \phi ; x_1 , y_1 \right) n_{q}(x_1) \otimes n_{q}(y_1)  \\
     & \quad + \sum_{x_1 , y_1 \in \Zd} \di^*_{x_1} \di^*_{y_1} \G_{\mathrm{der}, \sin \left( \phi , q_1 \right)} \left( x , y , \phi ; x_1 , y_1 \right)  n_{q_1} (x) \otimes n_{q_1}(y).
\end{align*}
We use the regularity estimates on the differentiated Green's function stated in Proposition~\ref{cor:corollary4.14} of Chapter 5 to obtain, for each pair of points $(x , y) \in \Zd \times \Zd$,
\begin{align} \label{eq:TV10395}
    \left\| u (x , y , \cdot) \right\|_{L^\infty \left( \mu_\beta \right)} & \leq \underbrace{C \sum_{q \in \mathcal{Q}} e^{-c \sqrt{\beta} \left\| q \right\|_{L^1}} \sum_{x_1 , y_1 \in \Zd} \frac{\left| n_q(x_1) \right| \left| n_q(y_1) \right| \left\| \left( \di^* \mathcal{U}_{q_1} , n_q \right) \right\|_{L^\infty \left( \mu_\beta \right)} }{|x - x_1|^{2d - \ep} + |y - y_1|^{2d - \ep}}}_{\eqref{eq:TV10395}-(i)} \\
    & \quad + \underbrace{\sum_{x_1 , y_1 \in \Zd} \frac{\left| n_{q_1}(x_1) \right| \left| n_{q_1}(y_1) \right| }{|x - x_1|^{2d - \ep} + |y - y_1|^{2d - \ep}}}_{\eqref{eq:TV10395}-(ii)}. \notag
\end{align}
We then estimate the two terms~\eqref{eq:TV10395}-(i) and~\eqref{eq:TV10395}-(ii) separately. We first focus on the term~\eqref{eq:TV10395}-(i) and prove the inequality
\begin{equation} \label{eq:TV16095}
    \eqref{eq:TV10395}-(i) \leq  \frac{C_{q_1}}{|x-y|^{d - \ep} \max \left( \left| x \right|, \left| y \right|\right)^{d-1}}
\end{equation}
To prove the estimate~\eqref{eq:TV16095}, we first decompose the set of charges $\mathcal{Q}$ according to the following procedure. For each $z \in \Zd$, we denote by $\mathcal{Q}_z$ the set of charges $q \in \mathcal{Q}$ such that the point $z$ belongs to the support of $n_q$, i.e., $\mathcal{Q}_z := \left\{ q \in \mathcal{Q} \, : \, z \in \supp n_q  \right\}$. We note that we have the equality $\mathcal{Q} := \bigcup_{z \in \Zd} \mathcal{Q}_z$ but the collection $\left( \mathcal{Q}_z\right)_{z \in \Zd}$ is not a partition of $\mathcal{Q}$. We first prove that, for each point $z \in \Zd$,
\begin{equation} \label{eq:TV16585}
    \sum_{q \in \mathcal{Q}_z} e^{-c\sqrt{\beta} \left\| q \right\|_{L^1}}\sum_{x_1 , y_1 \in \Zd} \frac{\left| n_q(x_1) \right| \left| n_q(y_1) \right| \left\| \left( \di^* \mathcal{U}_{q_1} , n_q \right) \right\|_{L^\infty \left( \mu_\beta \right)}}{|x - x_1|^{2d - \ep} + |y - y_1|^{2d - \ep}} \leq \frac{C_{q_1}}{\left(|x - z|^{2d-\ep} + |y - z|^{2d-\ep}\right) \times |z|^{d-\ep} }
\end{equation}
To prove the estimate~\eqref{eq:TV16585}, we first use Proposition~\ref{prop:prop6.5} to estimate the term $\left\| \left( \delta \mathcal{U}_{q_1} , n_q \right) \right\|_{L^\infty \left( \mu_\beta \right)}$. We write, for each charge $q \in \mathcal{Q}_z$,
\begin{align} \label{eq:TV17545}
    \left\| \left( \di^* \mathcal{U}_{q_1} , n_q \right) \right\|_{L^\infty \left( \mu_\beta \right)} & \leq \left\| \nabla \mathcal{U}_{q_1} \right\|_{L^\infty \left( \supp n_q , \mu_\beta \right)} \left\| n_q \right\|_{L^1} \\
    & \leq C_{q_1,q} \inf_{z_1 \in \supp n_q} \frac{1}{|z_1|^{d-\ep}}. \notag
\end{align}
Since we have assumed that the point $z$ belongs to the support of the charge $n_q$, we have the inequality
\begin{equation} \label{eq:TV17555}
    \inf_{z_1 \in \supp n_q} \frac{1}{|z_1|^{d-\ep}} \leq \frac{\left| \diam n_q\right|^{d - \ep}}{|z|^{d-\ep}} \leq \frac{C_q}{|z|^{d-\ep}}.
\end{equation}
Combining the estimates~\eqref{eq:TV17545},~\eqref{eq:TV17555}, we deduce that
\begin{equation} \label{eq:TV18015}
    \left\| \left( \di^* \mathcal{U}_{q_1} , n_q \right) \right\|_{L^\infty \left( \mu_\beta \right)} \leq \frac{C_{q_1,q}}{|z|^{d - \ep}}.
\end{equation}
Putting the inequality~\eqref{eq:TV18015} back into the left side of the estimate~\eqref{eq:TV16585}, we obtain
\begin{align} \label{eq:TV19005}
    \lefteqn{\sum_{q \in \mathcal{Q}_z} e^{-c\sqrt{\beta} \left\| q \right\|_{L^1}}\sum_{x_1 , y_1 \in \Zd} \frac{\left| n_q(x_1) \right| \left| n_q(y_1) \right| \left\| \left( \delta \mathcal{U}_{q_1} , n_q \right) \right\|_{L^\infty \left( \mu_\beta \right)}}{|x - x_1|^{2d - \ep} + |y - y_1|^{2d - \ep}}} \qquad & \\ &
    \leq \sum_{q \in \mathcal{Q}_z} \frac{Ce^{-c\sqrt{\beta}   \left\| q \right\|_{L^1}} C_{q,q_1}}{|z|^{d - \ep}} \sum_{x_1 , y_1 \in \supp n_q}  \frac{1}{|x - x_1|^{2d - \ep} + |y - y_1|^{2d - \ep}}. \notag
\end{align}
Using that, for a given charge $q \in \mathcal{Q}_z$, the point $z$ belongs to the support of $q$, we write
\begin{equation} \label{eq:TV19015}
     \frac{1}{|x - x_1|^{2d-\ep} + |y - y_1|^{2d - \ep}} \leq \frac{\left| \diam n_{q}\right|^{2d}}{|x - z|^{2d-\ep} + |y - z|^{2d - \ep}} \leq \frac{C_q}{|x - z|^{2d-\ep} + |y-z|^{2d - \ep}}.
\end{equation}
We then combine the estimates~\eqref{eq:TV19005} and~\eqref{eq:TV19015} and use the exponential decay of the coefficient $e^{-c \sqrt{\beta}\left\| q \right\|_{L^1}}$ to absorb the algebraic growth of the constant $C_{q_1 , q}$ in the variable $\left\| q_1 \right\|_{L^1}$. We obtain
\begin{equation*}
    \sum_{q \in \mathcal{Q}_z} e^{-c\sqrt{\beta} \left\| q \right\|_{L^1}}\sum_{x_1 , y_1 \in \Zd} \frac{\left| n_q(x_1) \right| \left| n_q(y_1) \right| \left\| \left( \di^* \mathcal{U}_{q_1} , n_q \right) \right\|_{L^\infty \left( \mu_\beta \right)}}{|x - x_1|^{2d - \ep} + |y - y_1|^{2d - \ep}} \leq \frac{C_{q_1}}{|z|^{d-\ep}\times \left( |x - z|^{2d-\ep} + |y - z|^{2d-\ep}  \right)}.
\end{equation*}
The proof of the estimate~\eqref{eq:TV16585} is complete. We then use the identity $\mathcal{Q} := \bigcup_{z \in \Zd} \mathcal{Q}_z$ to write
\begin{align} \label{eq:TV08086}
    \eqref{eq:TV10395}-(i) & =  \sum_{q \in \mathcal{Q}_z} e^{-c\sqrt{\beta} \left\| q \right\|_{L^1}}\sum_{x_1 , y_1 \in \Zd} \frac{\left| n_q(x_1) \right| \left| n_q(y_1) \right| \left\| \left( \di^* \mathcal{U}_{q_1} , n_q \right) \right\|_{L^\infty \left( \mu_\beta \right)}}{|x - x_1|^{2d - \ep} + |y - y_1|^{2d - \ep}} \\
    & \leq \sum_{z \in \Zd}  \sum_{q \in \mathcal{Q}_z} e^{-c\sqrt{\beta} \left\| q \right\|_{L^1}}\sum_{x_1 , y_1 \in \Zd} \frac{\left| n_q(x_1) \right| \left| n_q(y_1) \right| \left\| \left( \delta \mathcal{U}_{q_1} , n_q \right) \right\|_{L^\infty \left( \mu_\beta \right)}}{|x - x_1|^{2d - \ep} + |y - y_1|^{2d - \ep}} \notag \\
    & \leq  \sum_{z \in \Zd}  \frac{C_{q_1}}{|z|^{d-\ep} \times \left( |x - z|^{2d-\ep} + |y - z|^{2d-\ep}  \right)}. \notag
\end{align}
We estimate the sum in the right side of the estimate~\eqref{eq:TV08086}. To this end, we note that, for each triplet $(x,y,z) \in \Zd \times \Zd \times \Zd$,
\begin{align} \label{eq:TV08576}
    \left( |x - z|^{2d-\ep} + |y - z|^{2d-\ep}  \right) \geq c \dist_{\Z^{2d}} \left( (x,y) , (z,z) \right)^{^{2d-\ep}} & \geq c \left( \left| \frac{x-y}{2} \right|^2 + \left| \frac{x+y}{2} - z \right|^2 \right)^{\frac{2d-\ep}{2}} \\ & \geq c \left( \left| x-y \right|^{2d-\ep} + \left| \frac{x+y}{2} - z \right|^{2d-\ep} \right), \notag
\end{align}
where the notation $\dist_{\Z^{2d}}\left( (x,y) , (z,z) \right)$ is used to denote the euclidean distance in the lattice $\Z^{2d}$ between the points $(x,y)$ and $(z,z)$, the second inequality is obtained by computing the orthogonal projection of the point $(x,y) \in \Z^{2d}$ on the diagonal $\left\{ (z,z) \in \Z^{2d} \, : \, z \in \Zd \right\}$ and the third inequality is obtained by reducing the value of the constant $c$. Using the estimate~\eqref{eq:TV08576}, we deduce
\begin{align} \label{eq:TV10006}
    \sum_{z \in \Zd}  \frac{1}{|z|^{d-\ep} \times \left( |x - z|^{2d-\ep} + |y - z|^{2d-\ep}  \right)} & \leq \sum_{z \in \Zd} \frac{1}{|z|^{d-1}} \times \frac{1}{ \left| x-y \right|^{2d-\ep} + \left| \frac{x+y}{2} - z \right|^{2d-\ep}} \\
    & \leq \sum_{z \in \Zd} \frac{1}{|z|^{d-\ep}} \times \frac{1}{ \left| x-y \right|^{2d-\ep} + \left| \frac{x+y}{2} - z \right|^{2d-\ep}} \notag \\
    & \leq \frac{C}{|x-y|^{d - \ep} \max \left( \left| x \right|, \left| y \right|\right)^{d-\ep}}. \notag
\end{align}
\pdcomment{maybe we can prove this; maybe 2 $\ep$..}
Combining the estimates~\eqref{eq:TV08086} and~\eqref{eq:TV10006} completes the proof of the estimate~\eqref{eq:TV16095}.

To estimate the term~\eqref{eq:TV10395}-(ii), we use that $0$ belongs to the support of the charge $n_{q_1}$ to write, for each pair of points $x_1,y_1 \in \supp n_{q_1}$,
\begin{equation} \label{eq:TV14175}
    \frac{1}{|x - x_1|^{2d-\ep} + |y - y_1|^{2d - \ep}} \leq \frac{\left| \diam n_{q_1}\right|^{2d}}{|x|^{2d-\ep} + |y|^{2d-\ep}} \leq \frac{C_{q_1}}{|x|^{2d-\ep} + |y|^{2d - \ep}}.
\end{equation}
From the inequality~\eqref{eq:TV14175}, we deduce
\begin{equation} \label{eq:TV19375}
    \eqref{eq:TV10395}-(ii) = \sum_{x_1 , y_1 \in \Zd} \frac{\left| n_{q_1}(x_1) \right| \left| n_{q_1}(y_1) \right| }{|x - x_1|^{2d - \ep} + |y - y_1|^{2d - \ep}} \leq \frac{C_{q_1}}{|x|^{2d - \ep} + |y|^{2d-\ep}}.
\end{equation}
We then combine the estimates~\eqref{eq:TV10395},~\eqref{eq:TV16095},~\eqref{eq:TV19375} to deduce the inequality, for each pair of points $x , y \in \Zd$,
\begin{align} \label{eq:TV10186}
    \left\| u (x , y , \cdot) \right\|_{L^\infty \left( \mu_\beta \right)} & \leq \frac{C_{q_1}}{|x-y|^{d - \ep} \max \left( \left| x \right|, \left| y \right|\right)^{d-\ep}} + \frac{C_{q_1}}{|x|^{2d - \ep} + |y|^{2d-\ep}} \\
    & \leq \frac{C_{q_1}}{|x-y|^{d - \ep} \max \left( \left| x \right|, \left| y \right|\right)^{d-\ep}}. \notag
\end{align}
We then use this inequality to estimate the variance of the random variable $\mathcal{U}_{q_1}(x , \cdot)$ by using the formula~\eqref{eq:TV08435}. We obtain
\begin{equation*}
    \var \left[ \mathcal{U}_{q_1}(z, \cdot) \right] \leq C \sum_{y,y_1 \in \Zd} \frac{C_{q_1}}{|z-y|^{d - \ep} \max \left( \left| z \right|, \left| y \right|\right)^{d-1}} \cdot \frac{C}{|y - y_1|^{d-2}} \cdot \frac{C_{q_1}}{|z-y_1|^{d - \ep}  \max \left( \left| z \right|, \left| y_1 \right|\right)^{d-\ep}}.
\end{equation*}
We then use that the terms $\max \left( \left| z \right|, \left| y_1 \right|\right)$ and $\max \left( \left| z \right|, \left| y \right|\right)$ are both larger than the value $|z|$ to deduce that
\begin{equation*}
    \var \left[ \mathcal{U}_{q_1}(z, \cdot) \right] \leq \frac{C_{q_1}}{|z|^{2 d - 2 \ep}} \sum_{y,y_1 \in \Zd} \frac{1}{|z-y|^{d - \ep}} \cdot \frac{1}{|y - y_1|^{d-2}} \cdot \frac{1}{|z-y_1|^{d - \ep}} \leq \frac{C_{q_1}}{|z|^{2 d - 2 \ep}}.
\end{equation*}
The proof of the estimate~\eqref{eq:TV08015} is complete.

\medskip

\subsection{Homogenization of the mixed derivative of the Green's matrix} We fix a radius $R > 1$ and let $m$ be the smallest integer such that the annulus $A_R$ is included in the cube $\cu_m$. The proof relies on a two-scale expansion following the outline described in Section~\ref{sec3.2chap60851}. We define the function $\mathcal{H}_{q_1}$ by the formula
\begin{equation} \label{eq:TVdefHq12scexp}
    \mathcal{H}_{q_1} := \bar G_{q_1} + \sum_{i,j} \nabla_i \bar G_{q_1} \chi_{m,i}.
\end{equation}
We decompose the argument into three Steps.

\medskip

\textit{Step 1.} In this step, we prove that the $\underline{H}^{-1}\left( A_R , \mu_\beta \right)$-norm of the term $\mathcal{L} \mathcal{H}_{q_1}$ is small, more specifically, we prove that there exists an exponent $\gamma_\alpha > 0$ such that one has the estimate
\begin{equation} \label{eq:TV15356}
    \left\| \mathcal{L} \mathcal{H}_{q_1} \right\|_{\underline{H}^{-1}\left( A_R , \mu_\beta \right)} \leq \frac{C_{q_1}}{R^{d - \gamma_\alpha}}.
\end{equation}
The proof is essentially identical to the argument presented in Section~\ref{sec3.2chap60851}: we use the exact formula for the two-scale expansion $\mathcal{H}_{q_1}$ given in~\eqref{eq:TVdefHq12scexp} to compute the value of $\L \mathcal{H}_{q_1}$ and then use the quantitative properties of the corrector stated in Proposition~\ref{prop:prop5.25} to prove that the $\underline{H}^{-1}\left( A_R , \mu_\beta \right)$-norm of the term $ \mathcal{L} \mathcal{H}_{q_1}$ satisfies the estimate~\eqref{eq:TV15356}. Since the proof is rather long due to the technicalities caused by the specific structure of the operator $\mathcal{L}$ (iterations of the Laplacian, sum over all the charges $q \in \mathcal{Q}$), we do not rewrite it but only point out the main differences:
\begin{itemize}
    \item We work in the annulus $A_R$ and not in the ball $B_{R^{1+\delta}}$, this difference makes the proof simpler since we do not have to take the additional parameter $\delta$ into considerations;
    \item We can always assume that the diameter of the charge $q_1$ is smaller than $R/2$, otherwise the constant $C_{q_1}$ is larger than $R^k$ for some large number $k := k(d)$ (since it is allowed to have an algebraic growth in the parameter $\left\| q_1 \right\|_{L^1}$) and the estimate~\eqref{eq:TV15356} is trivial in this situation. Under the assumption $\diam q_1 \leq R/2$, we use the identity $- \ahom \Delta \bar G_{q_1} = 0$ in the annulus $A_R$ instead of the identity $- \ahom \Delta \bar G_\delta = \rho_\delta$ in the ball $B_{R^{1+\delta}}$;
    \item We use the regularity estimates on the function $\bar G_{q_1}$ stated in Proposition~\ref{prop:prop6.5} instead of the estimates on the Green's function $\bar G$ stated in Proposition~\ref{prop:prop6.2}. Since the map $\bar G_{q_1}$ scales like the gradient of the Green's function (in particular it decays like $|x|^{1-d}$), we obtain an additional factor $R$ in the right side of~\eqref{eq:TV15356} compared to~\eqref{eq:TV19578}, i.e., we obtain
    \begin{equation*}
        \left\| \mathcal{L} \mathcal{H}_{q_1} \right\|_{\underline{H}^{-1}\left( A_R , \mu_\beta \right)} \leq \frac{C_{q_1}}{R^{d - \gamma_\alpha}} \hspace{3mm} \mbox{instead of}  \hspace{3mm} \left\| \mathcal{L} \mathcal{H} - \rho_\delta \right\|_{\underline{H}^{-1}\left( A_R , \mu_\beta \right)} \leq \frac{C}{R^{d - 1 - \gamma_\alpha}}.
    \end{equation*}
\end{itemize}

\medskip


\textit{Step 2.} In this step, we use the main result~\eqref{eq:TV15356} of Substep 3.1 to prove that the gradient of the Green's function $\nabla \mathcal{U}_{q_1}$ is close to the gradient of the two-scale expansion $\nabla \mathcal{H}_{q_1}$ in the $\underline{L}^2\left(A_R , \mu_\beta \right)$-norm. We prove the estimate
\begin{equation} \label{eq:TV17086}
    \left\| \nabla \mathcal{U}_{q_1} - \nabla \mathcal{H}_{q_1} \right\|_{\underline{L}^2 \left( A_R , \mu_\beta \right)} \leq \frac{C_{q_1}}{R^{d+\gamma_\alpha}}.
\end{equation}

Since it is convenient in the rest of the argument, we do not prove the estimate~\eqref{eq:TV17086} directly. We slightly reduce the size of the annulus $A_R$ and define the set $A_R^1$ to be the annulus $A_R^1 := \left\{ x \in \Zd \, : \, 1.1 R \leq |x| \leq 1.9R \right\}$. We note that we have the inclusion, for each radius $R \geq 1$, $A_R^1 \subseteq A_R$. In this substep, we prove the inequality
\begin{equation} \label{eq:TV17096}
    \left\| \nabla \mathcal{U}_{q_1} - \nabla \mathcal{H}_{q_1} \right\|_{\underline{L}^2 \left( A_R^1 , \mu_\beta \right)} \leq \frac{C_{q_1}}{R^{d+\gamma_\delta}}.
\end{equation}
The inequality~\eqref{eq:TV17086} can then be deduced from~\eqref{eq:TV17096} by a covering argument.

The argument is similar to the one presented in Section~\ref{sec3.3chap60851} except that, instead of making use of the boundary layer exponent $\delta$ to prove that the $H^1$-norm is of the difference $\left( \nabla \mathcal{H}_\delta - \G_\delta \right)$ is small, as it was done in the estimates~\eqref{eq:TV07591} and~\eqref{eq:TV07601}, we use the main result~\eqref{eq:TV16256} of Section~\ref{SEctiocontracvar4.3chap7}. We first let $\eta$ be a cutoff function which satisfies the properties:
\begin{equation} \label{eq:propetebis}
    0 \leq \eta \leq 1, ~\supp \eta \subseteq A_R,~ \eta = 1 ~\mbox{in}~A_R^1,~\forall k \in \N, \, \left| \nabla^k \eta \right| \leq \frac{C}{R^k}.
\end{equation}
We then use the function $\eta \left( \mathcal{U}_{q_1} - \mathcal{H}_{q_1}\right)$ as a test function in the definition of the $\underline{H}^{-1} \left(A_R, \mu_\beta \right)$ of the inequality~\eqref{eq:TV15356} and use the identity $\L \mathcal{U}_{q_1} = 0$ in $A_R \times \Omega$. We obtain
\begin{align} \label{eq:TV10172112}
    \frac{1}{R^{d}}\sum_{x \in A_R} \left\langle \eta \left( \mathcal{U}_{q_1} - \mathcal{H}_{q_1}\right) \L \left( \mathcal{U}_{q_1} -  \mathcal{H}_{q_1} \right)  \right\rangle_{\mu_\beta} & \leq \left\| \L \left( \mathcal{U}_{q_1} - \mathcal{H}_{q_1} \right) \right\|_{\underline{H}^{-1} \left( B_{R^{1+\delta}} , \mu_\beta \right)} \left\|  \eta \left( \mathcal{U}_{q_1} -  \mathcal{H}_{q_1} \right)  \right\|_{\underline{H}^1 \left( A_R , \mu_\beta \right)} \\
    & \leq \frac{C}{R^{d + \gamma_\alpha}} \left\| \eta \left( \mathcal{U}_{q_1} - \mathcal{H}_{q_1} \right) \right\|_{\underline{H}^1 \left( A_R , \mu_\beta \right)}. \notag
\end{align}
We then estimate the $\underline{H}^1 \left( A_R , \mu_\beta \right)$-norm of the function $\mathcal{U}_{q_1} - \mathcal{H}_{q_1}$ with similar arguments as the one presented in the proof of the inequality~\eqref{eq:TV15049}, the only difference is that we use the regularity estimates stated in Proposition~\ref{prop:prop6.5} instead of the regularity estimates for the functions $\G_\delta$ and $\mathcal{H}$. We obtain
\begin{equation} \label{eq:TV10182112}
    \left\| \eta \left( \mathcal{U}_{q_1} - \mathcal{H}_{q_1} \right) \right\|_{\underline{H}^1 \left( A_R , \mu_\beta \right)} \leq \left\| \eta \mathcal{U}_{q_1} \right\|_{\underline{H}^1 \left( A_R , \mu_\beta \right)} + \left\| \eta  \mathcal{H}_{q_1} \right\|_{\underline{H}^1 \left( A_R , \mu_\beta \right)} \leq  \frac{C_{q_1}}{R^{d - \ep}}.
\end{equation}
For later use, we also note that the same argument yields to the inequality
\begin{equation} \label{eq:TV09577}
    \left\|\nabla  \mathcal{U}_{q_1} - \nabla \mathcal{H}_{q_1}  \right\|_{\underline{L}^2 \left( A_R , \mu_\beta \right)} \leq \left\|\nabla  \mathcal{U}_{q_1}  \right\|_{\underline{L}^2 \left( A_R , \mu_\beta \right)}  + \left\|\nabla  \mathcal{H}_{q_1} \right\|_{\underline{L}^2 \left( A_R , \mu_\beta \right)}  \leq  \frac{C_{q_1}}{R^{d - \ep}}.
\end{equation}
We then combine the inequalities~\eqref{eq:TV10172112} and~\eqref{eq:TV10172112} and use that $\ep \ll \gamma_\alpha$ to deduce that
\begin{equation} \label{eq:TV12287}
    \frac{1}{R^{d}}\sum_{x \in A_R} \left\langle \eta \left( \mathcal{U}_{q_1} - \mathcal{H}_{q_1}\right) \L \left( \mathcal{U}_{q_1} -  \mathcal{H}_{q_1} \right)  \right\rangle_{\mu_\beta} \leq \frac{C_{q_1}}{R^{2d + \gamma_\alpha}}.
\end{equation}
Thus to prove the inequality~\eqref{eq:TV17096}, it is sufficient to prove the estimate
\begin{equation*}
    \left\| \nabla \mathcal{U}_{q_1} - \nabla \mathcal{H}_{q_1} \right\|_{\underline{L}^2 \left( A_R^1 , \mu_\beta \right)}^2 \leq \frac{1}{R^{d}}\sum_{x \in A_R} \left\langle \eta \left( \mathcal{U}_{q_1} - \mathcal{H}_{q_1}\right) \L \left( \mathcal{U}_{q_1} -  \mathcal{H}_{q_1} \right)  \right\rangle_{\mu_\beta}  + \frac{C_{q_1}}{R^{2d+\gamma_\delta}}.
\end{equation*}
First, by definition of the Helffer-Sj{\"o}strand operator $\mathcal{L}$, we have the identity
\begin{align} \label{eq:TV081011}
\sum_{x \in \Zd} \left\langle \eta \left( \mathcal{U}_{q_1} -  \mathcal{H}_{q_1}\right) \L \left( \mathcal{U}_{q_1} -  \mathcal{H}_{q_1} \right)  \right\rangle_{\mu_\beta} & = \sum_{x , y \in \Zd} \eta(x) \left\langle \left( \partial_y \mathcal{U}_{q_1} (x , \cdot)  - \partial_y \mathcal{H}_{q_1} (x , \cdot) \right)^2 \right\rangle_{\mu_\beta} \\ & + \frac 1{2\beta}\sum_{x \in \Zd}  \left\langle  \left( \nabla \mathcal{U}_{q_1} - \nabla \mathcal{H}_{q_1}  \right)(x , \cdot) \cdot \nabla \left( \eta \left( \mathcal{U}_{q_1} -  \mathcal{H}_{q_1} \right)\right)(x , \cdot)  \right\rangle_{\mu_\beta} \notag \\ & +  \sum_{q \in \mathcal{Q}}  \left\langle \nabla_q \left(  \mathcal{U}_{q_1} -  \mathcal{H}_{q_1}\right) \cdot \a_q \nabla_q \left( \eta \left(  \mathcal{U}_{q_1} -  \mathcal{H}_{q_1} \right) \right) \right\rangle_{\mu_\beta} \notag \\ & +  \frac 1{2\beta} \sum_{n \geq 1} \sum_{x \in \Zd}  \frac{1}{\beta^{ \frac n2}} \left\langle  \nabla^{n+1} \left(  \mathcal{U}_{q_1} -  \mathcal{H}_{q_1} \right)(x , \cdot) \cdot \nabla^{n+1} \left( \eta \left(  \mathcal{U}_{q_1} -  \mathcal{H}_{q_1} \right) \right)(x,\cdot) \right\rangle_{\mu_\beta}. \notag
\end{align}
We then estimate the four terms on the right side separately. For the first one, we use that it is non-negative
\begin{equation} \label{eq:TV12137}
    \sum_{x , y \in \Zd} \eta(x)^2 \left\langle \left( \partial_y \mathcal{U}_{q_1} (x , \cdot)  - \partial_y \mathcal{H}_{q_1} (x , \cdot) \right)^2 \right\rangle_{\mu_\beta}  \geq 0.
\end{equation}
For the second one, we expand the gradient of the product $\eta^2 \left( \mathcal{U}_{q_1}  - \mathcal{H}_{q_1}  \right)$ and write
\begin{align} \label{eq:TV094901}
    \lefteqn{\sum_{x \in \Zd}  \left\langle  \left( \nabla \mathcal{U}_{q_1}  - \mathcal{H}_{q_1} \right)(x , \cdot) \cdot \nabla \left( \eta \left(\mathcal{U}_{q_1}  - \mathcal{H}_{q_1} \right)\right)(x , \cdot)  \right\rangle_{\mu_\beta}} \qquad & \\ &
    = \sum_{x \in \Zd}  \eta(x)  \left\langle  \left( \nabla \mathcal{U}_{q_1}  - \mathcal{H}_{q_1}\right)(x , \cdot) \cdot   \nabla \left(\mathcal{U}_{q_1}  - \mathcal{H}_{q_1} \right)(x , \cdot)  \right\rangle_{\mu_\beta} \notag \\
    & \quad + \sum_{x \in \Zd}  \left\langle  \left( \nabla \mathcal{U}_{q_1}  - \mathcal{H}_{q_1}\right)(x , \cdot) \cdot  \nabla \eta(x)\left( \mathcal{U}_{q_1}  - \mathcal{H}_{q_1} \right)(x , \cdot)  \right\rangle_{\mu_\beta}. \notag
\end{align}
Dividing the identity~\eqref{eq:TV094901} by the volume factor $R^{d}$ and using the properties of the function $\eta$ stated in~\eqref{eq:propetebis}, we obtain
\begin{multline} \label{eq:TV075917}
    R^{-d}\sum_{x \in \Zd}  \left\langle  \left( \nabla \mathcal{U}_{q_1} (x , \cdot)  - \nabla \mathcal{H}_{q_1} \right)(x , \cdot) \cdot \nabla \left( \eta \left( \G_\delta-  \mathcal{H} \right)\right)(x , \cdot)  \right\rangle_{\mu_\beta} \geq c \left\| \eta \left( \nabla \mathcal{U}_{q_1}  - \nabla \mathcal{H}_{q_1} \right) \right\|_{\underline{L}^2 \left(A_R , \mu_\beta \right)}^2 \\ -  \frac{C}{R} \left\| \nabla \mathcal{U}_{q_1}  \ - \nabla \mathcal{H}_{q_1} \right\|_{\underline{L}^2 \left( A_{R} , \mu_\beta \right)} \left\|  \mathcal{U}_{q_1}  - \mathcal{H}_{q_1} \right\|_{\underline{L}^2 \left( A_{R} , \mu_\beta \right)}.
\end{multline}
We then use the inequality~\eqref{eq:TV16256} and the estimate~\eqref{eq:TV09577} to deduce that
\begin{equation} \label{eq:TV10537}
    \frac{1}{R} \left\| \nabla \mathcal{U}_{q_1}  \ - \nabla \mathcal{H}_{q_1} \right\|_{\underline{L}^2 \left( A_{R} , \mu_\beta \right)} \left\|  \mathcal{U}_{q_1}  - \mathcal{H}_{q_1} \right\|_{\underline{L}^2 \left( A_{R} , \mu_\beta \right)} \leq \frac{1}{R} \cdot \frac{C}{R^{d - \ep}} \cdot \frac{C}{R^{d - 1 + \gamma_\delta}} \leq \frac{C}{R^{2d + \gamma_\delta}}.
\end{equation}
We then combine the inequalities~\eqref{eq:TV075917} and~\eqref{eq:TV10537} to deduce that
\begin{equation} \label{eq:TV11427}
     R^{-d}\sum_{x \in \Zd}  \left\langle  \left( \nabla \mathcal{U}_{q_1} (x , \cdot)  - \nabla \mathcal{H}_{q_1} \right)(x , \cdot) \cdot \nabla \left( \eta \left( \mathcal{U}_{q_1}  - \nabla \mathcal{H}_{q_1} \right)\right)(x , \cdot)  \right\rangle_{\mu_\beta} + \frac{C_{q_1}}{R^{2d + \gamma_\delta}} \geq c \left\| \eta \left( \nabla \mathcal{U}_{q_1}  - \nabla \mathcal{H}_{q_1} \right) \right\|_{\underline{L}^2 \left(A_R , \mu_\beta \right)}^2.
\end{equation}
The two remaining terms in the right side of the estimate~\eqref{eq:TV094901} (involving the iteration of the Laplacian and the sum over the charges) are estimated following the ideas developed in in Section~\ref{sec3.3chap60851} (see~\eqref{eq:TV11121} and~\eqref{eq:TV11131}) or in the proof of the Caccioppoli inequality (Proposition~\ref{Caccio.ineq} of Chapter 5). We skip the details and write the result: we obtain
\begin{equation} \label{eq:TV111211}
    R^{-d}\sum_{q \in \mathcal{Q}}  \left\langle \nabla_q \left(  \mathcal{U}_{q_1}  - \nabla \mathcal{H}_{q_1}\right) \cdot \a_q \nabla_q \left( \eta \left(  \mathcal{U}_{q_1}  - \nabla \mathcal{H}_{q_1} \right) \right) \right\rangle_{\mu_\beta}  + \frac{C_{q_1}}{R^{(2d-\gamma_\delta) }} \geq -C e^{-c \sqrt{\beta}} \left\| \eta \left( \nabla \mathcal{U}_{q_1}  - \nabla \mathcal{H}_{q_1} \right) \right\|_{\underline{L}^2 \left(A_R , \mu_\beta \right)}^2
\end{equation}
and
\begin{equation} \label{eq:TV111311}
    R^{-d} \sum_{n \geq 1} \sum_{x \in \Zd}  \frac{1}{\beta^{ \frac n2}} \left\langle  \nabla^{n+1} \left(  \mathcal{U}_{q_1}  - \mathcal{H}_{q_1} \right)(x , \cdot) \cdot \nabla^{n+1} \left( \eta \left(   \mathcal{U}_{q_1}  - \mathcal{H}_{q_1} \right) \right)(x,\cdot) \right\rangle_{\mu_\beta} + \frac{C_{q_1}}{R^{(2d+\gamma_\delta) }} \geq 0.
\end{equation}
We then combine the estimates~\eqref{eq:TV12137},~\eqref{eq:TV11427},~\eqref{eq:TV111211} and~\eqref{eq:TV111311} with the identity~\eqref{eq:TV081011}, choose the inverse temperature $\beta$ large enough so that the right side of~\eqref{eq:TV111211} can be absorbed by the right side of~\eqref{eq:TV075917} and use that the cutoff function $\eta$ is equal to $1$ in the annulus $A_R^1$. We obtain
\begin{equation} \label{eq:TV12277}
     \left\| \nabla \mathcal{U}_{q_1}  - \nabla \mathcal{H}_{q_1} \right\|_{\underline{L}^2 \left( A_{R}^1 , \mu_\beta \right)} \leq \frac{C}{R^d} \sum_{x \in \Zd} \left\langle \eta \left( \mathcal{U}_{q_1} -  \mathcal{H}_{q_1}\right) \L \left( \mathcal{U}_{q_1} -  \mathcal{H}_{q_1} \right)  \right\rangle_{\mu_\beta} + \frac{C_{q_1}}{R^{d + \gamma_\delta}}.
\end{equation}
We then combine the inequality~\eqref{eq:TV12277} with the estimate~\eqref{eq:TV12287} to complete the proof of~\eqref{eq:TV17096}. Step 2 is complete.

\medskip

\textit{Step 3. The conclusion.} In this step, we prove the $L^2$-estimate
\begin{equation} \label{eq:TV12337}
    \left\| \nabla \mathcal{U}_{q_1} - \sum_{i,j} \left( e_i + \nabla \chi_{ij} \right) \nabla \bar G_{q_1} \right\|_{\underline{L}^2 \left( A_R , \mu_\beta \right)} \leq \frac{C_{q_1}}{R^{d+ \gamma_\delta}}.
\end{equation}
In view of the estimate~\eqref{eq:TV17096} proved in Step 2, it is sufficient to prove the inequality
\begin{equation} \label{eq:TV12347}
    \left\| \nabla \mathcal{H}_{q_1} - \sum_{i,j} \left( e_i + \nabla \chi_{ij} \right) \nabla \bar G_{q_1} \right\|_{\underline{L}^2 \left( A_R , \mu_\beta \right)} \leq \frac{C_{q_1}}{R^{d+ \gamma_\delta}}.
\end{equation}
The proof of~\eqref{eq:TV12347} relies on the regularity estimate on the function $\bar G_{q_1}$ stated in Proposition~\ref{prop:prop6.5}, the quantitative sublinearity of the corrector stated in Proposition~\ref{prop:prop5.25} of Chapter 6 and the quantitative estimate for the difference of the finite and infinite-volume gradient of the corrector stated in Proposition~\ref{prop5.26} of Chapter 6. The argument is identical (and even simpler since we do not have to take into account the parameter $\delta$) to the argument given in Section~\ref{sec3.4chap60851} so we skip the details. The proof of Step 3, and thus of Theorem~\ref{thm:homogmixedder}, is complete.


==> draft.tex <==
\textit{Step 1.} Fix two integers $m,n \in \N$ such that $m \leq n$. To simplify the notation, we denote
\begin{equation*}
    v := v \left( \cdot , \cdot , \cu_n , p^* \right) \hspace{5mm} \mbox{and} \hspace{5mm} v_z := v \left( \cdot , \cdot , z + \cu_m , p^* \right).
\end{equation*}
We claim that for each $p \in B_1$, one has the inequality
\begin{equation} \label{eq:TV16155}
    \var_{\mu_\beta}^{\frac 12} \left[ \frac{1}{|\cu_n|} \sum_{x \in \cu_n} \nabla v \left( x, \cdot \right) \right] \leq  \var_{\mu_\beta}^{\frac 12} \left[ 3^{d \left( m-n \right)}\sum_{z \in \mathcal{Z}_{m,n}} \frac{1}{|\cu_m|} \sum_{x \in z + \cu_m} \nabla v_z \left( x, \cdot \right) \right] + C \left( \sum_{k = m}^{n-1} \tau_k \right)^{\frac12} + C3^{- \frac m2}.
\end{equation}
To this end, we use the identity, 
\begin{equation} \label{eq:TV15215}
    \sum_{x \in \cu_n} \nabla v \left( x, \cdot \right) = \underbrace{\sum_{z \in \mathcal{Z}_{m,n}} \sum_{x \in z + \cu_m} \nabla \left( v(x , \cdot) - v_z(x , \cdot ) \right)}_{\eqref{eq:TV15215}-(i)} + \underbrace{\sum_{x \in BL_{m,n}} \nabla v (x , \cdot)}_{\eqref{eq:TV15215}-(ii)} + \sum_{z \in \mathcal{Z}_{m,n}} \sum_{x \in z + \cu_m} \nabla v_z(x , \cdot ).
\end{equation}
We then divide the previous equality by the volume factor $\left| \cu_n \right|$ and estimate the variance of the terms~\eqref{eq:TV15215}-(i) and~\eqref{eq:TV15215}-(ii). We recall that by the definition of the triadic cubes stated in Definition~\ref{def:deftriadic}, we have the identity $\left| \cu_n \right| = 3^{d \left(n-m \right)} \left| \cu_n \right|+ \left| BL_{m,n}\right|$ and the volume estimate $\left| BL_{m,n}\right| \leq C 3^{-\frac m2} \left| \cu_n\right|$. For the term~\eqref{eq:TV15215}-(i), we use Proposition~\ref{p.subaddnustar} and write
\begin{align} \label{eq:TV16075}
    \var_{\mu_\beta} \left[ \frac{1}{|\cu_n|}\sum_{z \in \mathcal{Z}_{m,n}} \sum_{x \in z + \cu_m} \nabla  v(x , \cdot) - \nabla v_z(x , \cdot ) \right] & \leq \frac{1}{|\cu_n|}\sum_{z \in \mathcal{Z}_{m,n}} \sum_{x \in z + \cu_m} \left\| \nabla v(x , \cdot) - \nabla v_z(x , \cdot ) \right\|_{L^2 \left( \mu_\beta \right)}^2 \\&
    \leq \frac{1}{|\cu_n|}\sum_{z \in \mathcal{Z}_{m,n}} \left\|  \nabla v - \nabla v_z \right\|_{L^2 \left( z + \cu_m , \mu_\beta \right)}^2 \notag \\
    & \leq 3^{d \left( m-n \right)} \sum_{z \in \mathcal{Z}_{m,n}} \left\|  \nabla v - \nabla v_z \right\|_{\underline{L}^2 \left( z + \cu_m , \mu_\beta \right)}^2 \notag \\
    & \leq C \left( \sum_{k=m}^{n-1} \tau_k + 3^{-\frac m2} \right). \notag
\end{align}
For the term~\eqref{eq:TV15215}-(ii), we use the Cauchy-Schwarz inequality and the estimate~\eqref{eq:uppboundoptimi} on the $L^2$-norm of the gradient of the function $v$. We obtain
\begin{align} \label{eq:TV16085}
     \var_{\mu_\beta} \left[ \frac{1}{|\cu_n|}\sum_{x \in BL_{m,n}} \nabla v (x , \cdot) \right] & \leq \left( \frac{1}{|\cu_n|}\sum_{x \in BL_{m,n}} \left\| \nabla v (x , \cdot) \right\|_{L^2 \left( \mu_\beta \right)} \right)^2 \\
     & \leq \frac{\left| BL_{m,n} \right|}{\left| \cu_n \right|} \frac{1}{\left| \cu_n \right|}\sum_{x \in BL_{m,n}} \left\| \nabla v (x , \cdot) \right\|_{L^2 \left( \mu_\beta \right)}^2 \notag \\
     & \leq C 3^{-\frac m2}   \frac{1}{\left| \cu_n \right|}\sum_{x \in \cu_n} \left\| \nabla v (x , \cdot) \right\|_{L^2 \left( \mu_\beta \right)}^2 \notag \\
     & \leq C 3^{-\frac m2} . \notag
\end{align}
Combining the identity~\eqref{eq:TV15215} with the estimates~\eqref{eq:TV16075} and~\eqref{eq:TV16085}, we obtain the inequality~\eqref{eq:TV16155}. The proof of Step 1 is complete. \pd{an argument is missing to adjust the volume factor, I mean we do not have $\left| \cu_n \right| = 3^{d \left(n-m \right)} \left| \cu_n \right|$}

\medskip

\medskip



\textit{Step 2.} In this step, we claim that there exists a constant $\theta := \theta(d) \in (0,1)$ such that one has the estimate
\begin{equation} \label{eq:TV16475}
    \var_{\mu_\beta}^{\frac 12} \left[ 3^{-d }\sum_{z \in \mathcal{Z}_{n}} \frac{1}{|\cu_n|} \sum_{x \in z + \cu_m} \nabla v \left( x, \cdot, z+ \cu_n , p^* \right) \right] \leq \theta \var_{\mu_\beta}^{\frac 12} \left[ \frac{1}{|\cu_n|} \sum_{x \in \cu_m} \nabla v \left( x, \cdot, \cu_n , p^* \right) \right].
\end{equation}
To ease the notation, we set, for each $z \in \mathcal{Z}_n$,
\begin{equation} \label{eq:expformXz}
    X_z := \frac{1}{|\cu_n|} \sum_{x \in z + \cu_n} \nabla v \left( x, \cdot, z+ \cu_n , p^* \right).
\end{equation}
We first describe the strategy of the proof. First, by translation invariance of the measure $\mu_{\beta}$, we see that the random variables $X_z$ have the same law. The inequality~\eqref{eq:TV16475} states that the variance of the average $3^{-d }\sum_{z \in \mathcal{Z}_{n}} X_z$ is strictly smaller than the variance of the random variable $X_z$. This property is typical of independent or weekly correlated random variables. The objective of this step is to prove that this property is satisfied for the family of random variables $X_z$; more specifically, we prove that if two cubes of the form $(z + \cu_n)$ are distant from each other, then they are weakly correlated and we refer to REf for a precise statement. An heuristic reason justifying this decorrelation is the following. By definition of the function $v \left( \cdot , z + \cu_n, p^* \right)$, we expect that this function will mostly depend on the value of the field $\phi$ inside the the cube $\left( z + \cu_n \right)$.  In dimension $3$ and higher, the field $\phi$ should exhibit a behavior similar to the one of the Gaussian free field and in particular, we expect the field to be approximately local and in particular, if two cubes $\left( z + \cu_n \right)$ and $\left( z' + \cu_n \right)$ are far away from each other, then we expect the restrictions of the field $\phi$ to this two cubes to be weakly correlated. We claim that if $z , z' \in \mathcal{Z}_n$ are such that the two cubes $\left( z + \cu_n \right)$ and $\left( z' + \cu_n \right)$ are not neighbors, that is, if they satisfy $\dist \left(  z + \cu_n ,  z' + \cu_n  \right) \geq 2 l_n$ (see figure REF), and if the inverse temperature $\beta$ is chosen high enough so that the from the regularity theory stated in Section~\ref{section:section4} hold with exponent $\ep$ (in particular we choose $\beta$ large enough so that $\ep \leq \frac 14$) then we have the estimate
\begin{equation} \label{eq:TV06415}
    \cov_{\mu_{\beta}} \left[ X_z , X_{z'} \right] \leq C 3^{\left( 2\ep - 1\right)n } \leq C 3^{ \frac n2 }.
\end{equation}
To prove this result, we use the Hellfer-Sjostrand representation formula and the properties of the derived Helffer-Sjostrand equation presented in Section~\ref{sec.section4.5}. We decompose the rest of the proof into three substeps:
\begin{itemize}
    \item In Substep 2.1, we show how to deduce the inequality~\eqref{eq:TV16475} from the correlation estimate~\eqref{eq:TV06415}; 
    \item In Substeps 2.2 and 2.3, we prove the correlation estimate~\eqref{eq:TV06415}.
\end{itemize}


\textit{Case 1. The point $z$ belongs to the cube $\cu$.} In that case, we can use that for each $y_1 \in \Zd \setminus 2\cu$, we have the estimates $|y - y_1| \geq \frac 12 |y|$ and $|y - z| \geq \frac 12 |y|$. We obtain
\begin{equation} \label{eq:TV08147}
    \sum_{y_1  \in \Zd \setminus  2 \cu} \frac{  \left\| \nabla v \left( y_1 \right) \right\|_{L^2 \left(  \mu_\beta \right)}}{\left| y_1 - y \right|^{2d +1 - \ep} + \left| y_1 - z \right|^{2d +1 - \ep}} \leq C \sum_{y_1  \in \Zd \setminus  2 \cu} \frac{  \left\| \nabla v \left( y_1 \right) \right\|_{L^2 \left(  \mu_\beta \right)}}{\left| y_1 \right|^{2d +1 - \ep}}.
\end{equation}
To estimate the previous inequality, we split the space into cubes. We denote by $\mathcal{K} := \left\{ \kappa \, : \, \kappa \in 2l_n \Zd \right\}$ so that the family of cubes $\left( \kappa + 2 \cu\right)_{\kappa \in \mathcal{K}}$ forms a partition of $\Zd$. We also note that, for each point $\kappa \in \mathcal{K}\setminus \{ 0 \}$ and each point $y_1 \in \left( \kappa + 2 \cu \right)$, we have the inequality $c \left| \kappa \right| \leq \left| y_1 \right| \leq C |\kappa|$. We then use the inequality~\ref{} which states that the average $L^2$-norm of the gradient of the function $v$ over a cube of size larger than $l_n$ is bounded by a constant and rewrite the inequality~\eqref{eq:TV08147}. We obtain
\begin{align*}
     \sum_{y_1  \in \Zd \setminus  2 \cu} \frac{  \left\| \nabla v \left( y_1 \right) \right\|_{L^2 \left(  \mu_\beta \right)}}{\left| y_1 \right|^{2d +1 - \ep}}  \leq C \sum_{\kappa \in \mathcal{K} \setminus\{0\}} \sum_{y_1 \in \kappa + 2 \cu} \frac{  \left\| \nabla v \left( y_1 \right) \right\|_{L^2 \left(  \mu_\beta \right)}}{\left| y_1 \right|^{2d +1 - \ep}} 
     & \leq C \sum_{\kappa \in \mathcal{K} \setminus\{0\}} \frac{1}{|\kappa|^{2d+1-\ep}} \sum_{y_1 \in \kappa + 2 \cu} \left\| \nabla v \left( y_1 \right) \right\|_{L^2 \left(  \mu_\beta \right)} \\
     & \leq C \sum_{\kappa \in \mathcal{K} \setminus\{0\}} \frac{\left| 2 \cu \right|}{|\kappa|^{2d+1-\ep}}.
\end{align*}
To estimate the previous sum, we use that for each point $\kappa \in \mathcal{K}\setminus \{ 0 \}$ and each point $y_1 \in \left( \kappa + 2 \cu \right)$, we have the inequality $c \left| \kappa \right| \leq \left| y_1 \right| \leq C |\kappa|$ and note that, for each point $y \in \Zd \setminus 2\cu$, we have the estimate $\left| y_1 \right| \geq c 3^{n}$. We obtain
\begin{align*}
    \sum_{y_1  \in \Zd \setminus  2 \cu} \frac{  \left\| \nabla v \left( y_1 \right) \right\|_{L^2 \left(  \mu_\beta \right)}}{\left| y_1 \right|^{2d +1 - \ep}}  \leq C \sum_{\kappa \in \mathcal{K} \setminus\{0\}} \frac{\left| 2 \cu \right|}{|\kappa|^{2d+1-\ep}}
     \leq \sum_{\kappa \in \mathcal{K} \setminus\{0\}} \sum_{y_1 \in \kappa + 2 \cu }\frac{1}{|\kappa|^{2d+1-\ep}} 
    & \leq C \sum_{\kappa \in \mathcal{K} \setminus\{0\}} \sum_{y_1 \in \kappa + 2 \cu } \frac{1}{|y_1|^{2d+1-\ep}}  \\
    & \leq C \sum_{y_1 \in \Zd \setminus 2 \cu } \frac{1}{|y_1|^{2d+1-\ep}} \\
    & \leq C3^{\left( d+ 1 - \ep \right)n}.
\end{align*}
We have the proved
\begin{equation} \label{eq:TV11077}
    \sum_{y_1  \in \Zd \setminus  2 \cu} \frac{  \left\| \nabla v \left( y_1 \right) \right\|_{L^2 \left(  \mu_\beta \right)}}{\left| y_1 - y \right|^{2d +1 - \ep} + \left| y_1 - z \right|^{2d +1 - \ep}}  \leq   C3^{\left( d+ 1 - \ep \right)n}.
\end{equation}
The proof of Case 1 is complete.

\medskip







\begin{proposition}[Homogenization of the Green's function] \label{prop:prop6.1}
Let $\f$ be a smooth Lipschitz bounded from $\Rd$ to $\R$ and let $G$ be the Green's function associated to the Helffer-Sjostrand equation
\begin{equation*}
    \mathcal{L}_\beta G = \f(\nabla \phi (0))
\end{equation*}
and let $\bar G$ be the solution of the homogenized Helffer-Sjostrand equation
\begin{equation*}
    \bar \L_\beta \bar G = \Delta_\phi \bar G + \ahom_\beta \Delta \bar G = \f \left( \nabla \phi (0) \right) \delta_0
\end{equation*}
There exist and exponent $\alpha(d) > 0$ and an inverse temperature $\beta_0(d) < \infty$ such that for any radius $R \geq 1$, one has the estimate, in the annulus $A_R := B_{2R} \setminus B_R$,
\begin{equation*}
\left\| G  - \bar G \right\|_{\underline{L}^2 \left( A_R, \, \mu_\beta\right)} \leq C R^{ 2 - d - \alpha} ,
\end{equation*}
and the estimate on the gradient of the Green's function, for each integer $i \in \{ 1 , \ldots , d \}$,
\begin{equation*}
\left\| \nabla_i G - \left( 1 + \nabla_i \chi_{p} \right) \nabla_i \bar G \right\|_{L^2 \left(A_R,  \mu_\beta\right)} \leq C R^{ 1 - d - \alpha}.
\end{equation*}
\end{proposition}

The proof of this proposition relies on two ingredients: an approximation procedure and a two-scale expansion. We first describe the approximation procedure.

We first fix two strictly positive parameters $\delta$ and $\ep$. The parameter $\delta$ represents the size of a mesoscopic scale which needs to be taken into account in the approximation argument. The parameter $\ep$ is a regularity exponent: we choose the inverse temperature $\beta$ large enough (depending on $\ep$) such that all the estimates of Section REf are valid with this specific exponent. These exponents are chosen such that
\begin{equation} \label{eq:hierarchepdelal}
\ep \ll \delta \ll \alpha.
\end{equation}
We also let $\rho_\delta$ be a smooth non-negative compactly supported function which satisfies
\begin{equation*}
\rho_\delta \in C_c^\infty (\Rd),~\supp \rho_\delta \subseteq B_{R^{1 - \delta}}, ~\rho_\delta \geq 0, ~\int_{\Rd} \rho_\delta = 1, ~\mbox{and} ~\forall k \in \N, ~\left| \nabla^k \rho_\delta \right| \leq \frac{C}{R^{k(1 - \delta)}}
\end{equation*}

and we define the approximate Green's functions $G_\delta$ and $\bar G_\delta$ according to the formulas
\begin{equation*}
\mathcal{L}_\beta G_\delta = \f \left( \nabla \phi (0) \right) \rho_\delta
\end{equation*}
and
\begin{equation*}
    \bar \L_\beta \bar G_\delta = \f \left( \nabla \phi (0) \right) \rho_\delta
\end{equation*}
The first proposition shows that, in the annulus $A_R$, the functions $G_\delta$ and $\bar G_\delta$ are good approximations of the Green's functions $G$ and $\bar G$ respectively. 


 \textit{Step 5.} We combine the main estimates REF of Step 2, REF of Step 3 and REF of Step 4 and we obtain
\begin{align} \label{eq:Lwstep5}
    \L w & =  \Delta_\phi \bar G_\delta +  \frac{1}{2\beta}\sum_{i = 1}^d \left[ \nabla \cdot (\nabla_i \bar G_\delta  \left( e_i + \nabla \chi_{m,i} \right)) \right]  + \sum_{i = 1}^d \sum_{\di q = 0}  \left( \di^* \nabla_i \bar G_\delta\right) \a_q \nabla_q \left( l_{e_i} + \chi_{m,i} \right) n_q \\ 
                &  + \sum_{i=1}^d \nabla_i \bar G_\delta \left(  \Delta_{\phi} \chi_{m,i} + \frac{1}{2\beta} \sum_{i=1}^d \sum_{n \geq 1}  \frac{1}{\beta^{\frac n2}} \Delta^n \chi_{m,i} + \sum_{\di q = 0} \nabla_q^* \cdot \a_q \nabla_q \left( l_{e_i} + \chi_{m,i} \right) \right) + R_5. \notag
\end{align}
where we denote by $R_5$ the error term defined by the formula $R_5 := R_1 + R_2 + R_3 + R_4$ and satisfies the estimate
\begin{equation*}
    \left\| R_5 \right\|_{\underline{H}^{-1}\left( B_{R^{1+\delta}} , \mu_\beta \right)} \leq small.
\end{equation*}
We then use that, by definition of the corrector, one has the equality, for each $i\in \{1, \ldots, d \}$,
\begin{equation*}
      \Delta_{\phi} \chi_{m,i} + \frac{1}{2\beta} \sum_{i=1}^d \sum_{n \geq 1}  \frac{1}{\beta^{\frac n2}} \Delta^n \chi_{m,i} + \sum_{\di q = 0} \nabla_q^* \cdot \a_q \nabla_q \left( l_{e_i} + \chi_{m,i} \right) = 0.
\end{equation*}
Putting this estimate back into the identity~\eqref{eq:Lwstep5}, we obtain
\begin{equation*}
    \L w  =  \Delta_\phi \bar G_\delta +  \frac{1}{2\beta}\sum_{i = 1}^d  \nabla\nabla_i \bar G_\delta \cdot  \left( e_i + \nabla \chi_{m,i} \right) + \sum_{\di q = 0}  \left( \di^* \nabla_i \bar G_\delta\right) \a_q \nabla_q \left( l_{e_i} + \chi_{m,i} \right) n_q + R_5.
\end{equation*}
The next step of the proof is to use the the estimate on the weak norm of the flux of the corrector proved in REF to replace the second and third term of the sum REf by the term $\ahom_\beta \Delta \bar G_\delta$. We first compute
\begin{align*}
    \lefteqn{\left\| \frac{1}{2\beta}\sum_{i = 1}^d  \nabla\nabla_i \bar G_\delta \cdot  \left( e_i + \nabla \chi_{m,i} \right) + \sum_{\di q = 0}  \left( \di^* \nabla_i \bar G_\delta\right) \a_q \nabla_q \left( l_{e_i} + \chi_{m,i} \right) n_q - \ahom_\beta \Delta \bar G_\delta \right\|_{\underline{H}^{-1}\left( B_{R^{1+\delta} , \mu_\beta} \right)}} \qquad & \\  & \leq \left\| \nabla\nabla_i \bar G_\delta \right\|_{\underline{W}^{1,\infty} (B_{R^{1+\delta}}, \mu_\beta)} \sum_{i=1}^d\left\| \frac{1}{2\beta}\sum_{i = 1}^d    \left( e_i + \nabla \chi_{m,i} \right) + \sum_{\di q = 0}  \a_q \nabla_q \left( l_{e_i} + \chi_{m,i} \right) n_q - \ahom_\beta e_i \right\|_{\underline{H}^{-1}\left( B_{R^{1+\delta} , \mu_\beta} \right)}.
\end{align*}
We then use the regularity estimate REF and the estimate REF on the flux of the corrector to obtain the estimate
\begin{equation*}
   \left\| \frac{1}{2\beta}\sum_{i = 1}^d  \nabla\nabla_i \bar G_\delta \cdot  \left( e_i + \nabla \chi_{m,i} \right) + \sum_{\di q = 0}  \left( \di^* \nabla_i \bar G_\delta\right) \a_q \nabla_q \left( l_{e_i} + \chi_{m,i} \right) n_q - \ahom_\beta \Delta \bar G_\delta \right\|_{\underline{H}^{-1}\left( B_{R^{1+\delta} , \mu_\beta} \right)}  \leq small.
\end{equation*}
We then denote by
\begin{equation*}
R_6 := \frac{1}{2\beta}\sum_{i = 1}^d  \nabla\nabla_i \bar G_\delta \cdot  \left( e_i + \nabla \chi_{m,i} \right) + \sum_{\di q = 0}  \left( \di^* \nabla_i \bar G_\delta\right) \a_q \nabla_q \left( l_{e_i} + \chi_{m,i} \right) n_q - \ahom_\beta \Delta \bar G_\delta + R_5.
\end{equation*}
By the estimates REF and REF, it is an error term which satisfies
\begin{equation*}
    \left\| R_6 \right\|_{\underline{H}^{-1}\left( B_{R^{1+\delta} , \mu_\beta} \right)} \leq Bla.
\end{equation*}
Using the definition of $R_6$, the identity REF can be rewritten
\begin{equation*}
    \L w  =   \Delta_\phi \bar G_\delta + \ahom_\beta \Delta \bar G_\delta + R_6.
\end{equation*}
By the definition of $\bar G_\delta$ stated in REf, we obtain
\begin{equation*}
    \L w = \f(\phi) \rho_\delta + R_6.
\end{equation*}
Using the identity $\L_\beta  G_\delta  = \f(\phi) \rho_\delta$.
\begin{equation*}
    \L_\beta \left(w - G_\delta \right) = R_6.
\end{equation*}
This is the estimate REf and the proof is complete.



The proof relies on a two-scale expansion which is defined as follows. We first let $\eta$ be a cutoff function supported in the ball $B_{R^{1+ \delta}}$ such that
\begin{equation*}
    0 \leq \eta \leq \indc_{B_{R^{ 1 + \delta }}}, ~ \eta = 1 ~\mbox{in}~ B_{\frac{R^{ 1 + \delta }}{2}} , ~\mbox{and}~ \forall k \in \N, \, \left| \nabla^k \eta \right|\leq \frac{C}{R^{ (1 + \delta ) k }}.
\end{equation*}
We also let $m$ be the integer such that $3^{m-1} \leq R < 3^m$ and consider the corrector $\chi_m$.
We then define the two-scale expansion $w$ according to the formula
\begin{equation*}
    w :=  \bar G_\delta + \sum_{i=1}^d \left( \nabla_i  \bar G_\delta \right) \chi_{m,i}.
\end{equation*}

The objective is then to prove the estimate: there exists an exponent $\delta(d)>0$ such that the following estimate holds
\begin{equation} \label{mainest.homog}
    \sum_{x \in B_{R^{1+\delta}}} \left\langle \L_\beta \left(w - G_{\delta} \right), \eta \left( w -  G_{\delta} \right) \right\rangle_{\mu_\beta} \leq \frac{C}{R^{(1 + \delta)(d-2)}}.
\end{equation}

We then decompose the proof into N Steps.

\textit{Step 1.} In this step, we show how to deduce the estimates REF from~\eqref{mainest.homog}. Since the function $\eta \left( w -  G_{\delta} \right)$ belongs to the space $H^1_0 \left(B_{R^{1+\delta}} , \mu_\beta \right)$, we can perform the integration by part and obtain
\begin{multline*}
    \sum_{x \in B_{R^{1+\delta}}} \left\langle \L_\beta F, \eta F \right\rangle_{\mu_\beta}  = \sum_{y \in F} \int_F \eta(x)^2 \left\langle \left( \partial_y F(x) \right)^2 \right\rangle_{\mu_\beta} \, dx + \frac 1{2\beta}\int_F  \left\langle \nabla F \cdot \nabla \left( \eta^2 F\right) \right\rangle_{\mu_\beta} \\ +  \frac 1{2\beta} \sum_{n \geq 1} \int_F  \frac{1}{\beta^{ \frac n2}} \left\langle  \nabla^n F \cdot \nabla^n \left( \eta^2 F \right) \right\rangle_{\mu_\beta} + \sum_{q}  \left\langle \nabla_q F\cdot \a_q \nabla_q \left( \eta^2 F \right) \right\rangle_{\mu_\beta}.
\end{multline*}
Using the estimate~\eqref{mainest.homog}, we obtain
\begin{equation*}
    \frac 1{2\beta}\int_F  \left\langle \nabla F \cdot \nabla \left( \eta^2 F\right) \right\rangle_{\mu_\beta} +  \frac 1{2\beta} \sum_{n \geq 1} \int_F  \frac{1}{\beta^{ \frac n2}} \left\langle  \nabla^n F \cdot \nabla^n \left( \eta^2 F \right) \right\rangle_{\mu_\beta} + \sum_{q}  \left\langle \nabla_q F\cdot \a_q \nabla_q \left( \eta^2 F \right) \right\rangle_{\mu_\beta} \leq \frac{C}{R^{(1 + \delta)(d-2)}}.
\end{equation*}
We then use the commutation estimate proved in REF
\begin{equation*}
     \int_F \nabla^n F \cdot \nabla^n \left( \eta^2 F \right) - \int_F \eta^2 \nabla^n F \cdot \nabla^n  F \geq \frac{C^n}{R^{1+\delta}} \left\| \nabla  F \right\|_{L^2 \left( A_{R^{1+ \delta} + B_n}\right)} \left\| F \right\|_{L^2 \left( A_{R^{1+ \delta} + B_n}\right)},
\end{equation*}
and the estimate 
\begin{align*}
      \sum_{q} \nabla_q F\cdot \a_q \nabla_q \left( \eta^2 F \right) -  \sum_{q} \eta^2 \nabla_q F\cdot \a_q \nabla_q  F  & \geq - \frac{C}{R^{1+\delta}} \left\| \nabla  F \right\|_{L^2 \left( A_{R^{1+ \delta} + B_n}\right)} \left\| F \right\|_{L^2 \left( A_{R^{1+ \delta} + B_n}\right)} \\ & \quad  + e^{-c \sqrt{\beta} R} \left\| \nabla  F \right\|_{L^2 \left( B_{R^{1+\delta}}\right)} \left\| F \right\|_{L^2 \left(  B_{R^{1+\delta}} \right)}
\end{align*}
Combining the three previous estimates, we obtain
\begin{align*}
     \frac 1{2\beta} \eta^2 \int_F  \left\langle \nabla F \cdot \nabla  F \right\rangle_{\mu_\beta} & \leq \frac{C}{R^{(1 + \delta)(d-2)}} + \frac{C}{R^{1+\delta}} \left\| \nabla  F \right\|_{L^2 \left( A_{R^{1+ \delta}}\right)} \left\| F \right\|_{L^2 \left( A_{R^{1+ \delta}}\right)}  \\ & + e^{-c \sqrt{\beta} R} \left\| \nabla  F \right\|_{L^2 \left( B_{R^{1+\delta}}\right)} \left\| F \right\|_{L^2 \left(  B_{R^{1+\delta}} \right)}.
\end{align*}
Using the estimates REF on the functions $\bar G_\delta$, REf on the function $G$ and the sublinearity estimate REF on the corrector, we deduce
\begin{equation*}
     \left\| F \right\|_{L^2 \left( A_{R^{1+ \delta}}\right)} \leq \frac{C}{R^{(1+\delta)(d/2 - 2)}}~\mbox{and}~ \left\| \nabla F \right\|_{L^2 \left( A_{R^{1+ \delta}}\right)} \leq \frac{C}{R^{( 1+ \delta)(d/2 - 1)}}
\end{equation*}

We now prove the estimate REF pertaining to the gradient of the Green's function. We start from the estimate REF restrict the domain of integration to the annulus $A_R$ and note that the cutoff function $\eta$ is equal to $1$ on $A_R$. This gives
\begin{equation*}
    \left\| \nabla \left( w - G  \right) \right\|_{\underline{L}^2\left( A_R, \, \mu_\beta \right)} \leq \frac{1}{ R^{d}} \sum_{x \in B_{R^{1 + \delta}}} \left\langle \L_\beta \left(w -  G \right), \left( w -  G \right) \right\rangle_{\mu_\beta} \leq \frac{C}{R^{d-1 - \alpha}}.
\end{equation*}
Using the explicit formula REF to compute the gradient of $w$ and obtain
\begin{equation*}
    \nabla w = \nabla \bar G_\delta +
    \sum_{i = 1}^d  \nabla_i \bar G_\delta \nabla \chi_{m,i} + \sum_{i = 1}^d \nabla \nabla_i \bar G_\delta \chi_{m,i}.
\end{equation*}
The third term on the right side can be estimated thanks to the regularity estimates REF and the sublinearity of the corrector REF with an argument similar to the one of the inequality REF and we obtain
\begin{equation*}
    \left\|  \sum_{i = 1}^d \nabla \nabla_i \bar G_\delta \chi_{m,i} \right\|_{\underline{L}^2\left( A_R, \, \mu_\beta \right) } \leq \frac{C}{R^{d-1-\alpha}}.
\end{equation*}
Combining the estimate REF with REF, we deduce
\begin{equation*}
    \left\| \nabla  w -  \nabla \bar G_\delta -
    \sum_{i = 1}^d  \nabla_i \bar G_\delta \nabla \chi_{m,i} \right\|_{\underline{L}^2\left( A_R, \, \mu_\beta \right)} \leq \frac{C}{R^{d-1 - \alpha}}.
\end{equation*}
Their remains to replace the gradient of the finite volume corrector by the full-volume gradient $\nabla \chi_p$ and we use Proposition REF with the regularity estimate REF to obtain
\begin{equation*}
    \left\| \nabla  w -  \nabla \bar G_\delta -
    \sum_{i = 1}^d  \nabla_i \bar G_\delta \nabla \chi_i \right\|_{\underline{L}^2\left( A_R, \, \mu_\beta \right)} \leq \frac{C}{R^{d-1 - \alpha}}.
\end{equation*}
Combining the inequality REF with the estimate REF completes the proof of REF.


A FIRST VERSION OF THE TWO-SCALE EXPANSION



\subsection{Two-scale expansion and homogenization of the gradient of the Green's function} \label{sec:section6.1}

This section is devoted to the proof of Proposition~\ref{prop:prop6.1}. We first prove that the functions $\G_{\f}^\delta$ and $\G_{\mathrm{hom}, \f}^\delta$ are well-approximated by the functions $\G_{\f}^\delta$ and $\G_{\mathrm{hom}, \f}^\delta$. The result corresponds to the inequality~\eqref{eq:TV0421} and is stated in the following lemma.

\begin{lemma} \label{prop:prop6.2}
There exists an exponent $\gamma := \gamma (d) > 0$ such that one has the estimates
\begin{equation} \label{eq:TV20383}
\sup_{x \in A_R} \left\|\nabla \G_{\f} (x, \cdot) - \nabla \G_{\f}^\delta(x , \cdot ) \right\|_{L^\infty \left( \mu_\beta \right)} \leq C R^{1 - d - \gamma } \hspace{5mm} \mbox{and} \hspace{5mm} \sup_{x \in A_R} \left\|\nabla \G_{\mathrm{hom}, \f} (x, \cdot) - \nabla \G_{\mathrm{hom},\f}^\delta(x , \cdot ) \right\|_{L^\infty \left( \mu_\beta \right)} \leq C R^{1 - d - \gamma }.
\end{equation}
\end{lemma}


\begin{proof}[Proof of Lemma~\ref{prop:prop6.2}]
The proof relies on the regularity estimates established in Section~\ref{section:section4}. We first note that, by definitions of the functions $\G_\f \left( x , \phi \right)$ and $\G_\f^\delta \left( x , \phi \right)$, we have the identities 
\begin{equation} \label{eq:TV13219}
    \G_\f \left( x , \phi \right) = \G_\f \left( x , \phi ;0 \right) \hspace{5mm} \mbox{and} \hspace{5mm} \G_\f^\delta \left( x , \phi \right) = \sum_{y \in B_{R^{1-\delta}}} \rho_\delta(y) \G_\f \left( x , \phi ; y \right)
\end{equation}
Using that the map $\rho_\delta$ has total mass $1$ and the regularity estimate on the Green's function stated in Corollary~\ref{cor:corollary4.14}, we obtain, for each point $x$ in the annulus $A_R$
\begin{align*}
    \left\| \nabla_x \G_\f (x , \phi ; 0) - \nabla_x \G_\f^\delta (x , \phi ; y) \right\|_{L^\infty \left( \mu_\beta \right)}  & \leq  \sum_{y \in B_{R^{1-\delta}}} \rho_\delta (y) \left\|  \nabla_x \G_\f (x ,  \phi ; 0 ) -  \nabla_x  \G_\f (x , \phi ; y)  \right\|_{L^\infty \left( \mu_\beta \right)} \\
    & \leq R^{1 - \delta} \sup_{y \in B_{R^{1- \delta}}} \left\| \nabla_x \nabla_y \G_\f (x , \phi ; y ) \right\|_{L^\infty \left( \mu_\beta \right)} \\
    & \leq R^{1 - \delta} \sup_{y \in B_{R^{1-\delta}}}|x - y|^{- d - \ep}\\
    & \leq R^{1 - \delta} R^{- d - \ep},
\end{align*}
 This completes the proof of the estimate~\eqref{eq:TV20383} with the exponent $\gamma = \delta - \ep$ which is strictly positive by the assumption~\eqref{eq:TVexpord}.
 
The estimate on the homogenized Green's function is similar. We first note that, for each point $y \in \Zd$, the function $(x , \phi) \mapsto \G_{\mathrm{hom} , \f} \left( x - y , \phi \right)$ is solution of the Hellfer-Sjostrand equation
\begin{equation} \label{eq:TV}
    \Delta_\phi \G_{\mathrm{hom} , \f} \left( \cdot  - y , \cdot \right) + \ahom \Delta \G_{\mathrm{hom} , \f} \left( \cdot  - y , \cdot \right) = \f \delta_y.
\end{equation}
Using the equality and the definition~\eqref{def:GdeltaGhomdelta} of the function $\G_{\mathrm{hom} , \f}^\delta$, we deduce the identity, for each $(x , \phi) \in \Zd \times \Omega$,
\begin{equation} \label{eq:TV80004}
    \G_{\mathrm{hom} , \f}^\delta (x , \phi) = \sum_{y \in B_{R^{1-\delta}}} \rho_\delta(x) \G_{\mathrm{hom} , \f} \left( x - y , \phi \right).
\end{equation}
We then use the regularity estimates~\eqref{eq:TV21053} on the derivatives of the homogenized Green's function $\G_{\mathrm{hom}, \f}$ instead of the regularity estimates stated in Corollary~\ref{cor:corollary4.14} and we skip the details.
\end{proof}

Before starting the proof of Proposition~\ref{prop:prop6.2}, we need to record some regularity properties of the Green's function $\G_{\f}^\delta$ and the homogenized Green's function $\G_{\mathrm{hom}, \f}^\delta$, they are stated in Lemmas~\eqref{Lem6.4} and~\ref{Lem6.5} below.

\begin{lemma}  \label{Lem6.4}
The Green's function $\G_{\f}^\delta$ satisfies the following $L^\infty$-estimates
\begin{equation*}
    \left\| \G_{\f}^\delta  \right\|_{L^\infty \left( \Zd , \mu_\beta  \right)} \leq  \frac{1}{R^{(1-\delta) (d-2) }} ~\mbox{and}~ \left\| \nabla \G_{\f}^\delta  \right\|_{L^\infty \left( \Zd , \mu_\beta  \right)} \leq \frac{1}{R^{(1-\delta) (d-1 - \ep) }}
\end{equation*}
\end{lemma}

\begin{proof}
The proof relies on the estimates on the Green's function and its gradient established in Corollary~\ref{cor:cor5.23}. We use the identity~\eqref{eq:TV13219} and write, for each point $x \in \Zd$,
\begin{align*}
    \left\| \G_\f^\delta \left( x , \cdot \right) \right\|_{L^\infty \left( \mu_\beta \right)}  = \sum_{y \in B_{R^{1-\delta}}} \rho_\delta(y) \left\| \G_\f \left( x , \phi ; y \right)  \right\|_{L^\infty \left( \mu_\beta \right)} \leq \frac{1}{R^{(1-\delta) d }} \sum_{y \in B_{R^{1-\delta}}} \frac{C}{|x- y|^{d-2}} 
    & \leq  \frac{1}{R^{(1-\delta) d }} \sum_{y \in B_{R^{1-\delta}}} \frac{C}{| y|^{d-2}} \\
    & \leq \frac{1}{R^{(1-\delta) (d-2) }}.
\end{align*}
A similar computation shows the bound for the gradient of the Green's function and we skip the details.
\end{proof}

\begin{lemma} \label{Lem6.5}
The homogenized Green's function $\G_{\mathrm{hom} , \f}$ satisfies the regularity estimates:
\begin{itemize}
    \iffalse\item For each integer $k \in \{0 , 1 , 2 \}$ and each point $x \in \Zd $,
    \begin{equation} \label{eq:spatregbarG}
    \left\| \nabla^k \G_{\mathrm{hom}, \f }^\delta(x , \cdot) \right\|_{L^\infty \left( \mu_\beta \right)} \leq \frac{C \left\| \f \right\|_{L^\infty\left( \mu_\beta\right)}}{ \left(R^{1-\delta} \wedge |x| \right)^{d-2 + k}};
    \end{equation} \fi
    \item For each integer $k \in \N$, we have the $L^\infty$-estimate
    \begin{equation} \label{eq:spatregbarGgeq3}
         \left\| \nabla^k \G_{\mathrm{hom}, \f }^\delta \right\|_{L^\infty \left( \Zd , \mu_\beta \right)} \leq \frac{C}{R^{(1-\delta)(d-2+k)}};
    \end{equation}
   \iffalse \item For every pair $\left(x , y  \right) \in \Zd \times \Zd$
    \begin{equation}\label{eq:phiregbarG}
    \left\| \partial_y \G_{\mathrm{hom}, \f}^\delta (x , \cdot) \right\|_{L^\infty \left( \mu_\beta  \right)} \leq \frac{C\left\| \f \right\|_{L^\infty\left( \mu_\beta\right)}}{\left( R^{1-\delta} \wedge | x | + |y|\right)^{2d - 2 - \ep}}~\mbox{and}~\left\| \partial_y \nabla \G_{\mathrm{hom}, \f}^\delta (x , \cdot) \right\|_{L^\infty \left( \mu_\beta \right)} \leq \frac{C\left\| \f \right\|_{L^\infty\left( \mu_\beta\right)}}{\left( R^{1-\delta} \wedge | x | + |y|\right)^{2d -1  - \ep}};
    \end{equation} \fi
    \item For each $y \in \Zd$,
    \begin{equation} \label{eq:partialbarG}
    \left( \sum_{y \in \Zd} \left\| \partial_y \nabla \G_{\mathrm{hom}, \f}^\delta (x , \cdot) \right\|_{L^\infty \left( \mu_\beta \right)}^2 \right)^{\frac12} \leq C \left\| \f \right\|_{L^\infty\left( \mu_\beta\right)} R^{-d + \ep}.
    \end{equation}
\end{itemize}
\end{lemma}

\begin{proof}
To prove the regularity estimate~\eqref{eq:spatregbarG}, we use  is a consequence of the identity~\eqref{eq:TV80004} and the regularity estimate~\eqref{eq:TV21053} on on the homogenized Green's function $\G_{\mathrm{hom},\f}$ and its derivatives. We compute
\begin{align} \label{eq:TV09144}
    \left\| \nabla^k \G_{\mathrm{hom}, \f }^\delta(x , \cdot) \right\|_{L^\infty \left( \mu_\beta \right)}  \leq \sum_{y \in B_{R^{1-\delta}}} \rho_\delta(y) \left\| \nabla^k \G_{\mathrm{hom} , \f} \left( x - y , \cdot\right) \right\|_{L^\infty \left( \mu_\beta \right)} 
    & \leq \sum_{y \in B_{R^{1-\delta}}} \rho_\delta (y) \frac{C \left\| \f \right\|_{L^\infty \left( \mu_\beta \right)}}{|x - y|^{d-2+k}} \\
    & \leq \frac{C\left\| \f \right\|_{L^\infty \left( \mu_\beta \right)}}{R^{d(1-\delta)}} \sum_{y \in B_{R^{1-\delta}}} \frac{1}{|x - y|^{d-2+k}}. \notag
\end{align}
The second estimate in~\eqref{eq:defbarghom}, can be obtained by a similar argument and an integration by parts. We have
\begin{align} \label{eq:TV09144bis}
    \left\| \nabla^k \G_{\mathrm{hom}, \f }^\delta(x , \cdot) \right\|_{L^\infty \left( \mu_\beta \right)} & = \left\| \sum_{y \in B_{R^{1-\delta}}} \rho_\delta(y)  \nabla^k \G_{\mathrm{hom} , \f} \left( x - y , \cdot\right) \right\|_{L^\infty \left( \mu_\beta \right)} \\ &
    = \left\| \sum_{y \in B_{R^{1-\delta}}} \nabla^k \rho_\delta(y)   \G_{\mathrm{hom} , \f} \left( x - y , \cdot\right) \right\|_{L^\infty \left( \mu_\beta \right)} \notag \\&
    \leq \frac{C\left\| \f \right\|_{L^\infty \left( \mu_\beta \right)}}{R^{(1-\delta)(d+k)}} \sum_{y \in B_{R^{1-\delta}}} \frac{1}{|x - y|^{d-2}} \notag
\end{align}
The last term in the right side of~\eqref{eq:TV09144} can be explicitly computed and we obtain the estimate~\eqref{eq:spatregbarG}.

To prove the inequality~\eqref{eq:phiregbarG}, we take the partial derivative $\partial_x$ on both sides of the Helffer-Sjostrand equation
\begin{equation*}
\Delta_\phi \G_{\mathrm{hom} , \f} + \ahom \Delta \G_{\mathrm{hom} , \f}  = \f \rho_\delta. 
\end{equation*}
Following the arguments introduced in Section~\ref{sec.section4.5}, we introduce the function $g : (x , y , \phi) \mapsto \partial_y \G_{\mathrm{hom}, \f }^\delta (x , \phi)$ and obtain that this map is a solution of the equation
\begin{equation*}
 \Delta_\phi g (x , y , \phi)  + \ahom \Delta_y g (x , y , \phi)  + \mathcal{L}_{\mathrm{spat} , x} g (x , y , \phi)  = \partial_y \f \left( \phi \right) \rho_\delta (x).
\end{equation*}
Given a bounded random variable $\mathbf{g} : \Omega \to \R$ and two points $x_1 , y_1 \in \Zd$, we let $\G_{\mathrm{hom}, \mathrm{der}, \mathbf{g}}\left( \cdot , \cdot , \cdot ; x_1 , y_1 \right) : \Zd \times \Zd \times \Omega \mapsto \R$ be the Green's function associated to the equation
\begin{equation*}
    \Delta_\phi \G_{\mathrm{hom}, \mathrm{der}, \mathbf{g}}\left( \cdot , \cdot , \cdot ; x_1 , y_1 \right)  + \ahom \Delta_x \G_{\mathrm{hom}, \mathrm{der}, \mathbf{g}}\left( \cdot , \cdot , \cdot ; x_1 , y_1 \right)  + \mathcal{L}_{\mathrm{spat} , y} \G_{\mathrm{hom}, \mathrm{der}, \mathbf{g}}\left( \cdot , \cdot , \cdot ; x_1 , y_1 \right) = \mathbf{g} \delta_{(x_1,y_1)} ~\mbox{in}~ \Zd \times \Zd \times \Omega.
\end{equation*}
By using the same argument as the one presented in Section~\ref{sec.section4.5} and by noting that the operator $\Delta_\phi + \ahom \Delta_x + + \mathcal{L}_{\mathrm{spat} , y}$ is a perturbation of the operator $\Delta_\phi + \ahom \Delta_x  +  \frac 1{2\beta} \Delta_y$, we deduce that a $C^{0,1-\ep}$-regularity theory holds for the Green's function $\G_{\mathrm{hom}, \mathrm{der}, \mathbf{g}}$; in particular all the inequalities stated in Corollary~\ref{cor:corollary4.14} hold for the Green's function $\G_{\mathrm{hom}, \mathrm{der}, \mathbf{g}}$.

The function $g$ can then be expressed explicitly in terms of the Green's function $\G_{\mathrm{hom}, \mathrm{der}, \mathbf{g}}$ and estimated thanks to the arguments developed in the previous paragraph. We obtain the inequality, for each pair of points $(x , y) \in \Zd \times \Zd $, \pdcomment{clarify this}
\begin{equation} \label{eq:TV21274}
    \left\| g(x,y, \cdot) \right\|_{L^\infty \left( \mu_\beta \right)} \leq C \sum_{x_1 , y_1 \in \Zd} \frac{\left\| \partial_{y_1} \f  \right\|_{L^\infty \left( \mu_\beta \right)} \rho_\delta \left( x_1 \right)}{\left|x - x_1 \right|^{2d-1-\ep} + \left| y -  y_1 \right|^{2d-1-\ep}}  .
\end{equation}
The sum on the right side of the inequality~\eqref{eq:TV21274} can be explicitly estimated and we have
\begin{equation*}
    \left\| g(x,y, \cdot) \right\|_{L^\infty \left( \mu_\beta \right)} \leq \left\{\begin{aligned}
    \frac{C \left\| \partial \f \right\|_{L^\infty \left( \mu_\beta\right)}}{\left(  | x | + |y|\right)^{2d - 1 - \ep}} \\
     \frac{C \left\| \partial \f \right\|_{L^\infty \left( \mu_\beta\right)}}{R^{d(1-\delta)} |y|^{d - 1 - \ep}}.
    \end{aligned} \right.
\end{equation*}
\end{proof}

We have now collected all the necessary preliminary ingredients for the proof of Proposition~\ref{prop:prop6.1} and devote the rest of Section~\ref{sec:section6.1} to this demonstration. 

\begin{proof}[Proof of Proposition~\ref{prop:prop6.1}]
We decompose the proof into three steps, following the sketch presented at the beginning of Section~\ref{sec:section6}. We recall that through the proof, the exponent $\gamma$ is a small, strictly positive exponent which may vary from line to line and can be computed explicitly in terms of the values of $\ep$, $\delta$ and $\alpha$; in particular, it depends only on the dimension $d$. We also recall the ordering between the three exponents $\ep$, $\delta$ and $\alpha$ presented in~\eqref{eq:TVexpord}.

\smallskip

\textit{Step 1.} In this step, we let $\mathcal{H}$ be the two-scale expansion introduced in~\eqref{def.Ho2sc} and prove the estimate
\begin{equation} \label{eq:TV19578}
    \left\| \L \mathcal{H} - \f \rho_\delta \right\|_{\underline{H}^{-1}\left(B_{R^{1+\delta}} , \mu_\beta \right)} \leq \frac{C}{R^{d-1+\gamma}}.
\end{equation}

The strategy is to use the explicit formula for $\mathcal{H}$ to compute the value of the term $\mathcal{L} \mathcal{H}$ and then prove that its $\underline{H}^{-1}\left(B_{R^{1+\delta}} , \mu_\beta \right)$-norm is small by using the quantitative properties of the corrector stated in Proposition~\ref{prop:prop5.25}. 
We first write
\begin{equation} \label{eq:TV09577}
    \L \mathcal{H} = \underbrace{\Delta_\phi \mathcal{H}}_{\textnormal{Substep 1.1}} - \underbrace{\frac1{2\beta} \Delta \mathcal{H} + \sum_{q \in \mathcal{Q}} \nabla_q^* \cdot \a_q \nabla_q \mathcal{H}}_{\textnormal{Substep 1.2}} + \underbrace{\frac1{2\beta} \sum_{n \geq 1} \frac{1}{\sqrt{\beta}^n} \Delta^{n+1} \mathcal{H}}_{\textnormal{Substep 1.3}}= 0,
\end{equation}
and we treat the three terms in three distinct substeps.

\medskip

\textit{Substep 1.1} 
In this substep, we prove that the term $\Delta_\phi \mathcal{H}$ can be written 
\begin{equation} \label{eq:mainsub1.1hom}
    \Delta_\phi \mathcal{H} = \Delta_\phi \G_{\mathrm{hom}, \f }^\delta  + \sum_{i=1}^d \nabla_i \G_{\mathrm{hom}, \f }^\delta \left( \Delta_{\phi} \chi_{m,i}\right) + R_{\Delta_\phi},
\end{equation}
where the term $R_{\Delta_\phi}$ is an error term error which is small in the $\underline{H}^{-1}\left( B_{R^{1+\delta}} , \mu_\beta\right)$-norm; we prove that there exists an exponent $\gamma > 0$ such that
\begin{equation} \label{eq:TVRphi}
    \left\| R_{\Delta_\phi} \right\|_{\underline{H}^{-1}\left( B_{R^{1+\delta}} , \mu_\beta \right)} \leq \frac{C}{R^{d-1 + \gamma}}.
\end{equation}
We first compute the Laplacian in the $\phi$-variable of $\mathcal{H}$. We use the formula
\begin{equation*}
    \Delta_\phi \left( \mathbf{g} \mathbf{h} \right) =  \left(\Delta_\phi \mathbf{g} \right) \mathbf{h} + \mathbf{g}  \left(\Delta_\phi \mathbf{h}\right) + \sum_{y \in \Zd} \partial_y \mathbf{g} \partial_y \mathbf{h},
\end{equation*}
and obtain the identity \pd{We lost the norm $\left\| \f \right\|_{L^2 \left( \mu_\beta \right)}$}
\begin{equation*} 
    \Delta_\phi \mathcal{H} = \Delta_\phi \G_{\mathrm{hom}, \f }^\delta  + \sum_{i=1}^d \left( \Delta_\phi \nabla_i \G_{\mathrm{hom}, \f }^\delta \right) \chi_{m,i} + \sum_{i=1}^d \nabla_i \G_{\mathrm{hom}, \f }^\delta \left( \Delta_{\phi} \chi_{m,i}\right) +\sum_{i=1}^d \sum_{y \in \Zd} \left( \partial_y \nabla_i \G_{\mathrm{hom}, \f }^\delta \right) \partial_y  \chi_{m,i}.
\end{equation*}
We thus define the error term $R_{\Delta_\phi}$ according to the formula
\begin{equation} \label{eq:Laplaphi2sc1716}
    R_{\Delta_\phi} := \underbrace{ \sum_{i=1}^d \left( \Delta_\phi \nabla_i \G_{\mathrm{hom}, \f }^\delta \right) \chi_{m,i} }_{\eqref{eq:Laplaphi2sc1716}-(i)} + \underbrace{ \sum_{i=1}^d \sum_{y \in \Zd} \left( \partial_y \nabla_i \G_{\mathrm{hom}, \f }^\delta \right) \partial_y  \chi_{m,i} }_{\eqref{eq:Laplaphi2sc1716}-(ii)}
\end{equation}
The objective of this substep is to prove that terms~\eqref{eq:Laplaphi2sc1716}-(i) and~\eqref{eq:Laplaphi2sc1716}-(ii) are error terms which are small in the $H^{-1}\left( B_{R^{1+\delta}} , \mu_\beta\right)$-norm and we prove
\begin{equation} \label{eq:TV15445}
    \left\| \sum_{i=1}^d \left( \Delta_\phi \nabla_i \G_{\mathrm{hom}, \f }^\delta \right) \chi_{m,i} \right\|_{\underline{H}^{-1} \left( B_{R^{1+\delta} , \mu_\beta} \right)} \leq  \frac{C}{R^{d - 1 + \gamma}} \hspace{3mm}\mbox{and} \hspace{3mm} \left\| \sum_{i=1}^d \sum_{y \in \Zd} \left( \partial_y \nabla_i \G_{\mathrm{hom}, \f }^\delta \right) \partial_y  \chi_{m,i} \right\|_{\underline{H}^{-1}\left( B_{R^{1+\delta} }  , \mu_\beta \right)} \leq \frac{C}{R^{d-1+\gamma}}.
\end{equation}
We first focus on the term~\eqref{eq:Laplaphi2sc1716}-(i). To estimate it, we prove the following stronger $L^2$-estimate: there exists an exponent $\gamma > 0$ such that
\begin{equation} \label{eq:TV15455}
    \left\| \sum_{i=1}^d \left( \Delta_\phi \nabla_i \G_{\mathrm{hom}, \f }^\delta \right) \chi_{m,i} \right\|_{\underline{L}^2 \left( B_{R^{1+\delta} , \mu_\beta} \right)} \leq  \frac{C}{R^{d + \delta + \gamma}}.
\end{equation}
The estimate~\eqref{eq:TV15455} immediately implies the estimate~\eqref{eq:TV15445} since, by definition of the $\underline{H}^{-1}\left( B_{R^{1+\delta}} , \mu_\beta \right)$-norm and the Poincar\'e inequality, we have the estimate
\begin{equation*}
   \left\| \sum_{i=1}^d \left( \Delta_\phi \nabla_i \G_{\mathrm{hom}, \f }^\delta \right) \chi_{m,i} \right\|_{\underline{H}^{-1} \left( B_{R^{1+\delta} , \mu_\beta} \right)} \leq  C R^{1+ \delta}\left\| \sum_{i=1}^d \left( \Delta_\phi \nabla_i \G_{\mathrm{hom}, \f }^\delta \right) \chi_{m,i} \right\|_{\underline{L}^2 \left( B_{R^{1+\delta} , \mu_\beta} \right)} .
\end{equation*}
First, by applying the discrete gradient $\nabla_i$ to the identity on the function $\G_{\mathrm{hom}, \f }^\delta$ stated in~\eqref{def:GdeltaGhomdelta}, we deduce that, for each integer $i \in \{1 , \ldots, d \}$,
\begin{equation} \label{eq:TV10385}
    \left( \Delta_\phi \nabla_i \G_{\mathrm{hom}, \f }^\delta \right) = \left( - \ahom \Delta \nabla_i \G_{\mathrm{hom}, \f }^\delta + \f \nabla_i \rho_{\delta} \right).
\end{equation}
We then use the inequality
\begin{multline*}
    \left\| \left( - \ahom \Delta \nabla_i \G_{\mathrm{hom}, \f }^\delta + \f \nabla_i \rho_{\delta} \right) \chi_{m,i} \right\|_{\underline{L}^2 \left(B_{R^{1+\delta}} , \mu_\beta \right)} \\ \leq \left( \left\|  \ahom \Delta \nabla_i \G_{\mathrm{hom}, \f }^\delta \right\|_{L^\infty \left(B_{R^{1+\delta}} , \mu_\beta \right)} + \left\|\f \nabla_i \rho_{\delta}\right\|_{L^\infty \left(B_{R^{1+\delta}} , \mu_\beta \right)} \right) \left\| \chi_{m,i} \right\|_{\underline{L}^2 \left(B_{R^{1+\delta}} , \mu_\beta \right)}.
\end{multline*}
We then use the sublinearity of the corrector stated in~\eqref{eq:quantsublin}, the regularity estimates~\eqref{eq:spatregbarG} on the function $\G_{\mathrm{hom}, \f }^\delta$ and the estimate~\eqref{prop.rhodelta} on the function $\rho_\delta$ and its gradient. We obtain
\begin{equation} \label{eq:TV10215}
   \left\| \left( - \ahom \Delta \nabla_i \G_{\mathrm{hom}, \f }^\delta + \f \nabla_i \rho_{\delta} \right) \chi_{m,i} \right\|_{L^2 \left(B_{R^{1+\delta}} , \mu_\beta \right)} \leq \frac{C}{R^{(1-\delta)(d+1)}} \times R^{(1+\delta)(1-\alpha)} \leq  \frac{C}{R^{d} \times R^{\alpha (1 + \delta) - \delta (2+d)}}
\end{equation}
Recalling the assumption~\eqref{eq:TVexpord}, we set $\gamma := \alpha (1 + \delta) - \delta (3+d)$ and have $\gamma > 0$. The estimate~\eqref{eq:TV10215} can be rewritten in this notation
\begin{equation} \label{eq:TV10375}
    \left\| \left( - \ahom \Delta \nabla_i \G_{\mathrm{hom}, \f }^\delta + \f \nabla_i \rho_{\delta} \right) \chi_{m,i} \right\|_{L^2 \left(B_{R^{1+\delta}} , \mu_\beta \right)} \leq \frac{C}{R^{(1-\delta)(d+1)}} \times R^{(1+\delta)(1-\alpha)} \leq  \frac{C}{R^{d + \delta +  \gamma}}.
\end{equation}
Combining the inequality~\eqref{eq:TV10375} with the identity~\eqref{eq:TV10385} completes the estimate of the term~\eqref{eq:Laplaphi2sc1716}-(ii).

\smallskip

We now focus on the term~\eqref{eq:Laplaphi2sc1716}-(ii), we select and integer $i \in \{ 1 , \ldots, d \}$, a function $h$ in the space $H^1_0 \left( B_{R^{1+\delta}} , \mu_\beta \right)$ such that $\left\| h \right\|_{\underline{H}^1 \left( B_{R^{1+\delta}} , \mu_\beta \right)} \leq 1$. We prove the estimate
\begin{equation} \label{eq:TV15395}
    \frac{1}{R^{d(1+\delta)}}\sum_{x \in B_{R^{1+\delta}} }\sum_{y \in \Zd} \left\langle  \left( \partial_y \nabla_i  \G_{\mathrm{hom}, \f }^\delta(x , \cdot ) \right) \partial_y  \chi_{m,i}(x , \cdot) h(x, \cdot) \right\rangle_{\mu_{\beta}} \leq \frac{C}{R^{d-1+\gamma}}.
\end{equation}
The proof of this estimate relies on the quantative sublinearity of the corrector and the regularity estimates~\eqref{eq:partialbarG}. We first perform an integration by parts and use the formula $\partial_y^* \left( \mathbf{g} \mathbf{h} \right) =  \left( \partial_y^* \mathbf{g} \right) \mathbf{h} - \mathbf{g}  \left(\partial_y \mathbf{h}\right)$. We obtain
\begin{multline} \label{Deltaphimeter1841}
   \frac{1}{R^{d(1+\delta)}}\sum_{x \in B_{R^{1+\delta}} }\sum_{y \in \Zd} \left\langle  \left( \partial_y \nabla_i  \G_{\mathrm{hom}, \f }^\delta(x , \cdot ) \right) \partial_y  \chi_{m,i}(x , \cdot) h(x, \cdot) \right\rangle_{\mu_{\beta}} \\ = \underbrace{\frac{1}{R^{d(1+\delta)}}\sum_{x \in B_{R^{1+\delta}} } \left\langle  \chi_{m,i}(x , \cdot) \left( \Delta_\phi \nabla_i \bar G_\delta (x , \cdot)  \right) h(x , \cdot)  \right\rangle_{\mu_{\beta}}}_{\eqref{Deltaphimeter1841}-(i)} \\ -  \underbrace{\frac{1}{R^{d(1+\delta)}}\sum_{x \in B_{R^{1+\delta}} }\sum_{y \in \Zd} \left\langle \left( \partial_y \nabla_i \G_{\mathrm{hom}, \f }^\delta(x , \cdot ) \right) \chi_{m,i}(x , \cdot) \partial_y h(x ,\cdot) \right\rangle_{\mu_{\beta}}}_{\eqref{Deltaphimeter1841}-(ii)}.
\end{multline}
The term~\eqref{Deltaphimeter1841}-(i) is estimated with the same strategy as the term~\eqref{eq:Laplaphi2sc1716}-(i). We use the identity~\eqref{eq:TV10385}, the Cauchy-Schwarz inequality, the regularity estimate~\eqref{eq:spatregbarGgeq3} and the inequality $\left\|  h \right\|_{\underline{L}^2 \left( B_{R^{1+\delta}} , \mu_\beta \right)} \leq C R^{1+\delta}$ (which is a straightforward consequence of the assumption $\left\|  h \right\|_{\underline{H}^1 \left( B_{R^{1+\delta}} , \mu_\beta \right)} \leq 1$ and the Poincar\'e inequality). We obtain
\begin{align*}
    \frac{1}{R^{d(1+\delta)}}\sum_{x \in B_{R^{1+\delta}} } \left\langle  \chi_{m,i}(x , \cdot) \left( \Delta_\phi \nabla_i \bar G_\delta (x , \cdot)  \right) h(x , \cdot)  \right\rangle_{\mu_{\beta}}
    & \leq \left\| \chi_{m,i} \left( \Delta \nabla_i \bar G_\delta + \f \nabla_i \rho_{\delta} \right) \right\|_{\underline{L}^2 \left( B_{R^{1+\delta}} , \mu_\beta \right)} \left\|  h \right\|_{\underline{L}^2 \left( B_{R^{1+\delta}} , \mu_\beta \right)} \\
    & \leq  \frac{C}{R^{d} \times R^{\alpha (1 + \delta) - \delta (2+d)}} \times R^{1 + \delta}
    \\ & \leq \frac{C}{R^{d-1 + \gamma}},
\end{align*}
where we have set the value $\gamma := \alpha (1 + \delta) - \delta (3+d)$, we note that by the assumption~\eqref{eq:TVexpord}, we have $\gamma > 0$.
The term~\eqref{Deltaphimeter1841}-(ii) is estimated by the sublinearity of the corrector, the Cauchy Schwarz inequality and the regularity estimate~\eqref{eq:partialbarG}. We obtain
\begin{align*}
    \lefteqn{\frac{1}{R^{d(1+\delta)}}\sum_{x \in B_{R^{1+\delta}} }\sum_{y \in \Zd} \left\langle \left( \partial_y \nabla_i \G_{\mathrm{hom}, \f }^\delta(x , \cdot ) \right) \chi_{m,i}(x , \cdot) \partial_y h(x ,\cdot) \right\rangle_{\mu_{\beta}} } \qquad & \\ 
     & \leq \left\| \chi_{m,i} \right\|_{\underline{L}^2 \left(B_{R^{1 + \delta}}, \mu_\beta \right)}  \sum_{y \in \Zd} \left\| \partial_y \nabla_i \G_{\mathrm{hom}, \f }^\delta \right\|_{L^\infty \left( B_{R^{1+\delta}} , \mu_\beta \right)} \left\| \partial_y h \right\|_{\underline{L}^2 \left( B_{R^{1+\delta}} , \mu_\beta \right)} \\
    & \leq \left\| \chi_{m,i} \right\|_{\underline{L}^2 \left(B_{R^{1 + \delta}}, \mu_\beta \right)}  \left( \sum_{y \in \Zd} \left\| \partial_y \nabla_i \G_{\mathrm{hom}, \f }^\delta \right\|_{L^\infty \left( B_{R^{1+\delta}} , \mu_\beta \right)}^2 \right)^{\frac12}  \left(  \sum_{y \in \Zd} \left\| \partial_y h \right\|_{\underline{L}^2 \left( B_{R^{1+\delta}} , \mu_\beta \right)}^2 \right)^{\frac12} \\
    & \leq C R^{(1+\delta)(1 - \alpha)} \times R^{-d + \ep} \\
    & \leq C R^{-d - \gamma},
\end{align*}
where we have set $\gamma := \alpha (1 + \delta) - \delta - \ep$, according to the assumption~\eqref{eq:TVexpord}, we have $\gamma > 0$. The proof of the estimate~\eqref{eq:TV15395} and thus of the estimate~\eqref{eq:TV15445} is complete. 

\medskip


\textit{Sustep 1.2.} In this substep, we study the iteration of the Laplacian following the identity~\eqref{eq:TV09577}. We prove the estimate
\begin{equation} \label{eq:TV14557}
 	 \sum_{n \geq 1} \frac{1}{\beta^{\frac n2}} \Delta^{n+1} \mathcal{H} =  \sum_{i=1}^d \sum_{n \geq 1}  \frac{1}{\beta^{\frac n2}} \nabla_i \G_{\mathrm{hom}, \f }^\delta \Delta^{n+1} \chi_{m,i} + R_{\Delta^n},
\end{equation}
where $R_{\Delta^n}$ is an error term which satisfies the $\underline{H}^{-1}\left( B_{R^{1+\delta}} , \mu_\beta \right)$-estimate
\begin{equation}  \label{eq:TV14567}
\left\| R_{\Delta^n} \right\|_{\underline{H}^{-1}\left( B_{R^{1+\delta}} \mu_\beta \right)} \leq \frac{C}{R^{d-1+\gamma}}.
\end{equation}
We use the following identity for the iteration of the Laplacian on a product of functions: given two smooth functions $f , g \in \C^\infty \left( \Rd \right)$, we have the identity
\begin{equation} \label{eq:expandLap}
    \Delta^n \left( f g \right) = \sum_{k=0}^{n} \sum_{l = 0}^k \binom{n- k}{l} \left( \nabla^{k} \Delta^l  f  \right) \times \left( \nabla^{k} \Delta^{n- k - l} g \right),
\end{equation}
which can be obtained by induction. We note that this formula is valid for continuous functions (with the continuous Laplacian), it can nevertheless be adapted to the discrete setting considered in this article \pd{find a nice way to say it}.
Applying the formula~\eqref{eq:expandLap} to the two-scale expansion $\mathcal{H}$, we obtain
\begin{equation} \label{eq:TV11087}
\Delta^n \mathcal{H} = \Delta^n \G_{\mathrm{hom}, \f }^\delta + \sum_{i=1}^d \sum_{k=0}^{n} \sum_{l = 0}^k \binom{n- k}{l} \left( \nabla^{k} \Delta^l  \nabla_i  \G_{\mathrm{hom}, \f }^\delta  \right) \times \left( \nabla^{k} \Delta^{n- k - l} \chi_{m,i} \right) .
\end{equation}
We first focus on the term $\Delta^n \G_{\mathrm{hom}, \f }^\delta$ in the identity~\eqref{eq:TV11087} and prove that it is small. Using the regularity estimate~\eqref{eq:spatregbarGgeq3}, we have, for each integer $n \geq 2$,
\begin{align} \label{eq:TV14407}
    \left\| \Delta^n \G_{\mathrm{hom}, \f }^\delta  \right\|_{\underline{H}^{-1} \left( B_{R^{1+\delta}} , \mu_\beta \right)}  \leq C R^{1+\delta}\left\| \Delta^n \G_{\mathrm{hom}, \f }^\delta  \right\|_{\underline{L}^{2} \left( B_{R^{1+\delta}} , \mu_\beta \right)} 
    & \leq  C R^{1+\delta}\left\| \Delta^n \G_{\mathrm{hom}, \f }^\delta  \right\|_{L^{\infty} \left( B_{R^{1+\delta}} , \mu_\beta \right)} \\
    & \leq  \frac{C^{2n} R^{1+\delta}}{R^{(1-\delta)(d - 2 + 2n)}} \notag \\
    & \leq \frac{C^{2n} R^{1+\delta}}{R^{(1-\delta)(d - 2 + 4)}} \notag \\
    & \leq \frac{C^{2n} }{R^{d-1 + \gamma}}, \notag
\end{align}
where we have set $\gamma := 2 + \delta (d+1)$; it is in particular larger than $2$ and thus strictly larger than $0$.

Using the regularity estimate~\eqref{eq:spatregbarGgeq3} a second time, we estimate the terms of the right side of the identity~\eqref{eq:TV11087} with more than 3 derivatives on the homogenized Green's function $\G_{\mathrm{hom}, \f }^\delta$. We obtain the following inequality: for each integer $i \in \{ 1 , \ldots, d\}$, and each pair of integers $k, l \in \{ 1 , \ldots, d \}$ such that $l \leq n-k$ and $k + 2 l \geq 2$,
\begin{align} \label{eq:TV11047}
\lefteqn{ \left\| \left( \nabla^{k} \Delta^l  \nabla_i \G_{\mathrm{hom}, \f }^\delta  \right) \times \left( \nabla^{k} \Delta^{n- k - l} \chi_{m,i} \right) \right\|_{\underline{H}^{-1}(B_{R^{1+\delta}}, \mu_\beta)} } \qquad & \\  & \leq C R^{1+\delta} \left\| \left( \nabla^{k} \Delta^l  \nabla_i \G_{\mathrm{hom}, \f }^\delta \right) \times \left( \nabla^{k} \Delta^{n- k - l} \chi_{m,i} \right) \right\|_{\underline{L}^2(B_{R^{1+\delta}}, \mu_\beta)}\notag \\
 & \leq  C R^{1+\delta} \left\|  \nabla^{k} \Delta^l  \nabla_i \G_{\mathrm{hom}, \f }^\delta \right\|_{L^\infty \left( B_{R^{1+\delta}} , \mu_\beta \right)} \times \left\|  \nabla^{k} \Delta^{n- k - l} \chi_{m,i}  \right\|_{\underline{L}^2(B_{R^{1+\delta}}, \mu_\beta)} \notag \\
 & \leq \frac{C^{k + 2l} R^{1+\delta}}{R^{(1-\delta)(d-1+2l + k)}} \left\|  \nabla^{k} \Delta^{n- k - l} \chi_{m,i}  \right\|_{\underline{L}^2(B_{R^{1+\delta}}, \mu_\beta)}. \notag
 \end{align}
 We then use that the discrete operator $ \nabla^{k} \Delta^{n- k - l}$ is continuous on the space $L^2 \left( B_{R^{1+\delta}} \right)$ (since the discrete gradient is a continuous operator) and Proposition~\ref{prop:prop5.25} to estimate the $L^2$-norm of the corrector. We obtain
 \begin{equation} \label{eq:TV11037}
      \left\|  \nabla^{k} \Delta^{n- k - l} \chi_{m,i}  \right\|_{\underline{L}^2(B_{R^{1+\delta}}, \mu_\beta)} \leq C^{2n - 2l} \left\|   \chi_{m,i}  \right\|_{\underline{L}^2(B_{R^{1+\delta}}, \mu_\beta)} \leq  C^{2n - 2l} R^{(1+\delta)(1-\alpha)}.
 \end{equation}
 Putting the estimate~\eqref{eq:TV11047} and~\eqref{eq:TV11037} together and using the inequality $3 \leq 2l+k \leq 2n$, we deduce that
 \begin{equation} \label{eq:TV14387}
       \left\| \left( \nabla^{k} \Delta^l  \nabla_i \G_{\mathrm{hom}, \f }^\delta  \right) \times \left( \nabla^{k} \Delta^{n- k - l} \chi_{m,i} \right) \right\|_{\underline{H}^{-1}(B_{R^{1+\delta}}, \mu_\beta)} \leq  \frac{C^{2n} R^{1+\delta}}{R^{(1-\delta)(d+2)}} R^{(1+\delta)(1-\alpha)} \leq \frac{C^{2n}}{R^{d-1 + \gamma}},
 \end{equation}
where we have set $\gamma := 1 + \alpha - \alpha \delta + \delta \left( d-1 \right) + \delta$. We note that since we assumed that the value of the exponents $\alpha$ and $\delta$ us small, the exponent $\gamma$ is close to $1$, it satisfies in particular the weaker property to be strictly positive, as required.

We then estimate the $H^{-1}$-norm of the terms corresponding to the parameters $k=1$ and $l=0$ in the sum in the right side of the identity~\eqref{eq:TV11087}. To estimate it, we select a function $h \in H^1 \left(B_{R^{1+\delta}}, \mu_\beta \right)$ such that $\left\| h \right\|_{\underline{H}^1 \left( B_{R^{1+\delta}}, \mu_\beta \right)}\leq 1$. We use the function $h$ as a test function, perform an integration by parts in the first line, use the Cauchy-Schwarz inequality in the second and the continuity of the Laplacian in the third line. We obtain 
\begin{align} \label{eq:TV14097}
\lefteqn{\frac{1}{R^{(1+\delta)d}}\sum_{x \in B_{R^{1+\delta}}} \left\langle \left( \nabla \nabla_i \G_{\mathrm{hom}, \f }^\delta \left( x , \cdot \right)  \right) \times \left( \nabla \Delta^{n- 1} \chi_{m,i} (x , \cdot ) \right)  h(x , \cdot)  \right\rangle_{\mu_\beta} } \qquad & \\ 
			& = \frac{1}{R^{(1+\delta)d}} \sum_{x \in B_{R^{1+\delta}}} \left\langle \chi_{m,i} (x , \cdot )   \nabla \Delta^{n- 1} \left( \left( \nabla \nabla_i \G_{\mathrm{hom}, \f }^\delta \left( x , \cdot \right)  \right) h  (x , \cdot )\right) \right\rangle_{\mu_\beta} \notag \\
			& \leq  \left\| \chi_{m,i} \right\|_{L^2 \left( B_{R^{1+\delta}}, \mu_\beta \right) }   \left\| \nabla \Delta^{n- k}\left( \nabla \nabla_i \G_{\mathrm{hom}, \f }^\delta  h \right) \right\|_{\underline{L}^2 \left( B_{R^{1+\delta}} , \mu_\beta \right)} \notag \\
			& \leq C^{n} \left\| \chi_{m,i} \right\|_{L^2 \left( B_{R^{1+\delta}}, \mu_\beta \right) }   \left\| \nabla \left( \nabla \nabla_i \G_{\mathrm{hom}, \f }^\delta  h \right) \right\|_{\underline{L}^2 \left( B_{R^{1+\delta}} , \mu_\beta \right)} \notag
\end{align}
Using the regularity estimate for the homogenized Green's function stated in~\eqref{eq:spatregbarGgeq3} and the inequality $\left\| h \right\|_{\underline{L}^2 \left(B_{R^{1+\delta}} , \mu_\beta \right)} \leq R^{1+\delta}$ (which is a consequence of the assumption $\left\| h \right\|_{\underline{H}^1 \left(B_{R^{1+\delta}} , \mu_\beta \right)} \leq 1$ and the Poincar\'e inequality), we obtain
\begin{align} \label{eq:TV14047}
    \left\| \nabla \left(\left( \nabla \nabla_i \G_{\mathrm{hom}, \f }^\delta \right) h \right) \right\|_{\underline{L}^2 \left( B_{R^{1+\delta}} , \mu_\beta \right)} & \leq \left\| \nabla^3 \G_{\mathrm{hom}, \f }^\delta h \right\|_{\underline{L}^2 \left( B_{R^{1+\delta}} , \mu_\beta \right)} + \left\| \nabla^2 \G_{\mathrm{hom}, \f }^\delta  \nabla h \right\|_{\underline{L}^2 \left( B_{R^{1+\delta}} , \mu_\beta \right)} \\
    & \leq  \frac{CR^{1+\delta}}{R^{\left( 1-\delta \right)\left(d + 1 \right)}}  +  \frac{C}{R^{\left( 1-\delta \right)d}} \notag \\ &
    \leq \frac{C}{R^{d - \delta (d+2)}}. \notag
\end{align}
We then combine the estimate~\eqref{eq:TV14097} with the inequality~\eqref{eq:TV14047} and the quantitative sublinearity of the corrector stated in Proposition~\ref{prop:prop5.25}. We obtain
\begin{equation} \label{eq:TV14397}
    \frac{1}{R^{(1+\delta)d}}\sum_{x \in B_{R^{1+\delta}}} \left\langle \left( \nabla \nabla_i \G_{\mathrm{hom}, \f }^\delta \left( x , \cdot \right)  \right) \times \left( \nabla \Delta^{n- 1} \chi_{m,i} (x , \cdot ) \right)  h(x , \cdot)  \right\rangle_{\mu_\beta} \leq \frac{C^n R^{\left(1+\delta\right)(1 - \alpha) }}{R^{d - \delta (d+2)}} \leq  \frac{C^n}{R^{d - 1 + \gamma }},
\end{equation}
where we have set $\gamma :=\alpha (1+\delta) - \delta (d+3) $, using that the exponent $\alpha$ is much larger than the exponent $\delta$ by the assumption~\eqref{eq:TVexpord}, we deduce that $\gamma$ is strictly positive. By combining the identity~\eqref{eq:TV11087} with the estimates~\eqref{eq:TV14407},~\eqref{eq:TV14387},~\eqref{eq:TV14397} and choosing the inverse temperature $\beta$ large enough, in particular larger than the square of all the constants $C$ which appear in this substep (and depend only on the dimension $d$) so that the series $\left( \frac{C^n}{\beta^{\frac n2}}\right)_{n \in \N}$ is summable, we obtain the main result~\eqref{eq:TV14567} and~\eqref{eq:TV14557} of this substep.

\medskip

\textit{Substep 1.3.}  In this substep, we study the iteration of the term pertaining to the charges following the identity~\eqref{eq:TV09577}. We prove the estimate
\begin{equation} \label{eq:mainsub1.3hom}
 \frac{1}{2\beta} \Delta \mathcal{H} + \sum_{\di q=0} \nabla_q^* \cdot \a_q \nabla_q \mathcal{H}  = \ahom  \Delta \G_{\mathrm{hom}, \f }^\delta + \sum_{i=1}^d \frac{1}{2\beta} \nabla_i  \G_{\mathrm{hom}, \f }^\delta \Delta \chi_{m,i} +   \sum_{i=1}^d  \sum_{\di q=0} \nabla_i  \G_{\mathrm{hom}, \f }^\delta \nabla_q^* \cdot \a_q \nabla_q \chi_{m,i}+ R_{Q}.
\end{equation}
where $R_{Q}$ is an error term which satisfies the $\underline{H}^{-1}\left( B_{R^{1+\delta}} , \mu_\beta \right)$-estimate
\begin{equation}  \label{eq:TV14567}
\left\| R_{Q} \right\|_{\underline{H}^{-1}\left( B_{R^{1+\delta}} \mu_\beta \right)} \leq \frac{C}{R^{d-1+\gamma}}.
\end{equation}
We first compute the gradient and the Laplacian of the two-scale expansion $\mathcal{H}$ and obtain the following formulas
\begin{equation} \label{eq:formnablaH2sc}
\nabla \mathcal{H} = \nabla  \G_{\mathrm{hom}, \f }^\delta  + \sum_{i=1}^d \left[ \nabla \nabla_i  \G_{\mathrm{hom}, \f }^\delta  \chi_{m,i} + \nabla_i  \G_{\mathrm{hom}, \f }^\delta   \nabla \chi_{m,i} \right],
\end{equation}
and
\begin{equation*}
    \Delta \mathcal{H}  = \Delta \G_{\mathrm{hom}, \f }^\delta + \sum_{i=1}^d \left( \Delta \nabla_i  \G_{\mathrm{hom}, \f }^\delta  \right) \chi_{m,i} + \left( \nabla \nabla_i  \G_{\mathrm{hom}, \f }^\delta  \right) \cdot \left( \nabla \chi_{m,i} \right)  + \left(  \nabla_i  \G_{\mathrm{hom}, \f }^\delta  \right) \Delta \chi_{m,i} \\
\end{equation*}
We first treat the term $\Delta \mathcal{H}$ and use the two following ingredients:
\begin{enumerate}
    \item[(i)] First we introduce the notation $R_{Q,1} := \sum_{i=1}^d \left( \Delta \nabla_i  \G_{\mathrm{hom}, \f }^\delta  \right) \chi_{m,i} $. By using the regularity estimate~\eqref{eq:spatregbarGgeq3} on the homogenized Green's function and the quantitative sublinearity of the corrector stated in 
    Proposition~\ref{prop:prop5.25}, we prove that this term is an error term and estimate its $\underline{H}^{-1} \left( B_{R^{1+\delta}} , \mu_\beta \right)$-norm according to the following computation
    \begin{align*}
        \left\| R_{Q,1} \right\|_{\underline{H}^{-1} \left( B_{R^{1+\delta}} , \mu_\beta \right)} & \leq C R^{1+\delta} \left\|  R_{Q,1} \right\|_{\underline{L}^{2} \left( B_{R^{1+\delta}} , \mu_\beta \right)} \\
        & \leq \sum_{i=1}^d C R^{1+\delta} \left\|  \left( \Delta \nabla_i  \G_{\mathrm{hom}, \f }^\delta  \right) \right\|_{L^{\infty} \left( B_{R^{1+\delta}} , \mu_\beta \right)} \left\|  \chi_{m,i} \right\|_{\underline{L}^{2} \left( B_{R^{1+\delta}} , \mu_\beta \right)}\\
        & \leq \frac{C R^{1+\delta} R^{\left( 1 + \delta \right)\left(1-\alpha\right)}}{R^{(1-\delta) (d+1)}} \\
        & \leq \frac{C}{R^{d-1 + \gamma}},
    \end{align*}
    where we have set $\gamma :=\alpha (1+\delta) - \delta (d+3)$. By the assumption~\eqref{eq:TVexpord}, the exponent $\gamma$ is strictly positive; \smallskip
    \item[(ii)] Second, we use the identity $\Delta \mathcal{H} = \sum_{i=1}^d \nabla \cdot \left( \nabla_i \G_{\mathrm{hom}, \f }^\delta  e_i \right)$.
\end{enumerate}
We obtain
\begin{equation} \label{eq:TV21228}
     \Delta \mathcal{H}  = \sum_{i=1}^d  \left( \nabla \nabla_i  \G_{\mathrm{hom}, \f }^\delta  \right) \cdot \left( e_i + \nabla \chi_{m,i} \right) + \sum_{i=1}^d \left(  \nabla_i  \G_{\mathrm{hom}, \f }^\delta  \right) \Delta \chi_{m,i} + R_{Q,1}
\end{equation}
We then treat the term pertaining to the charges; the objective is to prove the identity 
\begin{equation} \label{eq:TV19558}
\sum_{\di q=0} \nabla_q^* \cdot \a_q \nabla_q \mathcal{H} = \sum_{i = 1}^d \sum_{\di q = 0}  \left( \di^* \nabla_i \G_{\mathrm{hom}, \f }^\delta \right) \a_q \nabla_q \left( l_{e_i} + \chi_{m,i} \right) n_q + \sum_{\di q = 0} \nabla_i  \G_{\mathrm{hom}, \f }^\delta \nabla_q^* \cdot \a_q \nabla_q \left( l_{e_i} + \chi_{m,i} \right) + R_{Q,2},
\end{equation}
where $R_{Q,2}$ is an error term which satisfies the estimate
\begin{equation} \label{eq:TV19568}
    \left\| R_{Q,2} \right\|_{\underline{H}^{-1}\left(B_{R^{1+\delta}} , \mu_\beta \right)} \leq \frac{C}{R^{d-1-\gamma}}
\end{equation}
To prove this result, we select a test function $h$ which belongs to the space $H^1_0 \left(B_{R^{1+\delta}} , \mu_\beta \right)$ which satisfies the estimate $\left\| h \right\|_{\underline{H}^1 \left(B_{R^{1+\delta}} , \mu_\beta \right)} \leq 1$. Moreover, for each charge $q \in \mathcal{Q}$, we select a point $x_q$ which belongs to the support of the charge $q$ arbitrarily. We then write
\begin{equation} \label{eq:TV21447}
    \sum_{\di q=0} \a_q \nabla_q \mathcal{H} \nabla_q h :=  \sum_{\di q=0}  \a_q \left( n_q , \di^* \mathcal{H} \right) \left( n_q , \di^* h \right) 
\end{equation}
We use the exact formula for $\mathcal{H}$, and recall that we have the identity $\di^* \G_{\mathrm{hom}, \f }^\delta = \sum_{i=1}^d \nabla_i \G_{\mathrm{hom}, \f }^\delta \di^* l_{e_i}$. We obtain 
\begin{equation} \label{eq:TV21357}
    \di^* \mathcal{H}  = \di^* \G_{\mathrm{hom}, \f }^\delta + \sum_{i = 1}^d \nabla_i \G_{\mathrm{hom}, \f }^\delta \di^* \chi_{m,i} +  \sum_{i = 1}^d \di^* \nabla_i \G_{\mathrm{hom}, \f }^\delta \chi_{m,i}
             = \sum_{i = 1}^d \nabla_i \G_{\mathrm{hom}, \f }^\delta \left( \di^* l_{e_i} + \di^* \chi_{m,i} \right) + \sum_{i=1}^d \di^* \nabla_i \G_{\mathrm{hom}, \f }^\delta \chi_{m,i}.
\end{equation}
Putting the identity~\eqref{eq:TV21357} back into~\eqref{eq:TV21447}, we obtain \pd{change $\sum_{\di q = 0}$ into $\sum_{q \in \Qa}$}
\begin{equation} \label{eq:TV22007}
     \sum_{q \in \Qa} \a_q \nabla_q \mathcal{H} \nabla_q h = \underbrace{\sum_{i = 1}^d \sum_{q \in \Qa}  \a_q \left( n_q , \nabla_i \G_{\mathrm{hom}, \f }^\delta \left( \di^* l_{e_i} + \di^* \chi_{m,i} \right) \right) \left( n_q , \di^* h \right)}_{\eqref{eq:TV22007}-(i)}  +  \underbrace{\sum_{q \in \Qa}  \a_q \left( n_q , \di^* \nabla_i \G_{\mathrm{hom}, \f }^\delta \chi_{m,i} \right) \left( n_q , \di^* h \right)}_{\eqref{eq:TV22007}-(ii)} .
\end{equation}
The second term~\eqref{eq:TV22007}-(ii) is an error term which is small can be estimated thanks to the regularity estimate~\eqref{eq:spatregbarGgeq3} and Young's inequality. We obtain
\begin{align*}
     \lefteqn{ \left| \left\langle \sum_{q \in \Qa}  \a_q \left( n_q , \di^* \nabla_i \G_{\mathrm{hom}, \f }^\delta \chi_{m,i} \right) \left( n_q , \di^* h \right) \right\rangle_{\mu_\beta} \right|} \qquad & \\ &  \leq \sum_{q \in \Qa} e^{-c \sqrt{\beta} \left\| q \right\|_1} \left\| n_q \right\|_2^2 \left\| \nabla^2 \G_{\mathrm{hom}, \f }^\delta\right\|_{L^\infty \left( \Zd , \mu_\beta \right)} \left\| \chi_{m,i} \right\|_{L^2 \left( \supp n_q , \mu_\beta \right)} \left\| \nabla h \right\|_{L^2 \left( \supp n_q , \mu_\beta \right)} \\
     & \leq \frac{C}{R^{(1-\delta)(d+1)}}  \sum_{q \in \Qa} e^{-c \sqrt{\beta} \left\| q \right\|_1} \left\| n_q \right\|_2^2 \left\| \chi_{m,i} \right\|_{L^2 \left( \supp n_q , \mu_\beta \right)} \left\| \nabla h \right\|_{L^2 \left( \supp n_q , \mu_\beta \right)} \\
     & \leq \frac{C}{R^{(1-\delta)(d+1)}}  \sum_{q \in \Qa} e^{-c \sqrt{\beta} \left\| q \right\|_1} \left\| n_q \right\|_2^2 \left( R^{1 + \alpha} \left\| \chi_{m,i} \right\|_{L^2 \left( \supp n_q , \mu_\beta \right)}^2 + R^{- 1 - \alpha} \left\| \nabla h \right\|_{L^2 \left( \supp n_q , \mu_\beta \right)}^2 \right).
\end{align*}
We then use the inequality, for each point $x \in \Zd$,
\begin{equation} \label{eq:TV09127}
    \sum_{q \in \Qa} e^{-c \sqrt{\beta} \left\| q \right\|_1} \left\| n_q \right\|_2^2 \indc_{\{ x \in \supp n_q\}} \leq C.
\end{equation}
We deduce that
\begin{equation*}
    \left| \left\langle \sum_{q \in \Qa}  \a_q \left( n_q , \di^* \nabla_i \G_{\mathrm{hom}, \f }^\delta \chi_{m,i} \right) \left( n_q , \di^* h \right) \right\rangle_{\mu_\beta} \right| \leq \frac{CR^{-1 + \alpha}}{R^{(1-\delta)(d+1)}}  \left\| \chi_{m,i} \right\|_{L^2 \left(B_{R^{1+\delta}, \mu_\beta } \right)}^2 + \frac{CR^{1-\alpha}}{R^{(1-\delta)(d+1)}} \left\| \nabla h \right\|_{L^2 \left(B_{R^{1+\delta}, \mu_\beta } \right)}^2.
\end{equation*}
We then use Proposition~\ref{prop:prop5.25} and the assumption $\left\| \nabla h \right\|_{L^2 \left(B_{R^{1+\delta}, \mu_\beta } \right)} \leq 1$. We obtain
\begin{equation} \label{eq:TV18538}
    \left| \left\langle \sum_{q \in \Qa}  \a_q \left( n_q , \di^* \nabla_i \G_{\mathrm{hom}, \f }^\delta \chi_{m,i} \right) \left( n_q , \di^* h \right) \right\rangle_{\mu_\beta} \right| \leq \frac{C R^{1-\alpha}}{R^{(1-\delta)(d+1)}} \leq \frac{C}{R^{d-1 + \gamma}},
\end{equation}
where we have set $\gamma = \alpha - \delta \left( d+1 \right)$, it is strictly positive by the assumption~\eqref{eq:TVexpord}.

To treat the term~\eqref{eq:TV22007}-(i), we first use the point $x_q$ as a pivotal point and write
\begin{align*}
     \sum_{\di q=0}  \a_q \left( n_q , \nabla_i \G_{\mathrm{hom}, \f }^\delta \left( \di^* l_{e_i} + \di^* \chi_{m,i} \right) \right) \left( n_q , \di^* h \right) & = \sum_{\di q=0}   \a_q \left( n_q ,  \left( \di^* l_{e_i} + \di^* \chi_{m,i} \right) \right) \left( n_q , \nabla_i \G_{\mathrm{hom}, \f }^\delta \di^* h \right) \\
     & + \sum_{\di q=0} \a_q \left( n_q ,\left( \nabla_i \G_{\mathrm{hom}, \f }^\delta - \nabla_i \G_{\mathrm{hom}, \f }^\delta(x_q) \right)  \left( \di^* l_{e_i} + \di^* \chi_{m,i} \right) \right) \left( n_q , \di^* h \right) \\
     & +  \sum_{\di q=0} \a_q \left( n_q   \left( \di^* l_{e_i} + \di^* \chi_{m,i} \right) \right) \left( n_q , \left( \nabla_i \G_{\mathrm{hom}, \f }^\delta - \nabla_i \G_{\mathrm{hom}, \f }^\delta(x_q) \right) \di^* h \right).
\end{align*}
The terms on the second and third line are error term which are small, they can be estimated by the regularity estimate~\eqref{eq:spatregbarGgeq3} on the gradient of the homogenized Green's function, Young's inequality. We obtain
\begin{align*}
    \lefteqn{\left| \left\langle \sum_{\di q=0} \a_q \left( n_q ,\left( \nabla_i \G_{\mathrm{hom}, \f }^\delta - \nabla_i \G_{\mathrm{hom}, \f }^\delta(x_q) \right)  \left( \di^* l_{e_i} + \di^* \chi_{m,i} \right) \right) \left( n_q , \di^* h \right) \right\rangle_{\mu_\beta} \right|  } \qquad & \\ & \leq \sum_{\di q=0} e^{-c \sqrt{\beta} \left\| q \right\|_1} \left\| n_q \right\|_2 \left\| \G_{\mathrm{hom}, \f }^\delta - \G_{\mathrm{hom}, \f }^\delta \right\|_{L^\infty \left( \supp n_q , \mu_\beta \right)} \left\|  \nabla \chi_{m,i} \right\|_{L^2 \left( \supp n_q , \mu_\beta \right)} \left\| \nabla h \right\|_{L^2 \left( \supp n_q , \mu_\beta \right)} \\
    & \leq \frac{C}{R^{(1-\delta)d}} \sum_{\di q=0} e^{-c \sqrt{\beta} \left\| q \right\|_1} \left\| n_q \right\|_2  \left( \left\|  \nabla \chi_{m,i} \right\|_{L^2 \left( \supp n_q , \mu_\beta \right)}^2 +  \left\| \nabla h \right\|_{L^2 \left( \supp n_q , \mu_\beta \right)}^2 \right). 
\end{align*}
We then the estimate~\eqref{eq:TV09127}, the bound $\left\| \nabla \chi_{m,i} \right\|_{\underline{L}^2 \left( B_{R^{1+\delta}} , \mu_\beta \right)} \leq C$ on the gradient of the corrector and the assumption $\left\| \nabla h \right\|_{\underline{L}^2 \left( B_{R^{1+\delta}} , \mu_\beta \right)} \leq 1$ to conclude that
\begin{equation} \label{eq:TV18538}
    \left| \left\langle \sum_{\di q=0} \a_q \left( n_q ,\left( \nabla_i \G_{\mathrm{hom}, \f }^\delta - \nabla_i \G_{\mathrm{hom}, \f }^\delta(x_q) \right)  \left( \di^* l_{e_i} + \di^* \chi_{m,i} \right) \right) \left( n_q , \di^* h \right) \right\rangle_{\mu_\beta} \right|  \leq \frac{C}{R^{(1-\delta)d}} \leq \frac{C}{R^{(d-1) + \gamma}},
\end{equation}
where we have set $\gamma = 1 - \delta$, it is close to $1$ and in particular strictly positive.
The same argument proves the inequality
\begin{equation} \label{eq:TV18528}
     \left| \left\langle \sum_{\di q=0} \a_q \left( n_q   \left( \di^* l_{e_i} + \di^* \chi_{m,i} \right) \right) \left( n_q , \left( \nabla_i \G_{\mathrm{hom}, \f }^\delta - \nabla_i \G_{\mathrm{hom}, \f }^\delta(x_q) \right) \di^* h \right) \right\rangle_{\mu_\beta} \right| \leq \frac{C}{R^{(d-1) + \gamma}},
\end{equation}
with the same exponent $\gamma >0$. Combining the identity~\eqref{eq:TV22007} with the estimates~\eqref{eq:TV18538},~\eqref{eq:TV18538},~\eqref{eq:TV18528}, we have obtained the following result: for each function $h \in H^1_0 \left( B_{R^{1+\delta}} , \mu_\beta \right)$ such that $\left\| h \right\|_{\underline{H}^1 \left(B_{R^{1+\delta}} , \mu_\beta \right)} \leq 1$, one has the estimate
\begin{equation*}
    \sum_{q \in \Qa} \a_q \nabla_q \mathcal{H} \nabla_q h =  \sum_{\di q=0}   \a_q \left( n_q ,  \left( \di^* l_{e_i} + \di^* \chi_{m,i} \right) \right) \left( n_q , \nabla_i \G_{\mathrm{hom}, \f }^\delta \di^* h \right) + O \left( \frac{1}{R^{d - 1 + \gamma}} \right).
\end{equation*}
We then use the identity $\nabla_i \G_{\mathrm{hom}, \f }^\delta \di^* h = \di^*  \left(\nabla_i \G_{\mathrm{hom}, \f }^\delta h \right) -  \di^* \nabla_i \G_{\mathrm{hom}, \f }^\delta h$ and deduce that
\begin{multline} \label{eq:TV19548}
    \sum_{q \in \Qa} \a_q \nabla_q \mathcal{H} \nabla_q h =  \sum_{\di q=0}   \a_q \left( n_q ,  \left( \di^* l_{e_i} + \di^* \chi_{m,i} \right) \right) \left( n_q , \di^* \left( \nabla_i \G_{\mathrm{hom}, \f }^\delta  h\right) \right) \\ + \sum_{\di q=0}   \a_q \left( n_q ,  \left( \di^* l_{e_i} + \di^* \chi_{m,i} \right) \right) \left( n_q , \di^* \nabla_i \G_{\mathrm{hom}, \f }^\delta  h \right) + O \left( \frac{1}{R^{d - 1 + \gamma}} \right).
\end{multline}
The inequality~\eqref{eq:TV19548} is exactly equivalent to the identity~\eqref{eq:TV19558} and the estimate~\eqref{eq:TV19568}.

We now complete the proof of~\eqref{eq:mainsub1.3hom}. To prove this identity, it is sufficient, in view of~\eqref{eq:TV21228} and~\eqref{eq:TV19558} to prove the estimate
\begin{equation} \label{eq:07499}
    \sum_{i=1}^d  \left( \nabla \nabla_i  \G_{\mathrm{hom}, \f }^\delta  \right) \cdot \left( e_i + \nabla \chi_{m,i} \right) + \sum_{i = 1}^d \sum_{\di q = 0}  \left( \di^* \nabla_i \G_{\mathrm{hom}, \f }^\delta \right) \a_q \nabla_q \left( l_{e_i} + \chi_{m,i} \right) n_q = \ahom \Delta \G_{\mathrm{hom}, \f }^\delta + R_{Q,3},
\end{equation}
where the term $R_{Q,3}$ satisfies the estimate
\begin{equation} \label{eq:07509}
    \left\| R_{Q,3} \right\|_{\underline{H}^{-1}\left( B_{R^{1+\delta}} , \mu_\beta\right)} \leq \frac{C}{R^{1-d+ \gamma}}.
\end{equation}
The proof relies on the quantitative estimate for the $\underline{H}^{-1}\left( B_{R^{1+\delta}} , \mu_\beta\right)$-norm of the flux corrector stated in Proposition~\ref{prop:prop5.25} and the regularity estimate~\eqref{eq:spatregbarGgeq3} on the homogenized function $\G_{\mathrm{hom}, \f }^\delta$. We select a function $h \in H^1_0 \left( B_{R^{1+\delta}} , \mu_\beta \right)$ such that $\left\| h \right\|_{\underline{H}^1 \left( B_{R^{1+\delta}} , \mu_\beta \right)} \leq 1$ and use it as a test function. We write
\begin{align} \label{eq:TV07399}
    \lefteqn{\frac{1}{R^{(1+\delta)d}} \left| \left\langle  \sum_{x \in B_{R^{1+\delta}}}\sum_{i=1}^d  \left( \nabla \nabla_i  \G_{\mathrm{hom}, \f }^\delta(x , \cdot )  \right) \cdot \left( e_i + \nabla \chi_{m,i}(x , \cdot) \right)  \right. \right.} \qquad & \\ & \left. \left. + \sum_{i = 1}^d \sum_{\di q = 0}   \a_q \nabla_q \left( l_{e_i} + \chi_{m,i} \right) \left( n_q, \di^* \nabla_i \G_{\mathrm{hom}, \f }^\delta h \right) - \sum_{x \in B_{R^{1+\delta}}} \sum_{i = 1}^d \ahom \Delta  \G_{\mathrm{hom}, \f }^\delta(x , \cdot ) h(x , \cdot) \right\rangle_{\mu_\beta}\right| \notag \\ & \leq C \sum_{i=1}^d  \left\| e_i + \frac 1{2 \beta} \nabla \chi_{m,i} + \sum_{q} \a_q \nabla_q \left( l_{e_i} + \chi_{n,i} \right) n_q - \ahom e_i \right\|_{\underline{H}^{-1}\left( B_{R^{1+\delta}} , \mu_\beta \right)} \left\| \nabla^2 \G_{\mathrm{hom}, \f }^\delta  h \right\|_{\underline{H}^1 \left(B_{R^{1+\delta}} , \mu_\beta \right)}. \notag
\end{align}
We then use Proposition~\ref{prop:prop5.25} to write
\begin{equation} \label{eq:TV07379}
    \sum_{i=1}^d  \left\| e_i + \frac 1{2 \beta} \nabla \chi_{m,i} + \sum_{q} \a_q \nabla_q \left( l_{e_i} + \chi_{n,i} \right) n_q - \ahom e_i \right\|_{\underline{H}^{-1}\left( B_{R^{1+\delta}} , \mu_\beta \right)} \leq CR^{(1+\delta)(1-\alpha)}
\end{equation}
and the regularity estimate~\eqref{eq:spatregbarGgeq3} to write 
\begin{align} \label{eq:TV07299}
    \left\| \nabla^2 \G_{\mathrm{hom}, \f }^\delta  h \right\|_{\underline{H}^1 \left(B_{R^{1+\delta}} , \mu_\beta \right)} & \leq  \frac{1}{R^{1+\delta}}\left\|  \nabla^2 \G_{\mathrm{hom}, \f }^\delta  \right\|_{L^\infty \left( B_{R^{1+\delta}} , \mu_\beta \right)}\left\|   h \right\|_{\underline{L}^2 \left( B_{R^{1+\delta}} , \mu_\beta \right)} + \left\|  \nabla^3 \G_{\mathrm{hom}, \f }^\delta  \right\|_{L^\infty \left( B_{R^{1+\delta}} , \mu_\beta \right)}\left\|  h \right\|_{\underline{L}^2 \left( B_{R^{1+\delta}} , \mu_\beta \right)}  \\ & \qquad + \left\|  \nabla^2 \G_{\mathrm{hom}, \f }^\delta  \right\|_{L^\infty \left( B_{R^{1+\delta}} , \mu_\beta \right)}\left\| \nabla h \right\|_{\underline{L}^2 \left( B_{R^{1+\delta}} , \mu_\beta \right)} \notag \\
    & \leq C \left(\frac{1}{R^{d(1-\delta)}} + \frac{1}{R^{(d-1)(1-\delta)}} + \frac{R^{1+\delta}}{R^{(d+1)(1-\delta)}} \right) \notag\\
    & \leq \frac{1}{R^{d - \delta\left( d+2 \right)}} \notag
\end{align}
Combining the estimates~\eqref{eq:TV07399},~\eqref{eq:TV07379} and~\eqref{eq:TV07299}, we have obtained that, for each function $h \in H^1_0 \left( B_{R^{1+\delta}} , \mu_\beta \right)$ such that $\left\| h \right\|_{\underline{H}^1 \left( B_{R^{1+\delta}} , \mu_\beta \right)} \leq 1$,
\begin{align} \label{eq:07489}
    \lefteqn{\frac{1}{R^{(1+\delta)d}} \left| \left\langle  \sum_{x \in B_{R^{1+\delta}}}\sum_{i=1}^d  \left( \nabla \nabla_i  \G_{\mathrm{hom}, \f }^\delta(x , \cdot )  \right) \cdot \left( e_i + \nabla \chi_{m,i}(x , \cdot) \right)  \right. \right.} \qquad & \\ & \left. \left. \qquad + \sum_{i = 1}^d \sum_{\di q = 0}   \a_q \nabla_q \left( l_{e_i} + \chi_{m,i} \right) \left( n_q, \di^* \nabla_i \G_{\mathrm{hom}, \f }^\delta h \right) - \sum_{x \in B_{R^{1+\delta}}} \sum_{i = 1}^d \ahom \Delta  \G_{\mathrm{hom}, \f }^\delta(x , \cdot ) h(x , \cdot) \right\rangle_{\mu_\beta}\right| \notag \\ & \leq \frac{CR^{(1+\delta)(1-\alpha)}}{R^{d - \delta\left( d+2 \right)}} \notag \\
    & \leq \frac{C}{R^{d-1 + \gamma}}, \notag
\end{align}
where we have set $\gamma := $; by the assumption~\eqref{eq:TVexpord}, it is strictly positive. Since the inequality~\eqref{eq:07489} is valid for any function  for each function $h \in H^1_0 \left( B_{R^{1+\delta}} , \mu_\beta \right)$ such that $\left\| h \right\|_{\underline{H}^1 \left( B_{R^{1+\delta}} , \mu_\beta \right)} \leq 1$, the estimate~\eqref{eq:07489} is equivalent to the identity~\eqref{eq:07499} and the $H^{-1}\left( B_{R^{1+\delta}} , \mu_\beta \right)$-norm estimate~\eqref{eq:07509}. The proof of~\eqref{eq:07499}, and thus of~\eqref{eq:mainsub1.3hom}, is complete. 

\medskip

\textit{Substep 1.4} In this substep, we conclude Step 1 and prove the estimate~\eqref{eq:TV19578}. We use the identity~\eqref{eq:TV09577} and the identities~\eqref{eq:mainsub1.1hom} proved in Substep 1,~\eqref{eq:TV14557} proved in Substep 2 and~\eqref{eq:mainsub1.3hom} proved in Substep 3. We obtain
\begin{align} \label{eq:TV08399}
    \L \mathcal{H} & = \Delta_\phi \G_{\mathrm{hom}, \f }^\delta + \ahom  \Delta \G_{\mathrm{hom}, \f }^\delta \\ & \quad + \sum_{i=1}^d  \nabla_i  \G_{\mathrm{hom}, \f }^\delta \left( \frac{1}{2\beta} \Delta \chi_{m,i} + \sum_{\di q=0}  \nabla_q^* \cdot \a_q \nabla_q \left( l_{e_i} + \chi_{m,i} \right)+   \Delta_{\phi} \chi_{m,i}  +  \sum_{n \geq 1}  \frac{1}{\beta^{\frac n2}} \Delta^{n+1} \chi_{m,i} \right) \notag \\ & \quad + R_{Q} + R_{\Delta_\phi} + R_{\Delta^n}, \notag
\end{align}
We then treat the three lines of the previous display separately. For the first line we note that, by definition of the homogenized function $\G_{\mathrm{hom}, \f}$, we have the identity
\begin{equation} \label{eq:TV09239}
    \Delta_\phi \G_{\mathrm{hom}, \f }^\delta + \ahom  \Delta \G_{\mathrm{hom}, \f }^\delta = \f \rho_\delta.
\end{equation}
For the second line, we use that, by the definition of the finite-volume corrector given in Definition~\ref{def.finivolcorr}, this map is a solution of the Hellfer-Sjostrand equation $\L \left( l_{e_i} + \chi_{m,i} \right) = 0$ in the set $B_{R^{1+\delta}} \times \Omega$. We obtain
\begin{align} \label{eq:TV09249}
    \sum_{i=1}^d  \nabla_i  \G_{\mathrm{hom}, \f }^\delta \left(  \Delta_{\phi} \chi_{m,i}  + \frac{1}{2\beta} \Delta \chi_{m,i} + \sum_{\di q=0}  \nabla_q^* \cdot \a_q \nabla_q \left( l_{e_i} + \chi_{m,i} \right)+    \sum_{n \geq 1}  \frac{1}{\beta^{\frac n2}} \Delta^{n+1} \chi_{m,i} \right) & =  \sum_{i=1}^d  \nabla_i  \G_{\mathrm{hom}, \f }^\delta \L \left( l_{e_i} + \chi_{m,i} \right) \\& = 0. \notag
    \end{align}
For the third line, we use the estimates~\eqref{eq:TVRphi},~\eqref{eq:TV14557} and~\eqref{eq:TV14567} on the error terms $R_{Q}$, $R_{\Delta_\phi}$ and $R_{\Delta^n}$ respectively. We obtain
\begin{equation} \label{eq:TV09259}
    \left\| R_{Q}+R_{\Delta_\phi}+R_{\Delta^n} \right\|_{\underline{H}^{-1}\left(B_{R^{1+\delta}} , \mu_\beta \right)} \leq \frac{C}{R^{d-1+\gamma}}.
\end{equation}
A combination of the identities~\eqref{eq:TV08399},~\eqref{eq:TV09239},~\eqref{eq:TV09249} and~\eqref{eq:TV09259} proves the inequality
\begin{equation*}
    \left\| \mathcal{L} \mathcal{H} - \f \rho_\delta \right\|_{\underline{H}^{-1}\left(B_{R^{1+\delta}} , \mu_\beta \right)} \leq \frac{C}{R^{d-1+\gamma}}.
\end{equation*}
The proof of Step 1 is complete.


\medskip

\textit{Step 2.} The objective of this step is to prove that the Green's function $\G_{\f}^\delta$ and the the two scale expansion $\mathcal{H}$ are close in the $H^1$-norm in the annulus $A_R$. More specifically, we prove that there exists an exponent $\gamma := \gamma(d) > 0$ such that one has the estimate 
\begin{equation} \label{eq:TV10039}
    \left\| \nabla \G_{\f}^\delta - \nabla \mathcal{H}  \right\|_{\underline{L}^2 \left( A_R , \mu_\beta \right)} \leq \frac{C}{R^{(d-1) + \gamma}}.
\end{equation}
To prove this estimate, we work on the larger set $B_{R^{1+\delta}/2}$ and prove the estimate
\begin{align} \label{eq:TV10039}
    \left\| \nabla \G_{\f}^\delta - \nabla \mathcal{H}  \right\|_{\underline{L}^2 \left( B_{R^{1+\delta}/2} , \mu_\beta \right)} \leq  \frac{C}{R^{(1+\delta)(d-1) - \ep}}.
\end{align}
The inequality~\eqref{eq:TV10039} implies~\eqref{eq:TV10039}; indeed by using that the annulus $A_R$ is included in the ball $B_{R^{1+\delta}}$ we can compute
\begin{align*}
    \left\| \nabla \G_{\f}^\delta - \nabla \mathcal{H}  \right\|_{\underline{L}^2 \left( A_R , \mu_\beta \right)} & \leq \left(\frac{\left| A_R \right|}{\left| B_{R^{1+\delta}/2} \right|}\right)^\frac 12 \left\| \nabla \G_{\f}^\delta - \nabla \mathcal{H}  \right\|_{\underline{L}^2 \left( B_{R^{1+\delta}/2} , \mu_\beta \right)} \\ 
    & C \left( \frac{R^d}{R^{d(1+\delta)}}\right)^\frac12 \frac{C}{R^{(1+\delta)(d-1) - \ep}} \\
    & \leq \frac{C}{R^{d-1 + \gamma}},
\end{align*}
where we have set $\gamma := \delta (\frac d2-1) - \ep$; it is strictly positive under the assumptions $d \geq 3$ and $\ep \ll \delta$.
We now focus on the proof of the estimate~\eqref{eq:TV10039}. The strategy is to first use the identity $\mathcal{L} \G_{\f}^\delta = \f \rho_{\delta}$ to rewrite the estimate~\eqref{eq:TV19578} in the following form
\begin{equation} \label{eq:TV10569}
    \left\| \L \left( \G_{\f}^\delta - \mathcal{H} \right)  \right\|_{\underline{H}^{-1} \left( B_{R^{1+\delta}} , \mu_\beta \right)} \leq \frac{C}{R^{d-1+\gamma}}.
\end{equation}
We then appeal to the $H^{-1}$-estimate~\eqref{eq:TV19578} proved in Step 1 and use the function $\G_{\f}^\delta - \mathcal{H}$ as a test function in the definition of the $H^{-1}$-norm to obtain the $H^1$-estimate stated in~\eqref{eq:TV10039}, as described in the outline of the proof at the beginning of Section~\ref{sec:section6}. The overall strategy is relatively straightforward; however, one has to deal with the following technical difficulty. By definition of the $H^{-1}$-estimate~\eqref{eq:TV19578}, one needs to use a function in $H^1_0 \left( B_{R^{1+\delta}} , \mu_\beta \right)$ as a test function; in particular the function must be equal to $0$ outside the ball $B_{R^{1+\delta}}$, this condition is not verified by the $\G_{\f}^\delta - \mathcal{H}$ which is thus not a suitable test function. To overcome this issue, we introduce a cutoff function $\eta$ supported in the ball $B_{R^{1+ \delta}}$ which satisfies the inequalities
\begin{equation} \label{eq:propeta}
    0 \leq \eta \leq \indc_{B_{R^{ 1 + \delta }}}, ~ \eta = 1 ~\mbox{in}~ B_{\frac{R^{ 1 + \delta }}{2}} , ~\mbox{and}~ \forall k \in \N, \, \left| \nabla^k \eta \right|\leq \frac{C}{R^{ (1 + \delta ) k }},
\end{equation}
and use the functions $\eta \left( \G_{\f}^\delta - \mathcal{H} \right)$ as a test function. The main difficulty is thus to treat the cutoff function. Nevertheless this difficulty is similar to the one treated in the proof of the Caccioppoli inequality stated in Proposition~\ref{Caccio.ineq}, where one also has to deal with a cutoff function. We thus omit some of the details of the argument and refer the reader to the proof of Proposition~\ref{Caccio.ineq} for the missing elements of the proof.

We use the function $\eta \left( \G_{\f}^\delta - \mathcal{H} \right)$ as a test function in the inequality~\eqref{eq:TV10569}. We obtain
\begin{align} \label{eq:TV11239}
    \frac{1}{R^{(1+\delta)d}}\sum_{x \in B_{R^{1+\delta}}} \left\langle \eta \left( \G_{\f}^\delta - \mathcal{H}\right) \L \left( \G_{\f}^\delta - \mathcal{H} \right)  \right\rangle_{\mu_\beta} & \leq \left\| \L \left( \G_{\f}^\delta - \mathcal{H} \right) \right\|_{\underline{H}^{-1} \left( B_{R^{1+\delta}} , \mu_\beta \right)} \left\|  \eta \left( \G_\f^\delta - \mathcal{H} \right)  \right\|_{\underline{H}^1 \left( B_{R^{1+\delta}} , \mu_\beta \right)} \\
    & \leq \frac{C}{R^{d-1 + \gamma}} \left\| \eta \left( \G_\f^\delta - \mathcal{H} \right) \right\|_{\underline{H}^1 \left( B_{R^{1+\delta}} , \mu_\beta \right)}. \notag
\end{align}
We then treat the terms in the left and right side of the inequality~\eqref{eq:TV11239} separately. Regarding the left side, we prove the estimate \pdcomment{check also $\partial$ of everything}
\begin{equation} \label{eq:TV15049}
    \left\| \eta \left( \G_\f^\delta - \mathcal{H} \right) \right\|_{\underline{H}^1 \left( B_{R^{1+\delta}} , \mu_\beta \right)} \leq \frac{C}{R^{d-1 - \delta (d-1 - \ep)}}.
\end{equation}
The proof relies on the properties of the cutoff function $\eta$ given in~\eqref{eq:propeta}, the regularity estimate on the Green's function stated in Lemma~\ref{Lem6.4}, the $L^\infty$-bound on the homogenized Green's function $\G_{\mathrm{hom} , \f}^\delta$ stated in~\eqref{eq:spatregbarGgeq3} and the bounds on the corrector and its gradient
\begin{equation*}
    \left\| \chi_{m,i} \right\|_{\underline{L}^2 \left( B_{R^{1+\delta}} , \mu_\beta  \right)} \leq C R^{(1+\delta)(1-\alpha)} ~\mbox{and}~ \left\| \nabla \chi_{m,i} \right\|_{\underline{L}^2 \left( B_{R^{1+\delta}} , \mu_\beta  \right)} \leq C.
\end{equation*}
We first write
\begin{multline} \label{eq:TV11579}
    \left\| \eta \left( \G_\f^\delta - \mathcal{H} \right) \right\|_{\underline{H}^1 \left( B_{R^{1+\delta}} , \mu_\beta \right)} \leq \underbrace{\frac{1}{R^{1+\delta}} \left\| \eta \left( \G_\f^\delta - \mathcal{H} \right) \right\|_{\underline{L}^2 \left( B_{R^{1+\delta}} , \mu_\beta \right)}}_{\eqref{eq:TV11579}-(i)} + \underbrace{ \left\| \nabla \eta \left( \G_\f^\delta - \mathcal{H} \right) \right\|_{\underline{L}^2 \left( B_{R^{1+\delta}} , \mu_\beta \right)} }_{\eqref{eq:TV11579}-(ii)} \\ + \underbrace{ \left\| \eta \left( \nabla \G_\f^\delta - \nabla \mathcal{H} \right) \right\|_{\underline{L}^2 \left( B_{R^{1+\delta}} , \mu_\beta \right)}}_{\eqref{eq:TV11579}-(iii)}+ \underbrace{\sum_{x \in \Zd}  \left\| \eta \left( \partial_x \G_\f^\delta - \partial_x \mathcal{H} \right) \right\|_{\underline{L}^2 \left( B_{R^{1+\delta}} , \mu_\beta \right)}}_{\eqref{eq:TV11579}-(iv)},
\end{multline}
and treats the three terms in the right side separately. For the term~\eqref{eq:TV11579}-(i), we use that the function $\eta$ is non-negative and smaller than $1$ to write
\begin{equation*}
    \frac{1}{R^{1+\delta}} \left\| \eta \left( \G_\f^\delta - \mathcal{H} \right) \right\|_{\underline{L}^2 \left( B_{R^{1+\delta}} , \mu_\beta \right)} \leq \frac{1}{R^{1+\delta}} \left( \left\| \G_\f^\delta  \right\|_{\underline{L}^2 \left( B_{R^{1+\delta}} , \mu_\beta \right)} + \left\| \mathcal{H}  \right\|_{\underline{L}^2 \left( B_{R^{1+\delta}} , \mu_\beta \right)} \right).
\end{equation*}
We then estimate the $L^2$-norm of the Green's function $ \G_\f^\delta$ thanks to the estimate
\begin{equation*}
    \left\| \G_\f^\delta  \right\|_{\underline{L}^2 \left( B_{R^{1+\delta}} , \mu_\beta \right)} \leq \left\| \G_\f^\delta \right\|_{L^\infty \left( \Zd , \mu_\beta \right)} \leq \frac{C}{R^{(1-\delta)(d-2)}}.
\end{equation*}
The $L^2$-norm of the two-scale expansion $\mathcal{H}$ can be estimated according to the following computation
\begin{align*}
     \left\| \mathcal{H}  \right\|_{\underline{L}^2 \left( B_{R^{1+\delta}} , \mu_\beta \right)} & \leq  \left\| \G_{\mathrm{hom}, \f}  \right\|_{\underline{L}^2 \left( B_{R^{1+\delta}} , \mu_\beta \right)} + \sum_{i=1}^d \left\| \nabla_i \G_{\mathrm{hom}, \f}  \right\|_{L^\infty \left( B_{R^{1+\delta}} , \mu_\beta \right)} \left\| \chi_{m,i} \right\|_{\underline{L}^2 \left( B_{R^{1+\delta}} , \mu_\beta \right)} \\
     & \leq \frac{C}{R^{(1-\delta)(d-2)}} + \frac{C^{1-\alpha}}{R^{(1-\delta)(d-1)}} \\
     & \leq \frac{C}{R^{(1-\delta)(d-2)}}.
\end{align*}
A combination of the three previous displays show the inequality
\begin{equation} \label{eq:TV15019}
    \frac{1}{R^{1+\delta}} \left\| \eta \left( \G_\f^\delta - \mathcal{H} \right) \right\|_{\underline{L}^2 \left( B_{R^{1+\delta}} , \mu_\beta \right)} \leq \frac{C}{R^{1+\delta} \times R^{(1-\delta)(d-2)}} \leq \frac{C}{ R^{d-1 + \delta (d-1)}}
\end{equation}
The proof of the term~\eqref{eq:TV11579}-(ii) is identical, we first use that, by the assumption made on the function $\eta$ in~\eqref{eq:propeta}, we have $\left| \nabla \eta \right| \leq \frac{C}{R^{1+\delta}}$ and apply the estimate obtained for the term~\eqref{eq:TV11579}-(ii). We obtain
\begin{equation} \label{eq:TV15029}
     \left\| \nabla \eta \left( \G_\f^\delta - \mathcal{H} \right) \right\|_{\underline{L}^2 \left( B_{R^{1+\delta}} , \mu_\beta \right)} \leq \frac{C}{ R^{d-1 + \delta (d-1)}}.
\end{equation}
For the term~\eqref{eq:TV11579}-(iii), we first write
\begin{equation*}
     \left\| \eta \left( \nabla \G_\f^\delta - \nabla \mathcal{H} \right) \right\|_{\underline{L}^2 \left( B_{R^{1+\delta}} , \mu_\beta \right)} \leq \left\| \nabla \G_\f^\delta  \right\|_{L^\infty \left(\Zd , \mu_\beta \right)} + \left\| \nabla \mathcal{H}  \right\|_{\underline{L}^2 \left( B_{R^{1+\delta}} , \mu_\beta \right)}.
\end{equation*}
The $L^\infty$-norm of the Green's function $\nabla \G_\f^\delta $ is estimated by Lemma~\ref{Lem6.4}. We have
\begin{equation*}
    \left\| \nabla \G_\f^\delta  \right\|_{L^\infty \left(\Zd , \mu_\beta \right)} \leq \frac{C}{R^{(1-\delta)(d-1-\ep)}}.
\end{equation*}
For the $L^2$-norm of the two-scale expansion $\mathcal{H}$, we use the formula~\eqref{eq:formnablaH2sc} and write
\begin{align*}
    \left\| \nabla \mathcal{H}  \right\|_{\underline{L}^2 \left( B_{R^{1+\delta}} , \mu_\beta \right)} & \leq  \left\| \nabla  \G_{\mathrm{hom}, \f }^\delta \right\|_{L^\infty \left( \Zd , \mu_\beta \right)}  + \sum_{i=1}^d \left\| \nabla \nabla_i  \G_{\mathrm{hom}, \f }^\delta \right\|_{L^\infty \left( \Zd , \mu_\beta \right)} \left\| \chi_{m,i} \right\|_{\underline{L}^2 \left( B_{R^{1+\delta}} , \mu_\beta  \right)} \\ & \quad + \sum_{i=1}^d \left\| \nabla_i  \G_{\mathrm{hom}, \f }^\delta \right\|_{L^\infty \left( \Zd , \mu_\beta \right)}  \left\| \nabla \chi_{m,i} \right\|_{\underline{L}^2 \left( B_{R^{1+\delta}} , \mu_\beta  \right)} \\
    & \leq \frac{C}{R^{(1-\delta)(d-1-\ep)}} + \frac{CR^{(1+\delta)(1-\alpha)}}{R^{(1-\delta)(d-\ep)}} + \frac{C}{R^{(1-\delta)(d-1-\ep)}} \\
    & \leq \frac{C}{R^{d-1 + \delta (d-1-\ep)}}.
\end{align*}
A combination of the three previous displays gives the inequality
\begin{equation} \label{eq:TV15039}
    \left\| \eta \left( \nabla \G_\f^\delta - \nabla \mathcal{H} \right) \right\|_{\underline{L}^2 \left( B_{R^{1+\delta}} , \mu_\beta \right)}  \leq \frac{C}{R^{d-1- \delta(d-1-\ep)}}.
\end{equation}
The inequality~\eqref{eq:TV15049} is then obtained by combining the estimates~\eqref{eq:TV15019}, \eqref{eq:TV15029} and~\eqref{eq:TV15039}. We then put the inequality back into the inequality~\eqref{eq:TV11239} and deduce that
\begin{equation} \label{eq:TV06520}
     \frac{1}{R^{(1+\delta)d}}\sum_{x \in B_{R^{1+\delta}}} \left\langle \eta \left( \G_{\f}^\delta - \mathcal{H}\right) \L \left( \G_{\f}^\delta - \mathcal{H} \right)  \right\rangle_{\mu_\beta} \leq \frac{C}{R^{d-1 + \gamma} \times R^{d-1 - \delta (d-1 - \ep)}} \leq  \frac{C}{R^{2d-2 + \gamma}},
\end{equation}
where we have reduced the value of the exponent $\gamma$ in the second inequality (by subtracting the value $\delta (d-1 - \ep)$ to it); this operation is justified by the fact that \pd{blabla}.

In the rest of this step, we treat the left side of~\eqref{eq:TV06520} and prove the inequality
\begin{equation} \label{eq:TV11321}
     \left\| \nabla \G_{\f}^\delta - \nabla \mathcal{H} \right\|_{\underline{L}^2 \left( B_{\frac{R^{1+\delta}}{2}} , \mu_\beta \right)} \leq \frac{1}{R^{(1+\delta)d}}\sum_{x \in B_{R^{1+\delta}}} \left\langle \eta \left( \G_{\f}^\delta - \mathcal{H}\right) \L \left( \G_{\f}^\delta - \mathcal{H} \right)  \right\rangle_{\mu_\beta} + \frac{C}{R^{(1+\delta)(2d-2 - \ep) }} .
\end{equation}
First, by definition of the Hellfer-Sjostrand operator $\mathcal{L}$, we have the identity
\begin{align} \label{eq:TV08101}
\sum_{x \in \Zd} \left\langle \eta \left( \G_{\f}^\delta - \mathcal{H}\right) \L \left( \G_{\f}^\delta - \mathcal{H} \right)  \right\rangle_{\mu_\beta} & = \sum_{x , y \in \Zd} \eta(x) \left\langle \left( \partial_y \G_{\f}^\delta (x , \cdot)  - \partial_y \mathcal{H} (x , \cdot) \right)^2 \right\rangle_{\mu_\beta} \\ & + \frac 1{2\beta}\sum_{x \in \Zd}  \left\langle  \left( \nabla \G_{\f}^\delta  - \nabla \mathcal{H}\right)(x , \cdot) \cdot \nabla \left( \eta \left( \G_{\f}^\delta-  \mathcal{H} \right)\right)(x , \cdot)  \right\rangle_{\mu_\beta} \notag \\ & +  \sum_{q}  \left\langle \nabla_q \left(  \G_{\f}^\delta -  \mathcal{H}\right) \cdot \a_q \nabla_q \left( \eta \left(  \G_{\f}^\delta  - \mathcal{H} \right) \right) \right\rangle_{\mu_\beta} \notag \\ & +  \frac 1{2\beta} \sum_{n \geq 1} \sum_{x \in \Zd}  \frac{1}{\beta^{ \frac n2}} \left\langle  \nabla^{n+1} \left(  \G_{\f}^\delta  -  \mathcal{H} \right)(x , \cdot) \cdot \nabla^{n+1} \left( \eta \left(  \G_{\f}^\delta  -  \mathcal{H} \right) \right)(x,\cdot) \right\rangle_{\mu_\beta}. \notag
\end{align}
We then estimate the various terms on the right side separately. For the first, we use that it is non-negative
\begin{equation*}
    \sum_{x , y \in \Zd} \eta(x)^2 \left\langle \left( \partial_y \G_{\f}^\delta (x , \cdot)  - \partial_y \mathcal{H} (x , \cdot) \right)^2 \right\rangle_{\mu_\beta}  \geq 0.
\end{equation*}
For the second one, we expand the gradient of the product $\eta^2 \left( \G_{\f}^\delta  - \mathcal{H} \right)$ and write
\begin{align} \label{eq:TV09490}
    \lefteqn{\sum_{x \in \Zd}  \left\langle  \left( \nabla \G_{\f}^\delta  - \nabla \mathcal{H}\right)(x , \cdot) \cdot \nabla \left( \eta \left( \G_{\f}^\delta-  \mathcal{H} \right)\right)(x , \cdot)  \right\rangle_{\mu_\beta}} \qquad & \\ &
    = \sum_{x \in \Zd}  \eta(x)  \left\langle  \left( \nabla \G_{\f}^\delta  - \nabla \mathcal{H}\right)(x , \cdot) \cdot   \nabla \left( \G_{\f}^\delta-  \mathcal{H} \right)(x , \cdot)  \right\rangle_{\mu_\beta} \notag \\
    & \quad + \sum_{x \in \Zd}  \left\langle  \left( \nabla \G_{\f}^\delta  - \nabla \mathcal{H}\right)(x , \cdot) \cdot  \nabla \eta(x)\left( \G_{\f}^\delta-  \mathcal{H} \right)(x , \cdot)  \right\rangle_{\mu_\beta}. \notag
\end{align}
Dividing the identity~\eqref{eq:TV09490} by the volume factor $R^{(1+\delta)d}$ and using the properties of the function $\eta$ stated in~\eqref{eq:propeta} and in particular, we use that the gradient of $\eta$ is supported in the annulus $A_{R^{1+\delta}} := B_{R^{1+\delta}} \setminus B_{\frac{R^{1+\delta}}{2}}$. We obtain
\begin{multline} \label{eq:TV07591}
    \sum_{x \in \Zd}  \left\langle  \left( \nabla \G_{\f}^\delta  - \nabla \mathcal{H}\right)(x , \cdot) \cdot \nabla \left( \eta \left( \G_{\f}^\delta-  \mathcal{H} \right)\right)(x , \cdot)  \right\rangle_{\mu_\beta} \geq c \left\| \eta \left( \nabla \G_{\f}^\delta  - \nabla \mathcal{H} \right) \right\|_{L^2 \left( \Zd , \mu_\beta \right)}^2 \\ -  \frac{C}{R^{1+\delta}} \left\| \nabla \G_{\f}^\delta  \ - \nabla \mathcal{H} \right\|_{L^2 \left( A_{R^{1+\delta}} , \mu_\beta \right)} \left\|  \G_{\f}^\delta  - \mathcal{H} \right\|_{L^2 \left( A_{R^{1+\delta}} , \mu_\beta \right)}.
\end{multline}
By a computation similar to the one performed for the term ~\eqref{eq:TV11579}-(iii), but using the estimates REF for the Green's function in the distant annulus $A_R$, instead of the $L^\infty$-estimates REF. We obtain
\begin{equation} \label{eq:TV07601}
    \left\| \nabla \G_{\f}^\delta  \ - \nabla \mathcal{H} \right\|_{L^2 \left( A_{R^{1+\delta}} , \mu_\beta \right)} \leq CR^{(1+\delta)(1+\ep)}~\mbox{and}~\left\|  \G_{\f}^\delta  - \mathcal{H} \right\|_{L^2 \left( A_{R^{1+\delta}}, \mu_\beta \right)} \leq CR^{2(1+\delta)}.
\end{equation}
A combination of the inequalities~\eqref{eq:TV07591} and~\eqref{eq:TV07601} proves the estimate
\begin{equation} \label{eq:TV11111}
    \frac{1}{2\beta}\sum_{x \in \Zd}  \left\langle  \left( \nabla \G_{\f}^\delta  - \nabla \mathcal{H}\right)(x , \cdot) \cdot \nabla \left( \eta \left( \G_{\f}^\delta-  \mathcal{H} \right)\right)(x , \cdot)  \right\rangle_{\mu_\beta} + \frac{C}{R^{(1+\delta)(2d-2 - \ep)}} \geq \frac{c}{\beta} \left\| \eta \left( \nabla \G_{\f}^\delta  - \nabla \mathcal{H} \right) \right\|_{L^2 \left( \Zd , \mu_\beta \right)}^2
\end{equation}
The other terms in the right side of the identity~\eqref{eq:TV08101} involving the sum over the iteration of the Laplacian and over the charges $q \in \mathcal{Q}$ are treated similarly. Instead of expanding the gradient as it was done in~\eqref{eq:TV09490}, we use the commutation estimates (see~\eqref{eq:Caccio1925} and~\eqref{eq:TV1549C}), for each integer $n \in \N$, and each pair $(x , \phi) \in \Zd \times \Omega$,
\begin{equation}
\left| \nabla^n \left( \eta \left ( \G_{\f}^\delta  - \mathcal{H} \right) \right) (x , \phi)  -  \eta(x) \nabla^n\left ( \G_{\f}^\delta  - \mathcal{H} \right)(x , \phi)  \right| \leq \frac{C^n}{R^{1+\delta}} \sum_{z \in B(x,n)} | \G_{\f}^\delta ( z, \phi)  - \mathcal{H}( z, \phi)|.
\end{equation}
and for each charge $q \in \mathcal{Q}$, each point $x$ in the support of the charge $q$ and each field $\phi \in \Omega$,
\begin{equation*}
\left| \nabla_q \left( \eta \left ( \G_{\f}^\delta  - \mathcal{H} \right) \right) - \eta(x) \nabla_q  \left( \G_{\f}^\delta  - \mathcal{H} \right) \right| \leq \frac{C}{R^{1+\delta}} \left(\diam q \right) \left\|q \right\|_{1} \sum_{z \in \supp q} | \G_{\f}^\delta  - \mathcal{H}|.
\end{equation*}
The details of the argument are similar to the one presented in the proof of the Caccioppoli inequality (Proposition~\ref{Caccio.ineq}) and are omitted. The result we obtain is stated below
\begin{equation} \label{eq:TV11121}
    \sum_{q}  \left\langle \nabla_q \left(  \G_{\f}^\delta -  \mathcal{H}\right) \cdot \a_q \nabla_q \left( \eta \left(  \G_{\f}^\delta  - \mathcal{H} \right) \right) \right\rangle_{\mu_\beta}  + \frac{C}{R^{(1+\delta)(2d-2 - \ep) }} \geq -C e^{-c \sqrt{\beta}} \left\| \eta \left( \nabla \G_{\f}^\delta  - \nabla \mathcal{H} \right) \right\|_{L^2 \left( \Zd , \mu_\beta \right)}^2
\end{equation}
and
\begin{align} \label{eq:TV11131}
    \lefteqn{\frac 1{2\beta} \sum_{n \geq 1} \sum_{x \in \Zd}  \frac{1}{\beta^{ \frac n2}} \left\langle  \nabla^{n+1} \left(  \G_{\f}^\delta  -  \mathcal{H} \right)(x , \cdot) \cdot \nabla^{n+1} \left( \eta \left(  \G_{\f}^\delta  -  \mathcal{H} \right) \right)(x,\cdot) \right\rangle_{\mu_\beta} + \frac{C}{R^{(1+\delta)(2d-2 - \ep) }} }  \qquad \qquad\qquad\qquad \qquad\qquad\qquad & \\ & \geq  \frac 1{2\beta} \sum_{n \geq 1} \sum_{x \in \Zd}  \frac{1}{\beta^{ \frac n2}} \left\langle \eta(x) \left| \nabla^{n+1} \left(  \G_{\f}^\delta  -  \mathcal{H} \right)(x , \cdot) \right|^2 \right\rangle_{\mu_{\beta}} \notag \\
    & \geq 0. \notag
\end{align}
We then combine the identity~\eqref{eq:TV08101} with the estimates~\eqref{eq:TV11121},~\eqref{eq:TV11121} and~\eqref{eq:TV11121} and assume that the inverse temperature $\beta$ is large enough. We obtain
\begin{align*}
    \sum_{x \in \Zd} \left\langle \eta \left( \G_{\f}^\delta - \mathcal{H}\right) \L \left( \G_{\f}^\delta - \mathcal{H} \right)  \right\rangle_{\mu_\beta} +  \frac{C}{R^{(1+\delta)(2d-2 - \ep) }} & \geq \frac{c}{\beta} \left\| \eta \left( \nabla \G_{\f}^\delta  - \nabla \mathcal{H} \right) \right\|_{L^2 \left( \Zd , \mu_\beta \right)}^2 \\ & \geq \frac{c}{\beta} \left\|  \nabla \G_{\f}^\delta  - \nabla \mathcal{H}  \right\|_{L^2 \left( B_{\frac{R^{1+\delta}}{2}}, \mu_\beta \right)}^2. \notag
\end{align*}
The proof of the inequality~\eqref{eq:TV11321} is then complete. To complete the proof of Step 2, we combine the estimates~\eqref{eq:TV11321} and~\eqref{eq:TV06520}. We obtain
\begin{equation} \label{eq:TV06520}
     \left\| \nabla \G_{\f}^\delta - \nabla \mathcal{H} \right\|_{L^2 \left( B_{\frac{R^{1+\delta}}{2}} , \mu_\beta \right)}^2 \leq \frac{C}{R^{2d-2 + \gamma}} + \frac{C}{R^{(1+\delta)(2d-2 - \ep) }} \leq \frac{C}{R^{(1+\delta)(d-1) - \ep}},
\end{equation}
where the last inequality is a consequence of the ordering $\alpha \gg \delta \gg \ep$. The proof of the estimate~\eqref{eq:TV10039}, and thus of Step 2, is complete.

\medskip

\textit{Step 3.} In this step, we post-process the conclusion~\eqref{eq:TV21003} and prove that the gradient of the two-scale expansion $\nabla \mathcal{H}$. The objective is to prove that there exists an exponent $\gamma := \gamma(d) > 0$ such that one has the estimate
\begin{equation} \label{eq:TV14282}
    \left\| \nabla \G_\f - \sum_{i=1}^d \left( e_i + \nabla \chi_{i} \right) \nabla_i \G_{\mathrm{hom} , \f} \right\|_{\underline{L}^2 \left( A_R , \mu_\beta \right)}  \leq \frac{C}{R^{d-1 + \gamma}}.
\end{equation}
First, we note that the Green's function $\G_\f$ and $\G_{\mathrm{hom} , \f}$ present in the inequality~\eqref{eq:TV14282} are different from the averaged Green's functions $\G_\f^\delta$, and $\G_{\mathrm{hom}, \f}^\delta$ studied in the previous steps. We thus first use the regularity estimates stated in Lemma~\ref{prop:prop6.2} and the $L^2$-bound on the gradient of the corrector, for each integer $i \in \{ 1 , \ldots , d \}$ $\left\| \nabla \chi_i \right\|_{L^2 \left( \mu_\beta \right)}$. We write
\begin{align} \label{eq:TV14272}
    \lefteqn{\left\| \nabla \left( \G_\f - \G_\f^\delta \right) - \sum_{i=1}^d \left( e_i + \nabla \chi_{i} \right) \nabla_i \left( \G_{\mathrm{hom} , \f} - \G_{\mathrm{hom} , \f} \right) \right\|_{\underline{L}^2 \left( A_R , \mu_\beta \right)}} \qquad & \\ & \leq \left\| \nabla \left( \G_\f - \G_\f^\delta \right) \right\|_{\underline{L}^2 \left( A_R , \mu_\beta \right)} + \sum_{i=1}^d \left\| \left( e_i + \nabla \chi_{i} \right) \right\|_{\underline{L}^2 \left( A_R , \mu_\beta \right)} \left\| \nabla_i \left( \G_{\mathrm{hom} , \f} - \G_{\mathrm{hom} , \f} \right) \right\|_{L^\infty \left( A_R , \mu_\beta \right)}  \notag \\
    & \leq \frac{C}{R^{d-1+\gamma}}. \notag
\end{align}
Using the inequality~\eqref{eq:TV14272}, we see that to prove~\eqref{eq:TV14282} it is sufficient to prove the estimate 
\begin{equation} \label{eq:TV15172}
 \left\| \nabla \G_\f^\delta - \sum_{i=1}^d \left( e_i + \nabla \chi_{i} \right) \nabla_i \G_{\mathrm{hom} , \f}^\delta \right\|_{\underline{L}^2 \left( A_R , \mu_\beta \right)}  \leq \frac{C}{R^{d-1 + \gamma}}.
 \end{equation}
We then use the main estimate~\eqref{eq:TV10039} and deduce that, to prove the inequality~\eqref{eq:TV15172}, it is sufficient to prove
\begin{equation} \label{eq:TV15182}
    \left\| \nabla \mathcal{H} - \sum_{i=1}^d \left( e_i + \nabla \chi_{i} \right) \nabla_i \G_{\mathrm{hom} , \f}^\delta \right\|_{\underline{L}^2 \left( A_R , \mu_\beta \right)} \leq \frac{C}{R^{d-1 + \gamma}}.
\end{equation}
The rest of the argument of this step is devoted to the proof of~\eqref{eq:TV15182}. We first use the explicit formula for the gradient of the two-scale expansion $\nabla \mathcal{H}$ stated in~\eqref{eq:formnablaH2sc} and write 
\begin{align*}
\left\| \nabla \mathcal{H} - \sum_{i=1}^d \left( e_i + \nabla \chi_{m,i} \right) \nabla_i \G_{\mathrm{hom} , \f}^\delta \right\|_{\underline{L}^2 \left( A_R , \mu_\beta \right)} \leq \sum_{i=1}^d \left\|  \nabla \nabla_i  \G_{\mathrm{hom}, \f }^\delta  \chi_{m,i} \right\|_{\underline{L}^2 \left( A_R , \mu_\beta \right)}+ \left\| \nabla_i  \G_{\mathrm{hom}, \f }^\delta  \left( \nabla \chi_{m,i} - \nabla \chi_i \right) \right\|_{\underline{L}^2 \left(A_R , \mu_\beta \right)}.
\end{align*}
We then use the regularity estimate~\eqref{eq:spatregbarGgeq3}, the quantitative sublinearity of the corrector stated in Proposition~\ref{prop:prop5.25} and Proposition~\ref{prop5.26} to quantify the $L^2$-norm of the difference between the gradient of finite-volume corrector and the gradient of the infinite-volume corrector. We obtain
\begin{align} \label{eq:TV13422}
    \left\| \nabla \mathcal{H} - \sum_{i=1}^d \left( e_i + \nabla \chi_{m,i} \right) \nabla_i \G_{\mathrm{hom} , \f}^\delta \right\|_{\underline{L}^2 \left( A_R , \mu_\beta \right)} & \leq \left( \frac{\left| A_R \right|}{\left| B_{R^{1+\delta}} \right|} \right)^\frac 12 \frac{C R^{1-\alpha}}{R^{d - \ep}} + \left( \frac{\left| A_R \right|}{\left| B_{R^{1+\delta}} \right|} \right)^\frac 12 \frac{C R^{-\alpha}}{R^{d - 1 - \ep}} \\
    & \leq \frac{C}{R^{d-1 + \gamma}}, \notag
\end{align}
where we have set $\gamma := \alpha - \ep - \frac{\delta}{2}$; under the assumption~\eqref{eq:TVexpord}, it is strictly positive. The proof of the estimate~\eqref{eq:TV13422} is complete.
\end{proof}



\begin{proposition}
For each $R > 0$, we let $w_R$ be the solution of the equation
\begin{equation*}
    \L^\beta w_R := \nabla^* F_R,
\end{equation*}
where the function is defined by the formula
\begin{equation*}
    F_R (x , \phi) := \cos \left( \nabla \phi(x) \right) \indc_{\{ x \in A_R\}}.
\end{equation*}
We also let $\bar w_R$ be the homogenized solution of the equation
\begin{equation*}
    \ahom \Delta \bar w_R = \left\langle \cos \left( \nabla \phi(0) \right) (1 + \nabla \chi(0)) \right\rangle_{\mu_\beta} \indc_{A_R},
\end{equation*}
then we have the estimate
\begin{equation*}
    \left\| w_R(0) - \bar w_R(0)\right\|_{L^2 \left( \mu_\beta \right)} \leq \frac{C}{R^{d - 1 - \alpha}}.
\end{equation*}
\end{proposition}

\begin{remark}
With a notational modification of the proof, we obtain the following more general result, for each $x \in B_{\frac R2}$,
\begin{equation*}
     \left\| w_R(x) - \bar w_R(x)\right\|_{L^2 \left( \mu_\beta \right)} \leq \frac{C}{R^{d - 1 - \alpha}}
\end{equation*}
\end{remark}

In this section, we fix a point $z \in A_R$ and let $H_z$ be the solution of the equation
\begin{equation*}
    \L^\beta H = \sin\left( \nabla \phi(z) \right) \delta_z.
\end{equation*}
We first prove that the function $\mathbf{f}(\phi) := \nabla H(0 , \phi)$ satisfies the assumption of Theorem REF. We first compute the derivative of $H(0 , \phi)$ with respect to the field. Using the derived Helffer-Sjostrand equation: the map $v(x, y , \phi) = \partial_y H(x , \phi)$ is solution of the equation
\begin{multline*}
    \Delta_\phi v (x , y , \phi) + \mathcal{L}_{\mathrm{spat}, x } v (x , y , \phi) + \mathcal{L}_{\mathrm{spat}, y} v (x , y , \phi)  = - \sum_{\di q=0}  z \left( \beta , q\right) \cos \left( \phi , q \right) \left( H, q \right) q(x) q(y) \\ + \sin\left( \nabla \phi(z) \right)  \nabla_{y} \cdot \delta_{(x,y) = (z,z)} .
\end{multline*}
We then write
\begin{equation*}
     v (x , y , \phi) := v_1 (x,y,\phi) + v_2 (x , y , \phi),
\end{equation*}
with
\begin{equation*}
    v_1 (x,y,\phi) = \int_{\Omega} \nabla \mathcal{G}_{\mathrm{der}} (x , y , \phi ; z,z,\psi) \sin(\nabla \psi(z)) \mu_\beta (d \psi)
\end{equation*}
and
\begin{equation*}
    v_2 (x , y , \phi) =  \int_{\Omega} \sum_{x_1,y_1} \sum_{\di q = 0} z(\beta , q) \cos (\psi , q) (H , q) q(x_1) q(y_1) \mathcal{G}_{\mathrm{der}} (x , y , \phi ; x_1,y_1,\psi)  \mu_\beta (d \psi).
\end{equation*}
The first term is estimated thanks to the regularity estimate REF, and we have
\begin{equation*}
   \left|  v_1 (x,y,\phi) \right| \leq  \frac{C}{|(x,y)- (z , z)|^{2d-1}} \leq  \frac{C}{|x - z |^{2d-1} + |y - z|^{2d-1}}.
\end{equation*}
The second term can be estimated by REF and we have
\begin{equation*}
    \left| v_2 (x , y , \phi) \right| \leq C \sum_{h} \frac{1}{|h - z|^{d-1 - \ep}} \times \frac{1}{|(x,y) - (h,h)|^{2d - \ep}} \leq C \sum_{h} \frac{1}{|h - z|^{d-1 - \ep}} \times \frac{1}{|x - h|^{2d - \ep} + |y - h|^{2d - \ep}} .
\end{equation*}
We then consider the value $x = 0$. This gives
\begin{equation*}
    \left| \partial_y H\left( 0 , \phi \right) \right| \leq \frac{C}{R^{2d - 1 - \ep} + |y - z|^{2d - 1 - \ep}} + C \sum_{h} \frac{1}{|h - z|^{d-1 - \ep}} \times  \frac{1}{| h|^{2d - \ep} + |y - h|^{2d - \ep}}.
\end{equation*}
The second term on the right side of the previous inequality can be estimated by the following argument. We first note that we have the identity
\begin{equation*}
    \frac{1}{| h|^{2d - \ep} + |y - h|^{2d - \ep}} \leq \frac{C}{\left( |h| \vee |y|\right)^{2d-\ep}}.
\end{equation*}
The sum ban thus be rewritten and estimated
\begin{align*}
    \sum_{h} \frac{1}{|h - z|^{d-1 - \ep}} \times  \frac{1}{| h|^{2d - \ep} + |y - h|^{2d - \ep}} & \leq C \sum_{h} \frac{1}{|h - z|^{d-1 - \ep}} \times  \frac{1}{\left( |h| \vee |y|\right)^{2d-\ep}} \\
                        & \leq  C \sum_{|h| \leq |y|}  \frac{1}{|h - z|^{d-1 - \ep}} \times  \frac{1}{|y|^{2d-\ep}} +  \sum_{|h| \geq |y|}  \frac{1}{|h - z|^{d-1 - \ep}} \times  \frac{1}{|h|^{2d-\ep}}
\end{align*}
which gives the estimate \pdcomment{add a gradient in the computation and I think the $R \vee |y|$ is false}
\begin{align*}
    \left| \partial_y \nabla H\left( 0 , \phi \right) \right| & \leq  C \frac{1}{R^{d-1- \ep}} \times \frac{1}{\left( R \vee |y| \right)^{d+1-\ep}}
\end{align*}

We now verify that if we define the function $\bar G_\delta$ according to the formula
\begin{equation*}
    \Delta_\phi \bar G_\delta + \Delta \bar G_\delta = \nabla H \left( 0 , \phi \right) \rho_\delta,
\end{equation*}
we want to prove that for any $x \in F$, one has the estimate
\begin{equation*}
    \left( \sum_{y \in F} \left| \partial_y \nabla \bar G_\delta (x , \phi)  \right|^2 \right)^{\frac{1}{2}} \leq C R^{-2d-1}.
\end{equation*}
We use the derived Helffer-Sjostrand equation; if we denote by $g(x , y , \phi) := \partial_y \nabla \bar G_\delta(x , \phi) $, we have
\begin{equation*}
 \Delta_\phi g(x , y , \phi) + \Delta_x g(x , y , \phi) + \mathcal{L}_{\mathrm{spat} , y} g(x , y , \phi) = \frac{1}{R^{1-\delta}}\partial_y \nabla H \left( 0 , \phi \right) \nabla \rho_\delta(x).
\end{equation*}
The objective is then to prove the estimate, for each $x \in F$,
\begin{equation*}
    \left( \sum_{y \in F} \left| g(x , y , \phi) \right|^2 \right)^{\frac12} \leq C R^{-2d - 1}
    \end{equation*}
This function $g$ can then be written in terms of the elliptic Green's matrix $ \mathcal{G}_{\mathrm{der}}$ associated to the operator $\Delta_\phi + \Delta_x  + \mathcal{L}_{\mathrm{spat} , y}$ and we have
\begin{equation*}
     g(x , y , \phi)  = \frac{1}{R^{1-\delta}} \int_{\Omega} \sum_{x_1 , y_1}  \mathcal{G}_{\mathrm{der}} \left(x , y , \phi ; x_1 , y_1 , \psi \right) \partial_{y_1} \nabla H \left( 0 , \phi \right) \nabla \rho_\delta(x_1) d \mu_\beta \left( \psi\right).
\end{equation*}
By using the estimates REF and REF, we obtain
\begin{equation*}
    \left| g(x , y , \phi) \right| \leq \frac{C}{R^{d-\delta - \ep}} \sum_{x_1 , y_1} \frac{1}{|x - x_1|^{2d-2} + |y - y_1|^{2d-2}} \times \frac{1}{\left( R \vee |y_1| \right)^{d+1-\ep}} \left| \nabla \rho_\delta(x_1) \right|
\end{equation*}
We then use that the function $ \nabla \rho_\delta$ is supported in the ball $B_{R^{1+\delta}}$ to obtain the estimate $\left|  \nabla \rho_\delta \right| \leq \frac{C}{R^{d(1-\delta)}} \indc_{B_{R^{1+\delta}}}$. This shows
\begin{equation*}
     \left| g(x , y , \phi) \right| \leq \frac{C}{R^{d-\delta - \ep}} \times \frac{1}{R^{d(1-\delta})} \sum_{x_1 , y_1} \frac{1}{|x - x_1|^{2d-2} + |y - y_1|^{2d-2}} \times \frac{1}{\left( R \vee |y_1| \right)^{d+1-\ep}} \indc_{B_{R^{1-\delta}}}(x_1).
\end{equation*}
By Youngs inequality with parameters $\frac{2d}{d-2}$ and $q = \frac{2d}{d+2}$. We have the estimate
\begin{align*}
    \left( \sum_{x,y}  \left| g(x , y , \phi) \right|^2 \right)^\frac 12 & \leq \frac{C}{R^{d-\delta - \ep}} \times \frac{1}{R^{d(1-\delta})} \left( \sum_{x,y} \frac{1}{|(x,y)|^{p(2d-2)} } \right)^{\frac1p} \left( \sum_{x,y} \frac{1}{\left( R \vee |y| \right)^{q(d+1-\ep)}} \indc_{B_{R^{1-\delta}}}(x) \right)^{\frac1p} \\
    & \leq \frac{C}{R^{d-\delta - \ep}} \times \frac{1}{R^{d(1-\delta})}  \left( \sum_{x,y} \frac{1}{\left( R \vee |y| \right)^{q(d+1-\ep)}} \indc_{B_{R^{1-\delta}}}(x) \right)^{\frac1q}.
\end{align*}
We then estimate the term on the right side
\begin{align*}
\sum_{x,y} \frac{1}{\left( R \vee |y| \right)^{q(d+1-\ep)}} \indc_{B_{R^{1-\delta}}}(x) & = \left( \sum_{y} \frac{1}{\left( R \vee |y| \right)^{q(d+1-\ep)}}\right) \left( \sum_x \indc_{B_{R^{1-\delta}}}(x) \right) \\
                    & = \left( \sum_{y} \frac{1}{\left( R \vee |y| \right)^{q(d+1-\ep)}}\right)  R^{d(1-\delta)} \\
                    & \leq R^{-q(d+1-\ep) - d} R^{d(1-\delta)}.
\end{align*}
Using the explicit value $q = \frac{2d}{d+2}$, we obtain
\begin{align*}
     \left( \sum_{x,y} \frac{1}{\left( R \vee |y| \right)^{q(d+1-\ep)}} \indc_{B_{R^{1-\delta}}}(x) \right)^{\frac1q} \leq R^{-(d+1-\ep) + \frac{(d+2)}{2}} R^{\frac{(1-\delta)(d+2)}{2}} \leq R^{1+ \ep}.
\end{align*}
This implies the result.


\begin{proposition}[Homogenization of mixed derivative] \label{prop:homhogmixedder}
For each $R > 0$, we let $w_R$ be the solution of the equation
\begin{equation*}
    \L^\beta w_R := \nabla^* F_R,
\end{equation*}
where the function is defined by the formula
\begin{equation*}
    F_R (x , \phi) := \cos \left( \nabla \phi(x) \right) \indc_{\{ x \in A_R\}}.
\end{equation*}
We also let $\bar w_R$ be the homogenized solution of the equation
\begin{equation*}
    \ahom \Delta \bar w_R = \left\langle \cos \left( \nabla \phi(0) \right) (1 + \nabla \chi(0)) \right\rangle_{\mu_\beta} \indc_{A_R},
\end{equation*}
then we have the estimate
\begin{equation*}
    \left\| \nabla w_R(0) - \left( I_d + \nabla \chi(0) \right) \nabla \bar w_R(0)\right\|_{L^2 \left( \mu_\beta \right)} \leq \frac{C}{R^{d - \alpha}}.
\end{equation*}
\end{proposition}


\textit{Step 1.} Since the function $\bar w_R$ is a solution of the equation REF, we have, by the standard results of the regularity theory for harmonic functions: for each integer $k \in \N$ and each $x \in B_{R/2}$,
\begin{equation*}
    \left| \nabla^k \bar w_R \right| \leq \frac{C}{R^{d - 2 + k}}.
\end{equation*}
We then define the two-scale expansion
    \begin{equation*}
    w^0_R := \bar w_R + \sum_{i = 1}^d \left( \nabla_i   \bar w_R\right) \chi_{m , i}
    \end{equation*}
The strategy is similar to the one of Proposition REF and even simpler since the map $w_R$ does not depend on the $\phi$-variable. We first prove the following estimate 
\begin{equation*}
    \left\| \mathcal{L}^\beta w^0_R \right\|_{\underline H^{-1} \left( B_R, \mu_\beta \right)} \leq small.
\end{equation*}
We first compute the Laplacian with respect to the $\phi$ variable $\Delta_\phi$ of the two scale expansion $w^0_R$. Since the map $\bar w_R$ is deterministic, we have
\begin{equation} \label{eq:w0RDeltaphi}
    \Delta_\phi w^0_R =  \sum_{i = 1}^d \left( \nabla_i   \bar w_R\right) \Delta_\phi \chi_{m , i}
\end{equation}
We then study the spatial derivative of the two-scale expansion $w^0_R$ and prove the two following estimates
\begin{equation} \label{eq:w0Riterglap}
     \sum_{n \geq 2} \frac{1}{\beta^{\frac n2}} \Delta^n w =  \sum_{i=1}^d \sum_{n \geq 2}  \frac{1}{\beta^{\frac n2}} \nabla_i \bar G_\delta \Delta^n \chi_{m,i} + R_1
\end{equation}
and
\begin{equation}\label{eq:w0Riterglap}
 \frac{1}{2\beta} \Delta w^0_R + \sum_{\di q=0} \nabla_q^* \cdot \a_q \nabla_q w^0_R  = \ahom \Delta  \bar w_R + \sum_{i= 1}^d \nabla_i \bar w_R \left( \frac{1}{2\beta} \Delta \chi_{m ,i} + \sum_{\di q=0} \nabla_q^* \cdot \a_q \nabla_q \chi_{m ,i}  \right) + R_2,
\end{equation}
where $R_1$ and $R_2$ are error terms which are small in the $H^{-1}$-norm. More specifically, they satisfy the estimate
\begin{equation*}
 \left\| R_1 \right\|_{\underline{H}^{-1}\left( B_R , \mu_\beta \right)} + \left\| R_2 \right\|_{\underline{H}^{-1}\left( B_R , \mu_\beta \right)} \leq C R^{1 - d - \alpha}.
\end{equation*}
The proof is identical to the proofs of the estimates REf anf REF in Proposition REF, the only difference is that we use the regularity estimate 
We then combine the identities~\eqref{eq:w0RDeltaphi},~\eqref{eq:w0RDeltaphi} and~\eqref{eq:w0RDeltaphi} with the equalities
\begin{equation*}
    \Delta_\phi \chi_{m ,i} + \frac{1}{2\beta} \Delta \chi_{m ,i} + \sum_{n \geq 2} \frac{1}{\beta^{\frac n2}} \Delta^n \chi_{m ,i} +  \sum_{\di q=0} \nabla_q^* \cdot \a_q \nabla_q \left( l_{e_i} + \chi_{m ,i} \right) = 0 ~\mbox{in}~\Omega \times B_R
\end{equation*}
and
\begin{equation*}
     \ahom \Delta \bar w_R = 0 ~\mbox{in}~B_R.
\end{equation*}
This shows the identity
\begin{align*}
        \mathcal{L}^\beta w^{0}_R & = \Delta_\phi w^{0}_R +  \frac{1}{2\beta} \Delta w^{0}_R + \sum_{n \geq 2} \frac{1}{\beta^{\frac n2}} \Delta^n w^{0}_R +  \sum_{\di q=0} \nabla_q^* \cdot \a_q \nabla_q w^{0}_R \\
                                    & = R_1 + R_2.
\end{align*}
The previous identity together with the estimate REF, we obtain REF.


\textit{Step 2.} In this step, we prove the estimate 
\begin{equation*}
    \left\| \nabla w_R - \nabla w^0_R \right\|_{\underline L^2 \left( B_{\frac{R}4} \right)} \leq \frac{C}{R^{d - 1 - \alpha}}.
\end{equation*}
The strategy of the proof relies on the following argument. By Proposition REF, we know that the function $w_R$ is close to the function $\bar w_R$ in the $L^2$ norm over the ball $B_R$. More specifically, we have the estimates
\begin{equation*}
        \left\| w_R - \bar w_R\right\|_{\underline{L}^2 \left(B_\frac R2 , \mu_\beta \right)} \leq \frac{C}{R^{d -1 - \alpha}}.
    \end{equation*}
We also record the following $L^2$-estimate on the gradients of the functions
\begin{equation*}
    \left\| \nabla w_R(x) \right\|_{\underline{L}^2\left(B_{\frac R2} , \mu_\beta\right)} + \left\| \nabla \bar w_R(x)\right\|_{\underline{L}^2 \left( \mu_\beta \right)} +  \left\| \nabla  \bar w_R(x)\right\|_{\underline{L}^2 \left( \mu_\beta \right)}
\end{equation*}
We let $\eta$ be a cutoff function in the ball $B_{\frac R2}$ satisfying
\begin{equation*}
\eta \in C_c^\infty (\Rd),\indc_{B_{\frac{R}4}} \leq \eta  \leq \indc_{B_{\frac{R}2}}, ~\mbox{and} ~\forall k \in \N, ~\left| \nabla^k \eta \right| \leq \frac{C}{R^{k}}
\end{equation*}
The function $\eta \left( w_R - \nabla w^0_R \right)$ belongs to the space $H^1_0 \left(B_R , \mu_\beta \right)$ and can be used as a test function in the equation REF. We obtain
\begin{equation} \label{eq:2sc1434}
    \sum_{x \in B_R} \left\langle \mathcal{L}^\beta \left( w_R - w_R^0 \right) , w_R - w_R^0  \right\rangle_{\mu_\beta} \leq \left\| \mathcal{L}^\beta \left( w_R - w_R^0 \right) \right\|_{\underline{H}^{-1}\left( B_R, \mu_\beta \right)} \left\|  w_R - w_R^0 \right\|_{\underline{H}^1 \left(  B_R, \mu_\beta \right)}.
\end{equation}
We then treat the terms on the right and left-hand side separately. The term on the right side can be estimated thanks to the equality $\mathcal{L}^\beta \left( w_R  \right) =0 $ in $\Omega \times B_R$, the estimate REF of Step 1 and the estimate REF. We obtain
\begin{align*}
    \sum_{x \in B_R} \left\langle \mathcal{L}^\beta \left( w_R - w_R^0 \right) , w_R - w_R^0  \right\rangle_{\mu_\beta} & \leq \left\| \mathcal{L}^\beta \left( w_R - w_R^0 \right) \right\|_{\underline{H}^{-1}\left( B_R, \mu_\beta \right)} \left\|  w_R - w_R^0 \right\|_{\underline{H}^1 \left(  B_R, \mu_\beta \right)} \\
                    & \leq \left\| \mathcal{L}^\beta  w_R^0  \right\|_{\underline{H}^{-1}\left( B_R, \mu_\beta \right)} \left\|  w_R - w_R^0 \right\|_{\underline{H}^1 \left(  B_R, \mu_\beta \right)} \\
                    & \leq C R^{d - 1 - \alpha} \times R^{d - 1 }.
\end{align*}
To estimate the term on the left side of~\eqref{eq:2sc1434}, we use the computation of REF, with the function $F =  w_R - w_R^0$,
\begin{align*}
    \sum_{x \in B_R} \left\langle \mathcal{L}^\beta \left( w_R - w_R^0 \right) , \eta \left( w_R - w_R^0 \right) \right\rangle_{\mu_\beta} = \sum_{y \in F} \int_F \eta(x)^2 \left\langle \left( \partial_y F(x) \right)^2 \right\rangle_{\mu_\beta} \, dx + \frac 1{2\beta}\int_F  \left\langle \nabla F \cdot \nabla \left( \eta^2 F\right) \right\rangle_{\mu_\beta} \\ +  \frac 1{2\beta} \sum_{n \geq 1} \int_F  \frac{1}{\beta^{ \frac n2}} \left\langle  \nabla^n F \cdot \nabla^n \left( \eta^2 F \right) \right\rangle_{\mu_\beta} + \sum_{q}  \left\langle \nabla_q F\cdot \a_q \nabla_q \left( \eta^2 F \right) \right\rangle_{\mu_\beta}
\end{align*}
with the estimates
\begin{equation*}
     \int_F \nabla^n F \cdot \nabla^n \left( \eta^2 F \right) - \int_F \eta^2 \nabla^n F \cdot \nabla^n  F \geq \frac{C^n}{R} \left\| \nabla  F \right\|_{L^2 \left( B_R\right)} \left\| F \right\|_{L^2 \left( B_R \right)},
\end{equation*}
and the estimate 
\begin{equation*}
      \sum_{q} \nabla_q F\cdot \a_q \nabla_q \left( \eta^2 F \right) -  \sum_{q} \eta^2 \nabla_q F\cdot \a_q \nabla_q  F  \geq - \frac{C}{R} \left\| \nabla  F \right\|_{L^2 \left( B_R\right)} \left\| F \right\|_{L^2 \left( B_R \right)}.
\end{equation*}
A combination of the three previous displays shows
\begin{equation*}
    \sum_{x \in B_R} \left\langle \mathcal{L}^\beta \left( w_R - w_R^0 \right) , \eta \left( w_R - w_R^0 \right) \right\rangle_{\mu_\beta} \geq c \left\| \nabla \left( w_R - w_R^0 \right) \right\|_{\underline{L}^2 \left(B_{\frac R2 , \mu_\beta} \right)}^2 - \frac{C}{R^2} \left\|  w_R - w_R^0 \right\|_{\underline{L}^2 \left(B_{R , \mu_\beta} \right)}^2
\end{equation*}
Combining REF and REf shows the estimate
\begin{equation*}
    \left\| \nabla \left( w_R - w_R^0 \right) \right\|_{\underline{L}^2 \left(B_{\frac R2 , \mu_\beta} \right)} \leq C R^{2d - 2 - \alpha} + \frac{C}{R} \left\|  w_R - w_R^0 \right\|_{\underline{L}^2 \left(B_{R , \mu_\beta} \right)}.
\end{equation*}
We complete the proof of the inequality REF by estimating the second term on the right side of the previous display. We use the estimate REF, which states that the functions $w_R$ and $\bar w_R$ are close in the $L^2$-norm, the regularity estimate on the harmonic function $\bar w_R$ stated in REf and the quantitative sublinearity of the corrector stated in REF. We obtain
\begin{align*}
    \left\|  w_R - w_R^0 \right\|_{\underline{L}^2 \left(B_{R , \mu_\beta} \right)} & \leq \left\|  w_R - \bar w_R \right\|_{\underline{L}^2 \left(B_{R , \mu_\beta} \right)} + \sum_{i = 1}^d \left\|   \left( \nabla_i   \bar w_R\right) \chi_{m , i} \right\|_{\underline{L}^2 \left(B_{R , \mu_\beta} \right)} \\
                    & \leq \frac{C}{R^{d - 1 - \alpha}} .
\end{align*}
Combining this estimate with the inequality REF shows
\begin{equation*}
     \left\| \nabla \left( w_R - w_R^0 \right) \right\|_{\underline{L}^2 \left(B_{\frac R2 , \mu_\beta} \right)} \leq \frac{C}{R^{d - 1 - \alpha}}.
\end{equation*}
We finally simplify the previous display and note that by an explicit computation, we have
\begin{equation*}
    \nabla  w_R^0 = \nabla \bar w_R + \sum_{i=1}^d \nabla_i \bar w_R \nabla \chi_{m,i} +  \nabla \bar w_R + \sum_{i=1}^d \nabla \nabla_i \bar w_R  \chi_{m,i}.
\end{equation*}
Using the regularity estimate on the function $ \bar w_R$ stated in REf and  we can estimate the $L^2$-norm of the second term on the right side and prove that it it small compared to the value $R^{d-2}$, we have the estimate
\begin{equation*}
   \sum_{i=1}^d \left\| \nabla \nabla_i \bar w_R  \chi_{m,i} \right\|_{\underline{L}^2 \left(B_R , \mu_\beta \right)} \leq \frac{C}{R^{d -\alpha}}
\end{equation*}
We also replace the gradient of the corrector $\chi_m$ by the gradient of the full-volume corrector thanks to Proposition REF and the regularity estimate REf on the function $\bar w_R$, according to the estimate
\begin{equation*}
   \sum_{i=1}^d \left\|  \nabla_i \bar w_R \left( \nabla \chi_{m,i} - \nabla \chi_i \right) \right\|_{\underline{L}^2 \left( B_R , \mu_\beta \right)} \leq \frac{C}{R^{d -\alpha}}
\end{equation*}
Combining the estimates
\begin{equation*}
    \left\| \nabla  w_R - \nabla \bar w_R + \sum_{i=1}^d \nabla_i \bar w_R \nabla \chi_i \right\|_{\underline{L}^2 \left(B_{\frac R2 , \mu_\beta} \right)} \leq \frac{C}{R^{d  - \alpha}}
\end{equation*}
This completes the proof of Step 2.

\medskip

\textit{Step 3.} In this step we deduce from the $L^2$-estimate REF obtained in Step 2, the pointwise estimate REF. This is achieved by using the stationarity of the measure $\mu_\beta$. We first define the exponent
\begin{equation*}
    \kappa := \frac{\alpha}{bla}
\end{equation*}
and reduce the domain of integration of the estimate REF: we write
\begin{align*}
    \left\| \nabla  w_R - \left( I_d + \nabla \chi \right) \nabla \bar w_R  \right\|_{\underline{L}^2 \left(B_{R^{1- \kappa} , \mu_\beta} \right)} & \leq R^{d\kappa} \left\| \nabla  w_R - \left( I_d + \nabla \chi \right) \nabla \bar w_R \right\|_{\underline{L}^2 \left(B_{\frac R2 , \mu_\beta} \right)}\\ & \leq \frac{C}{R^{d  - \alpha + d\kappa}} \\ & \leq \frac{C}{R^{d  - \alpha}},
\end{align*}
by reducing the value of the exponent $\alpha$ in the last line. For each $y \in B_{R^{1- \kappa}}$, we let $ w_R^y$ be the solution of the Helffer-Sjostrand equation, for each $(x , \phi) \in F \times \Omega$
\begin{equation*}
    \mathcal{L}_\beta w_R^y (x , \phi) = \nabla \cdot F_R(y + x , \phi),
\end{equation*}
This solution is related to the solution $w_R$ by the identity, for each pair $(x , \phi) \in F \times \Omega$,
\begin{equation*}
    w_R(x + y , \tau_y \phi) = w_R^y (x , \phi).
\end{equation*}
Reducing the space of integration to the ball $B_{R^{1-\kappa}}$ in the estimate REF is useful because it gives the following estimates.
\begin{itemize}
    \item For each $x \in B_{R^{1-\kappa}}$, one has the estimate
    \begin{equation*}
        \left| \nabla \bar w_R(x) - \nabla \bar w_R(0) \right|  \leq \frac{C}{R^{d+\kappa}},
    \end{equation*}
    which follows from the regularity estimate REF.
    \item For each $y \in B_{R^{1-\kappa}}$, one has the estimate
    \begin{equation*}
        \left| w^y_R (0 , \phi) - w_R (0 , \phi) \right| \leq small.
    \end{equation*}
    The proof of this estimate relies on the bounds on the mixed derivative of the Green's matrix $\mathcal{G}$. By the definitions of the function $w_R$ and $w_R^y$, the map $w_R - w_R^y$ is a solution of the equation
    \begin{equation*}
        \mathcal{L}_\beta \left( w_R - w_R^y \right) = \nabla \cdot \left( F_R(y + x , \phi) - F_R(y + x , \phi) \right).
    \end{equation*}
    By definition of the function $F_R$, we have the identity
    \begin{equation*}
        F_R(y + x , \phi) - F_R( x , \phi) = \cos \left(\nabla \phi (x) \right) \indc_{x \in A_R \Delta \left( y + A_R\right)}
    \end{equation*}
    where the symbol $\Delta$ denotes the symmetric difference. Using that the point $y$ belongs to the ball $B_{R^{1-\kappa}}$, we can estimate the volume of the symmetric difference $A_R \Delta \left( y + A_R\right)$. We obtain
    \begin{equation*}
        \left| A_R \Delta \left( y + A_R\right) \right| \leq R^{-\kappa} \left| A_R \right| \leq C R^{-\kappa} \left| A_R \right| \leq C R^{d -\kappa}.
    \end{equation*}
    Combining this estimate with the inequality REF on the mixed derivative of the Green's matrix, we deduce
    \begin{equation*}
    \left| w_R(0,\phi) - w_R^y(0, \phi)\right| \leq R^{-\kappa}.
    \end{equation*}
\end{itemize}
We then come back to the inequality REf and use the translation invariance of the measure $\mu_\beta$ and the identity REf and the identity REf on the gradient of the corrector to rewrite it in terms of the random variable $w_R^y(0,\cdot)$. We have
\begin{align*}
     \lefteqn{\left\| \nabla  w_R - \left( I_d + \nabla \chi \right) \nabla \bar w_R  \right\|_{\underline{L}^2 \left(B_{R^{1- \kappa} , \mu_\beta} \right)}^2} \qquad & \\ & = \frac{1}{R^{ \left(1-\kappa\right)}} \sum_{y \in B_{R^{1-\kappa}}} \int_\Omega \left|\nabla  w_R(y, \phi) - \left( I_d + \nabla \chi(y , \phi)) \right) \nabla \bar w_R(x) \right|^2 \mu_\beta\left( d \phi \right) \\ &
     = \frac{1}{R^{ \left(1-\kappa\right)}} \sum_{y \in B_{R^{1-\kappa}}} \int_\Omega \left|\nabla  w_R^y (0, \tau_y \phi) - \left( I_d + \nabla \chi(0 , \tau_y \phi)) \right) \nabla \bar w_R(x) \right|^2 \mu_\beta\left( d \phi \right) \\
     & = \frac{1}{R^{ \left(1-\kappa\right)}} \sum_{y \in B_{R^{1-\kappa}}} \int_\Omega \left|\nabla  w_R^y (0, \phi) - \left( I_d + \nabla \chi(0 , \phi)) \right) \nabla \bar w_R(y) \right|^2 \mu_\beta\left( d \phi \right)
\end{align*}
By the inequalities REf and REf, we have, for each $y \in B_{R^{1-\kappa}}$,
\begin{multline*}
    \int_\Omega \left|\nabla  w_R^y (0, \phi) - \left( I_d + \nabla \chi(0 , \phi)) \right) \nabla \bar w_R(y) \right|^2 \mu_\beta\left( d \phi \right) \\ = \int_\Omega \left|\nabla  w_R (0, \phi) - \left( I_d + \nabla \chi(0 , \phi)) \right) \nabla \bar w_R(0) \right|^2 \mu_\beta\left( d \phi \right) + O \left( R^{-\kappa}\right).
\end{multline*}
Combining the estimates REf and REf shows
\begin{equation*}
    \left\| \nabla  w_R - \left( I_d + \nabla \chi \right) \nabla \bar w_R  \right\|_{\underline{L}^2 \left(B_{R^{1- \kappa} , \mu_\beta} \right)}^2 = \left\| \nabla  w_R (0, \cdot) - \left( I_d + \nabla \chi(0 , \cdot)) \right) \nabla \bar w_R(0) \right\|_{L^2 \left( \mu_\beta \right)}^2 + O \left( R^{-\kappa} \right). 
\end{equation*}
Combining this estimate with the inequality REF and recalling the value of the exponent $\kappa$ defined in REf, we deduce the pointwise estimate
\begin{equation*}
    \left\| \nabla  w_R (0, \cdot) - \left( I_d + \nabla \chi(0 , \cdot)) \right) \nabla \bar w_R(0) \right\|_{L^2 \left( \mu_\beta \right)}^2  \leq C R^{-\kappa} + C R^{-\alpha}.
\end{equation*}
By reducing the size of the exponent $\alpha$, we deduce the estimate REF. This completes the proof of Proposition~\ref{prop:homhogmixedder}.

Un bout de l'ancienne estimee H-1 du flux

similar to the proof of~\eqref{eq:quantsublin}. We first combine Lemma~\ref{lem:lemma5.8} (estimate~\eqref{mainest.lamma4.2vH-1}) with Lemma~\ref{lem:lemma5.6} and Corollary~\ref{cor:cor5.23} to obtain the estimate
\begin{equation}
\left\| \nabla v (\cdot, \cu_{n+1} , p^*) - \ahom^{-1} p^*  \right\|_{\underline L^2(\cu_{n+1} , \mu_{\beta}) }^2 \leq  C |p^*|^2 3^{2n} \left( 3^{-\gamma n}+ \sum_{m = 0}^n 3^{-\gamma (m -n)} \tau_m \right).
\end{equation}



There are only two differences which are explained below:
\begin{itemize}
    \item We use the $H^{-1}$-version of the multiscale Poincar\'e inequality stated in~\eqref{eq:H-1multsc} instead of the $L^2$ version given in~\eqref{eq:L2multsc};
    \item We do not rely on the identity $\sum_{x \in \cu_m^-} u \left( x , \cdot, \cu_m^{-} , p \right) = p$ as it is done in the proof of the estimate~\eqref{mainest.lamma4.2u} (see the equality~\eqref{eq:TV17394}). Instead, we note that Proposition~\ref{prop:prop5.2} implies the inequality $\left| \a\left( \cu_m^- \right) - \ahom \right| \leq C 3^{-\alpha m}$ and use the identity~\eqref{eq:derivpnu} to write, for each integer $m \in \N$ and each slope $p \in \R^{d \binom d2}$,
    \begin{equation*}
\left| \sum_{x \in \cu_m^-} \left( \frac1{2\beta}  \left\langle \nabla  u(x , \cdot , \cu ,p ) \right\rangle_{\mu_\beta}  -  \sum_{q}  \left\langle \a_q  \nabla_q u(x , \cdot , \cu_m^- ,p )   \right\rangle_{\mu_{\beta}} n_q(x)  \right) -  \ahom p \right| \leq C |p| 3^{-\alpha m}.
\end{equation*}
\end{itemize}


(Old) Proof of the main Theorem

\subsubsection{Next Section} \label{section3.4.2}

The next lemma shows that only the terms $X_x$ and $Y_0$ give the main contribution of the two point function. The proof is deferred to Section REf.
\begin{proposition} \label{prop:propmun1246}
There exist constants such that
\begin{equation*}
     \frac{Z_\beta (\sigma)}{Z_\beta(0)} = \left\langle Y_0 X_x \right\rangle_{\mu_\beta} + \frac{c_1 \left\langle Y_0 X_x \right\rangle_{\mu_\beta}}{|x|^{d-2}} + O \left( \frac{1}{|x|^{d-1}}. \right)
\end{equation*}
In particular the following statements are equivalent
\begin{equation*}
    \exists c_1 , c_2 \in \R, \frac{Z_\beta (\sigma)}{Z_\beta(0)} = c_1 + \frac{c_2}{|x|^{d-2}} + O \left( \frac{1}{|x|^{d-2 + \alpha}} \right) \iff  \exists c_1, c_2 \in \R, \left\langle Y_0 X_x \right\rangle_{\mu_\beta} = c_1+ \frac{c_2}{|x|^{d-2}} + O \left( \frac{1}{|x|^{d-2 + \alpha}} \right).
\end{equation*}
\end{proposition}





By Proposition \ref{prop:propmun1246}, to prove Theorem REF it is sufficient to prove the identity: there exists two constants $c_0, c_1 \in \R$ such that
\begin{equation}
\label{e.cor31}
    \left\langle Y_0 X_x \right\rangle_{\mu_\beta} = c_0 + \frac{c_1}{|x|^{d-2}} + O \left( \frac{1}{|x|^{d-2+ \gamma}} \right).
\end{equation}
The first-order term $c_0$ in the expansion REF can be heuristically determined: by sending $x$ to infinity, the random variables $Y_0$ and $X_x$ becomes independent and this implies
\begin{equation*}
    \lim_{x \rightarrow \infty} \left\langle Y_0 X_x \right\rangle_{\mu_\beta} = \left\langle Y_0 \right\rangle_{\mu_\beta} \left\langle X_0 \right\rangle_{\mu_\beta},
\end{equation*}
since, by translation invariance of the measure $\mu_\beta$, the expectation $\left\langle X_x \right\rangle_{\mu_\beta}$ does not depend on the point $x$ and is equal to $\left\langle X_0 \right\rangle_{\mu_\beta}$. This allows to identify the value of $c_0$ and we expect to have $c_0 = \left\langle Y_0 \right\rangle_{\mu_\beta} \left\langle X_0 \right\rangle_{\mu_\beta}$. As a consequence, the expansion \eqref{e.cor31} can be rewritten as
\begin{equation*}
    \cov \left[ X_x , Y_0 \right] = \frac{c_1}{|x|^{d-2}} + O \left( \frac{1}{|x|^{d-2 + \alpha}} \right).
\end{equation*}
To prove this result, we appeal to the Helffer-Sjostrand representation formula and write the covariance in the following form
\begin{equation*}
     \cov \left[ X_x , Y_0 \right] = \sum_{y \in \Zd} \left\langle \left(\partial_y  X_x\right) w(y, \cdot ) \right\rangle_{\mu_\beta},
\end{equation*}
where $w$ is the solution of the Helffer-Sjostrand equation, for each $(x , \phi) \in \Zd \times \Omega$,
\begin{equation} \label{def.wVill}
    \mathcal{L}w(y , \phi) = \partial_y Y_0.
\end{equation}



The goal of the following proposition is to decouple the exponential terms $X_x$ and $Y_0$ from the Hellfer Sjostrand equation to simplify the analysis. The proof is deferred to Section REF.

\begin{proposition}[Removing the contribution of the cosine]\label{p.removecos}
One has the first-order expansion
\begin{equation}
\label{e.removecos}
    \cov \left[ X_x , Y_0 \right] = \sum_{y \in \Zd} \left\langle X_x Q_x(y) v(y, \cdot ) \right\rangle_{\mu_\beta},
\end{equation}
where $v$ is the solution of the Helffer Sjostrand equation, for each $(y, \phi ) \in \Zd \times \Omega$,
\begin{equation*}
    \mathcal{L} v(y , \phi) = Q_0(y) Y_0(\phi)
\end{equation*}
\end{proposition}



The next step in the analysis consist in further removing the exponential terms $X_x$ and $Y_0$ from the right hand side of \eqref{e.removecos}. The proof is based on the regularity theory developed in Section \ref{section:section4} and will be deferred to Section REF. 

\begin{proposition}[Decoupling the exponential]
\label{p.decoupleexp}
One has the following estimate
\begin{align*}
    \cov \left[ X_x , Y_0 \right] 
    %& = \sum_{y \in \Zd} \left\langle \left(\partial_y  X_x\right) w(y, \cdot ) \right\rangle_{\mu_\beta} \\
    & = \left\langle Y_0 \right\rangle_{\mu_\beta} \left\langle X_0 \right\rangle_{\mu_\beta}  \sum_{y \in \Zd} \left\langle Q_x(y) u(y, \cdot ) \right\rangle_{\mu_\beta} + O \left( \frac{1}{|x|^{d-1+\ep}} \right),
\end{align*}
where $u$ is the solution of the Hellfer Sjostrand equation
\begin{equation*}
    \mathcal{L} u = Q_0. 
\end{equation*}
\end{proposition}



\subsection{Proof of Theorem REF} This section is devoted to the proof of Theorem REF

\begin{proof}[Proof of Theorem REF]
By the Propositions \ref{p.decoupleexp}, it is sufficient to prove  the expansion
\begin{equation}
\label{e.expanQu}
    \sum_{y \in \Zd} \left\langle Q_x(y) u(y ,\cdot) \right\rangle_{\mu_\beta} = \frac{c_1}{|x|^{d-2}} + O \left( \frac{1}{|x|^{d-2 + \alpha}} \right),
\end{equation}
where $u$ is the solution of the Helffer Sjostrand equation $\mathcal{L}u = Q_0$.

\textit{Step 1. Decomposing along the charges.} We recall the definition of the quotient space for charges $Q / \Zd$. For each class $[q] \in Q / \Zd$, we choose a charge $q \in \Zd$ such that $0$ belongs to the support of the charge $q$ (and break ties thanks to an arbitrary criterion). We have the decomposition
\begin{align*}
    Q_0 & = \sum_{[q] \in Q/\Zd} z \left( \beta , q \right) \sum_{y \in \Zd} \cos \left( \phi , q(y + \cdot) \right) \sin\left( \sigma_0, q(y + \cdot) \right) q(y + \cdot) \\
    & = \sum_{[q] \in Q/\Zd} z \left( \beta , q \right) \sum_{y \in \Zd} \cos \left( \phi(y + \cdot ) , q \right) \sin\left( \sigma_0(y + \cdot), q \right) q(y + \cdot).
\end{align*}
We recall that we have the pointwise estimate, for each $x \in \Zd$,
\begin{equation*}
    \left| \sum_{y \in \Zd} \cos \left( \phi(y + \cdot ) , q \right) \sin\left( \sigma_0(y + \cdot), q \right) q(y + x) \right| \leq \frac{C\left\| q \right\|_1}{|x|^{d-1}}.
\end{equation*}
Given an equivalence class $[q] \in Q/\Zd$ and a point $y \in \Zd$, we denote by $u_q$ and $u_{q ,y}$ the solutions of the Hellfer Sjostrand equations 
\begin{equation*}
    \mathcal{L} u_q = \sum_{y \in \Zd} \cos \left( \phi(y + \cdot ) , q \right) \sin\left( \sigma_0(y + \cdot), q \right) q(y + \cdot) ~\mbox{and}~  \mathcal{L} u_{q,y} = \cos \left( \phi(y + \cdot ) , q \right) q(y + \cdot).
\end{equation*}
In particular, we have the identities
\begin{equation*}
    u = \sum_{[q] \in Q/\Zd} z \left(\beta ,q  \right) u_q ~\mbox{and}~  u_q = \sum_{y \in \Zd} \sin\left( \sigma_0(y + \cdot), q \right) u_{q , y} .
\end{equation*}
Making use of this notation, the expansion \eqref{e.expanQu} can be rewritten as 
\begin{multline}
    \sum_{[q_1], [q_2] \in Q/\Zd} z \left( \beta, q_1 \right) z \left( \beta, q_2 \right) \sum_{y , y_1, y_2 \in \Zd} \sin\left( \sigma_x(y_1 + \cdot), q_1\right) q_1( y - y_1) \left\langle \cos \left( \phi(y_1 + \cdot ) , q_1 \right) u_{q_2, y_2}(y) \right\rangle_{\mu_\beta} \sin\left( \sigma_0(y_2 + \cdot), q_2 \right)  \\
                    = \frac{c_1}{|x|^{d-2}} + O \left( \frac{1}{|x|^{d-2 + \alpha}} \right). \label{e.rewriteexpan}
\end{multline}
To prove REF, we fix two equivalence classes $[q_1] , [q_2] \in Q/\Zd$ and prove the following result: there exist two real constants $c_{q_1,q_2} \in \R$ and $C_{q_1, q_2} \in (0, \infty)$ such that
\begin{multline*}
    \sum_{z,y_1, y_2 \in \Zd} \sin\left( \sigma_x(y_1 + z), q_1\right) q_1(y_1 + \cdot) \left\langle \cos \left( \phi(y_1 + \cdot ) , q_1 \right) u_{q_2, y_2}(z , \phi ) \right\rangle_{\mu_\beta} \sin\left( \sigma_0(y_2 + \cdot), q_2 \right) \\ = \frac{c_{q_1,q_2}}{|x|^{d-2}} + O \left(\frac{C_{q_1, q_2}}{|x|^{d-2+\alpha}} \right).
\end{multline*}
The constants $c_{q_1,q_2}$ and $C_{q_1, q_2}$ depend on the charges $q_1,q_2$; we prove that they satisfy the estimates
\begin{equation}
\label{e.Cestimate}
    \left| c_{q_1,q_2} \right|+ \left| C_{q_1,q_2} \right| \leq \left\| q_1 \right\|_1^{10^{10}} \left\| q_2 \right\|_1^{10^{10}}.
\end{equation}
A combination of the expansion REF with the inequalities REF is then sufficient to prove the result REF; indeed by using the the estimate REf on the coefficient $z \left( \beta , q \right)$, we have that the sums $\sum_{[q_1], [q_2] \in Q/\Zd} \left| z \left( \beta, q_1 \right) z \left( \beta, q_2 \right)  c_{q_1, q_2} \right|$ and $\sum_{[q_1], [q_2] \in Q/\Zd} \left| z \left( \beta, q_1 \right) z \left( \beta, q_2 \right)  c_{q_1, q_2} \right|$ are finite. We can thus sum the expansion REf over all the equivalence classes (following the formula REF), to obtain the expansion REF with the value
\begin{equation*}
    c_1 := \sum_{[q_1], [q_2] \in Q/\Zd} z \left( \beta , q_1 \right) z \left( \beta , q_2 \right) c_{q_1 , q_2}.
\end{equation*}
We now focus on the proofs of the expansion \eqref{e.rewriteexpan} and the estimate \eqref{e.Cestimate}.

\medskip

\textit{Step 2. Simplifying the expansion REF.} We fix two equivalence classes $[q_1], [q_2] \in Q/\Zd$. The objective of this step is to simplify the estimate REf. More specifically, we prove the following result
\begin{multline*}
    \sum_{z,y_1, y_2 \in \Zd} \sin\left( \sigma_x(y_1 + z), q_1\right) q_1(y_1 + \cdot) \sum_{y \in y_1 + \supp  n_{q_1}}\left\langle \cos \left( \phi(y_1 + \cdot ) , q_1 \right) u_{q_2, y_2}(z , \phi ) \right\rangle_{\mu_\beta} \sin\left( \sigma_0(y_2 + \cdot), q_2 \right) \\ = (n_{q_1}) (n_{q_2}) \sum_{y_1, y_2 \in \Zd} \nabla G(y_1-x) \nabla G(y_2) \left\langle \cos \left( \phi(y_1 + \cdot ) , q_1 \right) \delta u_{q_2, y_2}(z , \phi )  \right\rangle_{\mu_\beta} + O \left( \frac{1}{|x|^{d-1-\ep}} \right). 
\end{multline*}
To prove this result, we first use the formulas $q_1 = \di n_{q_1}$, $\delta \sigma_0 = \nabla G$ and $\delta \sigma_x = \nabla G\left( \cdot  - x \right)$ to write
\begin{multline*}
    \sum_{z,y_1, y_2 \in \Zd} \sin\left( \sigma_x(y_1 + z), q_1\right) q_1(y_1 + \cdot) \left\langle \cos \left( \phi(y_1 + \cdot ) , q_1 \right) u_{q_2, y_2}(z , \phi ) \right\rangle_{\mu_\beta} \sin\left( \sigma_0(y_2 + \cdot), q_2 \right) \\ = \sum_{y, y_1, y_2 \in \Zd} \sin\left( \nabla G(y_1-x + \cdot), n_{q_1}\right) \sin\left( \nabla G(y_2 + \cdot), n_{q_2} \right) n_{q_1}(y - y_1) \left\langle \cos \left( \phi(y_1 + \cdot ) , q_1 \right) \delta u_{q_2, y_2}(y , \phi ) \right\rangle_{\mu_\beta}.
\end{multline*}
We compute
\begin{align*}
    \lefteqn{\sum_{y, y_1, y_2 \in \Zd} \sin\left( \nabla G(y_1-x + \cdot), n_{q_1}\right) \sin\left( \nabla G(y_2 + \cdot), n_{q_2} \right) n_{q_1}(y - y_1) \left\langle \cos \left( \phi(y_1 + \cdot ) , q_1 \right) \delta u_{q_2, y_2}(y , \phi ) \right\rangle_{\mu_\beta}} \qquad & \\ & = (n_{q_1}) (n_{q_2}) \sum_{y_1, y_2 \in \Zd} \nabla G(y_1-x)\nabla G(y_2 ) \left( \sum_{y} n_{q_1}(y - y_1) \left\langle \cos \left( \phi(y_1 + \cdot ) , q_1 \right) \delta u_{q_2, y_2}(y , \phi ) \right\rangle_{\mu_\beta} \right) \\
    & \quad + \sum_{y_1, y_2 \in \Zd} F_1(y_1-x) \sin\left( \nabla G(y_2 + \cdot), n_{q_2} \right) \left( \sum_y n_{q_1}(y - y_1) \left\langle \cos \left( \phi(y_1 + \cdot ) , q_1 \right) \delta u_{q_2, y_2}(y , \phi ) \right\rangle_{\mu_\beta}\right)\\
    & \quad + \sum_{ y_1, y_2 \in \Zd} \nabla G(y_1-x) F_2(y_2) \left( \sum_y n_{q_1}(y - y_1) \left\langle \cos \left( \phi(y_1 + \cdot ) , q_1 \right) \delta u_{q_2, y_2}(y , \phi ) \right\rangle_{\mu_\beta} \right),
\end{align*}
where the function $F_1$ and $F_2$ are defined by the formulas
\begin{equation*}
    \left\{ \begin{aligned}
    F_1(y_1) := \sin\left( \nabla G(y_1-x + \cdot), n_{q_1}\right) - (n_{q_1})\nabla G(y_1-x) \\
    F_2(y_2) := \sin\left( \nabla G(y_2 + \cdot), n_{q_2}\right) - (n_{q_2}) \nabla G(y_2)
    \end{aligned}
    \right.
\end{equation*}
These maps can be estimated thanks to the following ingredients:
\begin{itemize}
    \item Using the estimate REf and the Taylor expansion of the sine, we have the inequality
    \begin{equation*}
        \left|\sin\left( \nabla G(y_1-x + \cdot), n_{q_1}\right) - \left( \nabla G(y_1-x + \cdot), n_{q_1}\right) \right|  \leq C \left|\left( \nabla G(y_1-x + \cdot), n_{q_1}\right) \right|^3 \leq C \frac{\left\| n_q \right\|^{3d}}{\left| y_1-x \right|^{3d-3}};
    \end{equation*}
    \item Using the regularity for the Green's matrix $G$, we have the estimate $\left| \nabla \nabla G \left( y\right) \right| \leq \frac{C}{|y|^d},$
    which implies
    \begin{align*}
        \left|\left( \nabla G(y_1 -x + \cdot), n_{q_1}\right) - \nabla G(y_1-x) \left( n_{q_1} \right) \right| & \leq \left|\left( \nabla G(y_1-x + \cdot) - \nabla G(y_1-x), n_{q_1}\right) \right| \\
        & \leq \sup_{\supp n_{q_1}} \left|\nabla \nabla G (y_1 + \cdot) \right| \diam n_{q_1} \left\| n_{q_1}\right\|_1 \\
        & \leq \frac{C\left\| q_1 \right\|_1^{d+2}}{|y_1-x|^d}.
    \end{align*}
\end{itemize}
We obtain the upper bounds, for each $y_1 , y_2 \in \Zd$,
\begin{equation*}
    \left| F_1(y_1) \right| \leq C \left( \frac{\left\| q_1 \right\|^{3d}}{\left| y_1-x\right|^{3d-3}} + \frac{C\left\| q_1 \right\|_1^{d+2}}{|y_1-x|^d} \right) \leq \frac{\left\| q_1 \right\|^{3d}}{\left| y_1-x\right|^{d}} 
\end{equation*}
and similarly
\begin{equation*}
     \left| F_2(y_2) \right| \leq C \left( \frac{\left\| q_2 \right\|^{3d}}{\left| y_2\right|^{3d-3}} + \frac{C\left\| q_2 \right\|_1^{d+2}}{|y_2|^d} \right) \leq \frac{\left\| q_2 \right\|^{3d}}{\left| y_2\right|^{d}}.
\end{equation*}
We also record the estimate
\begin{equation*}
        \left| \left( \nabla G(y_2 + \cdot), n_{q_1}\right) \right| \leq \frac{C \left\| n_{q_1}\right\|^d }{|y_2|^{d-1}},
\end{equation*}
and the following inequality, which is a consequence of the estimate REf on the mixed derivative of the Green's matrix $\mathcal{G}$,
\begin{equation*}
    \left| \sum_y n_{q_1}(y - y_1) \left\langle \cos \left( \phi(y_1 + \cdot ) , q_1 \right) \delta u_{q_2, y_2}(y , \phi ) \right\rangle_{\mu_\beta} \right| \leq \frac{C \left\| q_1 \right\|_1 \left\| q_2 \right\|_1}{|y_1 - y_2|^{d-\ep}}.
\end{equation*}
Using the estimates REF, we can estimate the second and third term in the right-hand side of the identity REf, we obtain
\begin{align*}
    \lefteqn{\left| \sum_{y_1, y_2 \in \Zd} F_1(y_1) \sin\left( \nabla G(y_2 + \cdot), n_{q_2} \right) \left( \sum_y n_{q_1}(y - y_1) \left\langle \cos \left( \phi(y_1 + \cdot ) , q_1 \right) \delta u_{q_2, y_2}(y , \phi ) \right\rangle_{\mu_\beta}\right) \right|} \qquad & \\ & \leq 
    C \left\| q_1 \right\|_1 \left\| q_2 \right\|_1 \sum_{y_1 , y_2} \frac{1}{|y_1-x|^d} \frac{1}{|y_1 - y_2|^{d-\ep}} \frac{1}{| y_2|^{d-1}} \\
    & \leq
    C \left\| q_1 \right\|_1 \left\| q_2 \right\|_1 \frac{1}{|x|^{d-1-\ep}}.
\end{align*}
A similar computation gives the estimate
\begin{equation*}
    \sum_{ y_1, y_2 \in \Zd} \nabla G(y_1-x) F_2(y_2) \left( \sum_y n_{q_1}(y - y_1) \left\langle \cos \left( \phi(y_1 + \cdot ) , q_1 \right) \delta u_{q_2, y_2}(y , \phi ) \right\rangle_{\mu_\beta} \right) \leq C \left\| q_1 \right\|_1 \left\| q_2 \right\|_1 \frac{1}{|x|^{d-1-\ep}}.
\end{equation*}
Combining the estimates REf, REf and REf completes the proof of REF. A consequence of REf is that to prove Theorem REF it is sufficient to prove the following expansion
\begin{equation*}
    \sum_{y_1, y_2 \in \Zd} \nabla G(y_1-x) \nabla G(y_2) \left(\sum_{z} n_{q_1}\left(z + y_1 \right) \left\langle \cos \left( \phi(y_1 + \cdot ) , q_1 \right) \delta u_{q_2, y_2}(z , \phi )  \right\rangle_{\mu_\beta} \right) = \frac{\bar c}{|x|^{d-2}} + O \left( \frac{1}{|x|^{d-2-\alpha}}\right).
\end{equation*}
The proof of this result is the objective of Steps REF.


\medskip

\textit{Step 3. Using the translation invariance of the Gibbs measure $\mu_\beta$.} We fix two equivalence classes $[q_1], [q_2]$ in the set $Q/\Zd$. By translation invariance of the Gibbs measure $\mu_\beta$, we have the equality
 \begin{multline*}
    \sum_{y_1, y_2 \in \Zd} \nabla G(y_1-x) \nabla G(y_2) \left(\sum_{z} n_{q_1}\left(z + y_1 \right) \left\langle \cos \left( \phi(y_1 + \cdot ) , q_1 \right) \delta u_{q_2, y_2}(z , \phi )  \right\rangle_{\mu_\beta} \right)  \\ = \sum_{y_1, y_2 \in \Zd} \nabla G(y_1-x) \nabla G( y_2) \left(\sum_{z} n_{q_1}\left(z + y_1 - y_2 \right) \left\langle \cos \left( \phi(y_1 - y_2 + \cdot ) , q_1 \right) \delta u_{q_2, 0}(z + y_1-y_2 , \phi )  \right\rangle_{\mu_\beta} \right).
\end{multline*}
We then do the change of variables $\kappa = y_1 - y_2$ and rewrite the sum REF
\begin{multline*}
    \sum_{y_1, y_2 \in \Zd} \nabla G(y_1-x) \nabla G(y_2) \left(\sum_{z} n_{q_1}\left(z + y_1 \right) \left\langle \cos \left( \phi(y_1 + \cdot ) , q_1 \right) \delta u_{q_2, y_2}(z , \phi )  \right\rangle_{\mu_\beta} \right) \\ = \sum_{y_1, \kappa \in \Zd} \nabla G(y_1-x) \nabla G(y_1 - \kappa) \left(\sum_{z} n_{q_1}\left(z + \kappa \right) \left\langle \cos \left( \phi(\kappa + \cdot ) , q_1 \right) \delta u_{q_2, 0}(z + \kappa , \phi )  \right\rangle_{\mu_\beta} \right).
\end{multline*}
We then apply the homogenization theorem for the solution of the Helffer Sjostrand equation stated in Theorem REF. For an integer $n \in \N$, we define the dyadic annulus $A_n$ according to the formula $A_n = B_{2^{n+1}} \setminus B_{2^{n}}$. Theorem REf then reads \wwcomment{define the homogenized Green's matrix somewhere}
\begin{equation*}
    \sum_{\kappa \in A_n} \left| \sum_{z \in \Zd} n_{q_1}\left(z + \kappa \right) \left\langle \cos \left( \phi(\kappa + \cdot ) , q_1 \right) \delta u_{q_2, 0}(z + \kappa , \phi )  \right\rangle_{\mu_\beta} - \bar c_{q_1,q_2} \nabla \nabla G (\kappa) \right| \leq  C \left\| q_1 \right\|_1^{1000} \left\| q_2\right\|_1^{1000} 2^{-n \alpha}.
\end{equation*}
We introduce the following error term, for each $\kappa \in \Zd$,
\begin{equation*}
    \mathcal{E}_{q_1,q_2}(\kappa) = \sum_{z \in \Zd} n_{q_1}\left(z + \kappa \right) \left\langle \cos \left( \phi(\kappa + \cdot ) , q_1 \right) \delta u_{q_2, 0}(z + \kappa , \phi )  \right\rangle_{\mu_\beta} - \bar c_{q_1,q_2} \nabla \nabla G (\kappa).
\end{equation*}
We record that it satisfies the following estimates, by REF and REF, for each $\kappa \in \Zd$ and each $n \in \N$,
\begin{equation}
\label{est.mathcale}
    \left| \mathcal{E}_{q_1,q_2}(\kappa) \right| \leq \frac{C}{|\kappa|^{d- \ep}} ~\mbox{and}~ \sum_{\kappa \in A_n} \left| \mathcal{E}_{q_1 , q_2} \left( \kappa \right) \right| \leq C 2^{-n \alpha}.
\end{equation}
Using this notation, we deduce the following identity, for each point $y \in \Zd$ and each integer $n \in \N$,
\begin{multline} \label{eq:afthomog1125}
    \sum_{y_1, \kappa \in \Zd} \nabla G(y_1-x) \nabla G(\kappa - y_1) \left(\sum_{z} n_{q_1}\left(z + \kappa \right) \left\langle \cos \left( \phi(\kappa + \cdot ) , q_1 \right) \delta u_{q_2, 0}(z + \kappa , \phi )  \right\rangle_{\mu_\beta} \right) \\
    = \underbrace{\bar c \sum_{y_1, \kappa \in \Zd} \nabla G(y_1-x) \nabla G(\kappa - y_1) \nabla \nabla G (\kappa) }_{\eqref{eq:afthomog1125}-1}
    + \underbrace{\sum_{y_1, \kappa \in \Zd} \nabla G(y_1-x) \nabla G(x - \kappa - y_1) \mathcal{E}_{q_1 , q_2}(\kappa)}_{\eqref{eq:afthomog1125}-2}.
\end{multline}
We first estimate the term~\eqref{eq:afthomog1125}-1, thanks to two integration by parts and the definition of the Green's matrix, we have
\begin{equation*}
    \sum_{y_1, \kappa \in \Zd} \nabla G(y_1-x) \nabla G(\kappa - y_1) \nabla \nabla G (\kappa)  =  \sum_{y_1 \in \Zd} \nabla G(y_1) \nabla G (x - y_1) = G(x).
\end{equation*}
To estimate the term~\eqref{eq:afthomog1125}-2, we exchange the order of summation and integrate by parts
\begin{align*}
    \sum_{y_1, \kappa\in \Zd} \nabla G(y_1-x) \nabla G(\kappa - y_1) \mathcal{E}_{q_1 , q_2}(\kappa) & = \sum_{\kappa \in \Zd} \left(\sum_{y_1\in \Zd} \nabla G(y_1-x) \nabla G( \kappa - y_1)\right) \mathcal{E}_{q_1,q_2}(\kappa) \\
    & = \sum_{\kappa \in \Zd} G\left( x - \kappa \right) \mathcal{E}_{q_1,q_2}(\kappa).
\end{align*}
Using Proposition REF and the estimate \eqref{est.mathcale} of the error term $\mathcal{E}$, we obtain that there exists a constant $\bar c_2$ such that
\begin{equation*}
    \sum_{\kappa \in \Zd} G\left( x - \kappa \right) \mathcal{E}_{q_1,q_2}(\kappa) = \frac{\bar c_2}{|x|^{d-2}} + O \left( \frac{1}{|x|^{d-2+\alpha}}\right).
\end{equation*}
Combining the estimates REf proves the following expansion
\begin{equation*}
     \sum_{y_1, y_2 \in \Zd} \nabla G(y_1-x) \nabla G(y_2) \left(\sum_{z} n_{q_1}\left(z + y_1 \right) \left\langle \cos \left( \phi(y_1 + \cdot ) , q_1 \right) \delta u_{q_2, y_2}(z , \phi )  \right\rangle_{\mu_\beta} \right) = \frac{\bar c + \bar c_2}{|x|^{d-2}} + O \left( \frac{1}{|x|^{d-2+\alpha}}. \right)
\end{equation*}
Combining the identities REF completes the proof of Theorem REF.
\end{proof}

\textit{Step 3. Using the translation invariance of the Gibbs measure $\mu_\beta$.} We fix two equivalence classes $[q_1], [q_2]$ in the set $Q/\Zd$. By translation invariance of the Gibbs measure $\mu_\beta$, we have the equality
 \begin{multline*}
    \sum_{y_1, y_2 \in \Zd} \nabla G(y_1-x) \nabla G(y_2) \left(\sum_{z} n_{q_1}\left(z + y_1 \right) \left\langle \cos \left( \phi(y_1 + \cdot ) , q_1 \right) \delta u_{q_2, y_2}(z , \phi )  \right\rangle_{\mu_\beta} \right)  \\ = \sum_{y_1, y_2 \in \Zd} \nabla G(y_1-x) \nabla G( y_2) \left(\sum_{z} n_{q_1}\left(z + y_1 - y_2 \right) \left\langle \cos \left( \phi(y_1 - y_2 + \cdot ) , q_1 \right) \delta u_{q_2, 0}(z + y_1-y_2 , \phi )  \right\rangle_{\mu_\beta} \right).
\end{multline*}
We then do the change of variables $\kappa = y_1 - y_2$ and rewrite the sum REF
\begin{multline*}
    \sum_{y_1, y_2 \in \Zd} \nabla G(y_1-x) \nabla G(y_2) \left(\sum_{z} n_{q_1}\left(z + y_1 \right) \left\langle \cos \left( \phi(y_1 + \cdot ) , q_1 \right) \delta u_{q_2, y_2}(z , \phi )  \right\rangle_{\mu_\beta} \right) \\ = \sum_{y_1, \kappa \in \Zd} \nabla G(y_1-x) \nabla G(y_1 - \kappa) \left(\sum_{z} n_{q_1}\left(z + \kappa \right) \left\langle \cos \left( \phi(\kappa + \cdot ) , q_1 \right) \delta u_{q_2, 0}(z + \kappa , \phi )  \right\rangle_{\mu_\beta} \right).
\end{multline*}


Un bout de la preuve du theoreme principal (vers la fin de l'argument)

For an integer $n \in \N$, we define the dyadic annulus $A_n$ according to the formula $A_n = B_{2^{n+1}} \setminus B_{2^{n}}$. Theorem REf then reads \wwcomment{define the homogenized Green's matrix somewhere}
\begin{equation*}
    \sum_{\kappa \in A_n} \left| \sum_{z \in \Zd} n_{q_1}\left(z + \kappa \right) \left\langle \cos \left( \phi(\kappa + \cdot ) , q_1 \right) \delta u_{q_2, 0}(z + \kappa , \phi )  \right\rangle_{\mu_\beta} - \bar c_{q_1,q_2} \nabla \nabla G (\kappa) \right| \leq  C \left\| q_1 \right\|_1^{1000} \left\| q_2\right\|_1^{1000} 2^{-n \alpha}.
\end{equation*}
We introduce the following error term, for each $\kappa \in \Zd$,
\begin{equation*}
    \mathcal{E}_{q_1,q_2}(\kappa) = \sum_{z \in \Zd} n_{q_1}\left(z + \kappa \right) \left\langle \cos \left( \phi(\kappa + \cdot ) , q_1 \right) \delta u_{q_2, 0}(z + \kappa , \phi )  \right\rangle_{\mu_\beta} - \bar c_{q_1,q_2} \nabla \nabla G (\kappa).
\end{equation*}
We record that it satisfies the following estimates, by REF and REF, for each $\kappa \in \Zd$ and each $n \in \N$,
\begin{equation}
\label{est.mathcale}
    \left| \mathcal{E}_{q_1,q_2}(\kappa) \right| \leq \frac{C}{|\kappa|^{d- \ep}} ~\mbox{and}~ \sum_{\kappa \in A_n} \left| \mathcal{E}_{q_1 , q_2} \left( \kappa \right) \right| \leq C 2^{-n \alpha}.
\end{equation}
Using this notation, we deduce the following identity, for each point $y \in \Zd$ and each integer $n \in \N$,
\begin{multline} \label{eq:afthomog1125}
    \sum_{y_1, \kappa \in \Zd} \nabla G(y_1-x) \nabla G(\kappa - y_1) \left(\sum_{z} n_{q_1}\left(z + \kappa \right) \left\langle \cos \left( \phi(\kappa + \cdot ) , q_1 \right) \delta u_{q_2, 0}(z + \kappa , \phi )  \right\rangle_{\mu_\beta} \right) \\
    = \underbrace{\bar c \sum_{y_1, \kappa \in \Zd} \nabla G(y_1-x) \nabla G(\kappa - y_1) \nabla \nabla G (\kappa) }_{\eqref{eq:afthomog1125}-1}
    + \underbrace{\sum_{y_1, \kappa \in \Zd} \nabla G(y_1-x) \nabla G(x - \kappa - y_1) \mathcal{E}_{q_1 , q_2}(\kappa)}_{\eqref{eq:afthomog1125}-2}.
\end{multline}
We first estimate the term~\eqref{eq:afthomog1125}-1, thanks to two integration by parts and the definition of the Green's matrix, we have
\begin{equation*}
    \sum_{y_1, \kappa \in \Zd} \nabla G(y_1-x) \nabla G(\kappa - y_1) \nabla \nabla G (\kappa)  =  \sum_{y_1 \in \Zd} \nabla G(y_1) \nabla G (x - y_1) = G(x).
\end{equation*}
To estimate the term~\eqref{eq:afthomog1125}-2, we exchange the order of summation and integrate by parts
\begin{align*}
    \sum_{y_1, \kappa\in \Zd} \nabla G(y_1-x) \nabla G(\kappa - y_1) \mathcal{E}_{q_1 , q_2}(\kappa) & = \sum_{\kappa \in \Zd} \left(\sum_{y_1\in \Zd} \nabla G(y_1-x) \nabla G( \kappa - y_1)\right) \mathcal{E}_{q_1,q_2}(\kappa) \\
    & = \sum_{\kappa \in \Zd} G\left( x - \kappa \right) \mathcal{E}_{q_1,q_2}(\kappa).
\end{align*}
Using Proposition REF and the estimate \eqref{est.mathcale} of the error term $\mathcal{E}$, we obtain that there exists a constant $\bar c_2$ such that
\begin{equation*}
    \sum_{\kappa \in \Zd} G\left( x - \kappa \right) \mathcal{E}_{q_1,q_2}(\kappa) = \frac{\bar c_2}{|x|^{d-2}} + O \left( \frac{1}{|x|^{d-2+\alpha}}\right).
\end{equation*}
Combining the estimates REf proves the following expansion
\begin{equation*}
     \sum_{y_1, y_2 \in \Zd} \nabla G(y_1-x) \nabla G(y_2) \left(\sum_{z} n_{q_1}\left(z + y_1 \right) \left\langle \cos \left( \phi(y_1 + \cdot ) , q_1 \right) \delta u_{q_2, y_2}(z , \phi )  \right\rangle_{\mu_\beta} \right) = \frac{\bar c + \bar c_2}{|x|^{d-2}} + O \left( \frac{1}{|x|^{d-2+\alpha}}. \right)
\end{equation*}
Combining the identities REF completes the proof of Theorem REF.


Summing over all the points $y \in \Zd$, we deduce that \pdcomment{maybe a log correction somewhere}
\begin{equation*}
    \sum_{y \in \Zd} \sin(\sigma_0 , q(y + \cdot)) \sin(\sigma_x , q(y + \cdot)) = \left( n_q \right)^2 \sum_{y \in \Zd}  \nabla G(y, 0) \nabla G (y ,x) + O \left( \frac{\left\| n_q \right\|_1^2}{|y|^{d-1}} \right).
\end{equation*}
Thanks to an integration by parts, we obtain
\begin{equation*}
\sum_{y \in \Zd} \sin(\sigma_0 , q(y + \cdot)) \sin(\sigma_x , q(y + \cdot)) = \left( n_q \right)^2   G(0, x)+ O \left( \frac{\left\| n_q \right\|_1^2}{|y|^{d-1}} \right).
\end{equation*}
We complete the proof by summing over all the equivalence class of charges in $Q / \Zd$ and by noting that, by the estimate REF on the decay of the coefficient $z \left( \beta , q \right)$, the series $\sum_{[q] \in Q/ \Zd} z\left( \beta , q\right) \E \left[ \cos(\phi , q(y + \cdot))\right] (n_q)^2$ and $\sum_{[q] \in Q/ \Zd} z\left( \beta , q\right) \E \left[ \cos(\phi , q(y + \cdot))\right] \left\| n_q \right\|_1^2$ are summable. This implies
\begin{equation*}
    \E \left[ \sum_{q \in \mathcal{Q}} z(\beta , q) \cos(\phi , q) \sin(\sigma_0 , q) \sin(\sigma_x , q) \right] = \frac{c}{|x|^{d-2}} + O \left( \frac{1}{|x|^{d-1}} \right),
\end{equation*}
where the coefficient $c$ is equal to
\begin{equation*}
    c = \frac{\Gamma \left( d/2 - 1 \right)}{2 \pi^{d/2}} \sum_{[q] \in Q/\Zd} z(\beta , q) \E \left[ \cos(\phi , q) \right] \left( n_q \right)^2.
\end{equation*}
The proof of Proposition~\ref{prop:propmun1246} is complete.



REMOVING THE CONTRIBUTION OF THE COSINE

By Proposition REF, to prove Theorem REF it is sufficient to prove the identity: there exists two constants $c_0, c_1 \in \R$ such that
\begin{equation*}
    \left\langle Y_0 X_x \right\rangle_{\mu_\beta} = c_0 + \frac{c_1}{|x|^{d-2}} + O \left( \frac{1}{|x|^{d-2+ \alpha}}. \right)
\end{equation*}
The first-order term $c_0$ in the expansion REF can be heuristically determined: by sending $x$ to infinity, the random variables $Y_0$ and $X_x$ becomes independent and this implies
\begin{equation*}
    \lim_{x \rightarrow \infty} \left\langle Y_0 X_x \right\rangle_{\mu_\beta} = \left\langle Y_0 \right\rangle_{\mu_\beta} \left\langle X_0 \right\rangle_{\mu_\beta},
\end{equation*}
since, by translation invariance of the measure $\mu_\beta$, the expectation $\left\langle X_x \right\rangle_{\mu_\beta}$ does not depend on the point $x$ and is equal to $\left\langle X_0 \right\rangle_{\mu_\beta}$. This allows to identify the value of $c_0$ and we expect to have $c_0 = \left\langle Y_0 \right\rangle_{\mu_\beta} \left\langle X_0 \right\rangle_{\mu_\beta}$. As a consequence, the expansion REF can be rewritten
\begin{equation*}
    \cov \left[ X_x , Y_0 \right] = \frac{c_1}{|x|^{d-2}} + O \left( \frac{1}{|x|^{d-2 + \alpha}} \right).
\end{equation*}
To prove this result, we appeal to the Helffer-Sjostrand representation formula and write the covariance in the following form
\begin{equation*}
     \cov \left[ X_x , Y_0 \right] = \sum_{y \in \Zd} \left\langle \left(\partial_y  X_x\right) w(y, \cdot ) \right\rangle_{\mu_\beta},
\end{equation*}
where $w$ is the solution of the Helffer-Sjostrand equation, for each $(x , \phi) \in \Zd \times \Omega$,
\begin{equation} \label{def.wVill}
    \mathcal{L}w(y , \phi) = \partial_y Y_0.
\end{equation}

Preuve de l'estimee sur le terme d'erreur

We decompose the proof into two steps.
\begin{itemize}
    \item In Step 1, we prove the convergence
    \begin{equation*}
        \lim_{x \to \infty} \frac{1}{G(0,x)} \sum_{\kappa \in \Zd} G \left(x - \kappa \right) \mathcal{E}_{q_1 , q_2}\left( \kappa \right) = K
    \end{equation*}
    \item In Step 2, we prove the expansion REF.
\end{itemize}

\textit{Step 1.} To prove the convergence REF, define the exponent $\delta = \frac{\alpha}2$. By the assumption of the proposition, it satisfies the inequalities $\ep \leq \delta \leq \alpha$. We then split the sum REf into two terms according to the formula
\begin{equation*}
    \sum_{\kappa \in \Zd} G \left( x - \kappa \right) \mathcal{E}_{q_1,q_2} \left( \kappa \right) = \sum_{\kappa \in \Zd \setminus B\left(x , |x|^{1-\delta}\right)} G \left( x - \kappa \right) \mathcal{E}_{q_1,q_2} \left( \kappa \right) + \sum_{\kappa \in B(x , |x|^{1-\delta}} G \left( x - \kappa \right) \mathcal{E}_{q_1,q_2} \left( \kappa \right)
\end{equation*}
and estimate the two terms in the right side of REF separately. We first focus on the second term in the right side of REf and prove that it converges to $0$. We quantify the statement and prove the inequality
\begin{equation*}
    \sum_{\kappa \in B \left(x , |x|^{1-\delta} \right)} G \left( x - \kappa \right) \mathcal{E}_{q_1,q_2} \left( \kappa \right) \leq \frac{C}{|x|^{d - 2 +\delta - \ep}}.
\end{equation*}
The proof of this result relies on the following ingredients
\begin{itemize}
    \item The inequality REF;
    \item The fact that the Green's matrix $G$ can be bounded from above by the value $C|x|^{2-d}$;
    \item The observation, for each $x \in \Zd$ large enough and each $\kappa$ in the ball $B(x , |x|^{1-\delta})$, one can bracket the norm of $\kappa$ between the two values $\frac{|x|}{2}$ and $2 |x|$, i.e., we have $\frac{|x|}{2} \leq |\kappa| \leq 2|x|$.
\end{itemize}
We then compute
\begin{align*}
    \left| \sum_{\kappa \in B \left(x , |x|^{1-\delta} \right)} G \left( x - \kappa \right) \mathcal{E}_{q_1,q_2} \left( \kappa \right) \right|  \leq \frac{C}{|x|^{d - \ep}} \sum_{\kappa \in B \left(x , |x|^{1-\delta} \right)} G(x - \kappa) & \leq \frac{C}{|x|^{d - \ep}} \sum_{\kappa \in B \left(0 , |x|^{1-\delta} \right)} G(\kappa)\\
    & \leq \frac{C}{|x|^{d - \ep}} \sum_{\kappa \in B \left(0 , |x|^{1-\delta} \right)} \frac{1}{|\kappa|^{d-2}} \\
    & \leq \frac{C}{|x|^{d - 2 + 2 \delta - \ep}}.
\end{align*}
Using the assumption $\delta \geq \ep$ completes the proof of the estimate REF. We then focus on the on the first term in the right side of REF. The proof relies on the dominated convergence Theorem with the observations
\begin{itemize}
    \item One has the upper bounds: there exists a constant $C > 0$ such that for every $x \in \Zd$ and every $\kappa \in \Zd$,
    \begin{equation*}
        \frac{G \left( x- \kappa \right)}{G(x)} |\kappa|^{-\delta} \indc_{\kappa \in B \left( x , |x|^{1-\delta} \right)} \leq C;
    \end{equation*}
    \item One has the pointwise bound, for each $\kappa \in \Zd$,
    \begin{equation*}
        \frac{G \left( x- \kappa \right)}{G(x)} |\kappa|^{-\delta} \indc_{\kappa \in B \left( x , |x|^{1-\delta} \right)} \underset{x \to \infty}{\longrightarrow} 1.
    \end{equation*}
    \item Using the assumption REF, one has for each integer $n \in \N$,
    \begin{equation*}
        2^{n\delta} \sum_{\kappa \in A_n} \left| \mathcal{E}_{q_1,q_2}(\kappa) \right| \leq 2^{-n (\alpha - \delta)} \leq 2^{-n \frac{\alpha}2}.
    \end{equation*}
    This implies that the map $\kappa \mapsto \left| \kappa \right|^\delta \mathcal{E}_{q_1,q_2}(\kappa)$ is summable, i.e.,
    \begin{equation*}
        \sum_{\kappa \in \Zd} |\kappa|^{\delta} \left|\mathcal{E}_{q_1,q_2}(\kappa) \right| < \infty.
    \end{equation*}
\end{itemize}
By a combination of the three previous ingredients, we can apply the dominated convergence theorem and obtain
\begin{equation*}
    \frac{1}{G(x)}\sum_{\kappa \in \Zd \setminus B (x , |x|^{1-\delta})} G \left( x - \kappa \right) \mathcal{E}_{q_1,q_2} \left( \kappa \right) \underset{x \to \infty}{\longrightarrow} K.
\end{equation*}
Combining the convergence REF with the identity REf and the upper bound REF, we deduce 
\begin{equation*}
    \frac{1}{G(x)}\sum_{\kappa \in \Zd} G \left( x - \kappa \right) \mathcal{E}_{q_1,q_2} \left( \kappa \right) \underset{x \to \infty}{\longrightarrow} K.
\end{equation*}
The proof of Step 1 is complete.

\medskip

\textit{Step 2.}



\textit{Estimate for the term $\mathcal{V}_{\mathrm{der},1}$.}
We first express the function $\mathcal{V}_{\mathrm{der},1}$ in terms of the Greens function $\mathcal{G}$. We have
\begin{equation*}
    \delta H_{1,y}(z , \phi) = \sum_{z_1 \in \Zd} \int_{\Omega} \delta_z \delta_{z_1} \mathcal{G} \left( z , \phi ; z_1 , \psi \right) \left( \sum_{q \in \mathcal{Q}} z(\beta , q) \left( \sin(\psi , q) \sin(\sigma_x  , q)  \right) n_q(y) n_q(z_1) \right) \delta v(y , \psi)
\end{equation*}
Using the estimate REf on the derivative of the Green's matrix $\mathcal{G}$, the estimate REF on the $L^p\left( \mu_\beta \right)$-norm of the function $v(y,\cdot)$ and the pointwise estimate, for each $(y,\phi) \in \Zd \times \Omega$,
\begin{equation*}
    \left( \sum_{q \in \mathcal{Q}} z(\beta , q) \left( \sin(\psi , q) \sin(\sigma_x  , q)  \right) q(y) n_q(z_1) \right) \leq C e^{-c \beta \left| y - z_1 \right|} \frac{1}{|x - y|^{d-1}},
\end{equation*}
we obtain
\begin{align*}
    \left\| \nabla H_{1,y}(z , \cdot) \right\|_{L^p \left( \mu_\beta \right)} & \leq \sum_{z_1 \in \Zd} C e^{-c \beta \left| y - z_1 \right|} \frac{1}{|z - z_1|^{d-\ep}} \frac{1}{|x - y|^{d-1}} \frac{1}{|y|^{d-1-\ep}} \\
    & \leq \frac{C}{|z-y|^{d- \ep} \times |x-y|^{d-1 - \ep}\times |y|^{d-1-\ep}}.
\end{align*}


We first express the function $w_3$ in terms of the Green function $\mathcal{G}_{\mathrm{der}}$. We obtain
\begin{multline*}
   w_3 \left(y , z, \phi \right) = - \sum_{y_1 , z_1 \in \Zd} \int_\Omega  \delta_{y_1} \delta_{z_1} \mathcal{G}_{\mathrm{der}} \left( y , z , \phi ; y_1 , z_1 , \psi \right) \\ \times n_{Q_0}(y_1) \left(n_{Q_0}(z_1)  + \frac12 \sum_q z \left( \beta , q \right) \sin(\psi, q) \left( \cos (\sigma_0 , q) - 1 \right) n_q(z_1) \right) Y_0(\psi) \mu_\beta(d \psi).
\end{multline*}
We then use the bound on the mixed derivative of the Green's matrix $\mathcal{G}_{\mathrm{der}}$ stated in REF, the fact that the random variable $Y_0$ belongs to the space $L^p\left( \mu_\beta \right)$ and the pointwise estimates, for each $(y ,z , \phi) \in \Zd \times \Zd \times \Omega$,
\begin{equation*}
    \left| Q_0(y) \right| \leq \frac{C}{|y|^{d-1}} ~\mbox{and}~  \left| \sum_q z \left( \beta , q \right) \sin(\psi, q) \left( \cos (\sigma_0 , q) - 1 \right) q(z) \right| \leq \frac{C}{|z|^{2d-2}}.
\end{equation*}
We obtain
\begin{align*}
    \left\|  w_3 \left(y , z, \cdot \right) \right\|_{L^p \left( \mu_\beta \right)} & \leq C \sum_{y_1, z_1} \frac{1}{\left(|y - y_1|^{2d +1 - \ep} + |z - z_1|^{2d+ 1 - \ep} \right) \times |y_1|^{d-1} \times |z_1|^{d-1}} \\
    & \leq \frac{C}{|y|^{d-1} \times |z|^{d-1}}.
\end{align*}
\ww{To do: use $C^{0,1-\ep}$ estimate to obtain a better bound for $\delta_y w_3$} Multiplying the term by the value $n_{Q_x}(y)$ and applying the pointwise bound REf shows
\begin{equation*}
    \left\| n_{Q_x}(y) \delta_y w_2 \left( y,z,\phi\right) \right\|_{L^p \left( \mu_\beta \right)} \leq \frac{C}{|x-y|^{d-1} \times |y|^{d-1} \times |z|^{d-1}}.
\end{equation*}
We can then express the function $H_{3,y}$ in terms of the Green function $\mathcal{G}$. We obtain
\begin{equation*}
        \delta H_{3,y}(z , \phi) = \sum_{z_1 \in \Zd} \int_\Omega \delta_z \mathcal{G} \left( z , \phi ; z_1 , \psi \right) n_{Q_x}(y) \delta_y w_3 \left( y,z,\phi\right) \mu_\beta \left( d \psi\right).
\end{equation*}
The integral REf can be estimated thanks to the estimate REF on the derivative of the Green function $\mathcal{G}$ and the estimate REF. We obtain
\begin{align*}
    \left|\nabla H_{3,y}(z , \phi) \right| &\leq \sum_{z_1 \in \Zd} \frac{C}{|z - z_1|^{d-1-\ep}\times|x-y|^{d-1} \times |y|^{d-1} \times |z_1|^{d-1}} \\
    & \leq \frac{C}{|z |^{d-2-\ep}\times|x-y|^{d-1} \times |y|^{d-1}}.
\end{align*}





USING THE ROTATION INVARIANCE OF THE MODEL

\iffalse
\begin{proof}
We let $u: \Zd \to \R$ be the heat kernel associated to the discrete triharmonic heat equation
\begin{equation*}
   \left\{ \begin{aligned}
   \partial_t u + (- \Delta )^3 u &= 0 ~\mbox{in}~ (0, \infty) \times \Zd, \\
   u(0 , \cdot) &= \delta_0 ~\mbox{in}~ \Zd.
   \end{aligned} \right.
\end{equation*}
We let $\bar u(\xi) := \sum_{x \in \Zd} u(x) e^{i x \cdot \xi}$ be the discrete Fourier transform of $u$. It satisfies the equation, for each $\xi \in \Rd$,
\begin{equation*}
    \left\{ \begin{aligned}
   \partial_t u(\cdot , \xi) + \left( 2 \sum_{i=1}^d \left( 1- \cos \xi_i \right)\right)^3 u(\cdot , \xi) &= 0 ~\mbox{in}~ (0, \infty) , \\
   u(0 , \xi) &= 1,
   \end{aligned} \right.
\end{equation*}
which implies the explicit formula 
\begin{equation*}
    \forall (t , \xi) \in [0, \infty) \times \Rd, \hat u(t , \xi) = \exp \left( - t \left( 2 \sum_{i=1}^d \left( 1- \cos \xi_i \right)\right)^3 \right),
\end{equation*}
and consequently
\begin{equation*}
    bla    
\end{equation*}
\end{proof}
\fi


\iffalse

\begin{proposition} \label{prop:symmetriesGreenFourier}
Let $G$ be the standard Green's function on the lattice $\Zd$ in dimension $d \geq 3$. Then there exists a constant $c := c(d) \in \R$ such that for any pair of integers $i,j \in \{1 , \ldots, d \}$, one has the expansion
\begin{equation} \label{eq:TV13353}
    \sum_{h \in H} \sum_{y \in \Zd} \nabla_i G(y) \nabla_j G(y - h(x)) =
     \left\{ \begin{aligned}
    \frac{c}{|x|^{d-2}} + O \left( \frac{C}{|x|^{d-1}} \right) &~\mbox{if}~ i=j, \\
    O \left( \frac{C}{|x|^{d-1}} \right) &~\mbox{otherwise}.
    \end{aligned} \right.
\end{equation}
%Moreover, given any collection of coefficients $\left( c_{i,j} \right)_{1 \leq i,j \leq d}$, one has the expansion
%\begin{equation} \label{eq:TV06591}
 %   \sum_{h \in H} \sum_{i, i_1,j, j_1=1}^d c_{i,i_1} c_{j , j_1} \sum_{y,\kappa \in \Zd} \nabla_i G(y) \nabla_j G( y - \kappa - x)  \nabla_{i_1} \nabla_{j_1} G(\kappa) = \frac{c}{|x|^{d-2}} + O \left( \frac{C}{|x|^{d-1}} \right).
%\end{equation}
\end{proposition}

\begin{proof}
The proof uses an explicit formula for the Green's function and relies on the discrete Fourier transform. Let us try to construct the Green's function $G$ by Fourier transform. Given a function $F: \Zd \to \R$ which decays sufficiently fast at infinity, we define its discrete Fourier transform according to the formula, for each $\xi = \left( \xi_1 , \ldots, \xi_d \right) \in \Rd$,
\begin{equation*}
    \hat F (\xi) = \sum_{z \in \Zd} F(z) e^{-i\xi \cdot z}.
\end{equation*}
Then we have $\widehat{\Delta F} (\xi) = 2 \sum_{i=1}^d \left( \cos \xi_i - 1 \right) \hat F(\xi)$. Applying this formula to the Green's function $G$, we formally obtain that $\hat G = \left(2 \sum_{i=1}^d \left( \cos \xi_i - 1 \right)\right)^{-1}$. Applying the inverse Fourier transform, we formally obtain the formula, for each $z \in \Zd$,
\begin{equation} \label{eq:TV13013}
    G (z) = \frac{1}{\left( 2\pi\right)^d}\int_{[0,2\pi]^d} \frac{e^{i\xi \cdot z}}{2 \sum_{i=1}^d \left( \cos \xi_i - 1 \right)} \di \xi.
\end{equation}
One can then prove the formula~\eqref{eq:TV13013} rigorously. First, it is clear that the integral~\eqref{eq:TV13013} converges absolutely in dimension larger than $3$ and that it is bounded as a function of the variable $z$; one can then verify by an explicit computation that the discrete Laplacian in the variable $z$ of the integral~\eqref{eq:TV13013} is equal to the Dirac $\delta_0$. This argument provides a rigorous justification of the identity~\eqref{eq:TV13013}.

Once the formula~\eqref{eq:TV13013} is established, we obtain the identity for the gradient of the function $G$: for each integer $\left\{ 1 , \ldots,d \right\}$,
\begin{equation*}
    \nabla_i G (z) = \frac{1}{\left( 2\pi\right)^d}\int_{[0,2\pi]^d} \frac{\left( e^{i \xi_i} - 1\right)e^{i\xi \cdot z}}{2 \sum_{i=1}^d \left( \cos \xi_i - 1 \right)} \di \xi.
\end{equation*}
Using that the discrete Fourier transform turns discrete convolution into products, we obtain the formula
\begin{equation*}
    \sum_{y \in \Zd} \nabla_i G(y) \nabla_j G(y - x) = \frac{1}{\left( 2\pi\right)^d}\int_{[0,2\pi]^d} \frac{\left( e^{i \xi_i} - 1\right)\left( e^{-i \xi_j} - 1\right)e^{i\xi \cdot x}}{\left(2 \sum_{i=1}^d \left( \cos \xi_i - 1 \right)\right)^2} \di \xi.
\end{equation*}
We now prove the formula~\eqref{eq:TV13353}. We prove the identity, for each $h \in H$,
\begin{equation} \label{eq:TV13393}
    \sum_{y \in \Zd} \nabla_i G(y) \nabla_j G(y - h(x)) = \frac{1}{\left( 2\pi\right)^d}\int_{[0,2\pi]^d} \frac{\left( e^{i h(\xi) \cdot e_i} - 1\right)\left( e^{-i h(\xi) \cdot e_j} - 1\right)e^{i\xi \cdot x}}{\left(2 \sum_{i=1}^d \left( \cos \xi_i - 1 \right)\right)^2} \di \xi.
\end{equation}
We establish the formula~\eqref{eq:TV13393} for the functions $\left(h_i\right)_{1 \leq i \leq d}$ and $\left(h_{ij}\right)_{1\leq i,j \leq d} $: in that case the proof is simple and is obtained by a change of variable. For a general element $h \in H$, we use that every element $h$ of the group $H$ can be written a composition of a finite numbers of elements of the collections $\left( h_i \right)_{i = 1 , \cdots, d}$ and $\left( h_{ij} \right)_{1 \leq i < j \leq d}$ to obtain the result.

\smallskip

We prove the formula~\eqref{eq:TV13353} in the case $i=j$. We have
\begin{equation} \label{eq:TV14453}
    \sum_{h \in H} \left( e^{i h(\xi) \cdot e_i} - 1\right) \left( e^{ - i h(\xi) \cdot e_i} - 1\right) = - 2 \sum_{h \in H} \left( \cos (h(\xi) \cdot e_i) - 1 \right)= - \frac{2 \left|H \right|}{d} \sum_{k=1}^d \left( \cos (\xi_k) - 1 \right),
\end{equation}
where we used that, for each integer $k \in \{ 1 , \ldots , d\}$ and each $\xi \in \Rd$,
\begin{equation*}
    \left| \left\{ h \in H \, : \, h(\xi) \cdot e_i = \xi_k ~ \mbox{or}~ h(\xi) \cdot e_i = -\xi_k  \right\} \right| = \frac{|H|}{d}.
\end{equation*}
Combining the formula~\eqref{eq:TV14453} with the identity~\eqref{eq:TV13393}, we obtain that
\begin{align*}
    \frac{1}{|H|}\sum_{h \in H}\sum_{y \in \Zd} \nabla_i G(y) \nabla_j G(y - h(x)) & = \frac{1}{|H| \left( 2\pi\right)^d}\int_{[0,2\pi]^d} \sum_{h \in H} \frac{\left( e^{i h(\xi) \cdot e_i} - 1\right)\left( e^{-i h(\xi) \cdot e_j} - 1\right)e^{i\xi \cdot x}}{2 \sum_{i=1}^d \left( \cos \xi_i - 1 \right)} \di \xi \\
    & = \frac{-1}{d\left( 2\pi\right)^d}\int_{[0,2\pi]^d}  \frac{2\sum_{k=1}^d \left( \cos (\xi_k) - 1 \right)e^{i\xi \cdot x}}{\left(2 \sum_{i=1}^d \left( \cos \xi_i - 1 \right)\right)^2} \di \xi \\
    & = \frac{-1}{d\left( 2\pi\right)^d}\int_{[0,2\pi]^d}  \frac{e^{i\xi \cdot x}}{2 \sum_{i=1}^d \left( \cos \xi_i - 1 \right)} \di \xi \\
    & = - \frac{1}{d} G(x).
\end{align*}
We then complete the proof by noting that, by standard arguments, there exists a constant $c := c(d)$ such that $ - \frac{|H|}{d} G(x) = \frac{c}{|x|^{d-2}}+ O \left( \frac{C}{|x|^{d-1}} \right)$.

\medskip

We prove the formula~\eqref{eq:TV13353} in the case $i\neq j$. In that case, by summing over all the symmetries of the lattice, we have
\begin{equation*}
    \frac{1}{|H|}\sum_{h \in H} \left( e^{i h(\xi) \cdot e_i} - 1\right) \left( e^{ - i h(\xi) \cdot e_i} - 1\right) = \frac{4}{d(d-1)} \sum_{1 \leq k < l \leq d} \left( \cos \xi_k - 1\right) \left( \cos \xi_l - 1 \right).
\end{equation*}
Combining the formula~\eqref{eq:TV14453} with the identity~\eqref{eq:TV13393}, we obtain that
\begin{equation} \label{eq:TV15283}
    \frac{1}{|H|}\sum_{h \in H}\sum_{y \in \Zd} \nabla_i G(y) \nabla_j G(y - h(x)) = \frac{1}{\left( 2\pi\right)^d}\int_{[0,2\pi]^d} \frac{\sum_{1 \leq k < l \leq d} \left( \cos \xi_k - 1\right) \left( \cos \xi_l - 1 \right) e^{i\xi \cdot x}}{\left(2 \sum_{i=1}^d \left( \cos \xi_i - 1 \right)\right)^2} \di \xi.
\end{equation}
There only remains to prove that the integral on the right side of~\eqref{eq:TV15283} can be bounded from above by the value $C |x|^{1-d}$. To this end, we introduce the function $f$ defined by the formula, for each $\xi \in (0, 2\pi)^d$,
\begin{equation*}
    f (\xi) := \frac{\sum_{1 \leq k < l \leq d} \left( \cos \xi_k - 1\right) \left( \cos \xi_l - 1 \right)}{\left(2\pi \right)^d\left(2 \sum_{i=1}^d \left( \cos \xi_i - 1 \right)\right)^2}.
\end{equation*}
The identity~\eqref{eq:TV15283} can be rewritten in this notation
\begin{equation} \label{eq:TV17283}
     \frac{1}{|H|}\sum_{h \in H}\sum_{y \in \Zd} \nabla_i G(y) \nabla_j G(y - h(x)) = \int_{[0,2\pi]^d} f(\xi) e^{i\xi \cdot x} \di \xi.
\end{equation}
One can then compute explicitly the iterated gradients of the function $f$; we do not write the explicit formula, but note that for each integer $k \in \{ 1 , \ldots, d \}$, there exists a constant $C := C(d,k) < \infty$ such that
\begin{equation} \label{eq:TV17213}
    \left| \nabla^k f(\xi) \right| \leq \frac{C}{|\xi|^k}.
\end{equation}
This inequality can be used to perform integration by parts; indeed since the function $\xi \to |\xi|$ is integrable in around the point $0$ in $\Rd$, one can perform an the integration by parts with respect to the variable $\xi_1$. We obtain
\begin{equation*}
    \int_{[0,2\pi]^d} f(\xi) e^{i\xi \cdot x} \di \xi = \frac{-1}{i x_1}\int_{[0,2\pi]^d} \partial_{x_1} f(\xi) e^{i\xi \cdot x} \di \xi.
\end{equation*}
Since the function $\xi \to |\xi|^k$ is integrable around the point $0$ for each integer $k$ smaller than $d-1$, we can iterate the previous reasoning $(k-1)$ times. We obtain
\begin{equation} \label{eq:TV17243}
    \int_{[0,2\pi]^d} f(\xi) e^{i\xi \cdot x} \di \xi = \left( \frac{-1}{i x_1} \right)^{d-1} \int_{[0,2\pi]^d} \partial_{x_1}^{d-1} f(\xi) e^{i\xi \cdot x} \di \xi.
\end{equation}
Using the estimate~\eqref{eq:TV17213} and that the function $\xi \to |\xi|^{1-d}$ is integrable around $0$, we can bound the right side of the identity~\eqref{eq:TV17243}. We obtain
\begin{equation} \label{eq:TV17273}
    \int_{[0,2\pi]^d} f(\xi) e^{i\xi \cdot x} \di \xi \leq \frac{C}{|x_1|^{d-1}}.
\end{equation}
We can also perform the same the integrations by parts in the variables $\xi_2 , \ldots , \xi_d$ (instead of $\xi_1$). We obtain, for each integer $i \in \{1, \ldots , d\}$,
\begin{equation*}
    \int_{[0,2\pi]^d} f(\xi) e^{i\xi \cdot x} \di \xi \leq \frac{C}{|x_i|^{d-1}}.
\end{equation*}
This argument leads to the inequality
\begin{equation*}
    \int_{[0,2\pi]^d} f(\xi) e^{i\xi \cdot x} \di \xi \leq \min \left( \frac{C}{|x_1|^{d-1}} , \ldots ,  \frac{C}{|x_d|^{d-1}} \right) \leq \frac{C}{|x|^{d-1}}.
\end{equation*}
Combining the estimate~\eqref{eq:TV17273} with the identity~\eqref{eq:TV17283}, we deduce that
\begin{equation*}
    \left| \frac{1}{|H|}\sum_{h \in H}\sum_{y \in \Zd} \nabla_i G(y) \nabla_j G(y - h(x)) \right| \leq \frac{C}{|x|^{d-1}}.
\end{equation*}
The proof is complete.
\end{proof}
It only remains to prove~\eqref{eq:TV06591}. Using the same argument as the ones developed for the expansion~\eqref{eq:TV13353}, we obtain the formula
\begin{equation*}
    \sum_{y,\kappa \in \Zd} \nabla_i G(y) \nabla_j G( y - \kappa - x)  \nabla_{i_1} \nabla_{j_1} G(\kappa) = \frac{1}{\left( 2\pi\right)^d}\int_{[0,2\pi]^d} \frac{\left( e^{i \xi_i} - 1\right)\left( e^{-i \xi_{i_1}} - 1\right)\left( e^{i \xi_j} - 1\right) \left( e^{-i \xi_{j_1}} - 1\right)e^{i\xi \cdot x}}{\left(2 \sum_{i=1}^d \left( \cos \xi_i - 1 \right)\right)^4} \di \xi,
\end{equation*}
and for each lattice preserving transformation $h \in H$,
\begin{multline*}
    \sum_{y,\kappa \in \Zd} \nabla_i G(y) \nabla_j G( y - \kappa - h(x))  \nabla_{i_1} \nabla_{j_1} G(\kappa) \\ = \frac{1}{\left( 2\pi\right)^d}\int_{[0,2\pi]^d} \frac{\left( e^{i h(\xi_i)} - 1\right)\left( e^{-i h(\xi_{i_1})} - 1\right)\left( e^{i h(\xi_j)} - 1\right) \left( e^{-i h(\xi_{j_1})} - 1\right)e^{i\xi \cdot x}}{\left(2 \sum_{i=1}^d \left( \cos \xi_i - 1 \right)\right)^4} \di \xi,
\end{multline*}
We then note that we have the factorization
\begin{align*}
    \lefteqn{\sum_{i, i_1,j, j_1=1}^d c_{i,i_1} c_{j , j_1} \left( e^{i \xi_i} - 1\right)\left( e^{-i \xi_{i_1}} - 1\right)\left( e^{i \xi_j} - 1\right) \left( e^{-i \xi_{j_1}} - 1\right)} \qquad & \\& = \left( \sum_{i, i_1=1}^d c_{i,i_1}\left( e^{i \xi_i} - 1\right)\left( e^{-i \xi_{i_1}} - 1\right) \right) \left( \sum_{j, j_1=1}^d c_{j , j_1} \left( e^{i \xi_j} - 1\right) \left( e^{-i \xi_{j_1}} - 1\right)\right) \\
    & = \left( \sum_{i, i_1=1}^d c_{i,i_1}\left( e^{i \xi_i} - 1\right)\left( e^{-i \xi_{i_1}} - 1\right) \right)^2.
\end{align*}

\fi



More precisely, for each integer $i \in \{1 , \ldots, d\}$, we denote by $h_i$ the reflection of the lattice $\Zd$ with respect to the hyperplane $\left\{ z \in \Zd \, : \, z_i = 0 \right\}$, i.e.,
\begin{equation*}
    h_i := \left\{ \begin{aligned}
    \Zd &\to  \Zd \\
    (z_1 , \ldots, z_d) & \mapsto  (z_1 , \ldots, - z_i , \ldots,  z_d).
    \end{aligned}
    \right.
\end{equation*}
We then let $H$ be the group generated by the elements $\left( h_i\right)_{i \in \{1 , \ldots, d \}}$ for the composition law; it is a finite group of cardinality $2^d$. We then have
\begin{equation} \label{eq:TV06560}
    \forall h \in H, \hspace{2mm} \sum_{y \in \Zd} \left\langle Q_{h(x)}(y) \mathcal{U}(y, \cdot ) \right\rangle_{\mu_\beta} = \sum_{y \in \Zd} \left\langle Q_{x}(y) \mathcal{U}(y, \cdot ) \right\rangle_{\mu_\beta}.
\end{equation}
From the identity~\eqref{eq:TV06560}, we deduce that
\begin{equation} \label{eq:TV06401}
    \sum_{y \in \Zd} \left\langle Q_{h(x)}(y) \mathcal{U}(y, \cdot ) \right\rangle_{\mu_\beta} = 2^{-d} \sum_{h \in H}\sum_{y \in \Zd} \left\langle Q_{h(x)}(y) \mathcal{U}(y, \cdot ) \right\rangle_{\mu_\beta}.
\end{equation}
This symmetry provides some additional information which can be used to simplify the expansion~\eqref{eq:TV07030}. Using standard arguments about the discrete Green's function $G$, one can prove the following expansions, for each quadruplet $(i , j , k , l) \in \{ 1 , \ldots, d \}^4$ \wwcomment{fixed a typo in the first one, please check}
\begin{equation} \label{eq:TV06581}
    2^{-d} \sum_{h \in H} \sum_{y,\kappa \in \Zd} \nabla_i G( y) \nabla_j G(\kappa - h(x) - y ) = \left\{ \begin{aligned}
    \frac{c}{|x|^{d-2}} + O \left( \frac{C}{|x|^{d-1}} \right) &~\mbox{if}~ i=j \\
    O \left( \frac{C}{|x|^{d-1}} \right) &~\mbox{otherwise}
    \end{aligned} \right.
\end{equation}
and
\begin{equation} \label{eq:TV06591}
    2^{-d} \sum_{h \in H} \sum_{i, i_1,j, j_1=1}^d c_{i,i_1} c_{j , j_1} \sum_{y,\kappa \in \Zd} \nabla_i G(y) \nabla_j G( y - \kappa - h(x))  \nabla_{i_1} \nabla_{j_1} G(\kappa) = \frac{c}{|x|^{d-2}} + O \left( \frac{C}{|x|^{d-1}} \right).
\end{equation}
The proof of the expansions~\eqref{eq:TV06581} and~\eqref{eq:TV06591} relies on a discrete Fourier transform and exploits the symmetries of the lattice to simplify the first-order term of the expansion; it is deferred to Lemma~\ref{lem:lemma4.1chap8} of Chapter \ref{section7}.
A combination of the identities~\eqref{eq:TV07030}, ~\eqref{eq:TV06401},~\eqref{eq:TV06581} and~\eqref{eq:TV06591} completes the proof of~\eqref{eq:TV09355}.



MOST USEFUL PIECE OF CODE

$\sum_{\substack{q\in \mathcal{Q}_{\cu_{2^{k+1}R}} \setminus \mathcal{Q}_{\cu_{2^{k}R}}: \\ \supp q \cap (\cu_{2^{k+1}R} \setminus \cu_{2^{k}R}) \neq \emptyset}} z(\beta , q) \cos 2\pi(\phi , q) \left( \cos 2\pi(\sigma_{0x} , q) - 1  \right)}$


SECTION 6

\pd{Section 6 commented out as we discussed, a few references were in there.}
\iffalse
\section{Positivity} \label{section6chap4.l.}

In this section we derive Theorem \ref{t.main} from Theorem \ref{thm.expdualVil}, and conclude all constants in the statement of Theorem \ref{t.main}  are strictly positive and uniformly bounded in $\beta$. Recall that, the Green's function for simple random walk on $\Zd$ has the asymptotics
\begin{equation*}
\Delta^{-1}(0,x) = \frac{C_d}{|x|^{d-2}} + O\left(\frac{C}{|x|^d}\right),
\end{equation*}
where 
\begin{equation*}
C_d = \frac{d\Gamma(d/2)}{(d-2) \pi^{d/2}}.
\end{equation*}
 Combining Theorem \ref{thm.expdualVil} and Proposition \ref{p.FS} (proved in \cite{FS4d}), we conclude that 
\begin{equation*}
%\label{e.2ptmain}
    \left\langle S_0 \cdot S_x \right\rangle_{\mu^{V}_\beta} =
    \langle S_0 \rangle_{\mu^{V}_\beta} \langle S_x \rangle_{\mu^{V}_\beta}+ \frac{c_3}{|x|^{d-2}}+ O\left(\frac{C}{|x|^{d-2+\alpha}}\right),
 \end{equation*}
 where $c_3 = c_3 (d, \beta)$ admit the  low temperature expansion $c_3 = 
\frac {c'_3 }{\beta} + o(\frac 1\beta)$, with $c'_3 = c'_3 (d, \beta)\in [\frac12 C_d, C_d]$ uniformly for all large $\beta$. 

We now show that one can also keep track of the $\beta$ dependence in the constants for the low temperature expansion of the transversal and longitudinal correlations. We need the following a-priori bound for $\left\langle \exp(i(\theta_0 + \theta_x)) \right\rangle_{\mu^{V}_\beta}$, which can be proved using Jensen's inequality as in \cite{FS4d} and \cite{Bau}. 

\begin{lemma}
\label{l.apriori}
There exist constants $\beta_0 := \beta_0 (d)$, and $c=c(\beta)$, such that $c(\beta)= o(\frac 1\beta)$ as $\beta \to \infty$, and for every $\beta > \beta_0$, and every $x \in \Zd$,
\begin{equation*}
   1\geq \frac{Z \left(\bar \sigma_{0x} \right)}{Z(0)} \geq \exp \left(-c(\beta) (\indc_0+\indc_x, \Delta^{-1}(\indc_0+\indc_x) ) \right).
\end{equation*}
Consequently \pdcomment{I did the computation and did not obtain exactly the same result, for me the RHS should be like $\left( \frac1\beta -c(\beta) \right)\Delta^{-1}(0,0) + \left(\frac{1}{\beta} -c(\beta)\right) \Delta^{-1}(0,x)$}
\begin{equation*}
   \exp \left( \indc_0 - \indc_x, -\frac1{2\beta} \Delta^{-1}  (\indc_0 - \indc_x) \right) \geq
    \left\langle \exp(i(\theta_0 + \theta_x)) \right\rangle_{\mu^V_{\beta}} 
\geq 
\exp \left(-\frac1\beta \Delta^{-1}(0,0) + \left(\frac{1}{\beta} -c(\beta)\right) \Delta^{-1}(0,x)\right).
\end{equation*}
\end{lemma}

Using the trigonometric identity $\cos x = \frac12(e^{ix} + e^{-ix})$ and $\sin x= \frac1{2i}(e^{ix} - e^{-ix})$, we combine Theorem \ref{thm.expdualVil} and Lemma \ref{l.apriori} (in particular, use that for $\beta$ sufficiently large, $\left\langle \exp(i(\theta_0 + \theta_x)) \right\rangle_{\mu^V_{\beta}}
-  \langle e^{i\theta_0} \rangle_{\mu^{V}_\beta} \langle e^{i\theta_x}\rangle_{\mu^{V}_\beta} \ge 0$) to conclude 
\begin{multline*}
\langle \cos\theta(0)  \cos\theta(x)  \rangle_{\mu^{V}_\beta} - \langle \cos\theta(0) \rangle_{\mu^{V}_\beta}^2  \\
= \frac12  \left\langle \exp(i(\theta_0 - \theta_x)) \right\rangle_{\mu^V_{\beta}}
+  \frac12  \left\langle \exp(i(\theta_0 + \theta_x)) \right\rangle_{\mu^V_{\beta}}
-  \langle e^{i\theta_0} \rangle_{\mu^{V}_\beta} \langle e^{i\theta_x}\rangle_{\mu^{V}_\beta}
= \frac{c_1}{\beta |x|^{d-2}} + O\left(\frac{1}{|x|^{d-2+\alpha}}\right).
\end{multline*}
where $c_1 \in [\frac14 C_d, C_d]$ uniformly for all large $\beta$. Combining with the correlation inequality (see \cite{Dun, KPV})
\begin{equation}
\label{e.corr}
\langle \cos\theta(0)  \cos\theta(x)  \rangle_{\mu^{V}_\beta} - \langle \cos\theta(0) \rangle_{\mu^{V}_\beta}^2 \leq
\langle \sin\theta(0)  \sin\theta(x)  \rangle_{\mu^{V}_\beta},
\end{equation}
we conclude
\begin{equation*}
\langle \sin\theta(0)  \sin\theta(x)  \rangle_{\mu^{V}_\beta}
= \frac{c_2}{\beta |x|^{d-2}} + O\left(\frac{1}{|x|^{d-2+\alpha}}\right),
\end{equation*}
for some $c_2\in [c_1,C_d]$, and therefore completes the proof of Theorem \ref{t.main}. Notice that the correlation inequalities in \cite{Dun, KPV} are originally stated for the classical XY model. However, one may obtain the Villain model as a limit of XY models in which each edge $e\in\Zd$ is occupied by $N$ two-component spins interact with their nearest neighbors (see \cite{FSCoulomb, NW}). By taking the $N\to\infty$ limit we obtain the correlation \eqref{e.corr} for Villain models. 

\begin{proof}[Proof of Lemma \ref{l.apriori}]
The proof is almost identical with the proof of Proposition \ref{p.FS}, which we now sketch. Recall that both $\bar \sigma_{0x}$ and $n_q, q \pd{\in\mathcal{Q}}$ are interger valued, we thus have 
\begin{equation*}
(\bar \sigma_{0x},q) = (\di^*\bar \sigma_{0x},n_q )
= (\di^*\di \Delta^{-1} (h_0 + h_x), n_q )
= (\di\di^* \Delta^{-1} (h_0 + h_x), n_q )
= (\di \Delta^{-1} (\indc_0 + \indc_x), n_q)   \mod 1
\end{equation*}
Thus
\begin{equation*}
\cos (2\pi (\bar \sigma_{0x},q)) = \cos  (2\pi (\di \Delta^{-1} (\indc_0 + \indc_x), n_q)).
\end{equation*}
This implies
\begin{multline*}
|\cos (2\pi (\bar \sigma_{0x},q)) -1| \leq
2\pi^2 (\di \Delta^{-1} (\indc_0 + \indc_x), n_q)^2 \\
\leq 2\pi^2 (n_q, n_q) (\di \Delta^{-1} (\indc_0 + \indc_x),
\di \Delta^{-1} (\indc_0 + \indc_x))
=2\pi^2 (n_q, n_q) (\indc_0 + \indc_x, -\Delta^{-1} (\indc_0 + \indc_x)).
\end{multline*}
Therefore 
\begin{multline*}
\sum_{q \in \mathcal{Q}} \left| z(\beta , q) \cos 2\pi(\phi , q) \left( \cos 2\pi(\bar\sigma_{0x} , q) - 1  \right) \right| \\
\leq 2\pi^2 \sum_{q \in \mathcal{Q}}z(\beta , q) \|n_q\|^2_{L^2} (\indc_0 + \indc_x, -\Delta^{-1} (\indc_0 + \indc_x))
=c(\beta) (\indc_0 + \indc_x, -\Delta^{-1} (\indc_0 + \indc_x)),
\end{multline*}
where
\begin{equation*}
|c(\beta) | \leq C\sum_{q \in \mathcal{Q}}  e^{-c\beta^{1/2}\|q\|_1} \|q\|_1
\end{equation*}
satisfies $c(\beta)= O \left(e^{-c\beta^\frac 12}\right) $ as $\beta \to \infty$. Applying Jensen's inequality to \eqref{e.2ptplus} we obtain \pdcomment{ Can we not replace $\beta^{\frac 12}$ by $\beta$ here? Following Bauerschmidt?}
\begin{multline*}
\log \frac{Z \left(\bar \sigma_{0x} \right)}{Z(0)} \geq 
\left\langle \sum_{q \in \mathcal{Q}} z(\beta , q) \sin 2\pi (\phi , q) \sin 2\pi(\bar\sigma_{0x} , q) + \sum_q z(\beta , q) \cos 2\pi(\phi , q) \left( \cos 2\pi(\bar\sigma_{0x} , q) - 1  \right) \right\rangle_{\mu_\beta}\\
\geq
-c(\beta) (\indc_0 + \indc_x, \Delta^{-1}(\indc_0 + \indc_x) ).
\end{multline*}
\end{proof}
\fi


REST OF THE INTRODUCTION

\section{Rest of the introduction}

Our proof of Theorem \ref{t.main} starts from the insight of Fr{\"o}hlich and Spencer, that the two-point function of the Villain model in $\Zd$, $d\ge 3$ can be mapped, via duality, to a statistical mechanical model of lattice Coulomb gas on the 2-forms $\Lambda^2(\Zd)$. One may then perform a Fourier transform with respect to the charge variable, and obtain a random field representation of the Coulomb gas, known as the sine-Gordon representation. When the temperature is low enough, a one-step renormalization can be carried out and one obtains an effective model which is a small perturbation of a (non-local) Gaussian measure. The Hessian of the effective Hamiltonian is therefore a perturbation of the lattice Laplacian (thus uniformly positive definite), and one can use the insight of Naddaf and Spencer \cite{NS} that the fluctuations of the field are closely related to an elliptic homogenization
problem for the Helffer-Sj{\"o}strand equation \cite{HS, Sj}. Because of the quantitative nature of the question, we adapt and push forward recent ideas in \cite{AW}, that combine the Helffer-Sj{\"o}strand representation with some recent development in the theory of quantitative stochastic homogenization for elliptic equations in divergence-form \cite{AKM, AKMInvent} to obtain quantitative, algebraic rate of convergence of the finite volume
surface tension. Our strategy is therefore based on a multiscale analysis of subadditive quantities to obtain an algebraic rate of convergence of the mixed derivatives of Green's function associated to the Helffer-Sj{\"o}strand equation.

This adaptation of the methods of \cite{AW} is not straightforward since we are dealing with an (infinite order) elliptic operator with infinite range, and the  Helffer-Sj{\"o}strand equation is defined on differential forms. Plus, the statement in Theorem \ref{t.main} requires a precise description of the second order of the expansion. Our analysis relies crucially on the $C^{0,1-\ep}$ regularity theory of the Helffer-Sj{\"o}strand equation and the differentiated Helffer-Sj{\"o}strand equation, developed in Chapter~\ref{section:section4}, which implies quantitative convergence of higher order derivatives of the solution of these equations. 

The proof is based on a duality relation between the low temperature Villain model and a lattice model of Coulomb gas with integer valued and locally neutral charges defined on the faces of the lattice $\Zd$ which originates in~\cite{FS4d}. By performing a Fourier transform with respect to the charge variable, a classical random field representation of the Coulomb gas, known as the sine-Gordon representation is obtained. When the temperature is low enough, a one-step renormalization argument, following the presentation of~\cite{Bau}, can be applied in order to reduce the effective activity of the charges, and obtain an effective, vector-valued random interface model with infinite range and uniformly convex potential. The question of the asymptotic behavior of the two-point function is thus reduced to the question of the quantitative understanding of the large-scale properties of the random interface model. Naddaf and Spencer showed in~\cite{NS} that these properties, in the case of the unifomly convex $\nabla \phi$-interface model, are described by the asymptotic behavior of the solutions of an infinite dimensional and uniformly elliptic operator called the Helffer-Sj\"{o}strand PDE. Their strategy is adapted to the setting of the low temperature dual Villain model studied in this article and a Helffer-Sj\"{o}strand PDE is derived; in particular we prove that to establish the asymptotic decay of the truncated, longitudinal and transversal two-point functions, it is sufficient to obtain quantitative information on the large-scale behavior of the mixed derivative of the Green's function associated to the Helffer-Sj\"{o}strand operator. This is achieved by adapting the techniques of quantitative stochastic homogenization for uniformly elliptic equations in divergence-form developed by Armstrong, Mourrat and Kuusi in~\cite{AKM}.


\iffalse We complete this section by mentioning that in various computations in this article, we need to study the correlation between solutions of the Hellfer-Sj\"{o}strand equation. This is achieved by applying the strategy of Naddaf and Spencer on the Hellfer-Sj\"{o}strand operator~\eqref{introHS}, this operation shows that to study the correlations between solutions of the H-S equation, one needs to understand the behavior of the solutions of the $2d$-dimensional elliptic operator which takes the form
\begin{equation*}
    \Delta_\phi + \mathcal{L}_x + \mathcal{L}_y,
\end{equation*}
where given a map $u : \Z^{2d} \to \R$, the operator 
The properties of this operator are studied in Section~\ref{sec.section4.5} of Chapter~\ref{section:section4}. \fi

\iffalse  To prove~\eqref{eq:TV10010801}, we note that by the first variation
 \begin{equation} \label{eq:TV10020801}
    \forall v \in C^{k}_0 (\cu), ~\left( \di^* w , \di^* v \right)_\cu = \left( q , v \right)_\cu.
 \end{equation}
 We apply the identity with~\eqref{eq:TV10020801} with the form $v = q$ and use that the codifferential is a bounded operator. We obtain
 \begin{equation} \label{eq:TV10260801}
     \left( q , q \right)_\cu =  \left( \di^* w , \di^* q \right)_\cu \leq \left\| \di^* w \right\|_{L^2 \left( \cu \right)}^\frac 12 \left\| \di^* q \right\|_{L^2 \left( \cu \right)}^\frac 12 \leq C \left\| \di^* w \right\|_{L^2 \left( \cu \right)}^\frac 12 \left\|  q \right\|_{L^2 \left( \cu \right)}^\frac 12.
 \end{equation}
 The inequality~\eqref{eq:TV10010801} is a direct consequence of~\eqref{eq:TV10260801}.
 \fi
 
 \iffalse
To state the well-posedness for the Neumann problem, we introduce the set of boundary layer of $\cu$. This is defined as $\cu \setminus \cu^-$, where $\cu^-$ is the trimmed cube defined as follows. 

\begin{lemma}
\label{l.wellposeHS.neu}
Assume that $\beta$ is sufficiently large.  Fix a cube~$\cu$ and $G\in L^2(\cu,\mu_\beta)$ 
There exists a solution $u \in H^1(\cu,\mu_\beta)$ of the boundary-value problem 
\begin{equation}
\label{e.HS.eqn.neu}
\left\{ \begin{aligned}
\Delta_\phi v + \mathcal{L}_{\cu} v & = \di^*G &~\mbox{in}~ \cu \times \Omega,\\
\mathbf{n} \cdot \nabla v & = \mathbf{n} \cdot p &~\mbox{on}~ \partial \cu \times \Omega
\end{aligned} \right.
\end{equation}
satisfying
\begin{equation}
\label{e.neum.meanzero}
\left( v \right)_{\cu,\mu_\beta} = 0,
\end{equation}
where the operator $\mathcal{L}_{\cu}$ is the uniformly elliptic operator defined by the formula 
\begin{equation*}
    \mathcal{L}_{\cu} := - \frac{1}{2 \beta} \Delta +  \frac 1{2\beta}\sum_{n \geq 1} \frac1{\beta^{\frac n2}} \nabla^{n+1} \cdot \left( \indc_{\cu} \nabla^{n+1} \right) + \frac{1}{\beta^{\frac 54}} \nabla \cdot \left(\indc_{\cu \setminus \cu^-} \nabla\right) + \sum_{\di q=0, \supp q \subseteq \cu} \nabla_q \cdot \a_q \nabla_q.
\end{equation*}
Moreover, there exists a constant~$C(d,\beta)<\infty$ such that 
\begin{equation}
\label{e.HSsolest.neu}
|\cu|^{-\frac 1d} \left\| u \right\|_{L^2(\cu,\mu_\beta)}+ \left\llbracket v \right\rrbracket_{H^1(\cu,\mu_\beta)}
\leq 
C \left\| G \right\|_{L^2(\cu,\mu)}. 
\end{equation}
\end{lemma}
\begin{proof}
 A function $u\in H^1(\cu, \mu_\beta)$ is a solution of~\eqref{e.HS.eqn.neu} if and only if  
\begin{multline}
\sum_{y\in \cu} \sum_{x\in \cu} \left\langle (\partial_y u(x,\cdot) )(\partial_yw (x,\cdot) ) \right\rangle_{\mu_\beta}
+
\frac{1}{2\beta}\sum_{e\in E(\cu)} 
\left\langle \nabla u(e,\cdot) \nabla w(e,\cdot)  \right\rangle_{\mu_\beta} 
- \frac{1}{2\beta}\sum_{n \geq 1} \frac{1}{\beta^{ \frac n2}}\sum_{e\in E(\cu)} 
\left\langle   \nabla^{n-1} u(e,\cdot), \nabla^{n-1} w(e,\cdot)  \right\rangle_{\mu_\beta}  
\\
-\frac{1}{\beta^\frac 54}\sum_{e\in E(\cu\setminus \cu^-)} 
\left\langle \nabla u(e,\cdot) \nabla w(e,\cdot)  \right\rangle_{\mu_\beta} 
+
\sum_{\di q=0 ,\, \supp q \cap \cu \neq \emptyset }\left\langle \nabla_q u \cdot \a_q \nabla_q w \right\rangle_{\mu_\beta}  
=
\sum_{e\in E(\cu)}  \left\langle G(e,\cdot) \nabla w(e,\cdot) \right\rangle_{\mu_\beta}, \quad \forall w\in H^1(\cu,\mu_\beta). 
\end{multline} 
For large $\beta$,  the symmetric bilinear form on the left side of the previous display is is a small perturbation of the Laplacian term, and therefore $\left\llbracket u \right\rrbracket_{H^1(\cu,\mu_\beta)}
\leq 
C \left\| G \right\|_{ L^2(\cu,\mu_\beta)}$. Apply Lemma \ref{l.spectralgap.U} (ii), we see that the bilinear form is coercive with respect to the $H^1(\cu,\mu_\beta)$ norm. The
Lax-Milgram lemma therefore yields the existence of a unique solution $u\in H^1(\cu,\mu_\beta)$. It also follows that the solution to \eqref{e.HS.eqn.dir} admits a variational characterization: $v$ minimizes the energy 
\begin{align*}
  \sum_{y \in \Zd} \left\| \partial_y u \right\|_{L^2 \left( \cu , \mu_\beta \right)}^2 +  \frac1{2\beta}  \sum_{n \geq 1} \sum_{\dist \left( x , \partial \cu \right) \geq n} \frac1{\beta^{\frac n2}}\left\| \nabla^n  u(x , \cdot ) \right\|_{L^2 \left( \mu_\beta \right)}^2  - \frac{1}{\beta^{\frac 54}} \left\| \nabla u \right\|_{L^2 \left( \cu \setminus \cu^-, \mu_\beta\right)}^2 \\ -  \sum_{\supp q \subseteq \cu}  \left\langle \nabla_q u \cdot \a_q  \nabla_q u \right\rangle_{\mu_{\beta}} - 2\sum_{x\in\cu} p \cdot \langle \nabla u(x,\cdot)\rangle_{\mu_{\beta}}  - \sum_{e\in E(\cu)}  \left\langle G(e,\cdot) \nabla u(e,\cdot) \right\rangle_{\mu_\beta}.
\end{align*}
\end{proof}


%Notice that, since the measure $\mu_\beta$ is log-concave (and in fact, a perturbation of the Gaussian measure) for large $\beta$, the following Poincar\'e-type inequality is a direct consequence of the Bakry-Emery criteria [ref]. 

%\begin{lemma}[{Poincar\'e inequality for $H^1(\mu_{\beta})$}]
%\label{l.spectralgap.mu}
%Let $\beta$ be sufficiently large. There exists $C(d,\beta)<\infty$ such that, for every $F \in H^1(\mu_{\beta})$, 
%\begin{equation*}
%\left\langle \left( F - \left\langle F \right\rangle_{\mu_{\beta}} \right)^2 \right\rangle_{\mu_{\beta}} 
%\leq 
%C \sum_{x\in Q} \left\langle (\partial_x F)^2 \right\rangle_{\mu_{\beta}}.
%\end{equation*}
%\end{lemma}

\fi


Abstract talk


Title: Quantitative homogenization of Helffer-Sjostrand equations and application to Villain model.

Abstract: In 1997, Naddaf and Spencer proved that the scaling limit of the uniformly convex grad phi model is given by a continuous Gaussian free field. The proof is based on an application of tools from the qualitative theory of stochastic homogenization to an infinite dimensional elliptic operator called the Helffer-Sjostrand PDE. In this talk, we will see how these ideas can be revisited and combined with the recent progress in the quantitative theory of stochastic homogenization to obtain new information on a model of statistical physics: the Villain model.
